The Flux Auto- and Cross-Correlation of the Lyman-alpha Forest. II. Modelling Anisotropies with Cosmological Hydrodynamic Simulations

The isotropy of the Lyman-alpha forest in real-space uniquely provides a measurement of cosmic geometry at z > 2. The angular diameter distance for which the correlation function along the line of sight and in the transverse direction agree corresponds to the correct cosmological model. However, the Lyman-alpha forest is observed in redshift-space where distortions due to Hubble expansion, bulk flows, and thermal broadening introduce anisotropy. Similarly, a spectrograph's line spread function affects the autocorrelation and cross-correlation differently. In this the second paper of a series on using the Lyman-alpha forest observed in pairs of QSOs for a new application of the Alcock-Paczynski (AP) test, these anisotropies and related sources of potential systematic error are investigated with cosmological hydrodynamic simulations. Three prescriptions for galactic outflow were compared and found to have only a marginal effect on the Lyman-alpha flux correlation (which changed by at most 7% with use of the currently favored variable-momentum wind model vs. no winds at all). An approximate solution for obtaining the zero-lag cross-correlation corresponding to arbitrary spectral resolution directly from the zero-lag cross-correlation computed at full-resolution (good to within 2% at the scales of interest) is presented. Uncertainty in the observationally determined mean flux decrement of the Lyman-alpha forest was found to be the dominant source of systematic error; however, this is reduced significantly when considering correlation ratios. We describe a simple scheme for implementing our results, while mitigating systematic errors, in the context of a future application of the AP test.

==> tab3_full.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                       %%
%% THIS TEX FILE WAS CREATED BY AN IDL SCRIPT AND SHOULD %%
%%  NOT BE MODIFIED - MAKE CHANGES TO SCRIPT INSTEAD...  %%
%%                                                       %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{deluxetable}{crrrrrrrrrrrrrrr}
\tablecolumns{16}
\tabletypesize{\tiny}
\tablewidth{7.25in}
\tablecaption{Cross-Correlation (\citet{1993pre414apj64} Mean Flux Decrement).\label{tab_cross_p93}}
\tablehead{
\colhead{$\Delta v$\tablenotemark{a}} & \multicolumn{7}{c}{$10\times\xi_\perp\!\left(\Delta v\right)$ in real-space} & 
\colhead{} & \multicolumn{7}{c}{$10\times\xi_\perp\!\left(\Delta v\right)$ in \emph{z}-space}\\
\cline{2-8}
\cline{10-16}
\colhead{($\delta v_\perp\!\left(z\right)$)} & 
\colhead{$z=1.8$} & \colhead{2.0} & \colhead{2.2} & \colhead{2.4} & 
\colhead{2.6} & \colhead{2.8} & \colhead{3.0} & 
\colhead{} & 
\colhead{$z=1.8$} & \colhead{2.0} & \colhead{2.2} & \colhead{2.4} & 
\colhead{2.6} & \colhead{2.8} & \colhead{3.0}}
\startdata
0000 &  0.4315 &  0.5914 &  0.7994 &  1.0641 &  1.4036 &  1.8199 &  2.3333 & &  0.7489 &  0.9812 &  1.2594 &  1.5876 &  1.9748 &  2.4281 &  2.9558\\
0001 &  0.4263 &  0.5853 &  0.7917 &  1.0541 &  1.3907 &  1.8026 &  2.3094 & &  0.7302 &  0.9614 &  1.2392 &  1.5660 &  1.9499 &  2.3995 &  2.9216\\
0002 &  0.4151 &  0.5702 &  0.7718 &  1.0275 &  1.3555 &  1.7566 &  2.2504 & &  0.7089 &  0.9364 &  1.2103 &  1.5316 &  1.9089 &  2.3508 &  2.8630\\
0003 &  0.3997 &  0.5493 &  0.7436 &  0.9903 &  1.3067 &  1.6933 &  2.1686 & &  0.6870 &  0.9090 &  1.1772 &  1.4915 &  1.8593 &  2.2893 &  2.7876\\
0004 &  0.3817 &  0.5239 &  0.7089 &  0.9445 &  1.2480 &  1.6174 &  2.0722 & &  0.6627 &  0.8791 &  1.1375 &  1.4439 &  1.8025 &  2.2183 &  2.7004\\
0005 &  0.3628 &  0.4982 &  0.6743 &  0.8988 &  1.1874 &  1.5382 &  1.9677 & &  0.6399 &  0.8498 &  1.1014 &  1.3983 &  1.7451 &  2.1462 &  2.6092\\
0006 &  0.3431 &  0.4709 &  0.6373 &  0.8493 &  1.1220 &  1.4530 &  1.8579 & &  0.6154 &  0.8191 &  1.0628 &  1.3493 &  1.6840 &  2.0702 &  2.5134\\
0007 &  0.3231 &  0.4426 &  0.5984 &  0.7971 &  1.0533 &  1.3645 &  1.7455 & &  0.5905 &  0.7865 &  1.0221 &  1.2989 &  1.6202 &  1.9911 &  2.4162\\
0008 &  0.3032 &  0.4152 &  0.5615 &  0.7480 &  0.9879 &  1.2787 &  1.6339 & &  0.5682 &  0.7577 &  0.9865 &  1.2524 &  1.5618 &  1.9164 &  2.3213\\
0009 &  0.2836 &  0.3876 &  0.5239 &  0.6975 &  0.9223 &  1.1940 &  1.5257 & &  0.5452 &  0.7291 &  0.9487 &  1.2046 &  1.5020 &  1.8427 &  2.2287\\
0010 &  0.2647 &  0.3616 &  0.4885 &  0.6502 &  0.8600 &  1.1136 &  1.4233 & &  0.5232 &  0.7015 &  0.9136 &  1.1594 &  1.4452 &  1.7720 &  2.1397\\
0012 &  0.2303 &  0.3140 &  0.4243 &  0.5649 &  0.7480 &  0.9697 &  1.2414 & &  0.4838 &  0.6501 &  0.8491 &  1.0771 &  1.3413 &  1.6408 &  1.9774\\
0013 &  0.2147 &  0.2928 &  0.3956 &  0.5272 &  0.6989 &  0.9073 &  1.1625 & &  0.4655 &  0.6265 &  0.8192 &  1.0402 &  1.2938 &  1.5827 &  1.9049\\
0015 &  0.1876 &  0.2559 &  0.3464 &  0.4627 &  0.6152 &  0.8008 &  1.0295 & &  0.4336 &  0.5850 &  0.7666 &  0.9734 &  1.2101 &  1.4769 &  1.7747\\
0017 &  0.1653 &  0.2253 &  0.3060 &  0.4101 &  0.5470 &  0.7149 &  0.9219 & &  0.4068 &  0.5504 &  0.7212 &  0.9147 &  1.1370 &  1.3855 &  1.6598\\
0020 &  0.1390 &  0.1903 &  0.2603 &  0.3504 &  0.4692 &  0.6151 &  0.7967 & &  0.3727 &  0.5070 &  0.6645 &  0.8424 &  1.0442 &  1.2689 &  1.5179\\
0022 &  0.1250 &  0.1720 &  0.2361 &  0.3194 &  0.4304 &  0.5664 &  0.7344 & &  0.3534 &  0.4814 &  0.6335 &  0.8024 &  0.9956 &  1.2098 &  1.4426\\
0023 &  0.1191 &  0.1642 &  0.2258 &  0.3060 &  0.4130 &  0.5441 &  0.7062 & &  0.3444 &  0.4705 &  0.6189 &  0.7839 &  0.9718 &  1.1807 &  1.4069\\
0025 &  0.1087 &  0.1504 &  0.2078 &  0.2825 &  0.3824 &  0.5047 &  0.6562 & &  0.3285 &  0.4495 &  0.5922 &  0.7498 &  0.9289 &  1.1267 &  1.3407\\
0030 &  0.0893 &  0.1248 &  0.1740 &  0.2383 &  0.3234 &  0.4276 &  0.5566 & &  0.2983 &  0.4082 &  0.5363 &  0.6791 &  0.8367 &  1.0110 &  1.1993\\
0033 &  0.0808 &  0.1135 &  0.1587 &  0.2182 &  0.2968 &  0.3930 &  0.5120 & &  0.2826 &  0.3880 &  0.5091 &  0.6431 &  0.7920 &  0.9554 &  1.1316\\
0035 &  0.0759 &  0.1070 &  0.1500 &  0.2070 &  0.2821 &  0.3736 &  0.4873 & &  0.2716 &  0.3753 &  0.4927 &  0.6217 &  0.7665 &  0.9225 &  1.0923\\
0037 &  0.0719 &  0.1016 &  0.1423 &  0.1964 &  0.2681 &  0.3555 &  0.4630 & &  0.2653 &  0.3639 &  0.4779 &  0.6025 &  0.7406 &  0.8912 &  1.0530\\
0040 &  0.0668 &  0.0944 &  0.1333 &  0.1839 &  0.2524 &  0.3337 &  0.4330 & &  0.2557 &  0.3489 &  0.4574 &  0.5765 &  0.7087 &  0.8511 &  1.0012\\
0042 &  0.0633 &  0.0899 &  0.1263 &  0.1745 &  0.2393 &  0.3185 &  0.4150 & &  0.2461 &  0.3380 &  0.4441 &  0.5584 &  0.6855 &  0.8225 &  0.9693\\
0043 &  0.0618 &  0.0879 &  0.1235 &  0.1707 &  0.2342 &  0.3119 &  0.4065 & &  0.2426 &  0.3338 &  0.4376 &  0.5505 &  0.6750 &  0.8096 &  0.9539\\
0045 &  0.0592 &  0.0842 &  0.1183 &  0.1636 &  0.2247 &  0.2994 &  0.3906 & &  0.2366 &  0.3247 &  0.4256 &  0.5346 &  0.6551 &  0.7848 &  0.9244\\
0050 &  0.0536 &  0.0761 &  0.1074 &  0.1479 &  0.2047 &  0.2746 &  0.3563 & &  0.2228 &  0.3054 &  0.3967 &  0.4977 &  0.6113 &  0.7341 &  0.8590\\
0055 &  0.0485 &  0.0691 &  0.0977 &  0.1358 &  0.1865 &  0.2485 &  0.3253 & &  0.2086 &  0.2867 &  0.3738 &  0.4678 &  0.5705 &  0.6801 &  0.7975\\
0060 &  0.0455 &  0.0644 &  0.0916 &  0.1283 &  0.1759 &  0.2323 &  0.3032 & &  0.2000 &  0.2736 &  0.3574 &  0.4443 &  0.5394 &  0.6414 &  0.7507\\
0065 &  0.0417 &  0.0592 &  0.0832 &  0.1165 &  0.1610 &  0.2149 &  0.2804 & &  0.1880 &  0.2572 &  0.3346 &  0.4161 &  0.5053 &  0.6001 &  0.7024\\
0068 &  0.0399 &  0.0567 &  0.0796 &  0.1116 &  0.1545 &  0.2063 &  0.2692 & &  0.1823 &  0.2491 &  0.3236 &  0.4019 &  0.4879 &  0.5789 &  0.6771\\
0070 &  0.0390 &  0.0552 &  0.0789 &  0.1102 &  0.1518 &  0.2017 &  0.2628 & &  0.1784 &  0.2446 &  0.3182 &  0.3956 &  0.4774 &  0.5656 &  0.6621\\
0072 &  0.0377 &  0.0537 &  0.0756 &  0.1055 &  0.1462 &  0.1961 &  0.2558 & &  0.1752 &  0.2393 &  0.3107 &  0.3851 &  0.4670 &  0.5539 &  0.6474\\
0077 &  0.0352 &  0.0503 &  0.0710 &  0.0989 &  0.1370 &  0.1843 &  0.2406 & &  0.1660 &  0.2273 &  0.2951 &  0.3650 &  0.4427 &  0.5251 &  0.6132\\
0078 &  0.0347 &  0.0496 &  0.0701 &  0.0976 &  0.1353 &  0.1819 &  0.2375 & &  0.1641 &  0.2251 &  0.2920 &  0.3613 &  0.4381 &  0.5194 &  0.6064\\
0080 &  0.0337 &  0.0483 &  0.0682 &  0.0951 &  0.1319 &  0.1775 &  0.2321 & &  0.1612 &  0.2202 &  0.2862 &  0.3541 &  0.4291 &  0.5082 &  0.5942\\
0090 &  0.0300 &  0.0428 &  0.0608 &  0.0860 &  0.1202 &  0.1626 &  0.2099 & &  0.1488 &  0.2013 &  0.2594 &  0.3217 &  0.3912 &  0.4673 &  0.5406\\
0100 &  0.0270 &  0.0386 &  0.0557 &  0.0777 &  0.1071 &  0.1439 &  0.1849 & &  0.1365 &  0.1860 &  0.2408 &  0.2971 &  0.3573 &  0.4197 &  0.4848\\
0105 &  0.0256 &  0.0365 &  0.0523 &  0.0740 &  0.1019 &  0.1355 &  0.1766 & &  0.1295 &  0.1762 &  0.2272 &  0.2829 &  0.3388 &  0.3978 &  0.4617\\
0125 &  0.0207 &  0.0300 &  0.0434 &  0.0604 &  0.0827 &  0.1104 &  0.1428 & &  0.1103 &  0.1493 &  0.1919 &  0.2365 &  0.2818 &  0.3281 &  0.3790\\
0130 &  0.0200 &  0.0286 &  0.0414 &  0.0580 &  0.0800 &  0.1068 &  0.1376 & &  0.1066 &  0.1446 &  0.1855 &  0.2262 &  0.2708 &  0.3174 &  0.3654\\
0135 &  0.0189 &  0.0271 &  0.0390 &  0.0545 &  0.0746 &  0.0991 &  0.1274 & &  0.1030 &  0.1396 &  0.1773 &  0.2174 &  0.2579 &  0.2995 &  0.3435\\
0138 &  0.0184 &  0.0263 &  0.0379 &  0.0529 &  0.0723 &  0.0955 &  0.1233 & &  0.1006 &  0.1366 &  0.1739 &  0.2122 &  0.2516 &  0.2911 &  0.3338\\
0142 &  0.0178 &  0.0254 &  0.0366 &  0.0511 &  0.0695 &  0.0916 &  0.1181 & &  0.0979 &  0.1330 &  0.1689 &  0.2055 &  0.2431 &  0.2806 &  0.3213\\
0147 &  0.0171 &  0.0244 &  0.0350 &  0.0484 &  0.0662 &  0.0874 &  0.1136 & &  0.0936 &  0.1279 &  0.1623 &  0.1960 &  0.2323 &  0.2692 &  0.3078\\
0148 &  0.0169 &  0.0242 &  0.0347 &  0.0480 &  0.0656 &  0.0866 &  0.1127 & &  0.0931 &  0.1268 &  0.1608 &  0.1942 &  0.2307 &  0.2669 &  0.3053\\
0150 &  0.0166 &  0.0237 &  0.0340 &  0.0470 &  0.0642 &  0.0850 &  0.1109 & &  0.0919 &  0.1244 &  0.1579 &  0.1903 &  0.2265 &  0.2618 &  0.3005\\
0165 &  0.0148 &  0.0212 &  0.0305 &  0.0435 &  0.0593 &  0.0789 &  0.1029 & &  0.0845 &  0.1115 &  0.1418 &  0.1714 &  0.2022 &  0.2337 &  0.2689\\
0170 &  0.0140 &  0.0202 &  0.0291 &  0.0413 &  0.0575 &  0.0770 &  0.0988 & &  0.0812 &  0.1079 &  0.1364 &  0.1656 &  0.1976 &  0.2243 &  0.2556\\
0185 &  0.0124 &  0.0182 &  0.0268 &  0.0377 &  0.0520 &  0.0715 &  0.0922 & &  0.0743 &  0.0987 &  0.1252 &  0.1511 &  0.1775 &  0.2019 &  0.2295\\
0195 &  0.0115 &  0.0172 &  0.0257 &  0.0370 &  0.0495 &  0.0676 &  0.0861 & &  0.0707 &  0.0939 &  0.1180 &  0.1421 &  0.1671 &  0.1904 &  0.2152\\
0198 &  0.0113 &  0.0170 &  0.0253 &  0.0365 &  0.0487 &  0.0658 &  0.0847 & &  0.0693 &  0.0921 &  0.1158 &  0.1390 &  0.1637 &  0.1869 &  0.2122\\
0202 &  0.0111 &  0.0165 &  0.0247 &  0.0355 &  0.0479 &  0.0635 &  0.0831 & &  0.0677 &  0.0898 &  0.1119 &  0.1344 &  0.1593 &  0.1837 &  0.2080\\
0205 &  0.0111 &  0.0162 &  0.0238 &  0.0341 &  0.0485 &  0.0622 &  0.0811 & &  0.0664 &  0.0876 &  0.1088 &  0.1305 &  0.1555 &  0.1812 &  0.2083\\
0207 &  0.0108 &  0.0159 &  0.0240 &  0.0345 &  0.0475 &  0.0613 &  0.0812 & &  0.0657 &  0.0863 &  0.1079 &  0.1289 &  0.1528 &  0.1800 &  0.2027\\
0208 &  0.0108 &  0.0158 &  0.0239 &  0.0344 &  0.0471 &  0.0610 &  0.0807 & &  0.0653 &  0.0856 &  0.1072 &  0.1278 &  0.1519 &  0.1794 &  0.2016\\
0210 &  0.0107 &  0.0157 &  0.0236 &  0.0339 &  0.0464 &  0.0603 &  0.0796 & &  0.0648 &  0.0845 &  0.1061 &  0.1261 &  0.1505 &  0.1780 &  0.1994\\
0220 &  0.0107 &  0.0157 &  0.0229 &  0.0327 &  0.0426 &  0.0577 &  0.0756 & &  0.0625 &  0.0811 &  0.0993 &  0.1203 &  0.1454 &  0.1713 &  0.1913\\
0225 &  0.0102 &  0.0147 &  0.0212 &  0.0313 &  0.0414 &  0.0564 &  0.0707 & &  0.0607 &  0.0784 &  0.0954 &  0.1170 &  0.1428 &  0.1688 &  0.1851\\
0235 &  0.0098 &  0.0140 &  0.0212 &  0.0287 &  0.0398 &  0.0523 &  0.0669 & &  0.0584 &  0.0745 &  0.0912 &  0.1126 &  0.1369 &  0.1618 &  0.1756\\
0238 &  0.0098 &  0.0139 &  0.0212 &  0.0282 &  0.0391 &  0.0508 &  0.0655 & &  0.0577 &  0.0732 &  0.0899 &  0.1110 &  0.1356 &  0.1592 &  0.1737\\
0242 &  0.0097 &  0.0138 &  0.0205 &  0.0278 &  0.0379 &  0.0491 &  0.0637 & &  0.0561 &  0.0722 &  0.0882 &  0.1087 &  0.1340 &  0.1563 &  0.1702\\
0247 &  0.0096 &  0.0139 &  0.0197 &  0.0273 &  0.0372 &  0.0473 &  0.0613 & &  0.0542 &  0.0702 &  0.0862 &  0.1058 &  0.1298 &  0.1531 &  0.1660\\
0248 &  0.0095 &  0.0139 &  0.0195 &  0.0271 &  0.0368 &  0.0470 &  0.0608 & &  0.0538 &  0.0699 &  0.0858 &  0.1053 &  0.1294 &  0.1526 &  0.1654\\
0250 &  0.0094 &  0.0139 &  0.0192 &  0.0268 &  0.0364 &  0.0465 &  0.0598 & &  0.0532 &  0.0694 &  0.0851 &  0.1043 &  0.1281 &  0.1515 &  0.1636\\
0255 &  0.0092 &  0.0135 &  0.0187 &  0.0260 &  0.0352 &  0.0443 &  0.0605 & &  0.0524 &  0.0671 &  0.0826 &  0.1018 &  0.1249 &  0.1491 &  0.1589\\
0275 &  0.0088 &  0.0122 &  0.0169 &  0.0245 &  0.0303 &  0.0362 &  0.0508 & &  0.0488 &  0.0611 &  0.0731 &  0.0908 &  0.1159 &  0.1358 &  0.1427\\
0285 &  0.0084 &  0.0113 &  0.0169 &  0.0236 &  0.0281 &  0.0316 &  0.0502 & &  0.0485 &  0.0584 &  0.0687 &  0.0877 &  0.1112 &  0.1281 &  0.1368\\
0288 &  0.0084 &  0.0111 &  0.0170 &  0.0235 &  0.0273 &  0.0301 &  0.0494 & &  0.0485 &  0.0577 &  0.0677 &  0.0868 &  0.1097 &  0.1258 &  0.1358\\
0292 &  0.0082 &  0.0108 &  0.0172 &  0.0233 &  0.0262 &  0.0277 &  0.0481 & &  0.0487 &  0.0570 &  0.0667 &  0.0858 &  0.1076 &  0.1225 &  0.1328\\
0297 &  0.0079 &  0.0107 &  0.0174 &  0.0232 &  0.0248 &  0.0252 &  0.0468 & &  0.0489 &  0.0560 &  0.0658 &  0.0848 &  0.1048 &  0.1183 &  0.1290\\
0298 &  0.0079 &  0.0107 &  0.0175 &  0.0231 &  0.0245 &  0.0247 &  0.0466 & &  0.0490 &  0.0557 &  0.0657 &  0.0845 &  0.1042 &  0.1175 &  0.1284\\
0300 &  0.0078 &  0.0107 &  0.0176 &  0.0230 &  0.0238 &  0.0237 &  0.0461 & &  0.0489 &  0.0555 &  0.0654 &  0.0840 &  0.1030 &  0.1158 &  0.1270\\
\enddata
\tablenotetext{a}{74 $\Delta v$ values given in units of $\delta v_\perp\!\left(z\right) \equiv 0.67455\,z + 0.38896$ km s$^{-1}$ (or, alternatively, arcseconds)}
\tablecomments{These are the hybrid correlation 
values for full-resolution.}
\end{deluxetable}


==> tab4_full.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                       %%
%% THIS TEX FILE WAS CREATED BY AN IDL SCRIPT AND SHOULD %%
%%  NOT BE MODIFIED - MAKE CHANGES TO SCRIPT INSTEAD...  %%
%%                                                       %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{deluxetable}{crrrrrrrrrrrrrrr}
\tablecolumns{16}
\tabletypesize{\tiny}
\tablewidth{7.25in}
\tablecaption{Autocorrelation (\citet{1993pre414apj64} Mean Flux Decrement).\label{tab_auto_p93}}
\tablehead{
\colhead{$\Delta v$\tablenotemark{a}} & \multicolumn{7}{c}{$10\times\xi_\parallel\!\left(\Delta v\right)$ in real-space} & 
\colhead{} & \multicolumn{7}{c}{$10\times\xi_\parallel\!\left(\Delta v\right)$ in \emph{z}-space}\\
\cline{2-8}
\cline{10-16}
\colhead{($\delta v_\parallel\!\left(z\right)$)} & 
\colhead{$z=1.8$} & \colhead{2.0} & \colhead{2.2} & \colhead{2.4} & 
\colhead{2.6} & \colhead{2.8} & \colhead{3.0} & 
\colhead{} & 
\colhead{$z=1.8$} & \colhead{2.0} & \colhead{2.2} & \colhead{2.4} & 
\colhead{2.6} & \colhead{2.8} & \colhead{3.0}}
\startdata
0000 &  0.4315 &  0.5914 &  0.7994 &  1.0641 &  1.4036 &  1.8199 &  2.3333 & &  0.7489 &  0.9812 &  1.2594 &  1.5876 &  1.9748 &  2.4281 &  2.9558\\
0001 &  0.4250 &  0.5837 &  0.7902 &  1.0530 &  1.3902 &  1.8036 &  2.3135 & &  0.7478 &  0.9797 &  1.2572 &  1.5847 &  1.9709 &  2.4231 &  2.9493\\
0002 &  0.4097 &  0.5649 &  0.7672 &  1.0249 &  1.3558 &  1.7616 &  2.2622 & &  0.7445 &  0.9750 &  1.2507 &  1.5759 &  1.9593 &  2.4081 &  2.9303\\
0003 &  0.3897 &  0.5398 &  0.7359 &  0.9862 &  1.3079 &  1.7027 &  2.1899 & &  0.7392 &  0.9674 &  1.2400 &  1.5615 &  1.9404 &  2.3838 &  2.8994\\
0004 &  0.3673 &  0.5111 &  0.6998 &  0.9411 &  1.2519 &  1.6334 &  2.1043 & &  0.7319 &  0.9570 &  1.2256 &  1.5421 &  1.9148 &  2.3509 &  2.8579\\
0005 &  0.3436 &  0.4804 &  0.6608 &  0.8920 &  1.1906 &  1.5572 &  2.0100 & &  0.7229 &  0.9440 &  1.2077 &  1.5181 &  1.8834 &  2.3107 &  2.8071\\
0006 &  0.3193 &  0.4487 &  0.6200 &  0.8404 &  1.1258 &  1.4765 &  1.9097 & &  0.7123 &  0.9289 &  1.1868 &  1.4902 &  1.8469 &  2.2641 &  2.7487\\
0007 &  0.2952 &  0.4169 &  0.5788 &  0.7878 &  1.0593 &  1.3932 &  1.8058 & &  0.7002 &  0.9118 &  1.1633 &  1.4589 &  1.8061 &  2.2124 &  2.6840\\
0008 &  0.2720 &  0.3859 &  0.5381 &  0.7355 &  0.9927 &  1.3093 &  1.7009 & &  0.6870 &  0.8932 &  1.1378 &  1.4249 &  1.7621 &  2.1566 &  2.6145\\
0009 &  0.2501 &  0.3563 &  0.4990 &  0.6847 &  0.9275 &  1.2268 &  1.5975 & &  0.6729 &  0.8732 &  1.1105 &  1.3888 &  1.7154 &  2.0978 &  2.5414\\
0010 &  0.2299 &  0.3287 &  0.4621 &  0.6364 &  0.8652 &  1.1475 &  1.4977 & &  0.6579 &  0.8522 &  1.0820 &  1.3511 &  1.6670 &  2.0367 &  2.4658\\
0011 &  0.2114 &  0.3033 &  0.4280 &  0.5914 &  0.8066 &  1.0727 &  1.4033 & &  0.6424 &  0.8305 &  1.0525 &  1.3124 &  1.6173 &  1.9744 &  2.3886\\
0012 &  0.1947 &  0.2803 &  0.3968 &  0.5500 &  0.7525 &  1.0034 &  1.3156 & &  0.6264 &  0.8083 &  1.0226 &  1.2731 &  1.5669 &  1.9112 &  2.3107\\
0013 &  0.1798 &  0.2596 &  0.3686 &  0.5124 &  0.7032 &  0.9399 &  1.2350 & &  0.6102 &  0.7858 &  0.9923 &  1.2336 &  1.5164 &  1.8480 &  2.2326\\
0014 &  0.1665 &  0.2411 &  0.3434 &  0.4786 &  0.6586 &  0.8823 &  1.1618 & &  0.5938 &  0.7633 &  0.9621 &  1.1942 &  1.4661 &  1.7851 &  2.1551\\
0015 &  0.1548 &  0.2247 &  0.3208 &  0.4483 &  0.6185 &  0.8304 &  1.0957 & &  0.5774 &  0.7408 &  0.9320 &  1.1551 &  1.4163 &  1.7230 &  2.0786\\
0016 &  0.1443 &  0.2100 &  0.3008 &  0.4212 &  0.5825 &  0.7838 &  1.0361 & &  0.5612 &  0.7185 &  0.9024 &  1.1167 &  1.3674 &  1.6620 &  2.0034\\
0017 &  0.1351 &  0.1970 &  0.2829 &  0.3970 &  0.5503 &  0.7419 &  0.9824 & &  0.5451 &  0.6966 &  0.8733 &  1.0790 &  1.3196 &  1.6023 &  1.9300\\
0018 &  0.1268 &  0.1855 &  0.2669 &  0.3754 &  0.5214 &  0.7042 &  0.9339 & &  0.5292 &  0.6751 &  0.8449 &  1.0423 &  1.2731 &  1.5443 &  1.8587\\
0019 &  0.1195 &  0.1751 &  0.2526 &  0.3561 &  0.4955 &  0.6702 &  0.8902 & &  0.5137 &  0.6541 &  0.8172 &  1.0066 &  1.2279 &  1.4882 &  1.7896\\
0020 &  0.1129 &  0.1658 &  0.2397 &  0.3386 &  0.4721 &  0.6394 &  0.8505 & &  0.4985 &  0.6337 &  0.7903 &  0.9720 &  1.1843 &  1.4340 &  1.7230\\
0021 &  0.1070 &  0.1575 &  0.2281 &  0.3229 &  0.4509 &  0.6116 &  0.8144 & &  0.4837 &  0.6138 &  0.7643 &  0.9387 &  1.1423 &  1.3818 &  1.6591\\
0022 &  0.1017 &  0.1500 &  0.2177 &  0.3087 &  0.4317 &  0.5862 &  0.7814 & &  0.4693 &  0.5946 &  0.7392 &  0.9066 &  1.1019 &  1.3318 &  1.5978\\
0023 &  0.0969 &  0.1432 &  0.2082 &  0.2957 &  0.4142 &  0.5630 &  0.7513 & &  0.4554 &  0.5760 &  0.7151 &  0.8758 &  1.0633 &  1.2840 &  1.5393\\
0024 &  0.0925 &  0.1370 &  0.1996 &  0.2839 &  0.3981 &  0.5418 &  0.7235 & &  0.4419 &  0.5581 &  0.6918 &  0.8462 &  1.0262 &  1.2384 &  1.4836\\
0025 &  0.0886 &  0.1313 &  0.1917 &  0.2731 &  0.3834 &  0.5223 &  0.6980 & &  0.4288 &  0.5408 &  0.6695 &  0.8178 &  0.9909 &  1.1949 &  1.4306\\
0026 &  0.0850 &  0.1262 &  0.1845 &  0.2631 &  0.3699 &  0.5043 &  0.6743 & &  0.4162 &  0.5242 &  0.6480 &  0.7907 &  0.9571 &  1.1535 &  1.3803\\
0027 &  0.0817 &  0.1214 &  0.1778 &  0.2539 &  0.3574 &  0.4876 &  0.6524 & &  0.4041 &  0.5082 &  0.6275 &  0.7647 &  0.9250 &  1.1141 &  1.3326\\
0028 &  0.0786 &  0.1171 &  0.1717 &  0.2454 &  0.3458 &  0.4721 &  0.6320 & &  0.3923 &  0.4929 &  0.6078 &  0.7399 &  0.8943 &  1.0768 &  1.2875\\
0029 &  0.0758 &  0.1131 &  0.1660 &  0.2375 &  0.3350 &  0.4577 &  0.6129 & &  0.3810 &  0.4781 &  0.5889 &  0.7163 &  0.8651 &  1.0413 &  1.2447\\
0030 &  0.0732 &  0.1093 &  0.1607 &  0.2302 &  0.3250 &  0.4442 &  0.5951 & &  0.3702 &  0.4639 &  0.5708 &  0.6936 &  0.8373 &  1.0076 &  1.2042\\
0031 &  0.0708 &  0.1059 &  0.1558 &  0.2233 &  0.3155 &  0.4316 &  0.5784 & &  0.3597 &  0.4503 &  0.5535 &  0.6720 &  0.8108 &  0.9756 &  1.1658\\
0032 &  0.0686 &  0.1026 &  0.1512 &  0.2169 &  0.3067 &  0.4198 &  0.5627 & &  0.3496 &  0.4372 &  0.5369 &  0.6513 &  0.7856 &  0.9451 &  1.1295\\
0033 &  0.0665 &  0.0996 &  0.1469 &  0.2110 &  0.2984 &  0.4086 &  0.5479 & &  0.3399 &  0.4246 &  0.5210 &  0.6316 &  0.7615 &  0.9162 &  1.0950\\
0034 &  0.0645 &  0.0968 &  0.1429 &  0.2053 &  0.2906 &  0.3981 &  0.5340 & &  0.3305 &  0.4126 &  0.5058 &  0.6127 &  0.7385 &  0.8887 &  1.0624\\
0035 &  0.0627 &  0.0941 &  0.1390 &  0.2000 &  0.2833 &  0.3882 &  0.5208 & &  0.3215 &  0.4010 &  0.4912 &  0.5946 &  0.7166 &  0.8625 &  1.0313\\
0036 &  0.0610 &  0.0916 &  0.1354 &  0.1950 &  0.2763 &  0.3788 &  0.5083 & &  0.3128 &  0.3898 &  0.4771 &  0.5773 &  0.6957 &  0.8376 &  1.0018\\
0037 &  0.0593 &  0.0892 &  0.1320 &  0.1903 &  0.2697 &  0.3699 &  0.4964 & &  0.3044 &  0.3791 &  0.4637 &  0.5607 &  0.6756 &  0.8137 &  0.9737\\
0038 &  0.0578 &  0.0869 &  0.1288 &  0.1858 &  0.2634 &  0.3615 &  0.4851 & &  0.2964 &  0.3688 &  0.4508 &  0.5448 &  0.6564 &  0.7910 &  0.9470\\
0039 &  0.0563 &  0.0847 &  0.1257 &  0.1815 &  0.2574 &  0.3534 &  0.4744 & &  0.2886 &  0.3588 &  0.4383 &  0.5295 &  0.6380 &  0.7692 &  0.9215\\
0040 &  0.0549 &  0.0827 &  0.1228 &  0.1774 &  0.2518 &  0.3457 &  0.4642 & &  0.2811 &  0.3493 &  0.4264 &  0.5148 &  0.6204 &  0.7483 &  0.8971\\
0041 &  0.0536 &  0.0808 &  0.1200 &  0.1736 &  0.2464 &  0.3384 &  0.4544 & &  0.2738 &  0.3401 &  0.4149 &  0.5007 &  0.6035 &  0.7284 &  0.8737\\
0042 &  0.0524 &  0.0789 &  0.1174 &  0.1699 &  0.2413 &  0.3314 &  0.4451 & &  0.2668 &  0.3312 &  0.4038 &  0.4871 &  0.5872 &  0.7092 &  0.8514\\
0043 &  0.0512 &  0.0772 &  0.1149 &  0.1663 &  0.2363 &  0.3247 &  0.4362 & &  0.2601 &  0.3226 &  0.3931 &  0.4741 &  0.5716 &  0.6908 &  0.8300\\
0044 &  0.0501 &  0.0755 &  0.1125 &  0.1630 &  0.2317 &  0.3183 &  0.4277 & &  0.2535 &  0.3143 &  0.3828 &  0.4615 &  0.5566 &  0.6731 &  0.8094\\
0045 &  0.0490 &  0.0739 &  0.1102 &  0.1598 &  0.2272 &  0.3122 &  0.4195 & &  0.2472 &  0.3063 &  0.3729 &  0.4493 &  0.5421 &  0.6560 &  0.7896\\
0046 &  0.0479 &  0.0724 &  0.1080 &  0.1567 &  0.2229 &  0.3063 &  0.4117 & &  0.2411 &  0.2986 &  0.3633 &  0.4376 &  0.5281 &  0.6396 &  0.7706\\
0047 &  0.0470 &  0.0709 &  0.1059 &  0.1538 &  0.2188 &  0.3007 &  0.4042 & &  0.2352 &  0.2912 &  0.3541 &  0.4263 &  0.5146 &  0.6238 &  0.7523\\
0048 &  0.0460 &  0.0695 &  0.1039 &  0.1509 &  0.2149 &  0.2953 &  0.3969 & &  0.2295 &  0.2840 &  0.3451 &  0.4154 &  0.5016 &  0.6085 &  0.7346\\
0049 &  0.0451 &  0.0682 &  0.1020 &  0.1482 &  0.2111 &  0.2901 &  0.3900 & &  0.2240 &  0.2770 &  0.3365 &  0.4048 &  0.4890 &  0.5938 &  0.7176\\
0050 &  0.0443 &  0.0669 &  0.1001 &  0.1457 &  0.2075 &  0.2851 &  0.3833 & &  0.2186 &  0.2702 &  0.3282 &  0.3946 &  0.4768 &  0.5795 &  0.7011\\
0051 &  0.0435 &  0.0657 &  0.0984 &  0.1432 &  0.2040 &  0.2803 &  0.3769 & &  0.2135 &  0.2637 &  0.3201 &  0.3847 &  0.4651 &  0.5657 &  0.6852\\
0052 &  0.0427 &  0.0645 &  0.0966 &  0.1407 &  0.2006 &  0.2757 &  0.3707 & &  0.2084 &  0.2574 &  0.3122 &  0.3752 &  0.4537 &  0.5523 &  0.6698\\
0053 &  0.0419 &  0.0634 &  0.0950 &  0.1384 &  0.1974 &  0.2713 &  0.3647 & &  0.2036 &  0.2513 &  0.3047 &  0.3659 &  0.4426 &  0.5394 &  0.6548\\
0054 &  0.0412 &  0.0623 &  0.0934 &  0.1362 &  0.1942 &  0.2669 &  0.3589 & &  0.1989 &  0.2454 &  0.2974 &  0.3570 &  0.4319 &  0.5269 &  0.6404\\
0055 &  0.0405 &  0.0612 &  0.0918 &  0.1340 &  0.1912 &  0.2628 &  0.3533 & &  0.1943 &  0.2397 &  0.2903 &  0.3483 &  0.4216 &  0.5147 &  0.6263\\
0056 &  0.0398 &  0.0602 &  0.0903 &  0.1318 &  0.1882 &  0.2587 &  0.3479 & &  0.1899 &  0.2341 &  0.2834 &  0.3399 &  0.4116 &  0.5029 &  0.6127\\
0057 &  0.0391 &  0.0593 &  0.0889 &  0.1298 &  0.1853 &  0.2548 &  0.3426 & &  0.1856 &  0.2287 &  0.2767 &  0.3318 &  0.4018 &  0.4914 &  0.5995\\
0058 &  0.0385 &  0.0583 &  0.0875 &  0.1278 &  0.1825 &  0.2509 &  0.3375 & &  0.1815 &  0.2235 &  0.2703 &  0.3239 &  0.3924 &  0.4803 &  0.5866\\
0059 &  0.0378 &  0.0574 &  0.0861 &  0.1258 &  0.1798 &  0.2472 &  0.3325 & &  0.1774 &  0.2185 &  0.2641 &  0.3163 &  0.3832 &  0.4695 &  0.5741\\
0060 &  0.0372 &  0.0565 &  0.0848 &  0.1239 &  0.1771 &  0.2436 &  0.3277 & &  0.1735 &  0.2136 &  0.2580 &  0.3089 &  0.3744 &  0.4590 &  0.5619\\
0061 &  0.0365 &  0.0557 &  0.0835 &  0.1221 &  0.1746 &  0.2400 &  0.3230 & &  0.1697 &  0.2089 &  0.2522 &  0.3017 &  0.3658 &  0.4489 &  0.5501\\
0062 &  0.0359 &  0.0548 &  0.0822 &  0.1203 &  0.1721 &  0.2366 &  0.3184 & &  0.1661 &  0.2043 &  0.2465 &  0.2948 &  0.3574 &  0.4390 &  0.5386\\
0063 &  0.0353 &  0.0540 &  0.0810 &  0.1185 &  0.1696 &  0.2332 &  0.3139 & &  0.1625 &  0.1998 &  0.2410 &  0.2881 &  0.3493 &  0.4293 &  0.5273\\
0064 &  0.0348 &  0.0532 &  0.0798 &  0.1168 &  0.1673 &  0.2300 &  0.3096 & &  0.1590 &  0.1955 &  0.2357 &  0.2816 &  0.3415 &  0.4200 &  0.5164\\
0065 &  0.0342 &  0.0523 &  0.0787 &  0.1152 &  0.1650 &  0.2268 &  0.3054 & &  0.1557 &  0.1913 &  0.2305 &  0.2752 &  0.3339 &  0.4109 &  0.5058\\
0066 &  0.0337 &  0.0516 &  0.0776 &  0.1136 &  0.1627 &  0.2237 &  0.3012 & &  0.1524 &  0.1872 &  0.2255 &  0.2691 &  0.3265 &  0.4021 &  0.4954\\
0067 &  0.0332 &  0.0508 &  0.0765 &  0.1120 &  0.1606 &  0.2207 &  0.2973 & &  0.1493 &  0.1832 &  0.2206 &  0.2632 &  0.3194 &  0.3936 &  0.4854\\
0068 &  0.0327 &  0.0500 &  0.0754 &  0.1105 &  0.1585 &  0.2178 &  0.2934 & &  0.1462 &  0.1794 &  0.2159 &  0.2575 &  0.3125 &  0.3853 &  0.4756\\
0069 &  0.0323 &  0.0493 &  0.0744 &  0.1090 &  0.1565 &  0.2150 &  0.2896 & &  0.1432 &  0.1756 &  0.2113 &  0.2519 &  0.3058 &  0.3773 &  0.4660\\
0070 &  0.0318 &  0.0486 &  0.0734 &  0.1075 &  0.1545 &  0.2123 &  0.2859 & &  0.1403 &  0.1720 &  0.2068 &  0.2465 &  0.2993 &  0.3695 &  0.4568\\
0071 &  0.0314 &  0.0479 &  0.0724 &  0.1061 &  0.1525 &  0.2097 &  0.2823 & &  0.1375 &  0.1685 &  0.2025 &  0.2413 &  0.2930 &  0.3619 &  0.4477\\
0072 &  0.0310 &  0.0472 &  0.0714 &  0.1047 &  0.1506 &  0.2071 &  0.2788 & &  0.1347 &  0.1650 &  0.1983 &  0.2362 &  0.2869 &  0.3545 &  0.4390\\
0073 &  0.0306 &  0.0465 &  0.0704 &  0.1033 &  0.1486 &  0.2045 &  0.2754 & &  0.1321 &  0.1617 &  0.1942 &  0.2313 &  0.2810 &  0.3474 &  0.4305\\
0074 &  0.0302 &  0.0459 &  0.0695 &  0.1020 &  0.1468 &  0.2020 &  0.2720 & &  0.1295 &  0.1584 &  0.1902 &  0.2265 &  0.2752 &  0.3405 &  0.4222\\
0075 &  0.0298 &  0.0453 &  0.0686 &  0.1007 &  0.1449 &  0.1995 &  0.2688 & &  0.1270 &  0.1553 &  0.1864 &  0.2218 &  0.2697 &  0.3338 &  0.4141\\
0076 &  0.0294 &  0.0447 &  0.0676 &  0.0994 &  0.1431 &  0.1971 &  0.2655 & &  0.1245 &  0.1522 &  0.1826 &  0.2173 &  0.2643 &  0.3272 &  0.4063\\
0077 &  0.0291 &  0.0441 &  0.0668 &  0.0981 &  0.1413 &  0.1947 &  0.2623 & &  0.1221 &  0.1492 &  0.1789 &  0.2129 &  0.2590 &  0.3209 &  0.3986\\
0078 &  0.0287 &  0.0435 &  0.0659 &  0.0968 &  0.1395 &  0.1923 &  0.2592 & &  0.1198 &  0.1462 &  0.1754 &  0.2086 &  0.2539 &  0.3147 &  0.3912\\
0079 &  0.0284 &  0.0429 &  0.0650 &  0.0956 &  0.1377 &  0.1899 &  0.2560 & &  0.1175 &  0.1434 &  0.1719 &  0.2044 &  0.2489 &  0.3087 &  0.3840\\
0080 &  0.0280 &  0.0424 &  0.0642 &  0.0944 &  0.1360 &  0.1875 &  0.2529 & &  0.1153 &  0.1406 &  0.1685 &  0.2003 &  0.2441 &  0.3029 &  0.3770\\
0081 &  0.0277 &  0.0419 &  0.0634 &  0.0932 &  0.1342 &  0.1852 &  0.2498 & &  0.1131 &  0.1379 &  0.1652 &  0.1964 &  0.2394 &  0.2972 &  0.3701\\
0082 &  0.0274 &  0.0414 &  0.0626 &  0.0920 &  0.1325 &  0.1829 &  0.2468 & &  0.1110 &  0.1352 &  0.1620 &  0.1925 &  0.2348 &  0.2917 &  0.3634\\
0083 &  0.0271 &  0.0409 &  0.0618 &  0.0909 &  0.1309 &  0.1807 &  0.2438 & &  0.1090 &  0.1327 &  0.1588 &  0.1887 &  0.2303 &  0.2863 &  0.3569\\
0084 &  0.0268 &  0.0404 &  0.0610 &  0.0897 &  0.1292 &  0.1784 &  0.2408 & &  0.1070 &  0.1301 &  0.1557 &  0.1850 &  0.2259 &  0.2810 &  0.3506\\
0085 &  0.0265 &  0.0399 &  0.0603 &  0.0886 &  0.1276 &  0.1762 &  0.2378 & &  0.1051 &  0.1277 &  0.1528 &  0.1814 &  0.2216 &  0.2759 &  0.3444\\
0086 &  0.0263 &  0.0395 &  0.0595 &  0.0875 &  0.1260 &  0.1740 &  0.2349 & &  0.1032 &  0.1253 &  0.1498 &  0.1779 &  0.2174 &  0.2709 &  0.3383\\
0087 &  0.0260 &  0.0391 &  0.0588 &  0.0865 &  0.1245 &  0.1718 &  0.2320 & &  0.1013 &  0.1230 &  0.1470 &  0.1744 &  0.2133 &  0.2660 &  0.3324\\
0088 &  0.0257 &  0.0387 &  0.0581 &  0.0854 &  0.1229 &  0.1697 &  0.2292 & &  0.0995 &  0.1207 &  0.1442 &  0.1710 &  0.2094 &  0.2612 &  0.3266\\
0089 &  0.0254 &  0.0383 &  0.0575 &  0.0844 &  0.1214 &  0.1676 &  0.2264 & &  0.0977 &  0.1185 &  0.1415 &  0.1678 &  0.2054 &  0.2565 &  0.3210\\
0090 &  0.0252 &  0.0379 &  0.0568 &  0.0834 &  0.1200 &  0.1656 &  0.2237 & &  0.0960 &  0.1164 &  0.1389 &  0.1645 &  0.2016 &  0.2519 &  0.3155\\
0091 &  0.0249 &  0.0375 &  0.0562 &  0.0825 &  0.1185 &  0.1635 &  0.2210 & &  0.0944 &  0.1143 &  0.1363 &  0.1614 &  0.1979 &  0.2474 &  0.3101\\
0092 &  0.0246 &  0.0372 &  0.0556 &  0.0816 &  0.1171 &  0.1615 &  0.2184 & &  0.0927 &  0.1122 &  0.1338 &  0.1583 &  0.1942 &  0.2430 &  0.3048\\
0093 &  0.0244 &  0.0368 &  0.0550 &  0.0807 &  0.1158 &  0.1596 &  0.2158 & &  0.0911 &  0.1102 &  0.1313 &  0.1553 &  0.1907 &  0.2387 &  0.2996\\
0094 &  0.0241 &  0.0364 &  0.0545 &  0.0798 &  0.1145 &  0.1577 &  0.2133 & &  0.0895 &  0.1083 &  0.1289 &  0.1524 &  0.1872 &  0.2345 &  0.2945\\
0095 &  0.0238 &  0.0361 &  0.0539 &  0.0789 &  0.1132 &  0.1559 &  0.2109 & &  0.0880 &  0.1064 &  0.1266 &  0.1496 &  0.1838 &  0.2304 &  0.2896\\
0096 &  0.0235 &  0.0357 &  0.0534 &  0.0781 &  0.1120 &  0.1541 &  0.2085 & &  0.0865 &  0.1045 &  0.1244 &  0.1468 &  0.1804 &  0.2264 &  0.2847\\
0097 &  0.0233 &  0.0354 &  0.0528 &  0.0773 &  0.1108 &  0.1524 &  0.2061 & &  0.0851 &  0.1027 &  0.1222 &  0.1441 &  0.1772 &  0.2225 &  0.2799\\
0098 &  0.0230 &  0.0350 &  0.0523 &  0.0765 &  0.1097 &  0.1507 &  0.2038 & &  0.0836 &  0.1010 &  0.1200 &  0.1414 &  0.1740 &  0.2186 &  0.2753\\
0099 &  0.0227 &  0.0347 &  0.0518 &  0.0757 &  0.1086 &  0.1491 &  0.2016 & &  0.0822 &  0.0992 &  0.1179 &  0.1389 &  0.1709 &  0.2149 &  0.2707\\
0100 &  0.0225 &  0.0343 &  0.0513 &  0.0749 &  0.1076 &  0.1475 &  0.1994 & &  0.0809 &  0.0976 &  0.1159 &  0.1364 &  0.1679 &  0.2112 &  0.2663\\
0101 &  0.0222 &  0.0339 &  0.0508 &  0.0742 &  0.1065 &  0.1460 &  0.1973 & &  0.0795 &  0.0959 &  0.1139 &  0.1339 &  0.1649 &  0.2076 &  0.2619\\
0102 &  0.0219 &  0.0335 &  0.0503 &  0.0735 &  0.1055 &  0.1445 &  0.1952 & &  0.0782 &  0.0943 &  0.1120 &  0.1316 &  0.1620 &  0.2041 &  0.2576\\
0103 &  0.0216 &  0.0332 &  0.0498 &  0.0727 &  0.1045 &  0.1432 &  0.1933 & &  0.0770 &  0.0927 &  0.1101 &  0.1293 &  0.1592 &  0.2007 &  0.2534\\
0104 &  0.0214 &  0.0328 &  0.0492 &  0.0720 &  0.1036 &  0.1418 &  0.1913 & &  0.0757 &  0.0912 &  0.1083 &  0.1270 &  0.1565 &  0.1974 &  0.2493\\
0105 &  0.0211 &  0.0324 &  0.0487 &  0.0713 &  0.1026 &  0.1406 &  0.1895 & &  0.0745 &  0.0897 &  0.1065 &  0.1248 &  0.1538 &  0.1941 &  0.2454\\
0106 &  0.0208 &  0.0320 &  0.0482 &  0.0706 &  0.1017 &  0.1394 &  0.1878 & &  0.0733 &  0.0883 &  0.1047 &  0.1227 &  0.1513 &  0.1909 &  0.2415\\
0107 &  0.0205 &  0.0316 &  0.0477 &  0.0699 &  0.1008 &  0.1382 &  0.1861 & &  0.0721 &  0.0869 &  0.1030 &  0.1207 &  0.1488 &  0.1879 &  0.2376\\
0108 &  0.0203 &  0.0311 &  0.0471 &  0.0692 &  0.0999 &  0.1370 &  0.1845 & &  0.0710 &  0.0855 &  0.1014 &  0.1187 &  0.1463 &  0.1849 &  0.2339\\
0109 &  0.0200 &  0.0307 &  0.0466 &  0.0685 &  0.0991 &  0.1359 &  0.1829 & &  0.0698 &  0.0841 &  0.0998 &  0.1167 &  0.1440 &  0.1819 &  0.2303\\
0110 &  0.0197 &  0.0303 &  0.0461 &  0.0679 &  0.0982 &  0.1348 &  0.1814 & &  0.0687 &  0.0828 &  0.0982 &  0.1149 &  0.1417 &  0.1791 &  0.2268\\
0111 &  0.0195 &  0.0299 &  0.0455 &  0.0672 &  0.0974 &  0.1337 &  0.1799 & &  0.0677 &  0.0815 &  0.0967 &  0.1130 &  0.1395 &  0.1764 &  0.2233\\
0112 &  0.0192 &  0.0295 &  0.0450 &  0.0666 &  0.0965 &  0.1327 &  0.1785 & &  0.0666 &  0.0802 &  0.0952 &  0.1113 &  0.1373 &  0.1737 &  0.2200\\
0113 &  0.0190 &  0.0291 &  0.0445 &  0.0659 &  0.0957 &  0.1316 &  0.1771 & &  0.0656 &  0.0790 &  0.0937 &  0.1096 &  0.1353 &  0.1711 &  0.2167\\
0114 &  0.0187 &  0.0288 &  0.0440 &  0.0653 &  0.0949 &  0.1306 &  0.1757 & &  0.0646 &  0.0777 &  0.0923 &  0.1079 &  0.1333 &  0.1686 &  0.2136\\
0115 &  0.0185 &  0.0284 &  0.0435 &  0.0646 &  0.0941 &  0.1295 &  0.1744 & &  0.0636 &  0.0765 &  0.0909 &  0.1063 &  0.1313 &  0.1662 &  0.2105\\
0116 &  0.0183 &  0.0281 &  0.0430 &  0.0640 &  0.0932 &  0.1285 &  0.1730 & &  0.0626 &  0.0754 &  0.0896 &  0.1047 &  0.1294 &  0.1638 &  0.2076\\
0117 &  0.0181 &  0.0278 &  0.0425 &  0.0634 &  0.0924 &  0.1274 &  0.1716 & &  0.0617 &  0.0742 &  0.0882 &  0.1032 &  0.1276 &  0.1616 &  0.2047\\
0118 &  0.0178 &  0.0274 &  0.0421 &  0.0628 &  0.0916 &  0.1264 &  0.1703 & &  0.0607 &  0.0731 &  0.0869 &  0.1017 &  0.1259 &  0.1594 &  0.2020\\
0119 &  0.0176 &  0.0272 &  0.0416 &  0.0622 &  0.0908 &  0.1253 &  0.1689 & &  0.0598 &  0.0720 &  0.0857 &  0.1003 &  0.1242 &  0.1572 &  0.1993\\
0120 &  0.0174 &  0.0269 &  0.0412 &  0.0616 &  0.0901 &  0.1243 &  0.1675 & &  0.0589 &  0.0710 &  0.0845 &  0.0989 &  0.1226 &  0.1552 &  0.1967\\
0121 &  0.0172 &  0.0266 &  0.0408 &  0.0611 &  0.0893 &  0.1232 &  0.1661 & &  0.0580 &  0.0699 &  0.0833 &  0.0976 &  0.1210 &  0.1532 &  0.1942\\
0122 &  0.0171 &  0.0264 &  0.0404 &  0.0606 &  0.0885 &  0.1222 &  0.1647 & &  0.0572 &  0.0689 &  0.0821 &  0.0963 &  0.1195 &  0.1513 &  0.1918\\
0123 &  0.0169 &  0.0261 &  0.0401 &  0.0600 &  0.0878 &  0.1212 &  0.1632 & &  0.0564 &  0.0679 &  0.0810 &  0.0950 &  0.1180 &  0.1495 &  0.1895\\
0124 &  0.0167 &  0.0259 &  0.0397 &  0.0595 &  0.0870 &  0.1201 &  0.1618 & &  0.0555 &  0.0669 &  0.0799 &  0.0938 &  0.1166 &  0.1478 &  0.1872\\
0125 &  0.0165 &  0.0257 &  0.0394 &  0.0591 &  0.0863 &  0.1191 &  0.1604 & &  0.0547 &  0.0660 &  0.0788 &  0.0926 &  0.1152 &  0.1461 &  0.1851\\
0126 &  0.0163 &  0.0255 &  0.0391 &  0.0586 &  0.0856 &  0.1181 &  0.1590 & &  0.0539 &  0.0650 &  0.0777 &  0.0914 &  0.1139 &  0.1444 &  0.1830\\
0127 &  0.0162 &  0.0252 &  0.0388 &  0.0581 &  0.0850 &  0.1171 &  0.1575 & &  0.0532 &  0.0641 &  0.0767 &  0.0903 &  0.1126 &  0.1428 &  0.1810\\
0128 &  0.0160 &  0.0250 &  0.0385 &  0.0577 &  0.0843 &  0.1161 &  0.1561 & &  0.0524 &  0.0632 &  0.0757 &  0.0892 &  0.1113 &  0.1413 &  0.1790\\
0129 &  0.0158 &  0.0248 &  0.0382 &  0.0572 &  0.0836 &  0.1152 &  0.1547 & &  0.0516 &  0.0623 &  0.0747 &  0.0881 &  0.1101 &  0.1398 &  0.1771\\
0130 &  0.0156 &  0.0246 &  0.0379 &  0.0568 &  0.0830 &  0.1142 &  0.1533 & &  0.0509 &  0.0614 &  0.0737 &  0.0870 &  0.1089 &  0.1384 &  0.1753\\
0131 &  0.0155 &  0.0243 &  0.0376 &  0.0564 &  0.0824 &  0.1132 &  0.1519 & &  0.0502 &  0.0606 &  0.0728 &  0.0860 &  0.1077 &  0.1370 &  0.1735\\
0132 &  0.0153 &  0.0241 &  0.0373 &  0.0559 &  0.0817 &  0.1123 &  0.1505 & &  0.0495 &  0.0597 &  0.0718 &  0.0850 &  0.1066 &  0.1357 &  0.1718\\
0133 &  0.0151 &  0.0239 &  0.0369 &  0.0555 &  0.0811 &  0.1113 &  0.1491 & &  0.0488 &  0.0589 &  0.0709 &  0.0840 &  0.1055 &  0.1343 &  0.1701\\
0134 &  0.0150 &  0.0236 &  0.0366 &  0.0550 &  0.0804 &  0.1103 &  0.1477 & &  0.0481 &  0.0581 &  0.0700 &  0.0831 &  0.1044 &  0.1331 &  0.1685\\
0135 &  0.0148 &  0.0233 &  0.0363 &  0.0545 &  0.0798 &  0.1093 &  0.1463 & &  0.0474 &  0.0573 &  0.0691 &  0.0821 &  0.1034 &  0.1318 &  0.1669\\
0136 &  0.0147 &  0.0231 &  0.0360 &  0.0541 &  0.0791 &  0.1083 &  0.1449 & &  0.0467 &  0.0565 &  0.0683 &  0.0812 &  0.1023 &  0.1306 &  0.1654\\
0137 &  0.0145 &  0.0228 &  0.0356 &  0.0535 &  0.0783 &  0.1073 &  0.1435 & &  0.0461 &  0.0558 &  0.0674 &  0.0803 &  0.1013 &  0.1294 &  0.1638\\
0138 &  0.0144 &  0.0225 &  0.0352 &  0.0530 &  0.0776 &  0.1063 &  0.1422 & &  0.0454 &  0.0550 &  0.0665 &  0.0794 &  0.1003 &  0.1282 &  0.1624\\
0139 &  0.0143 &  0.0222 &  0.0349 &  0.0525 &  0.0769 &  0.1053 &  0.1408 & &  0.0448 &  0.0543 &  0.0657 &  0.0785 &  0.0993 &  0.1270 &  0.1609\\
0140 &  0.0142 &  0.0220 &  0.0345 &  0.0519 &  0.0761 &  0.1043 &  0.1394 & &  0.0441 &  0.0535 &  0.0648 &  0.0776 &  0.0983 &  0.1258 &  0.1595\\
0141 &  0.0140 &  0.0217 &  0.0341 &  0.0514 &  0.0753 &  0.1033 &  0.1381 & &  0.0435 &  0.0528 &  0.0640 &  0.0767 &  0.0973 &  0.1247 &  0.1581\\
0142 &  0.0139 &  0.0214 &  0.0337 &  0.0508 &  0.0746 &  0.1023 &  0.1367 & &  0.0429 &  0.0521 &  0.0632 &  0.0758 &  0.0963 &  0.1236 &  0.1567\\
0143 &  0.0138 &  0.0212 &  0.0333 &  0.0502 &  0.0738 &  0.1012 &  0.1354 & &  0.0423 &  0.0514 &  0.0624 &  0.0750 &  0.0954 &  0.1224 &  0.1554\\
0144 &  0.0137 &  0.0210 &  0.0329 &  0.0497 &  0.0730 &  0.1002 &  0.1341 & &  0.0417 &  0.0507 &  0.0616 &  0.0741 &  0.0944 &  0.1213 &  0.1540\\
0145 &  0.0136 &  0.0208 &  0.0325 &  0.0491 &  0.0722 &  0.0992 &  0.1328 & &  0.0411 &  0.0500 &  0.0608 &  0.0733 &  0.0935 &  0.1202 &  0.1527\\
0146 &  0.0135 &  0.0206 &  0.0321 &  0.0486 &  0.0715 &  0.0982 &  0.1315 & &  0.0405 &  0.0493 &  0.0600 &  0.0724 &  0.0925 &  0.1191 &  0.1514\\
0147 &  0.0134 &  0.0204 &  0.0317 &  0.0480 &  0.0707 &  0.0972 &  0.1303 & &  0.0399 &  0.0486 &  0.0592 &  0.0716 &  0.0916 &  0.1180 &  0.1501\\
0148 &  0.0133 &  0.0202 &  0.0314 &  0.0475 &  0.0700 &  0.0962 &  0.1291 & &  0.0394 &  0.0479 &  0.0584 &  0.0707 &  0.0907 &  0.1170 &  0.1489\\
0149 &  0.0132 &  0.0201 &  0.0310 &  0.0470 &  0.0693 &  0.0953 &  0.1279 & &  0.0388 &  0.0473 &  0.0576 &  0.0699 &  0.0898 &  0.1159 &  0.1476\\
0150 &  0.0131 &  0.0199 &  0.0307 &  0.0466 &  0.0686 &  0.0944 &  0.1267 & &  0.0382 &  0.0466 &  0.0568 &  0.0691 &  0.0888 &  0.1148 &  0.1464\\
0151 &  0.0130 &  0.0198 &  0.0305 &  0.0461 &  0.0680 &  0.0935 &  0.1256 & &  0.0377 &  0.0459 &  0.0561 &  0.0682 &  0.0879 &  0.1138 &  0.1451\\
0152 &  0.0129 &  0.0197 &  0.0302 &  0.0457 &  0.0673 &  0.0926 &  0.1244 & &  0.0371 &  0.0453 &  0.0553 &  0.0674 &  0.0870 &  0.1127 &  0.1439\\
0153 &  0.0128 &  0.0196 &  0.0300 &  0.0453 &  0.0667 &  0.0917 &  0.1233 & &  0.0366 &  0.0446 &  0.0545 &  0.0666 &  0.0861 &  0.1117 &  0.1427\\
0154 &  0.0127 &  0.0195 &  0.0298 &  0.0449 &  0.0662 &  0.0909 &  0.1223 & &  0.0360 &  0.0440 &  0.0538 &  0.0658 &  0.0852 &  0.1107 &  0.1415\\
0155 &  0.0126 &  0.0194 &  0.0296 &  0.0446 &  0.0656 &  0.0901 &  0.1212 & &  0.0355 &  0.0434 &  0.0530 &  0.0650 &  0.0843 &  0.1097 &  0.1404\\
0156 &  0.0126 &  0.0193 &  0.0294 &  0.0443 &  0.0651 &  0.0894 &  0.1202 & &  0.0350 &  0.0428 &  0.0523 &  0.0642 &  0.0834 &  0.1087 &  0.1393\\
0157 &  0.0125 &  0.0192 &  0.0293 &  0.0440 &  0.0646 &  0.0886 &  0.1192 & &  0.0344 &  0.0421 &  0.0516 &  0.0634 &  0.0826 &  0.1077 &  0.1381\\
0158 &  0.0124 &  0.0191 &  0.0291 &  0.0437 &  0.0642 &  0.0879 &  0.1182 & &  0.0339 &  0.0415 &  0.0509 &  0.0626 &  0.0817 &  0.1068 &  0.1371\\
0159 &  0.0123 &  0.0190 &  0.0290 &  0.0434 &  0.0637 &  0.0873 &  0.1173 & &  0.0334 &  0.0409 &  0.0502 &  0.0618 &  0.0808 &  0.1059 &  0.1360\\
0160 &  0.0122 &  0.0188 &  0.0289 &  0.0432 &  0.0633 &  0.0866 &  0.1164 & &  0.0329 &  0.0404 &  0.0495 &  0.0611 &  0.0800 &  0.1049 &  0.1350\\
0161 &  0.0121 &  0.0187 &  0.0287 &  0.0430 &  0.0630 &  0.0861 &  0.1155 & &  0.0325 &  0.0398 &  0.0488 &  0.0603 &  0.0792 &  0.1040 &  0.1339\\
0162 &  0.0121 &  0.0186 &  0.0286 &  0.0428 &  0.0626 &  0.0855 &  0.1147 & &  0.0320 &  0.0392 &  0.0481 &  0.0596 &  0.0783 &  0.1032 &  0.1330\\
0163 &  0.0120 &  0.0185 &  0.0285 &  0.0425 &  0.0622 &  0.0850 &  0.1140 & &  0.0315 &  0.0387 &  0.0475 &  0.0589 &  0.0775 &  0.1023 &  0.1320\\
0164 &  0.0119 &  0.0184 &  0.0283 &  0.0423 &  0.0619 &  0.0844 &  0.1132 & &  0.0310 &  0.0381 &  0.0469 &  0.0582 &  0.0767 &  0.1015 &  0.1311\\
0165 &  0.0118 &  0.0182 &  0.0282 &  0.0421 &  0.0616 &  0.0840 &  0.1125 & &  0.0306 &  0.0376 &  0.0462 &  0.0575 &  0.0760 &  0.1006 &  0.1301\\
0166 &  0.0117 &  0.0181 &  0.0280 &  0.0419 &  0.0613 &  0.0835 &  0.1119 & &  0.0301 &  0.0371 &  0.0456 &  0.0569 &  0.0752 &  0.0998 &  0.1293\\
0167 &  0.0116 &  0.0180 &  0.0279 &  0.0417 &  0.0610 &  0.0831 &  0.1113 & &  0.0297 &  0.0366 &  0.0450 &  0.0562 &  0.0745 &  0.0990 &  0.1284\\
0168 &  0.0115 &  0.0179 &  0.0277 &  0.0415 &  0.0607 &  0.0827 &  0.1107 & &  0.0293 &  0.0361 &  0.0444 &  0.0556 &  0.0737 &  0.0982 &  0.1275\\
0169 &  0.0114 &  0.0177 &  0.0276 &  0.0413 &  0.0604 &  0.0823 &  0.1101 & &  0.0289 &  0.0356 &  0.0439 &  0.0550 &  0.0730 &  0.0975 &  0.1267\\
0170 &  0.0113 &  0.0176 &  0.0274 &  0.0412 &  0.0601 &  0.0819 &  0.1096 & &  0.0285 &  0.0351 &  0.0433 &  0.0544 &  0.0723 &  0.0967 &  0.1259\\
0171 &  0.0113 &  0.0175 &  0.0273 &  0.0410 &  0.0599 &  0.0815 &  0.1090 & &  0.0281 &  0.0346 &  0.0428 &  0.0538 &  0.0716 &  0.0960 &  0.1251\\
0172 &  0.0112 &  0.0174 &  0.0272 &  0.0408 &  0.0596 &  0.0812 &  0.1085 & &  0.0277 &  0.0342 &  0.0423 &  0.0532 &  0.0710 &  0.0952 &  0.1243\\
0173 &  0.0111 &  0.0173 &  0.0271 &  0.0407 &  0.0594 &  0.0809 &  0.1080 & &  0.0273 &  0.0338 &  0.0418 &  0.0527 &  0.0703 &  0.0945 &  0.1235\\
0174 &  0.0110 &  0.0172 &  0.0270 &  0.0405 &  0.0592 &  0.0806 &  0.1075 & &  0.0269 &  0.0333 &  0.0413 &  0.0521 &  0.0697 &  0.0938 &  0.1228\\
0175 &  0.0109 &  0.0171 &  0.0269 &  0.0404 &  0.0590 &  0.0803 &  0.1071 & &  0.0266 &  0.0329 &  0.0408 &  0.0516 &  0.0691 &  0.0931 &  0.1220\\
0176 &  0.0109 &  0.0170 &  0.0267 &  0.0402 &  0.0588 &  0.0800 &  0.1066 & &  0.0262 &  0.0325 &  0.0403 &  0.0511 &  0.0685 &  0.0924 &  0.1212\\
0177 &  0.0108 &  0.0169 &  0.0266 &  0.0401 &  0.0586 &  0.0798 &  0.1062 & &  0.0258 &  0.0321 &  0.0399 &  0.0506 &  0.0679 &  0.0918 &  0.1205\\
0178 &  0.0107 &  0.0168 &  0.0265 &  0.0399 &  0.0584 &  0.0795 &  0.1058 & &  0.0255 &  0.0317 &  0.0394 &  0.0502 &  0.0674 &  0.0911 &  0.1198\\
0179 &  0.0107 &  0.0168 &  0.0264 &  0.0398 &  0.0581 &  0.0792 &  0.1054 & &  0.0252 &  0.0313 &  0.0390 &  0.0497 &  0.0668 &  0.0905 &  0.1190\\
0180 &  0.0106 &  0.0167 &  0.0262 &  0.0396 &  0.0579 &  0.0790 &  0.1050 & &  0.0248 &  0.0310 &  0.0386 &  0.0493 &  0.0663 &  0.0898 &  0.1183\\
0181 &  0.0105 &  0.0166 &  0.0261 &  0.0394 &  0.0577 &  0.0787 &  0.1046 & &  0.0245 &  0.0306 &  0.0382 &  0.0489 &  0.0658 &  0.0892 &  0.1176\\
0182 &  0.0104 &  0.0165 &  0.0259 &  0.0392 &  0.0574 &  0.0784 &  0.1042 & &  0.0242 &  0.0302 &  0.0378 &  0.0485 &  0.0652 &  0.0886 &  0.1169\\
0183 &  0.0104 &  0.0163 &  0.0257 &  0.0389 &  0.0571 &  0.0781 &  0.1039 & &  0.0239 &  0.0299 &  0.0374 &  0.0481 &  0.0648 &  0.0880 &  0.1162\\
0184 &  0.0103 &  0.0162 &  0.0255 &  0.0387 &  0.0568 &  0.0778 &  0.1035 & &  0.0236 &  0.0296 &  0.0370 &  0.0477 &  0.0643 &  0.0874 &  0.1155\\
0185 &  0.0102 &  0.0161 &  0.0253 &  0.0384 &  0.0565 &  0.0774 &  0.1032 & &  0.0233 &  0.0292 &  0.0367 &  0.0473 &  0.0638 &  0.0868 &  0.1148\\
0186 &  0.0101 &  0.0160 &  0.0251 &  0.0380 &  0.0561 &  0.0770 &  0.1028 & &  0.0230 &  0.0289 &  0.0363 &  0.0469 &  0.0634 &  0.0862 &  0.1141\\
0187 &  0.0101 &  0.0159 &  0.0249 &  0.0377 &  0.0557 &  0.0767 &  0.1024 & &  0.0228 &  0.0286 &  0.0360 &  0.0466 &  0.0629 &  0.0857 &  0.1135\\
0188 &  0.0100 &  0.0157 &  0.0246 &  0.0373 &  0.0553 &  0.0762 &  0.1021 & &  0.0225 &  0.0283 &  0.0356 &  0.0463 &  0.0625 &  0.0851 &  0.1128\\
0189 &  0.0099 &  0.0156 &  0.0244 &  0.0370 &  0.0549 &  0.0758 &  0.1017 & &  0.0222 &  0.0280 &  0.0353 &  0.0459 &  0.0621 &  0.0846 &  0.1122\\
0190 &  0.0098 &  0.0155 &  0.0242 &  0.0366 &  0.0545 &  0.0754 &  0.1013 & &  0.0220 &  0.0277 &  0.0350 &  0.0456 &  0.0617 &  0.0841 &  0.1116\\
0191 &  0.0098 &  0.0154 &  0.0240 &  0.0363 &  0.0541 &  0.0749 &  0.1009 & &  0.0217 &  0.0274 &  0.0347 &  0.0453 &  0.0613 &  0.0836 &  0.1110\\
0192 &  0.0097 &  0.0153 &  0.0238 &  0.0360 &  0.0537 &  0.0745 &  0.1004 & &  0.0215 &  0.0271 &  0.0344 &  0.0450 &  0.0610 &  0.0831 &  0.1104\\
0193 &  0.0097 &  0.0152 &  0.0236 &  0.0357 &  0.0533 &  0.0740 &  0.1000 & &  0.0212 &  0.0269 &  0.0341 &  0.0447 &  0.0606 &  0.0826 &  0.1098\\
0194 &  0.0096 &  0.0151 &  0.0234 &  0.0354 &  0.0529 &  0.0736 &  0.0995 & &  0.0210 &  0.0266 &  0.0339 &  0.0445 &  0.0603 &  0.0822 &  0.1093\\
0195 &  0.0096 &  0.0150 &  0.0233 &  0.0351 &  0.0525 &  0.0731 &  0.0990 & &  0.0207 &  0.0263 &  0.0336 &  0.0442 &  0.0600 &  0.0817 &  0.1088\\
0196 &  0.0096 &  0.0149 &  0.0232 &  0.0349 &  0.0521 &  0.0727 &  0.0985 & &  0.0205 &  0.0261 &  0.0334 &  0.0440 &  0.0597 &  0.0813 &  0.1083\\
0197 &  0.0096 &  0.0149 &  0.0231 &  0.0347 &  0.0518 &  0.0722 &  0.0980 & &  0.0203 &  0.0258 &  0.0331 &  0.0437 &  0.0594 &  0.0810 &  0.1079\\
0198 &  0.0095 &  0.0148 &  0.0230 &  0.0346 &  0.0514 &  0.0718 &  0.0974 & &  0.0201 &  0.0256 &  0.0329 &  0.0435 &  0.0591 &  0.0806 &  0.1074\\
0199 &  0.0095 &  0.0148 &  0.0229 &  0.0344 &  0.0511 &  0.0714 &  0.0969 & &  0.0199 &  0.0254 &  0.0326 &  0.0433 &  0.0589 &  0.0803 &  0.1071\\
0200 &  0.0095 &  0.0147 &  0.0228 &  0.0343 &  0.0508 &  0.0709 &  0.0965 & &  0.0196 &  0.0251 &  0.0324 &  0.0431 &  0.0586 &  0.0800 &  0.1065\\
0201 &  0.0095 &  0.0147 &  0.0227 &  0.0341 &  0.0505 &  0.0705 &  0.0955 & &  0.0194 &  0.0249 &  0.0322 &  0.0428 &  0.0584 &  0.0797 &  0.1056\\
0202 &  0.0096 &  0.0147 &  0.0227 &  0.0340 &  0.0502 &  0.0700 &  0.0949 & &  0.0192 &  0.0247 &  0.0320 &  0.0426 &  0.0582 &  0.0795 &  0.1047\\
0203 &  0.0096 &  0.0146 &  0.0226 &  0.0339 &  0.0499 &  0.0696 &  0.0945 & &  0.0190 &  0.0244 &  0.0317 &  0.0425 &  0.0580 &  0.0793 &  0.1038\\
0204 &  0.0096 &  0.0146 &  0.0225 &  0.0337 &  0.0495 &  0.0691 &  0.0936 & &  0.0188 &  0.0242 &  0.0315 &  0.0423 &  0.0578 &  0.0791 &  0.1030\\
0205 &  0.0096 &  0.0146 &  0.0225 &  0.0336 &  0.0492 &  0.0687 &  0.0930 & &  0.0186 &  0.0240 &  0.0313 &  0.0421 &  0.0577 &  0.0785 &  0.1021\\
0206 &  0.0096 &  0.0146 &  0.0224 &  0.0335 &  0.0489 &  0.0681 &  0.0926 & &  0.0184 &  0.0238 &  0.0311 &  0.0419 &  0.0575 &  0.0778 &  0.1013\\
0207 &  0.0096 &  0.0145 &  0.0223 &  0.0333 &  0.0486 &  0.0678 &  0.0918 & &  0.0182 &  0.0236 &  0.0309 &  0.0417 &  0.0574 &  0.0772 &  0.1004\\
0208 &  0.0095 &  0.0145 &  0.0223 &  0.0332 &  0.0483 &  0.0674 &  0.0912 & &  0.0180 &  0.0233 &  0.0307 &  0.0416 &  0.0573 &  0.0765 &  0.0996\\
0209 &  0.0095 &  0.0145 &  0.0222 &  0.0331 &  0.0480 &  0.0668 &  0.0909 & &  0.0178 &  0.0231 &  0.0305 &  0.0414 &  0.0572 &  0.0759 &  0.0988\\
0210 &  0.0095 &  0.0145 &  0.0221 &  0.0329 &  0.0477 &  0.0665 &  0.0900 & &  0.0176 &  0.0229 &  0.0303 &  0.0412 &  0.0567 &  0.0753 &  0.0979\\
0211 &  0.0095 &  0.0144 &  0.0220 &  0.0328 &  0.0473 &  0.0661 &  0.0895 & &  0.0174 &  0.0227 &  0.0301 &  0.0411 &  0.0562 &  0.0746 &  0.0971\\
0212 &  0.0095 &  0.0144 &  0.0220 &  0.0327 &  0.0471 &  0.0655 &  0.0892 & &  0.0172 &  0.0225 &  0.0299 &  0.0409 &  0.0558 &  0.0740 &  0.0963\\
0213 &  0.0094 &  0.0144 &  0.0219 &  0.0326 &  0.0468 &  0.0652 &  0.0884 & &  0.0170 &  0.0223 &  0.0297 &  0.0407 &  0.0553 &  0.0734 &  0.0955\\
0214 &  0.0094 &  0.0144 &  0.0218 &  0.0325 &  0.0464 &  0.0648 &  0.0878 & &  0.0168 &  0.0220 &  0.0294 &  0.0406 &  0.0548 &  0.0728 &  0.0947\\
0215 &  0.0094 &  0.0143 &  0.0218 &  0.0323 &  0.0462 &  0.0643 &  0.0875 & &  0.0166 &  0.0218 &  0.0292 &  0.0402 &  0.0544 &  0.0722 &  0.0939\\
0216 &  0.0094 &  0.0143 &  0.0217 &  0.0321 &  0.0459 &  0.0640 &  0.0867 & &  0.0164 &  0.0216 &  0.0290 &  0.0399 &  0.0539 &  0.0716 &  0.0932\\
0217 &  0.0093 &  0.0143 &  0.0216 &  0.0319 &  0.0456 &  0.0636 &  0.0862 & &  0.0161 &  0.0214 &  0.0288 &  0.0395 &  0.0535 &  0.0710 &  0.0924\\
0218 &  0.0093 &  0.0142 &  0.0216 &  0.0317 &  0.0454 &  0.0631 &  0.0859 & &  0.0159 &  0.0211 &  0.0286 &  0.0392 &  0.0530 &  0.0704 &  0.0916\\
0219 &  0.0093 &  0.0142 &  0.0215 &  0.0315 &  0.0451 &  0.0628 &  0.0852 & &  0.0157 &  0.0209 &  0.0284 &  0.0389 &  0.0526 &  0.0699 &  0.0909\\
0220 &  0.0093 &  0.0142 &  0.0214 &  0.0313 &  0.0447 &  0.0624 &  0.0846 & &  0.0155 &  0.0207 &  0.0281 &  0.0385 &  0.0521 &  0.0693 &  0.0901\\
0221 &  0.0093 &  0.0142 &  0.0213 &  0.0312 &  0.0445 &  0.0620 &  0.0843 & &  0.0153 &  0.0204 &  0.0279 &  0.0382 &  0.0517 &  0.0687 &  0.0893\\
0222 &  0.0093 &  0.0142 &  0.0212 &  0.0309 &  0.0442 &  0.0616 &  0.0836 & &  0.0151 &  0.0202 &  0.0276 &  0.0379 &  0.0513 &  0.0681 &  0.0886\\
0223 &  0.0093 &  0.0142 &  0.0211 &  0.0308 &  0.0439 &  0.0613 &  0.0830 & &  0.0149 &  0.0200 &  0.0274 &  0.0376 &  0.0509 &  0.0676 &  0.0879\\
0224 &  0.0093 &  0.0142 &  0.0210 &  0.0306 &  0.0436 &  0.0609 &  0.0827 & &  0.0147 &  0.0197 &  0.0271 &  0.0373 &  0.0504 &  0.0670 &  0.0871\\
0225 &  0.0093 &  0.0141 &  0.0208 &  0.0304 &  0.0434 &  0.0605 &  0.0821 & &  0.0145 &  0.0195 &  0.0269 &  0.0369 &  0.0500 &  0.0665 &  0.0864\\
0226 &  0.0093 &  0.0141 &  0.0207 &  0.0302 &  0.0431 &  0.0601 &  0.0815 & &  0.0143 &  0.0193 &  0.0267 &  0.0366 &  0.0496 &  0.0659 &  0.0857\\
0227 &  0.0093 &  0.0140 &  0.0206 &  0.0300 &  0.0428 &  0.0598 &  0.0812 & &  0.0141 &  0.0192 &  0.0264 &  0.0363 &  0.0492 &  0.0654 &  0.0850\\
0228 &  0.0093 &  0.0139 &  0.0205 &  0.0298 &  0.0426 &  0.0594 &  0.0806 & &  0.0139 &  0.0190 &  0.0262 &  0.0360 &  0.0488 &  0.0649 &  0.0842\\
0229 &  0.0093 &  0.0138 &  0.0204 &  0.0296 &  0.0423 &  0.0590 &  0.0800 & &  0.0137 &  0.0188 &  0.0260 &  0.0357 &  0.0484 &  0.0643 &  0.0835\\
0230 &  0.0093 &  0.0138 &  0.0202 &  0.0294 &  0.0421 &  0.0587 &  0.0797 & &  0.0135 &  0.0186 &  0.0258 &  0.0354 &  0.0480 &  0.0638 &  0.0828\\
0231 &  0.0093 &  0.0137 &  0.0201 &  0.0292 &  0.0418 &  0.0583 &  0.0791 & &  0.0133 &  0.0185 &  0.0255 &  0.0351 &  0.0476 &  0.0633 &  0.0821\\
0232 &  0.0093 &  0.0136 &  0.0200 &  0.0291 &  0.0415 &  0.0580 &  0.0785 & &  0.0132 &  0.0183 &  0.0253 &  0.0348 &  0.0472 &  0.0628 &  0.0815\\
0233 &  0.0092 &  0.0136 &  0.0199 &  0.0289 &  0.0413 &  0.0576 &  0.0782 & &  0.0131 &  0.0181 &  0.0251 &  0.0345 &  0.0468 &  0.0622 &  0.0808\\
0234 &  0.0092 &  0.0135 &  0.0197 &  0.0287 &  0.0411 &  0.0572 &  0.0776 & &  0.0130 &  0.0180 &  0.0249 &  0.0342 &  0.0465 &  0.0617 &  0.0801\\
0235 &  0.0091 &  0.0134 &  0.0196 &  0.0285 &  0.0408 &  0.0569 &  0.0771 & &  0.0129 &  0.0178 &  0.0247 &  0.0340 &  0.0461 &  0.0612 &  0.0794\\
0236 &  0.0091 &  0.0133 &  0.0195 &  0.0284 &  0.0406 &  0.0566 &  0.0768 & &  0.0127 &  0.0177 &  0.0244 &  0.0337 &  0.0457 &  0.0607 &  0.0787\\
0237 &  0.0090 &  0.0132 &  0.0193 &  0.0281 &  0.0403 &  0.0562 &  0.0763 & &  0.0126 &  0.0175 &  0.0242 &  0.0334 &  0.0453 &  0.0602 &  0.0781\\
0238 &  0.0090 &  0.0131 &  0.0192 &  0.0280 &  0.0401 &  0.0558 &  0.0757 & &  0.0125 &  0.0173 &  0.0240 &  0.0331 &  0.0450 &  0.0597 &  0.0774\\
0239 &  0.0089 &  0.0131 &  0.0191 &  0.0278 &  0.0398 &  0.0555 &  0.0754 & &  0.0124 &  0.0172 &  0.0238 &  0.0329 &  0.0446 &  0.0592 &  0.0768\\
0240 &  0.0089 &  0.0130 &  0.0189 &  0.0276 &  0.0396 &  0.0552 &  0.0749 & &  0.0123 &  0.0170 &  0.0236 &  0.0326 &  0.0442 &  0.0587 &  0.0761\\
0241 &  0.0088 &  0.0129 &  0.0188 &  0.0275 &  0.0393 &  0.0548 &  0.0744 & &  0.0122 &  0.0169 &  0.0234 &  0.0323 &  0.0439 &  0.0582 &  0.0755\\
0242 &  0.0088 &  0.0128 &  0.0187 &  0.0273 &  0.0391 &  0.0545 &  0.0741 & &  0.0120 &  0.0167 &  0.0232 &  0.0320 &  0.0435 &  0.0577 &  0.0749\\
0243 &  0.0087 &  0.0127 &  0.0186 &  0.0271 &  0.0389 &  0.0542 &  0.0736 & &  0.0119 &  0.0166 &  0.0230 &  0.0318 &  0.0431 &  0.0572 &  0.0742\\
0244 &  0.0087 &  0.0126 &  0.0185 &  0.0270 &  0.0386 &  0.0539 &  0.0731 & &  0.0118 &  0.0164 &  0.0228 &  0.0315 &  0.0428 &  0.0568 &  0.0736\\
0245 &  0.0086 &  0.0125 &  0.0184 &  0.0269 &  0.0384 &  0.0536 &  0.0728 & &  0.0117 &  0.0163 &  0.0226 &  0.0313 &  0.0424 &  0.0563 &  0.0730\\
0246 &  0.0086 &  0.0124 &  0.0182 &  0.0267 &  0.0382 &  0.0533 &  0.0724 & &  0.0116 &  0.0161 &  0.0224 &  0.0310 &  0.0421 &  0.0558 &  0.0724\\
0247 &  0.0085 &  0.0123 &  0.0181 &  0.0265 &  0.0379 &  0.0529 &  0.0719 & &  0.0115 &  0.0160 &  0.0222 &  0.0307 &  0.0417 &  0.0553 &  0.0718\\
0248 &  0.0084 &  0.0123 &  0.0180 &  0.0264 &  0.0377 &  0.0527 &  0.0716 & &  0.0114 &  0.0158 &  0.0220 &  0.0305 &  0.0414 &  0.0549 &  0.0712\\
0249 &  0.0084 &  0.0122 &  0.0179 &  0.0262 &  0.0375 &  0.0524 &  0.0712 & &  0.0113 &  0.0157 &  0.0218 &  0.0302 &  0.0410 &  0.0544 &  0.0706\\
0250 &  0.0083 &  0.0121 &  0.0178 &  0.0260 &  0.0373 &  0.0520 &  0.0707 & &  0.0112 &  0.0155 &  0.0217 &  0.0300 &  0.0407 &  0.0540 &  0.0701\\
0251 &  0.0083 &  0.0120 &  0.0177 &  0.0259 &  0.0371 &  0.0518 &  0.0704 & &  0.0110 &  0.0154 &  0.0215 &  0.0297 &  0.0403 &  0.0535 &  0.0695\\
0252 &  0.0082 &  0.0120 &  0.0176 &  0.0257 &  0.0368 &  0.0515 &  0.0701 & &  0.0109 &  0.0153 &  0.0213 &  0.0295 &  0.0400 &  0.0530 &  0.0689\\
0253 &  0.0081 &  0.0119 &  0.0175 &  0.0256 &  0.0366 &  0.0512 &  0.0696 & &  0.0108 &  0.0151 &  0.0211 &  0.0292 &  0.0396 &  0.0526 &  0.0684\\
0254 &  0.0081 &  0.0118 &  0.0174 &  0.0254 &  0.0365 &  0.0509 &  0.0693 & &  0.0107 &  0.0150 &  0.0209 &  0.0290 &  0.0393 &  0.0521 &  0.0678\\
0255 &  0.0080 &  0.0117 &  0.0173 &  0.0253 &  0.0362 &  0.0506 &  0.0690 & &  0.0106 &  0.0149 &  0.0207 &  0.0287 &  0.0389 &  0.0517 &  0.0673\\
0256 &  0.0080 &  0.0116 &  0.0172 &  0.0251 &  0.0360 &  0.0503 &  0.0685 & &  0.0105 &  0.0147 &  0.0206 &  0.0285 &  0.0386 &  0.0513 &  0.0667\\
0257 &  0.0079 &  0.0116 &  0.0171 &  0.0250 &  0.0358 &  0.0501 &  0.0683 & &  0.0104 &  0.0146 &  0.0204 &  0.0282 &  0.0383 &  0.0508 &  0.0662\\
0258 &  0.0079 &  0.0115 &  0.0170 &  0.0248 &  0.0356 &  0.0498 &  0.0679 & &  0.0103 &  0.0145 &  0.0202 &  0.0280 &  0.0379 &  0.0504 &  0.0657\\
0259 &  0.0078 &  0.0114 &  0.0169 &  0.0247 &  0.0354 &  0.0495 &  0.0674 & &  0.0102 &  0.0143 &  0.0200 &  0.0277 &  0.0376 &  0.0500 &  0.0652\\
0260 &  0.0078 &  0.0114 &  0.0168 &  0.0245 &  0.0352 &  0.0493 &  0.0672 & &  0.0101 &  0.0142 &  0.0198 &  0.0275 &  0.0373 &  0.0495 &  0.0646\\
0261 &  0.0077 &  0.0113 &  0.0167 &  0.0244 &  0.0350 &  0.0490 &  0.0669 & &  0.0100 &  0.0141 &  0.0197 &  0.0272 &  0.0369 &  0.0491 &  0.0641\\
0262 &  0.0077 &  0.0112 &  0.0166 &  0.0243 &  0.0348 &  0.0487 &  0.0664 & &  0.0099 &  0.0139 &  0.0195 &  0.0270 &  0.0366 &  0.0487 &  0.0636\\
0263 &  0.0076 &  0.0112 &  0.0165 &  0.0241 &  0.0347 &  0.0486 &  0.0661 & &  0.0098 &  0.0138 &  0.0193 &  0.0267 &  0.0363 &  0.0483 &  0.0631\\
0264 &  0.0076 &  0.0111 &  0.0164 &  0.0240 &  0.0345 &  0.0483 &  0.0659 & &  0.0097 &  0.0137 &  0.0191 &  0.0265 &  0.0359 &  0.0479 &  0.0626\\
0265 &  0.0075 &  0.0110 &  0.0163 &  0.0239 &  0.0343 &  0.0480 &  0.0653 & &  0.0096 &  0.0135 &  0.0189 &  0.0262 &  0.0356 &  0.0475 &  0.0621\\
0266 &  0.0075 &  0.0110 &  0.0162 &  0.0237 &  0.0341 &  0.0478 &  0.0651 & &  0.0095 &  0.0134 &  0.0188 &  0.0260 &  0.0353 &  0.0471 &  0.0616\\
0267 &  0.0074 &  0.0109 &  0.0161 &  0.0236 &  0.0339 &  0.0476 &  0.0648 & &  0.0095 &  0.0133 &  0.0186 &  0.0257 &  0.0350 &  0.0467 &  0.0611\\
0268 &  0.0074 &  0.0108 &  0.0160 &  0.0235 &  0.0337 &  0.0473 &  0.0643 & &  0.0094 &  0.0132 &  0.0184 &  0.0255 &  0.0347 &  0.0463 &  0.0606\\
0269 &  0.0073 &  0.0108 &  0.0159 &  0.0233 &  0.0336 &  0.0470 &  0.0640 & &  0.0093 &  0.0130 &  0.0182 &  0.0252 &  0.0343 &  0.0459 &  0.0601\\
0270 &  0.0073 &  0.0107 &  0.0158 &  0.0232 &  0.0334 &  0.0468 &  0.0637 & &  0.0092 &  0.0129 &  0.0180 &  0.0250 &  0.0340 &  0.0455 &  0.0596\\
0271 &  0.0072 &  0.0106 &  0.0157 &  0.0231 &  0.0332 &  0.0465 &  0.0632 & &  0.0091 &  0.0128 &  0.0179 &  0.0248 &  0.0337 &  0.0451 &  0.0592\\
0272 &  0.0072 &  0.0106 &  0.0157 &  0.0230 &  0.0331 &  0.0463 &  0.0629 & &  0.0090 &  0.0127 &  0.0177 &  0.0245 &  0.0334 &  0.0447 &  0.0587\\
0273 &  0.0072 &  0.0105 &  0.0156 &  0.0229 &  0.0329 &  0.0461 &  0.0627 & &  0.0089 &  0.0125 &  0.0175 &  0.0243 &  0.0331 &  0.0443 &  0.0582\\
0274 &  0.0071 &  0.0105 &  0.0155 &  0.0227 &  0.0327 &  0.0457 &  0.0621 & &  0.0088 &  0.0124 &  0.0173 &  0.0240 &  0.0328 &  0.0439 &  0.0577\\
0275 &  0.0071 &  0.0104 &  0.0154 &  0.0226 &  0.0326 &  0.0455 &  0.0618 & &  0.0087 &  0.0123 &  0.0172 &  0.0238 &  0.0325 &  0.0436 &  0.0573\\
0276 &  0.0070 &  0.0104 &  0.0153 &  0.0225 &  0.0324 &  0.0453 &  0.0616 & &  0.0086 &  0.0121 &  0.0170 &  0.0236 &  0.0322 &  0.0432 &  0.0568\\
0277 &  0.0070 &  0.0103 &  0.0153 &  0.0224 &  0.0322 &  0.0450 &  0.0610 & &  0.0085 &  0.0120 &  0.0168 &  0.0233 &  0.0319 &  0.0428 &  0.0563\\
0278 &  0.0069 &  0.0102 &  0.0152 &  0.0222 &  0.0320 &  0.0447 &  0.0607 & &  0.0085 &  0.0119 &  0.0166 &  0.0231 &  0.0316 &  0.0424 &  0.0559\\
0279 &  0.0069 &  0.0102 &  0.0151 &  0.0222 &  0.0319 &  0.0445 &  0.0605 & &  0.0084 &  0.0118 &  0.0164 &  0.0229 &  0.0313 &  0.0421 &  0.0554\\
0280 &  0.0069 &  0.0101 &  0.0150 &  0.0220 &  0.0316 &  0.0442 &  0.0599 & &  0.0083 &  0.0116 &  0.0163 &  0.0226 &  0.0310 &  0.0417 &  0.0549\\
0281 &  0.0068 &  0.0101 &  0.0149 &  0.0219 &  0.0315 &  0.0439 &  0.0596 & &  0.0082 &  0.0115 &  0.0161 &  0.0224 &  0.0307 &  0.0413 &  0.0545\\
0282 &  0.0068 &  0.0100 &  0.0148 &  0.0218 &  0.0313 &  0.0437 &  0.0595 & &  0.0081 &  0.0114 &  0.0159 &  0.0222 &  0.0304 &  0.0410 &  0.0540\\
0283 &  0.0067 &  0.0100 &  0.0148 &  0.0217 &  0.0311 &  0.0435 &  0.0589 & &  0.0080 &  0.0112 &  0.0158 &  0.0220 &  0.0301 &  0.0406 &  0.0536\\
0284 &  0.0067 &  0.0099 &  0.0147 &  0.0215 &  0.0310 &  0.0432 &  0.0586 & &  0.0079 &  0.0111 &  0.0156 &  0.0217 &  0.0299 &  0.0403 &  0.0531\\
0285 &  0.0066 &  0.0099 &  0.0146 &  0.0215 &  0.0308 &  0.0430 &  0.0585 & &  0.0078 &  0.0110 &  0.0154 &  0.0215 &  0.0296 &  0.0399 &  0.0527\\
0286 &  0.0066 &  0.0098 &  0.0145 &  0.0213 &  0.0306 &  0.0428 &  0.0579 & &  0.0077 &  0.0109 &  0.0152 &  0.0213 &  0.0293 &  0.0396 &  0.0522\\
0287 &  0.0066 &  0.0097 &  0.0145 &  0.0212 &  0.0304 &  0.0425 &  0.0576 & &  0.0076 &  0.0107 &  0.0151 &  0.0211 &  0.0290 &  0.0393 &  0.0518\\
0288 &  0.0065 &  0.0097 &  0.0143 &  0.0211 &  0.0303 &  0.0423 &  0.0575 & &  0.0075 &  0.0106 &  0.0149 &  0.0209 &  0.0288 &  0.0389 &  0.0513\\
0289 &  0.0065 &  0.0096 &  0.0143 &  0.0210 &  0.0300 &  0.0421 &  0.0569 & &  0.0075 &  0.0105 &  0.0148 &  0.0207 &  0.0285 &  0.0386 &  0.0509\\
0290 &  0.0065 &  0.0096 &  0.0142 &  0.0208 &  0.0299 &  0.0418 &  0.0566 & &  0.0074 &  0.0104 &  0.0146 &  0.0205 &  0.0283 &  0.0383 &  0.0505\\
0291 &  0.0064 &  0.0096 &  0.0141 &  0.0208 &  0.0298 &  0.0416 &  0.0565 & &  0.0073 &  0.0102 &  0.0144 &  0.0202 &  0.0280 &  0.0379 &  0.0500\\
0292 &  0.0064 &  0.0095 &  0.0141 &  0.0207 &  0.0295 &  0.0414 &  0.0559 & &  0.0072 &  0.0101 &  0.0143 &  0.0200 &  0.0277 &  0.0376 &  0.0496\\
0293 &  0.0064 &  0.0094 &  0.0140 &  0.0205 &  0.0295 &  0.0411 &  0.0556 & &  0.0071 &  0.0100 &  0.0141 &  0.0198 &  0.0275 &  0.0373 &  0.0492\\
0294 &  0.0063 &  0.0094 &  0.0139 &  0.0204 &  0.0293 &  0.0409 &  0.0556 & &  0.0070 &  0.0099 &  0.0140 &  0.0196 &  0.0272 &  0.0370 &  0.0488\\
0295 &  0.0063 &  0.0093 &  0.0139 &  0.0203 &  0.0291 &  0.0407 &  0.0550 & &  0.0069 &  0.0098 &  0.0138 &  0.0195 &  0.0270 &  0.0367 &  0.0483\\
0296 &  0.0063 &  0.0093 &  0.0138 &  0.0201 &  0.0290 &  0.0405 &  0.0547 & &  0.0068 &  0.0097 &  0.0137 &  0.0193 &  0.0268 &  0.0364 &  0.0479\\
0297 &  0.0062 &  0.0093 &  0.0137 &  0.0201 &  0.0288 &  0.0403 &  0.0546 & &  0.0068 &  0.0095 &  0.0135 &  0.0191 &  0.0265 &  0.0360 &  0.0475\\
0298 &  0.0062 &  0.0092 &  0.0137 &  0.0200 &  0.0286 &  0.0401 &  0.0540 & &  0.0067 &  0.0094 &  0.0134 &  0.0189 &  0.0263 &  0.0357 &  0.0471\\
0299 &  0.0062 &  0.0091 &  0.0136 &  0.0198 &  0.0285 &  0.0398 &  0.0537 & &  0.0066 &  0.0093 &  0.0132 &  0.0187 &  0.0261 &  0.0355 &  0.0467\\
0300 &  0.0061 &  0.0091 &  0.0135 &  0.0198 &  0.0284 &  0.0396 &  0.0537 & &  0.0065 &  0.0092 &  0.0131 &  0.0185 &  0.0258 &  0.0352 &  0.0463\\
0301 &  0.0061 &  0.0091 &  0.0135 &  0.0197 &  0.0282 &  0.0395 &  0.0531 & &  0.0064 &  0.0091 &  0.0129 &  0.0183 &  0.0256 &  0.0349 &  0.0459\\
0302 &  0.0061 &  0.0090 &  0.0134 &  0.0195 &  0.0281 &  0.0392 &  0.0528 & &  0.0064 &  0.0090 &  0.0128 &  0.0182 &  0.0254 &  0.0346 &  0.0455\\
0303 &  0.0060 &  0.0090 &  0.0133 &  0.0195 &  0.0279 &  0.0390 &  0.0528 & &  0.0063 &  0.0089 &  0.0127 &  0.0180 &  0.0252 &  0.0343 &  0.0452\\
0304 &  0.0060 &  0.0090 &  0.0132 &  0.0194 &  0.0277 &  0.0389 &  0.0523 & &  0.0062 &  0.0088 &  0.0125 &  0.0178 &  0.0250 &  0.0340 &  0.0448\\
0305 &  0.0060 &  0.0089 &  0.0132 &  0.0192 &  0.0277 &  0.0386 &  0.0520 & &  0.0061 &  0.0087 &  0.0124 &  0.0177 &  0.0248 &  0.0337 &  0.0444\\
0306 &  0.0059 &  0.0089 &  0.0131 &  0.0191 &  0.0275 &  0.0384 &  0.0520 & &  0.0060 &  0.0086 &  0.0123 &  0.0175 &  0.0245 &  0.0335 &  0.0440\\
0307 &  0.0059 &  0.0088 &  0.0130 &  0.0190 &  0.0273 &  0.0383 &  0.0514 & &  0.0060 &  0.0085 &  0.0121 &  0.0173 &  0.0243 &  0.0332 &  0.0437\\
0308 &  0.0059 &  0.0088 &  0.0129 &  0.0189 &  0.0273 &  0.0380 &  0.0511 & &  0.0059 &  0.0084 &  0.0120 &  0.0172 &  0.0241 &  0.0329 &  0.0433\\
0309 &  0.0059 &  0.0088 &  0.0129 &  0.0188 &  0.0271 &  0.0378 &  0.0511 & &  0.0058 &  0.0083 &  0.0119 &  0.0170 &  0.0239 &  0.0327 &  0.0430\\
0310 &  0.0059 &  0.0087 &  0.0128 &  0.0187 &  0.0269 &  0.0377 &  0.0506 & &  0.0058 &  0.0082 &  0.0118 &  0.0169 &  0.0237 &  0.0324 &  0.0426\\
0311 &  0.0059 &  0.0087 &  0.0127 &  0.0186 &  0.0268 &  0.0374 &  0.0503 & &  0.0057 &  0.0081 &  0.0117 &  0.0167 &  0.0236 &  0.0321 &  0.0423\\
0312 &  0.0058 &  0.0086 &  0.0126 &  0.0185 &  0.0267 &  0.0372 &  0.0503 & &  0.0056 &  0.0080 &  0.0115 &  0.0166 &  0.0234 &  0.0319 &  0.0419\\
0313 &  0.0058 &  0.0086 &  0.0125 &  0.0184 &  0.0265 &  0.0371 &  0.0498 & &  0.0056 &  0.0079 &  0.0114 &  0.0164 &  0.0232 &  0.0316 &  0.0416\\
0314 &  0.0058 &  0.0085 &  0.0125 &  0.0183 &  0.0264 &  0.0368 &  0.0495 & &  0.0055 &  0.0078 &  0.0113 &  0.0163 &  0.0230 &  0.0314 &  0.0412\\
0315 &  0.0058 &  0.0085 &  0.0124 &  0.0182 &  0.0263 &  0.0366 &  0.0495 & &  0.0054 &  0.0078 &  0.0112 &  0.0161 &  0.0228 &  0.0311 &  0.0409\\
0316 &  0.0058 &  0.0084 &  0.0123 &  0.0181 &  0.0261 &  0.0365 &  0.0490 & &  0.0054 &  0.0077 &  0.0111 &  0.0160 &  0.0226 &  0.0309 &  0.0406\\
0317 &  0.0057 &  0.0083 &  0.0122 &  0.0180 &  0.0261 &  0.0362 &  0.0487 & &  0.0053 &  0.0076 &  0.0110 &  0.0158 &  0.0224 &  0.0306 &  0.0402\\
0318 &  0.0057 &  0.0083 &  0.0122 &  0.0179 &  0.0259 &  0.0360 &  0.0487 & &  0.0052 &  0.0075 &  0.0108 &  0.0157 &  0.0222 &  0.0304 &  0.0399\\
0319 &  0.0057 &  0.0082 &  0.0121 &  0.0179 &  0.0257 &  0.0359 &  0.0483 & &  0.0052 &  0.0074 &  0.0107 &  0.0156 &  0.0221 &  0.0301 &  0.0396\\
0320 &  0.0056 &  0.0082 &  0.0120 &  0.0177 &  0.0257 &  0.0357 &  0.0480 & &  0.0051 &  0.0073 &  0.0106 &  0.0154 &  0.0219 &  0.0299 &  0.0393\\
0321 &  0.0056 &  0.0081 &  0.0119 &  0.0177 &  0.0255 &  0.0354 &  0.0480 & &  0.0050 &  0.0072 &  0.0105 &  0.0153 &  0.0217 &  0.0296 &  0.0390\\
0322 &  0.0056 &  0.0081 &  0.0118 &  0.0176 &  0.0253 &  0.0353 &  0.0476 & &  0.0050 &  0.0072 &  0.0104 &  0.0152 &  0.0215 &  0.0294 &  0.0387\\
0323 &  0.0055 &  0.0080 &  0.0118 &  0.0175 &  0.0253 &  0.0351 &  0.0474 & &  0.0049 &  0.0071 &  0.0103 &  0.0150 &  0.0213 &  0.0291 &  0.0384\\
0324 &  0.0055 &  0.0079 &  0.0117 &  0.0174 &  0.0251 &  0.0348 &  0.0474 & &  0.0049 &  0.0070 &  0.0102 &  0.0149 &  0.0212 &  0.0289 &  0.0380\\
0325 &  0.0054 &  0.0079 &  0.0116 &  0.0173 &  0.0249 &  0.0347 &  0.0470 & &  0.0048 &  0.0069 &  0.0101 &  0.0147 &  0.0210 &  0.0286 &  0.0377\\
0326 &  0.0054 &  0.0078 &  0.0115 &  0.0172 &  0.0248 &  0.0345 &  0.0468 & &  0.0048 &  0.0068 &  0.0100 &  0.0146 &  0.0208 &  0.0284 &  0.0374\\
0327 &  0.0054 &  0.0078 &  0.0115 &  0.0171 &  0.0247 &  0.0342 &  0.0468 & &  0.0047 &  0.0067 &  0.0099 &  0.0145 &  0.0206 &  0.0281 &  0.0371\\
0328 &  0.0053 &  0.0077 &  0.0114 &  0.0170 &  0.0245 &  0.0341 &  0.0465 & &  0.0046 &  0.0067 &  0.0098 &  0.0144 &  0.0204 &  0.0279 &  0.0368\\
0329 &  0.0053 &  0.0076 &  0.0113 &  0.0169 &  0.0244 &  0.0339 &  0.0462 & &  0.0046 &  0.0066 &  0.0097 &  0.0142 &  0.0202 &  0.0277 &  0.0366\\
0330 &  0.0052 &  0.0076 &  0.0113 &  0.0169 &  0.0243 &  0.0337 &  0.0462 & &  0.0045 &  0.0065 &  0.0095 &  0.0141 &  0.0201 &  0.0274 &  0.0363\\
0331 &  0.0051 &  0.0075 &  0.0112 &  0.0168 &  0.0241 &  0.0336 &  0.0459 & &  0.0045 &  0.0064 &  0.0094 &  0.0140 &  0.0199 &  0.0272 &  0.0360\\
0332 &  0.0051 &  0.0074 &  0.0111 &  0.0167 &  0.0240 &  0.0334 &  0.0457 & &  0.0044 &  0.0063 &  0.0093 &  0.0138 &  0.0197 &  0.0269 &  0.0357\\
0333 &  0.0051 &  0.0074 &  0.0111 &  0.0166 &  0.0239 &  0.0332 &  0.0457 & &  0.0043 &  0.0062 &  0.0092 &  0.0137 &  0.0195 &  0.0267 &  0.0354\\
0334 &  0.0050 &  0.0073 &  0.0110 &  0.0165 &  0.0237 &  0.0331 &  0.0454 & &  0.0043 &  0.0061 &  0.0091 &  0.0136 &  0.0193 &  0.0265 &  0.0351\\
0335 &  0.0050 &  0.0072 &  0.0110 &  0.0164 &  0.0236 &  0.0329 &  0.0451 & &  0.0042 &  0.0061 &  0.0090 &  0.0134 &  0.0192 &  0.0262 &  0.0348\\
0336 &  0.0049 &  0.0072 &  0.0109 &  0.0163 &  0.0234 &  0.0327 &  0.0451 & &  0.0041 &  0.0060 &  0.0089 &  0.0133 &  0.0190 &  0.0260 &  0.0346\\
0337 &  0.0049 &  0.0071 &  0.0109 &  0.0163 &  0.0233 &  0.0326 &  0.0449 & &  0.0041 &  0.0059 &  0.0088 &  0.0132 &  0.0188 &  0.0258 &  0.0343\\
0338 &  0.0048 &  0.0071 &  0.0108 &  0.0162 &  0.0232 &  0.0325 &  0.0446 & &  0.0040 &  0.0058 &  0.0087 &  0.0130 &  0.0186 &  0.0255 &  0.0340\\
0339 &  0.0048 &  0.0070 &  0.0108 &  0.0161 &  0.0231 &  0.0323 &  0.0446 & &  0.0039 &  0.0057 &  0.0086 &  0.0129 &  0.0184 &  0.0253 &  0.0338\\
0340 &  0.0047 &  0.0070 &  0.0107 &  0.0160 &  0.0229 &  0.0322 &  0.0444 & &  0.0039 &  0.0056 &  0.0085 &  0.0128 &  0.0182 &  0.0251 &  0.0335\\
0341 &  0.0047 &  0.0069 &  0.0106 &  0.0159 &  0.0228 &  0.0320 &  0.0441 & &  0.0038 &  0.0056 &  0.0084 &  0.0126 &  0.0181 &  0.0249 &  0.0332\\
0342 &  0.0046 &  0.0069 &  0.0106 &  0.0158 &  0.0227 &  0.0319 &  0.0440 & &  0.0038 &  0.0055 &  0.0083 &  0.0125 &  0.0179 &  0.0247 &  0.0330\\
0343 &  0.0046 &  0.0068 &  0.0106 &  0.0158 &  0.0226 &  0.0317 &  0.0438 & &  0.0037 &  0.0054 &  0.0082 &  0.0124 &  0.0177 &  0.0244 &  0.0327\\
0344 &  0.0045 &  0.0068 &  0.0105 &  0.0157 &  0.0225 &  0.0316 &  0.0435 & &  0.0036 &  0.0053 &  0.0081 &  0.0122 &  0.0175 &  0.0242 &  0.0325\\
0345 &  0.0045 &  0.0068 &  0.0105 &  0.0156 &  0.0223 &  0.0315 &  0.0435 & &  0.0036 &  0.0052 &  0.0080 &  0.0121 &  0.0174 &  0.0240 &  0.0322\\
0346 &  0.0044 &  0.0067 &  0.0104 &  0.0155 &  0.0222 &  0.0314 &  0.0432 & &  0.0035 &  0.0052 &  0.0079 &  0.0120 &  0.0172 &  0.0238 &  0.0320\\
0347 &  0.0044 &  0.0067 &  0.0104 &  0.0154 &  0.0221 &  0.0313 &  0.0429 & &  0.0034 &  0.0051 &  0.0079 &  0.0118 &  0.0170 &  0.0236 &  0.0318\\
0348 &  0.0044 &  0.0067 &  0.0104 &  0.0153 &  0.0220 &  0.0311 &  0.0429 & &  0.0034 &  0.0050 &  0.0078 &  0.0117 &  0.0169 &  0.0234 &  0.0315\\
0349 &  0.0043 &  0.0067 &  0.0103 &  0.0153 &  0.0219 &  0.0310 &  0.0427 & &  0.0033 &  0.0049 &  0.0077 &  0.0116 &  0.0167 &  0.0232 &  0.0313\\
0350 &  0.0043 &  0.0066 &  0.0103 &  0.0152 &  0.0218 &  0.0309 &  0.0423 & &  0.0032 &  0.0049 &  0.0076 &  0.0114 &  0.0165 &  0.0230 &  0.0311\\
0351 &  0.0043 &  0.0066 &  0.0103 &  0.0151 &  0.0217 &  0.0308 &  0.0422 & &  0.0032 &  0.0048 &  0.0075 &  0.0113 &  0.0164 &  0.0228 &  0.0308\\
0352 &  0.0042 &  0.0066 &  0.0102 &  0.0150 &  0.0216 &  0.0306 &  0.0421 & &  0.0031 &  0.0047 &  0.0074 &  0.0112 &  0.0162 &  0.0226 &  0.0306\\
0353 &  0.0042 &  0.0066 &  0.0102 &  0.0150 &  0.0215 &  0.0305 &  0.0417 & &  0.0031 &  0.0046 &  0.0073 &  0.0111 &  0.0160 &  0.0224 &  0.0304\\
0354 &  0.0042 &  0.0066 &  0.0101 &  0.0148 &  0.0214 &  0.0304 &  0.0416 & &  0.0030 &  0.0046 &  0.0072 &  0.0109 &  0.0159 &  0.0223 &  0.0302\\
0355 &  0.0042 &  0.0066 &  0.0101 &  0.0148 &  0.0213 &  0.0302 &  0.0414 & &  0.0029 &  0.0045 &  0.0071 &  0.0108 &  0.0157 &  0.0221 &  0.0300\\
0356 &  0.0041 &  0.0065 &  0.0100 &  0.0147 &  0.0213 &  0.0301 &  0.0411 & &  0.0029 &  0.0044 &  0.0070 &  0.0107 &  0.0156 &  0.0219 &  0.0297\\
0357 &  0.0041 &  0.0065 &  0.0100 &  0.0146 &  0.0211 &  0.0300 &  0.0410 & &  0.0028 &  0.0044 &  0.0069 &  0.0106 &  0.0154 &  0.0217 &  0.0295\\
0358 &  0.0041 &  0.0065 &  0.0100 &  0.0146 &  0.0210 &  0.0298 &  0.0408 & &  0.0028 &  0.0043 &  0.0068 &  0.0105 &  0.0153 &  0.0216 &  0.0293\\
0359 &  0.0041 &  0.0065 &  0.0099 &  0.0145 &  0.0210 &  0.0297 &  0.0404 & &  0.0027 &  0.0042 &  0.0068 &  0.0103 &  0.0152 &  0.0214 &  0.0291\\
0360 &  0.0041 &  0.0065 &  0.0099 &  0.0144 &  0.0209 &  0.0296 &  0.0404 & &  0.0027 &  0.0042 &  0.0067 &  0.0102 &  0.0150 &  0.0212 &  0.0289\\
0361 &  0.0041 &  0.0065 &  0.0099 &  0.0143 &  0.0208 &  0.0294 &  0.0402 & &  0.0026 &  0.0041 &  0.0066 &  0.0101 &  0.0149 &  0.0211 &  0.0288\\
0362 &  0.0041 &  0.0065 &  0.0098 &  0.0143 &  0.0208 &  0.0292 &  0.0398 & &  0.0026 &  0.0040 &  0.0065 &  0.0100 &  0.0147 &  0.0209 &  0.0286\\
0363 &  0.0041 &  0.0065 &  0.0097 &  0.0142 &  0.0206 &  0.0292 &  0.0397 & &  0.0025 &  0.0040 &  0.0064 &  0.0099 &  0.0146 &  0.0207 &  0.0284\\
0364 &  0.0041 &  0.0065 &  0.0097 &  0.0141 &  0.0205 &  0.0290 &  0.0396 & &  0.0025 &  0.0039 &  0.0063 &  0.0098 &  0.0145 &  0.0206 &  0.0282\\
0365 &  0.0041 &  0.0065 &  0.0097 &  0.0141 &  0.0205 &  0.0289 &  0.0392 & &  0.0024 &  0.0039 &  0.0062 &  0.0097 &  0.0144 &  0.0204 &  0.0280\\
0366 &  0.0041 &  0.0065 &  0.0096 &  0.0140 &  0.0204 &  0.0288 &  0.0391 & &  0.0024 &  0.0038 &  0.0062 &  0.0096 &  0.0142 &  0.0203 &  0.0279\\
0367 &  0.0041 &  0.0065 &  0.0095 &  0.0139 &  0.0202 &  0.0286 &  0.0390 & &  0.0023 &  0.0038 &  0.0061 &  0.0095 &  0.0141 &  0.0201 &  0.0277\\
0368 &  0.0042 &  0.0065 &  0.0095 &  0.0139 &  0.0202 &  0.0285 &  0.0386 & &  0.0023 &  0.0037 &  0.0060 &  0.0094 &  0.0140 &  0.0200 &  0.0276\\
0369 &  0.0042 &  0.0065 &  0.0094 &  0.0138 &  0.0201 &  0.0284 &  0.0385 & &  0.0023 &  0.0036 &  0.0059 &  0.0093 &  0.0139 &  0.0198 &  0.0274\\
0370 &  0.0042 &  0.0065 &  0.0094 &  0.0138 &  0.0200 &  0.0282 &  0.0384 & &  0.0022 &  0.0036 &  0.0058 &  0.0092 &  0.0138 &  0.0197 &  0.0272\\
0371 &  0.0042 &  0.0064 &  0.0094 &  0.0137 &  0.0200 &  0.0281 &  0.0380 & &  0.0022 &  0.0035 &  0.0058 &  0.0091 &  0.0137 &  0.0195 &  0.0271\\
0372 &  0.0042 &  0.0064 &  0.0093 &  0.0137 &  0.0198 &  0.0280 &  0.0379 & &  0.0021 &  0.0035 &  0.0057 &  0.0090 &  0.0135 &  0.0194 &  0.0270\\
0373 &  0.0042 &  0.0064 &  0.0092 &  0.0136 &  0.0197 &  0.0278 &  0.0379 & &  0.0021 &  0.0034 &  0.0056 &  0.0089 &  0.0134 &  0.0193 &  0.0268\\
0374 &  0.0042 &  0.0063 &  0.0092 &  0.0136 &  0.0197 &  0.0277 &  0.0375 & &  0.0021 &  0.0034 &  0.0055 &  0.0088 &  0.0133 &  0.0191 &  0.0267\\
0375 &  0.0042 &  0.0063 &  0.0091 &  0.0135 &  0.0196 &  0.0276 &  0.0374 & &  0.0020 &  0.0033 &  0.0055 &  0.0087 &  0.0132 &  0.0190 &  0.0265\\
0376 &  0.0042 &  0.0063 &  0.0091 &  0.0134 &  0.0195 &  0.0274 &  0.0374 & &  0.0020 &  0.0033 &  0.0054 &  0.0086 &  0.0131 &  0.0189 &  0.0264\\
0377 &  0.0042 &  0.0062 &  0.0091 &  0.0134 &  0.0195 &  0.0273 &  0.0370 & &  0.0020 &  0.0032 &  0.0053 &  0.0086 &  0.0130 &  0.0187 &  0.0263\\
0378 &  0.0042 &  0.0062 &  0.0090 &  0.0133 &  0.0194 &  0.0272 &  0.0369 & &  0.0019 &  0.0032 &  0.0053 &  0.0085 &  0.0129 &  0.0186 &  0.0261\\
0379 &  0.0043 &  0.0062 &  0.0090 &  0.0132 &  0.0192 &  0.0270 &  0.0369 & &  0.0019 &  0.0031 &  0.0052 &  0.0084 &  0.0128 &  0.0185 &  0.0260\\
0380 &  0.0042 &  0.0061 &  0.0089 &  0.0132 &  0.0192 &  0.0269 &  0.0365 & &  0.0019 &  0.0031 &  0.0051 &  0.0083 &  0.0127 &  0.0183 &  0.0259\\
0381 &  0.0042 &  0.0061 &  0.0089 &  0.0131 &  0.0191 &  0.0268 &  0.0364 & &  0.0018 &  0.0030 &  0.0051 &  0.0083 &  0.0126 &  0.0182 &  0.0258\\
0382 &  0.0042 &  0.0061 &  0.0088 &  0.0131 &  0.0190 &  0.0266 &  0.0365 & &  0.0018 &  0.0030 &  0.0050 &  0.0082 &  0.0125 &  0.0181 &  0.0257\\
0383 &  0.0042 &  0.0060 &  0.0088 &  0.0131 &  0.0190 &  0.0265 &  0.0361 & &  0.0018 &  0.0029 &  0.0050 &  0.0081 &  0.0124 &  0.0180 &  0.0255\\
0384 &  0.0042 &  0.0060 &  0.0088 &  0.0130 &  0.0189 &  0.0265 &  0.0360 & &  0.0017 &  0.0029 &  0.0049 &  0.0080 &  0.0123 &  0.0178 &  0.0254\\
0385 &  0.0042 &  0.0060 &  0.0087 &  0.0129 &  0.0187 &  0.0263 &  0.0360 & &  0.0017 &  0.0028 &  0.0049 &  0.0080 &  0.0122 &  0.0177 &  0.0253\\
0386 &  0.0042 &  0.0059 &  0.0087 &  0.0129 &  0.0187 &  0.0262 &  0.0357 & &  0.0017 &  0.0028 &  0.0048 &  0.0079 &  0.0121 &  0.0176 &  0.0252\\
0387 &  0.0041 &  0.0059 &  0.0086 &  0.0129 &  0.0186 &  0.0262 &  0.0356 & &  0.0017 &  0.0028 &  0.0048 &  0.0078 &  0.0120 &  0.0175 &  0.0251\\
0388 &  0.0041 &  0.0059 &  0.0086 &  0.0128 &  0.0185 &  0.0260 &  0.0357 & &  0.0016 &  0.0027 &  0.0047 &  0.0078 &  0.0119 &  0.0174 &  0.0250\\
0389 &  0.0041 &  0.0058 &  0.0086 &  0.0128 &  0.0185 &  0.0259 &  0.0353 & &  0.0016 &  0.0027 &  0.0047 &  0.0077 &  0.0118 &  0.0173 &  0.0248\\
0390 &  0.0040 &  0.0058 &  0.0085 &  0.0127 &  0.0184 &  0.0258 &  0.0352 & &  0.0016 &  0.0026 &  0.0046 &  0.0076 &  0.0117 &  0.0171 &  0.0247\\
0391 &  0.0040 &  0.0058 &  0.0085 &  0.0126 &  0.0182 &  0.0257 &  0.0353 & &  0.0015 &  0.0026 &  0.0046 &  0.0076 &  0.0116 &  0.0170 &  0.0246\\
0392 &  0.0040 &  0.0057 &  0.0085 &  0.0126 &  0.0182 &  0.0256 &  0.0349 & &  0.0015 &  0.0026 &  0.0045 &  0.0075 &  0.0115 &  0.0169 &  0.0245\\
0393 &  0.0039 &  0.0057 &  0.0084 &  0.0126 &  0.0182 &  0.0255 &  0.0348 & &  0.0015 &  0.0025 &  0.0045 &  0.0074 &  0.0114 &  0.0168 &  0.0244\\
0394 &  0.0039 &  0.0057 &  0.0084 &  0.0125 &  0.0180 &  0.0254 &  0.0350 & &  0.0015 &  0.0025 &  0.0044 &  0.0074 &  0.0113 &  0.0167 &  0.0243\\
0395 &  0.0039 &  0.0056 &  0.0084 &  0.0125 &  0.0180 &  0.0253 &  0.0346 & &  0.0014 &  0.0025 &  0.0044 &  0.0073 &  0.0112 &  0.0166 &  0.0242\\
0396 &  0.0039 &  0.0056 &  0.0084 &  0.0124 &  0.0180 &  0.0252 &  0.0345 & &  0.0014 &  0.0024 &  0.0043 &  0.0072 &  0.0111 &  0.0165 &  0.0241\\
0397 &  0.0038 &  0.0056 &  0.0083 &  0.0123 &  0.0178 &  0.0252 &  0.0346 & &  0.0014 &  0.0024 &  0.0043 &  0.0072 &  0.0110 &  0.0164 &  0.0240\\
0398 &  0.0038 &  0.0055 &  0.0083 &  0.0123 &  0.0178 &  0.0251 &  0.0342 & &  0.0014 &  0.0024 &  0.0043 &  0.0071 &  0.0109 &  0.0163 &  0.0239\\
0399 &  0.0038 &  0.0055 &  0.0083 &  0.0123 &  0.0177 &  0.0249 &  0.0341 & &  0.0013 &  0.0023 &  0.0042 &  0.0070 &  0.0108 &  0.0162 &  0.0237\\
0400 &  0.0038 &  0.0055 &  0.0082 &  0.0122 &  0.0176 &  0.0249 &  0.0343 & &  0.0013 &  0.0023 &  0.0042 &  0.0070 &  0.0108 &  0.0161 &  0.0236\\
0401 &  0.0038 &  0.0055 &  0.0082 &  0.0122 &  0.0176 &  0.0249 &  0.0339 & &  0.0013 &  0.0023 &  0.0042 &  0.0069 &  0.0107 &  0.0160 &  0.0235\\
0402 &  0.0037 &  0.0054 &  0.0082 &  0.0121 &  0.0175 &  0.0247 &  0.0338 & &  0.0013 &  0.0023 &  0.0041 &  0.0068 &  0.0106 &  0.0159 &  0.0234\\
0403 &  0.0037 &  0.0055 &  0.0082 &  0.0120 &  0.0174 &  0.0247 &  0.0340 & &  0.0012 &  0.0022 &  0.0041 &  0.0068 &  0.0105 &  0.0158 &  0.0233\\
0404 &  0.0037 &  0.0054 &  0.0081 &  0.0120 &  0.0174 &  0.0246 &  0.0336 & &  0.0012 &  0.0022 &  0.0040 &  0.0067 &  0.0104 &  0.0157 &  0.0232\\
0405 &  0.0037 &  0.0054 &  0.0081 &  0.0120 &  0.0174 &  0.0244 &  0.0335 & &  0.0012 &  0.0022 &  0.0040 &  0.0067 &  0.0103 &  0.0156 &  0.0231\\
0406 &  0.0036 &  0.0054 &  0.0081 &  0.0119 &  0.0173 &  0.0245 &  0.0337 & &  0.0012 &  0.0022 &  0.0040 &  0.0066 &  0.0103 &  0.0155 &  0.0229\\
0407 &  0.0036 &  0.0054 &  0.0080 &  0.0119 &  0.0173 &  0.0244 &  0.0333 & &  0.0012 &  0.0021 &  0.0039 &  0.0065 &  0.0102 &  0.0155 &  0.0228\\
0408 &  0.0036 &  0.0053 &  0.0080 &  0.0118 &  0.0172 &  0.0242 &  0.0332 & &  0.0011 &  0.0021 &  0.0039 &  0.0065 &  0.0101 &  0.0154 &  0.0227\\
0409 &  0.0036 &  0.0054 &  0.0080 &  0.0117 &  0.0171 &  0.0243 &  0.0334 & &  0.0011 &  0.0021 &  0.0039 &  0.0064 &  0.0100 &  0.0153 &  0.0226\\
0410 &  0.0036 &  0.0053 &  0.0079 &  0.0117 &  0.0171 &  0.0242 &  0.0331 & &  0.0011 &  0.0021 &  0.0039 &  0.0064 &  0.0100 &  0.0152 &  0.0224\\
0411 &  0.0036 &  0.0053 &  0.0079 &  0.0117 &  0.0170 &  0.0240 &  0.0329 & &  0.0011 &  0.0021 &  0.0038 &  0.0063 &  0.0099 &  0.0151 &  0.0223\\
0412 &  0.0035 &  0.0053 &  0.0079 &  0.0116 &  0.0169 &  0.0240 &  0.0331 & &  0.0011 &  0.0021 &  0.0038 &  0.0063 &  0.0098 &  0.0150 &  0.0222\\
0413 &  0.0035 &  0.0053 &  0.0078 &  0.0116 &  0.0169 &  0.0240 &  0.0328 & &  0.0011 &  0.0020 &  0.0038 &  0.0062 &  0.0097 &  0.0149 &  0.0220\\
0414 &  0.0035 &  0.0052 &  0.0078 &  0.0116 &  0.0169 &  0.0238 &  0.0326 & &  0.0011 &  0.0020 &  0.0037 &  0.0061 &  0.0097 &  0.0148 &  0.0219\\
0415 &  0.0035 &  0.0053 &  0.0078 &  0.0115 &  0.0168 &  0.0238 &  0.0328 & &  0.0010 &  0.0020 &  0.0037 &  0.0061 &  0.0096 &  0.0147 &  0.0217\\
0416 &  0.0035 &  0.0052 &  0.0077 &  0.0115 &  0.0168 &  0.0237 &  0.0325 & &  0.0010 &  0.0020 &  0.0037 &  0.0060 &  0.0095 &  0.0146 &  0.0216\\
0417 &  0.0035 &  0.0052 &  0.0077 &  0.0115 &  0.0167 &  0.0235 &  0.0323 & &  0.0010 &  0.0020 &  0.0036 &  0.0060 &  0.0095 &  0.0145 &  0.0215\\
0418 &  0.0035 &  0.0052 &  0.0077 &  0.0114 &  0.0166 &  0.0235 &  0.0325 & &  0.0010 &  0.0020 &  0.0036 &  0.0059 &  0.0094 &  0.0144 &  0.0213\\
0419 &  0.0035 &  0.0051 &  0.0076 &  0.0114 &  0.0166 &  0.0234 &  0.0322 & &  0.0010 &  0.0020 &  0.0036 &  0.0059 &  0.0093 &  0.0143 &  0.0211\\
0420 &  0.0035 &  0.0051 &  0.0076 &  0.0114 &  0.0165 &  0.0232 &  0.0320 & &  0.0010 &  0.0020 &  0.0036 &  0.0058 &  0.0093 &  0.0143 &  0.0210\\
0421 &  0.0034 &  0.0051 &  0.0076 &  0.0113 &  0.0165 &  0.0232 &  0.0321 & &  0.0010 &  0.0020 &  0.0035 &  0.0058 &  0.0092 &  0.0142 &  0.0208\\
0422 &  0.0034 &  0.0051 &  0.0075 &  0.0112 &  0.0165 &  0.0231 &  0.0318 & &  0.0010 &  0.0020 &  0.0035 &  0.0057 &  0.0091 &  0.0141 &  0.0207\\
0423 &  0.0034 &  0.0050 &  0.0075 &  0.0112 &  0.0164 &  0.0229 &  0.0316 & &  0.0010 &  0.0020 &  0.0035 &  0.0057 &  0.0091 &  0.0140 &  0.0205\\
0424 &  0.0034 &  0.0050 &  0.0075 &  0.0112 &  0.0163 &  0.0229 &  0.0317 & &  1.0E-3 &  0.0020 &  0.0035 &  0.0057 &  0.0090 &  0.0139 &  0.0204\\
0425 &  0.0034 &  0.0050 &  0.0075 &  0.0111 &  0.0163 &  0.0228 &  0.0314 & &  1.0E-3 &  0.0019 &  0.0034 &  0.0056 &  0.0089 &  0.0138 &  0.0202\\
0426 &  0.0034 &  0.0049 &  0.0074 &  0.0111 &  0.0162 &  0.0226 &  0.0312 & &  1.0E-3 &  0.0019 &  0.0034 &  0.0056 &  0.0089 &  0.0137 &  0.0200\\
0427 &  0.0034 &  0.0049 &  0.0074 &  0.0111 &  0.0161 &  0.0226 &  0.0313 & &  0.0010 &  0.0019 &  0.0034 &  0.0055 &  0.0088 &  0.0136 &  0.0199\\
0428 &  0.0034 &  0.0049 &  0.0074 &  0.0110 &  0.0161 &  0.0225 &  0.0310 & &  0.0010 &  0.0019 &  0.0034 &  0.0055 &  0.0087 &  0.0134 &  0.0197\\
0429 &  0.0033 &  0.0049 &  0.0073 &  0.0110 &  0.0159 &  0.0223 &  0.0308 & &  0.0010 &  0.0019 &  0.0033 &  0.0054 &  0.0087 &  0.0133 &  0.0195\\
0430 &  0.0033 &  0.0049 &  0.0073 &  0.0110 &  0.0159 &  0.0222 &  0.0308 & &  0.0010 &  0.0019 &  0.0033 &  0.0054 &  0.0086 &  0.0132 &  0.0194\\
0431 &  0.0033 &  0.0048 &  0.0073 &  0.0109 &  0.0158 &  0.0221 &  0.0305 & &  0.0010 &  0.0019 &  0.0033 &  0.0054 &  0.0085 &  0.0131 &  0.0192\\
0432 &  0.0033 &  0.0048 &  0.0073 &  0.0109 &  0.0157 &  0.0219 &  0.0303 & &  0.0010 &  0.0019 &  0.0033 &  0.0053 &  0.0085 &  0.0130 &  0.0190\\
0433 &  0.0032 &  0.0048 &  0.0073 &  0.0109 &  0.0156 &  0.0219 &  0.0303 & &  0.0010 &  0.0019 &  0.0032 &  0.0053 &  0.0084 &  0.0129 &  0.0188\\
0434 &  0.0032 &  0.0048 &  0.0072 &  0.0108 &  0.0156 &  0.0217 &  0.0300 & &  0.0010 &  0.0019 &  0.0032 &  0.0052 &  0.0083 &  0.0128 &  0.0187\\
0435 &  0.0032 &  0.0047 &  0.0072 &  0.0108 &  0.0154 &  0.0216 &  0.0297 & &  0.0010 &  0.0019 &  0.0032 &  0.0052 &  0.0083 &  0.0127 &  0.0185\\
0436 &  0.0032 &  0.0048 &  0.0072 &  0.0107 &  0.0153 &  0.0215 &  0.0297 & &  0.0010 &  0.0019 &  0.0032 &  0.0051 &  0.0082 &  0.0126 &  0.0183\\
0437 &  0.0032 &  0.0047 &  0.0072 &  0.0106 &  0.0153 &  0.0214 &  0.0295 & &  0.0010 &  0.0019 &  0.0031 &  0.0051 &  0.0081 &  0.0125 &  0.0181\\
0438 &  0.0032 &  0.0047 &  0.0071 &  0.0106 &  0.0152 &  0.0212 &  0.0292 & &  0.0011 &  0.0019 &  0.0031 &  0.0051 &  0.0081 &  0.0124 &  0.0180\\
0439 &  0.0031 &  0.0047 &  0.0071 &  0.0106 &  0.0150 &  0.0211 &  0.0292 & &  0.0011 &  0.0019 &  0.0031 &  0.0050 &  0.0080 &  0.0123 &  0.0178\\
0440 &  0.0031 &  0.0047 &  0.0071 &  0.0105 &  0.0150 &  0.0210 &  0.0289 & &  0.0011 &  0.0019 &  0.0031 &  0.0050 &  0.0079 &  0.0122 &  0.0176\\
0441 &  0.0031 &  0.0047 &  0.0070 &  0.0105 &  0.0149 &  0.0209 &  0.0286 & &  0.0011 &  0.0019 &  0.0031 &  0.0049 &  0.0078 &  0.0120 &  0.0174\\
0442 &  0.0031 &  0.0047 &  0.0070 &  0.0104 &  0.0147 &  0.0208 &  0.0286 & &  0.0011 &  0.0019 &  0.0030 &  0.0049 &  0.0078 &  0.0119 &  0.0173\\
0443 &  0.0031 &  0.0046 &  0.0070 &  0.0103 &  0.0147 &  0.0207 &  0.0283 & &  0.0011 &  0.0019 &  0.0030 &  0.0048 &  0.0077 &  0.0118 &  0.0171\\
0444 &  0.0031 &  0.0046 &  0.0069 &  0.0103 &  0.0146 &  0.0206 &  0.0280 & &  0.0011 &  0.0018 &  0.0030 &  0.0048 &  0.0076 &  0.0117 &  0.0169\\
0445 &  0.0031 &  0.0046 &  0.0069 &  0.0102 &  0.0145 &  0.0205 &  0.0280 & &  0.0011 &  0.0018 &  0.0030 &  0.0048 &  0.0076 &  0.0116 &  0.0168\\
0446 &  0.0030 &  0.0046 &  0.0069 &  0.0101 &  0.0144 &  0.0204 &  0.0278 & &  0.0011 &  0.0018 &  0.0029 &  0.0047 &  0.0075 &  0.0115 &  0.0166\\
0447 &  0.0030 &  0.0045 &  0.0068 &  0.0101 &  0.0143 &  0.0203 &  0.0274 & &  0.0011 &  0.0018 &  0.0029 &  0.0047 &  0.0074 &  0.0114 &  0.0165\\
0448 &  0.0030 &  0.0045 &  0.0068 &  0.0100 &  0.0142 &  0.0201 &  0.0274 & &  0.0011 &  0.0018 &  0.0029 &  0.0046 &  0.0073 &  0.0113 &  0.0163\\
0449 &  0.0030 &  0.0045 &  0.0068 &  0.0099 &  0.0141 &  0.0200 &  0.0272 & &  0.0011 &  0.0018 &  0.0029 &  0.0046 &  0.0073 &  0.0112 &  0.0161\\
0450 &  0.0030 &  0.0044 &  0.0068 &  0.0099 &  0.0140 &  0.0200 &  0.0269 & &  0.0011 &  0.0018 &  0.0028 &  0.0045 &  0.0072 &  0.0111 &  0.0160\\
0451 &  0.0030 &  0.0044 &  0.0068 &  0.0098 &  0.0139 &  0.0198 &  0.0269 & &  0.0011 &  0.0018 &  0.0028 &  0.0045 &  0.0071 &  0.0110 &  0.0158\\
0452 &  0.0030 &  0.0044 &  0.0067 &  0.0097 &  0.0139 &  0.0197 &  0.0267 & &  0.0011 &  0.0018 &  0.0028 &  0.0044 &  0.0071 &  0.0109 &  0.0157\\
0453 &  0.0029 &  0.0044 &  0.0067 &  0.0097 &  0.0138 &  0.0197 &  0.0264 & &  0.0011 &  0.0018 &  0.0028 &  0.0044 &  0.0070 &  0.0108 &  0.0156\\
0454 &  0.0029 &  0.0044 &  0.0067 &  0.0096 &  0.0137 &  0.0195 &  0.0264 & &  0.0011 &  0.0018 &  0.0027 &  0.0043 &  0.0069 &  0.0107 &  0.0154\\
0455 &  0.0029 &  0.0044 &  0.0067 &  0.0095 &  0.0137 &  0.0194 &  0.0263 & &  0.0011 &  0.0018 &  0.0027 &  0.0043 &  0.0069 &  0.0106 &  0.0153\\
0456 &  0.0029 &  0.0043 &  0.0066 &  0.0095 &  0.0136 &  0.0193 &  0.0260 & &  0.0011 &  0.0018 &  0.0027 &  0.0042 &  0.0068 &  0.0105 &  0.0152\\
0457 &  0.0029 &  0.0043 &  0.0066 &  0.0094 &  0.0136 &  0.0192 &  0.0260 & &  0.0011 &  0.0018 &  0.0027 &  0.0042 &  0.0067 &  0.0104 &  0.0150\\
0458 &  0.0029 &  0.0043 &  0.0066 &  0.0093 &  0.0135 &  0.0190 &  0.0259 & &  0.0011 &  0.0017 &  0.0026 &  0.0041 &  0.0067 &  0.0103 &  0.0149\\
0459 &  0.0028 &  0.0043 &  0.0065 &  0.0093 &  0.0134 &  0.0190 &  0.0256 & &  0.0011 &  0.0017 &  0.0026 &  0.0041 &  0.0066 &  0.0102 &  0.0148\\
0460 &  0.0028 &  0.0043 &  0.0065 &  0.0093 &  0.0134 &  0.0188 &  0.0255 & &  0.0011 &  0.0017 &  0.0026 &  0.0040 &  0.0065 &  0.0101 &  0.0146\\
0461 &  0.0028 &  0.0043 &  0.0064 &  0.0092 &  0.0134 &  0.0187 &  0.0255 & &  0.0011 &  0.0017 &  0.0025 &  0.0040 &  0.0065 &  0.0100 &  0.0145\\
0462 &  0.0028 &  0.0043 &  0.0064 &  0.0091 &  0.0133 &  0.0187 &  0.0252 & &  0.0011 &  0.0017 &  0.0025 &  0.0039 &  0.0064 &  0.0099 &  0.0144\\
0463 &  0.0028 &  0.0043 &  0.0064 &  0.0091 &  0.0132 &  0.0185 &  0.0252 & &  0.0011 &  0.0017 &  0.0025 &  0.0039 &  0.0064 &  0.0098 &  0.0143\\
0464 &  0.0027 &  0.0043 &  0.0063 &  0.0090 &  0.0132 &  0.0184 &  0.0251 & &  0.0011 &  0.0017 &  0.0024 &  0.0039 &  0.0063 &  0.0097 &  0.0142\\
0465 &  0.0027 &  0.0043 &  0.0063 &  0.0090 &  0.0131 &  0.0184 &  0.0248 & &  0.0011 &  0.0017 &  0.0024 &  0.0038 &  0.0062 &  0.0096 &  0.0141\\
0466 &  0.0027 &  0.0043 &  0.0063 &  0.0090 &  0.0130 &  0.0182 &  0.0248 & &  0.0011 &  0.0016 &  0.0024 &  0.0038 &  0.0062 &  0.0095 &  0.0140\\
0467 &  0.0027 &  0.0043 &  0.0062 &  0.0089 &  0.0130 &  0.0181 &  0.0248 & &  0.0011 &  0.0016 &  0.0023 &  0.0037 &  0.0061 &  0.0094 &  0.0139\\
0468 &  0.0027 &  0.0043 &  0.0062 &  0.0089 &  0.0129 &  0.0181 &  0.0245 & &  0.0011 &  0.0016 &  0.0023 &  0.0037 &  0.0060 &  0.0093 &  0.0138\\
0469 &  0.0027 &  0.0043 &  0.0061 &  0.0089 &  0.0128 &  0.0180 &  0.0245 & &  0.0011 &  0.0016 &  0.0023 &  0.0036 &  0.0060 &  0.0093 &  0.0137\\
0470 &  0.0027 &  0.0043 &  0.0061 &  0.0088 &  0.0128 &  0.0178 &  0.0245 & &  0.0011 &  0.0016 &  0.0022 &  0.0036 &  0.0059 &  0.0092 &  0.0136\\
0471 &  0.0027 &  0.0042 &  0.0061 &  0.0088 &  0.0127 &  0.0178 &  0.0242 & &  0.0011 &  0.0015 &  0.0022 &  0.0036 &  0.0059 &  0.0091 &  0.0135\\
0472 &  0.0027 &  0.0042 &  0.0060 &  0.0088 &  0.0126 &  0.0177 &  0.0241 & &  0.0011 &  0.0015 &  0.0021 &  0.0035 &  0.0058 &  0.0090 &  0.0134\\
0473 &  0.0027 &  0.0043 &  0.0060 &  0.0087 &  0.0126 &  0.0176 &  0.0242 & &  0.0011 &  0.0015 &  0.0021 &  0.0035 &  0.0057 &  0.0089 &  0.0133\\
0474 &  0.0027 &  0.0042 &  0.0060 &  0.0087 &  0.0125 &  0.0176 &  0.0239 & &  0.0011 &  0.0015 &  0.0021 &  0.0034 &  0.0057 &  0.0088 &  0.0132\\
0475 &  0.0027 &  0.0042 &  0.0059 &  0.0087 &  0.0124 &  0.0174 &  0.0238 & &  0.0011 &  0.0014 &  0.0020 &  0.0034 &  0.0056 &  0.0087 &  0.0131\\
0476 &  0.0027 &  0.0042 &  0.0059 &  0.0087 &  0.0124 &  0.0173 &  0.0239 & &  0.0010 &  0.0014 &  0.0020 &  0.0034 &  0.0055 &  0.0086 &  0.0130\\
0477 &  0.0027 &  0.0042 &  0.0059 &  0.0086 &  0.0123 &  0.0173 &  0.0236 & &  0.0010 &  0.0014 &  0.0020 &  0.0033 &  0.0055 &  0.0086 &  0.0129\\
0478 &  0.0027 &  0.0042 &  0.0059 &  0.0086 &  0.0122 &  0.0172 &  0.0235 & &  0.0010 &  0.0014 &  0.0019 &  0.0033 &  0.0054 &  0.0085 &  0.0128\\
0479 &  0.0027 &  0.0042 &  0.0058 &  0.0086 &  0.0122 &  0.0171 &  0.0236 & &  0.0010 &  0.0013 &  0.0019 &  0.0032 &  0.0054 &  0.0084 &  0.0127\\
0480 &  0.0028 &  0.0041 &  0.0058 &  0.0085 &  0.0122 &  0.0171 &  0.0233 & &  1.0E-3 &  0.0013 &  0.0019 &  0.0032 &  0.0053 &  0.0083 &  0.0125\\
0481 &  0.0028 &  0.0041 &  0.0058 &  0.0085 &  0.0120 &  0.0169 &  0.0233 & &  9.8E-4 &  0.0013 &  0.0019 &  0.0031 &  0.0052 &  0.0082 &  0.0124\\
0482 &  0.0028 &  0.0041 &  0.0058 &  0.0084 &  0.0121 &  0.0169 &  0.0233 & &  9.7E-4 &  0.0012 &  0.0018 &  0.0031 &  0.0052 &  0.0081 &  0.0123\\
0483 &  0.0028 &  0.0041 &  0.0057 &  0.0084 &  0.0120 &  0.0168 &  0.0230 & &  9.5E-4 &  0.0012 &  0.0018 &  0.0031 &  0.0051 &  0.0080 &  0.0122\\
0484 &  0.0028 &  0.0041 &  0.0057 &  0.0083 &  0.0119 &  0.0168 &  0.0230 & &  9.3E-4 &  0.0012 &  0.0018 &  0.0030 &  0.0050 &  0.0079 &  0.0121\\
0485 &  0.0028 &  0.0041 &  0.0057 &  0.0083 &  0.0119 &  0.0167 &  0.0231 & &  9.1E-4 &  0.0012 &  0.0017 &  0.0030 &  0.0049 &  0.0078 &  0.0120\\
0486 &  0.0028 &  0.0040 &  0.0057 &  0.0082 &  0.0118 &  0.0167 &  0.0227 & &  8.9E-4 &  0.0011 &  0.0017 &  0.0029 &  0.0049 &  0.0078 &  0.0119\\
0487 &  0.0028 &  0.0040 &  0.0057 &  0.0082 &  0.0117 &  0.0166 &  0.0226 & &  8.7E-4 &  0.0011 &  0.0017 &  0.0029 &  0.0048 &  0.0077 &  0.0118\\
0488 &  0.0028 &  0.0040 &  0.0057 &  0.0081 &  0.0117 &  0.0166 &  0.0228 & &  8.5E-4 &  0.0011 &  0.0016 &  0.0028 &  0.0047 &  0.0076 &  0.0117\\
0489 &  0.0028 &  0.0039 &  0.0056 &  0.0081 &  0.0116 &  0.0165 &  0.0224 & &  8.3E-4 &  0.0010 &  0.0016 &  0.0028 &  0.0047 &  0.0075 &  0.0115\\
0490 &  0.0028 &  0.0039 &  0.0056 &  0.0081 &  0.0115 &  0.0165 &  0.0223 & &  8.1E-4 &  0.0010 &  0.0016 &  0.0027 &  0.0046 &  0.0074 &  0.0114\\
0491 &  0.0029 &  0.0039 &  0.0056 &  0.0080 &  0.0115 &  0.0165 &  0.0225 & &  7.9E-4 &  9.9E-4 &  0.0015 &  0.0027 &  0.0045 &  0.0073 &  0.0113\\
0492 &  0.0028 &  0.0039 &  0.0055 &  0.0079 &  0.0115 &  0.0164 &  0.0221 & &  7.7E-4 &  9.7E-4 &  0.0015 &  0.0026 &  0.0044 &  0.0072 &  0.0112\\
0493 &  0.0028 &  0.0039 &  0.0055 &  0.0079 &  0.0114 &  0.0164 &  0.0220 & &  7.5E-4 &  9.4E-4 &  0.0015 &  0.0026 &  0.0044 &  0.0071 &  0.0111\\
0494 &  0.0028 &  0.0039 &  0.0055 &  0.0079 &  0.0114 &  0.0164 &  0.0222 & &  7.2E-4 &  9.1E-4 &  0.0014 &  0.0025 &  0.0043 &  0.0071 &  0.0109\\
0495 &  0.0028 &  0.0038 &  0.0054 &  0.0078 &  0.0114 &  0.0163 &  0.0218 & &  7.0E-4 &  8.8E-4 &  0.0014 &  0.0025 &  0.0042 &  0.0070 &  0.0108\\
0496 &  0.0028 &  0.0038 &  0.0054 &  0.0078 &  0.0113 &  0.0163 &  0.0218 & &  6.8E-4 &  8.5E-4 &  0.0014 &  0.0024 &  0.0041 &  0.0069 &  0.0107\\
0497 &  0.0028 &  0.0038 &  0.0054 &  0.0077 &  0.0113 &  0.0162 &  0.0220 & &  6.6E-4 &  8.3E-4 &  0.0013 &  0.0023 &  0.0040 &  0.0068 &  0.0106\\
0498 &  0.0028 &  0.0038 &  0.0053 &  0.0077 &  0.0113 &  0.0162 &  0.0216 & &  6.3E-4 &  8.0E-4 &  0.0013 &  0.0023 &  0.0040 &  0.0067 &  0.0105\\
0499 &  0.0027 &  0.0038 &  0.0053 &  0.0077 &  0.0112 &  0.0161 &  0.0215 & &  6.1E-4 &  7.7E-4 &  0.0012 &  0.0022 &  0.0039 &  0.0066 &  0.0103\\
0500 &  0.0027 &  0.0038 &  0.0053 &  0.0076 &  0.0112 &  0.0161 &  0.0217 & &  5.9E-4 &  7.4E-4 &  0.0012 &  0.0022 &  0.0038 &  0.0065 &  0.0102\\
0501 &  0.0027 &  0.0037 &  0.0052 &  0.0075 &  0.0112 &  0.0160 &  0.0213 & &  5.6E-4 &  7.1E-4 &  0.0012 &  0.0021 &  0.0037 &  0.0065 &  0.0101\\
0502 &  0.0027 &  0.0037 &  0.0052 &  0.0076 &  0.0111 &  0.0160 &  0.0213 & &  5.4E-4 &  6.8E-4 &  0.0011 &  0.0020 &  0.0037 &  0.0064 &  0.0100\\
0503 &  0.0027 &  0.0037 &  0.0051 &  0.0075 &  0.0112 &  0.0160 &  0.0215 & &  5.2E-4 &  6.5E-4 &  0.0011 &  0.0020 &  0.0036 &  0.0063 &  0.0098\\
0504 &  0.0027 &  0.0037 &  0.0051 &  0.0075 &  0.0111 &  0.0159 &  0.0211 & &  4.9E-4 &  6.2E-4 &  0.0010 &  0.0019 &  0.0035 &  0.0062 &  0.0097\\
0505 &  0.0026 &  0.0036 &  0.0051 &  0.0074 &  0.0112 &  0.0159 &  0.0210 & &  4.7E-4 &  5.9E-4 &  9.8E-4 &  0.0019 &  0.0034 &  0.0061 &  0.0096\\
0506 &  0.0026 &  0.0036 &  0.0050 &  0.0074 &  0.0112 &  0.0159 &  0.0212 & &  4.4E-4 &  5.6E-4 &  9.4E-4 &  0.0018 &  0.0034 &  0.0061 &  0.0095\\
0507 &  0.0026 &  0.0036 &  0.0050 &  0.0074 &  0.0111 &  0.0157 &  0.0209 & &  4.2E-4 &  5.3E-4 &  8.9E-4 &  0.0017 &  0.0033 &  0.0060 &  0.0093\\
0508 &  0.0026 &  0.0036 &  0.0050 &  0.0073 &  0.0111 &  0.0158 &  0.0208 & &  3.9E-4 &  4.9E-4 &  8.5E-4 &  0.0017 &  0.0032 &  0.0059 &  0.0092\\
0509 &  0.0026 &  0.0036 &  0.0049 &  0.0074 &  0.0112 &  0.0157 &  0.0210 & &  3.7E-4 &  4.6E-4 &  8.0E-4 &  0.0016 &  0.0032 &  0.0058 &  0.0091\\
0510 &  0.0026 &  0.0035 &  0.0049 &  0.0074 &  0.0111 &  0.0156 &  0.0207 & &  3.4E-4 &  4.3E-4 &  7.5E-4 &  0.0015 &  0.0031 &  0.0058 &  0.0090\\
0511 &  0.0025 &  0.0035 &  0.0049 &  0.0073 &  0.0111 &  0.0156 &  0.0206 & &  3.2E-4 &  3.9E-4 &  7.1E-4 &  0.0014 &  0.0030 &  0.0057 &  0.0089\\
0512 &  0.0025 &  0.0035 &  0.0049 &  0.0074 &  0.0111 &  0.0156 &  0.0208 & &  2.9E-4 &  3.6E-4 &  6.6E-4 &  0.0014 &  0.0030 &  0.0056 &  0.0088\\
0513 &  0.0025 &  0.0034 &  0.0048 &  0.0073 &  0.0110 &  0.0154 &  0.0206 & &  2.7E-4 &  3.2E-4 &  6.1E-4 &  0.0013 &  0.0029 &  0.0055 &  0.0086\\
0514 &  0.0025 &  0.0034 &  0.0048 &  0.0073 &  0.0111 &  0.0154 &  0.0205 & &  2.4E-4 &  2.9E-4 &  5.5E-4 &  0.0012 &  0.0028 &  0.0054 &  0.0085\\
0515 &  0.0025 &  0.0034 &  0.0048 &  0.0074 &  0.0111 &  0.0154 &  0.0207 & &  2.1E-4 &  2.5E-4 &  5.0E-4 &  0.0012 &  0.0028 &  0.0054 &  0.0084\\
0516 &  0.0024 &  0.0033 &  0.0048 &  0.0073 &  0.0110 &  0.0152 &  0.0204 & &  1.9E-4 &  2.2E-4 &  4.5E-4 &  0.0011 &  0.0027 &  0.0053 &  0.0083\\
0517 &  0.0024 &  0.0033 &  0.0047 &  0.0073 &  0.0110 &  0.0152 &  0.0203 & &  1.6E-4 &  1.8E-4 &  4.0E-4 &  0.0010 &  0.0026 &  0.0052 &  0.0082\\
0518 &  0.0024 &  0.0033 &  0.0047 &  0.0074 &  0.0110 &  0.0151 &  0.0204 & &  1.3E-4 &  1.4E-4 &  3.4E-4 &  9.8E-4 &  0.0026 &  0.0052 &  0.0081\\
0519 &  0.0024 &  0.0032 &  0.0047 &  0.0074 &  0.0109 &  0.0149 &  0.0202 & &  1.1E-4 &  1.0E-4 &  2.9E-4 &  9.2E-4 &  0.0025 &  0.0051 &  0.0080\\
0520 &  0.0023 &  0.0032 &  0.0047 &  0.0073 &  0.0109 &  0.0149 &  0.0201 & &  7.9E-5 &  6.6E-5 &  2.3E-4 &  8.6E-4 &  0.0025 &  0.0050 &  0.0079\\
0521 &  0.0024 &  0.0032 &  0.0047 &  0.0074 &  0.0109 &  0.0149 &  0.0202 & &  5.1E-5 &  2.7E-5 &  1.7E-4 &  7.9E-4 &  0.0024 &  0.0049 &  0.0078\\
0522 &  0.0023 &  0.0031 &  0.0047 &  0.0074 &  0.0108 &  0.0147 &  0.0200 & &  2.2E-5 &  1.1E-5 &  1.1E-4 &  7.3E-4 &  0.0024 &  0.0049 &  0.0077\\
0523 &  0.0023 &  0.0031 &  0.0047 &  0.0073 &  0.0108 &  0.0147 &  0.0198 & &  6.7E-6 &  5.1E-5 &  5.6E-5 &  6.7E-4 &  0.0023 &  0.0048 &  0.0076\\
0524 &  0.0023 &  0.0031 &  0.0047 &  0.0074 &  0.0108 &  0.0147 &  0.0200 & &  3.6E-5 &  9.0E-5 &  2.7E-6 &  6.2E-4 &  0.0023 &  0.0047 &  0.0075\\
0525 &  0.0023 &  0.0031 &  0.0047 &  0.0074 &  0.0107 &  0.0145 &  0.0197 & &  6.5E-5 &  1.3E-4 &  6.2E-5 &  5.6E-4 &  0.0022 &  0.0047 &  0.0074\\
0526 &  0.0022 &  0.0031 &  0.0046 &  0.0073 &  0.0107 &  0.0145 &  0.0196 & &  9.5E-5 &  1.7E-4 &  1.2E-4 &  5.0E-4 &  0.0022 &  0.0046 &  0.0073\\
0527 &  0.0022 &  0.0031 &  0.0047 &  0.0073 &  0.0106 &  0.0144 &  0.0197 & &  1.3E-4 &  2.1E-4 &  1.8E-4 &  4.5E-4 &  0.0021 &  0.0045 &  0.0073\\
0528 &  0.0022 &  0.0030 &  0.0047 &  0.0073 &  0.0105 &  0.0143 &  0.0195 & &  1.6E-4 &  2.5E-4 &  2.4E-4 &  4.0E-4 &  0.0021 &  0.0044 &  0.0072\\
0529 &  0.0021 &  0.0030 &  0.0046 &  0.0073 &  0.0105 &  0.0142 &  0.0193 & &  1.9E-4 &  3.0E-4 &  3.0E-4 &  3.4E-4 &  0.0020 &  0.0044 &  0.0071\\
0530 &  0.0021 &  0.0030 &  0.0047 &  0.0073 &  0.0104 &  0.0142 &  0.0194 & &  2.2E-4 &  3.4E-4 &  3.6E-4 &  2.9E-4 &  0.0020 &  0.0043 &  0.0070\\
0531 &  0.0021 &  0.0030 &  0.0047 &  0.0073 &  0.0103 &  0.0141 &  0.0192 & &  2.5E-4 &  3.8E-4 &  4.2E-4 &  2.4E-4 &  0.0019 &  0.0042 &  0.0069\\
0532 &  0.0021 &  0.0030 &  0.0047 &  0.0072 &  0.0102 &  0.0140 &  0.0190 & &  2.8E-4 &  4.3E-4 &  4.8E-4 &  2.0E-4 &  0.0019 &  0.0042 &  0.0069\\
0533 &  0.0020 &  0.0030 &  0.0046 &  0.0072 &  0.0102 &  0.0140 &  0.0191 & &  3.1E-4 &  4.7E-4 &  5.3E-4 &  1.5E-4 &  0.0018 &  0.0041 &  0.0068\\
0534 &  0.0021 &  0.0030 &  0.0047 &  0.0072 &  0.0101 &  0.0139 &  0.0189 & &  3.4E-4 &  5.2E-4 &  5.9E-4 &  1.0E-4 &  0.0018 &  0.0040 &  0.0067\\
0535 &  0.0020 &  0.0029 &  0.0047 &  0.0071 &  0.0100 &  0.0138 &  0.0187 & &  3.7E-4 &  5.7E-4 &  6.5E-4 &  5.8E-5 &  0.0017 &  0.0039 &  0.0066\\
0536 &  0.0020 &  0.0029 &  0.0046 &  0.0071 &  0.0100 &  0.0138 &  0.0188 & &  4.0E-4 &  6.1E-4 &  7.0E-4 &  1.5E-5 &  0.0017 &  0.0039 &  0.0066\\
0537 &  0.0020 &  0.0029 &  0.0046 &  0.0071 &  0.0098 &  0.0137 &  0.0186 & &  4.4E-4 &  6.6E-4 &  7.6E-4 &  2.7E-5 &  0.0017 &  0.0038 &  0.0065\\
0538 &  0.0020 &  0.0029 &  0.0046 &  0.0070 &  0.0098 &  0.0137 &  0.0184 & &  4.7E-4 &  7.1E-4 &  8.1E-4 &  6.7E-5 &  0.0016 &  0.0037 &  0.0064\\
0539 &  0.0019 &  0.0029 &  0.0046 &  0.0070 &  0.0097 &  0.0136 &  0.0185 & &  5.0E-4 &  7.6E-4 &  8.7E-4 &  1.1E-4 &  0.0016 &  0.0037 &  0.0064\\
0540 &  0.0020 &  0.0029 &  0.0046 &  0.0070 &  0.0096 &  0.0136 &  0.0183 & &  5.3E-4 &  8.1E-4 &  9.2E-4 &  1.4E-4 &  0.0015 &  0.0036 &  0.0063\\
0541 &  0.0020 &  0.0029 &  0.0046 &  0.0069 &  0.0096 &  0.0135 &  0.0181 & &  5.6E-4 &  8.6E-4 &  9.7E-4 &  1.8E-4 &  0.0015 &  0.0035 &  0.0062\\
0542 &  0.0019 &  0.0029 &  0.0046 &  0.0068 &  0.0095 &  0.0135 &  0.0181 & &  6.0E-4 &  9.1E-4 & -0.0010 &  2.2E-4 &  0.0014 &  0.0035 &  0.0061\\
0543 &  0.0019 &  0.0029 &  0.0046 &  0.0068 &  0.0094 &  0.0134 &  0.0180 & &  6.3E-4 &  9.7E-4 & -0.0011 &  2.5E-4 &  0.0014 &  0.0034 &  0.0061\\
0544 &  0.0019 &  0.0029 &  0.0046 &  0.0067 &  0.0094 &  0.0134 &  0.0178 & &  6.6E-4 & -0.0010 & -0.0011 &  2.9E-4 &  0.0013 &  0.0033 &  0.0060\\
0545 &  0.0019 &  0.0029 &  0.0045 &  0.0066 &  0.0094 &  0.0133 &  0.0178 & &  7.0E-4 & -0.0011 & -0.0012 &  3.2E-4 &  0.0012 &  0.0032 &  0.0059\\
0546 &  0.0019 &  0.0029 &  0.0045 &  0.0066 &  0.0093 &  0.0133 &  0.0177 & &  7.3E-4 & -0.0011 & -0.0012 &  3.5E-4 &  0.0012 &  0.0032 &  0.0058\\
0547 &  0.0019 &  0.0028 &  0.0045 &  0.0065 &  0.0092 &  0.0132 &  0.0174 & &  7.7E-4 & -0.0012 & -0.0013 &  3.9E-4 &  0.0011 &  0.0031 &  0.0057\\
0548 &  0.0018 &  0.0028 &  0.0044 &  0.0065 &  0.0092 &  0.0132 &  0.0175 & &  8.0E-4 & -0.0012 & -0.0013 &  4.2E-4 &  0.0011 &  0.0030 &  0.0057\\
0549 &  0.0018 &  0.0028 &  0.0044 &  0.0064 &  0.0091 &  0.0131 &  0.0173 & &  8.4E-4 & -0.0013 & -0.0013 &  4.6E-4 &  0.0010 &  0.0030 &  0.0056\\
0550 &  0.0019 &  0.0028 &  0.0044 &  0.0063 &  0.0091 &  0.0131 &  0.0171 & &  8.8E-4 & -0.0013 & -0.0014 &  4.9E-4 &  9.7E-4 &  0.0029 &  0.0055\\
0551 &  0.0018 &  0.0028 &  0.0043 &  0.0063 &  0.0091 &  0.0130 &  0.0171 & &  9.2E-4 & -0.0014 & -0.0014 &  5.3E-4 &  9.1E-4 &  0.0028 &  0.0054\\
0552 &  0.0018 &  0.0028 &  0.0043 &  0.0062 &  0.0090 &  0.0130 &  0.0171 & &  9.6E-4 & -0.0014 & -0.0015 &  5.7E-4 &  8.5E-4 &  0.0027 &  0.0053\\
0553 &  0.0018 &  0.0027 &  0.0043 &  0.0062 &  0.0090 &  0.0129 &  0.0168 & &  1.0E-3 & -0.0015 & -0.0015 &  6.0E-4 &  7.9E-4 &  0.0027 &  0.0052\\
0554 &  0.0018 &  0.0027 &  0.0042 &  0.0061 &  0.0090 &  0.0129 &  0.0169 & & -0.0010 & -0.0015 & -0.0015 &  6.4E-4 &  7.3E-4 &  0.0026 &  0.0051\\
0555 &  0.0018 &  0.0027 &  0.0042 &  0.0061 &  0.0090 &  0.0128 &  0.0168 & & -0.0011 & -0.0016 & -0.0016 &  6.8E-4 &  6.7E-4 &  0.0025 &  0.0050\\
0556 &  0.0017 &  0.0027 &  0.0042 &  0.0060 &  0.0089 &  0.0127 &  0.0166 & & -0.0011 & -0.0016 & -0.0016 &  7.2E-4 &  6.0E-4 &  0.0024 &  0.0049\\
0557 &  0.0017 &  0.0027 &  0.0041 &  0.0060 &  0.0089 &  0.0126 &  0.0166 & & -0.0012 & -0.0017 & -0.0016 &  7.7E-4 &  5.4E-4 &  0.0023 &  0.0048\\
0558 &  0.0017 &  0.0027 &  0.0041 &  0.0060 &  0.0089 &  0.0126 &  0.0166 & & -0.0012 & -0.0017 & -0.0017 &  8.1E-4 &  4.8E-4 &  0.0023 &  0.0048\\
0559 &  0.0017 &  0.0026 &  0.0040 &  0.0059 &  0.0089 &  0.0125 &  0.0164 & & -0.0012 & -0.0018 & -0.0017 &  8.5E-4 &  4.1E-4 &  0.0022 &  0.0047\\
0560 &  0.0017 &  0.0026 &  0.0040 &  0.0059 &  0.0089 &  0.0124 &  0.0165 & & -0.0013 & -0.0018 & -0.0017 &  9.0E-4 &  3.5E-4 &  0.0021 &  0.0046\\
0561 &  0.0017 &  0.0026 &  0.0040 &  0.0059 &  0.0088 &  0.0124 &  0.0165 & & -0.0013 & -0.0019 & -0.0018 &  9.4E-4 &  2.8E-4 &  0.0020 &  0.0044\\
0562 &  0.0016 &  0.0025 &  0.0039 &  0.0058 &  0.0088 &  0.0123 &  0.0163 & & -0.0014 & -0.0019 & -0.0018 &  9.9E-4 &  2.1E-4 &  0.0019 &  0.0043\\
0563 &  0.0016 &  0.0025 &  0.0039 &  0.0058 &  0.0088 &  0.0121 &  0.0163 & & -0.0014 & -0.0020 & -0.0018 & -0.0010 &  1.4E-4 &  0.0018 &  0.0042\\
0564 &  0.0016 &  0.0025 &  0.0038 &  0.0058 &  0.0088 &  0.0121 &  0.0164 & & -0.0015 & -0.0020 & -0.0019 & -0.0011 &  6.9E-5 &  0.0017 &  0.0041\\
0565 &  0.0016 &  0.0025 &  0.0038 &  0.0057 &  0.0087 &  0.0120 &  0.0162 & & -0.0015 & -0.0020 & -0.0019 & -0.0011 &  3.3E-6 &  0.0016 &  0.0040\\
0566 &  0.0016 &  0.0025 &  0.0038 &  0.0057 &  0.0087 &  0.0119 &  0.0163 & & -0.0016 & -0.0021 & -0.0019 & -0.0012 &  7.7E-5 &  0.0015 &  0.0039\\
0567 &  0.0016 &  0.0025 &  0.0037 &  0.0057 &  0.0087 &  0.0119 &  0.0163 & & -0.0016 & -0.0021 & -0.0020 & -0.0012 &  1.5E-4 &  0.0014 &  0.0038\\
0568 &  0.0015 &  0.0024 &  0.0037 &  0.0057 &  0.0086 &  0.0118 &  0.0161 & & -0.0016 & -0.0022 & -0.0020 & -0.0013 &  2.3E-4 &  0.0013 &  0.0037\\
0569 &  0.0015 &  0.0024 &  0.0037 &  0.0056 &  0.0086 &  0.0116 &  0.0162 & & -0.0017 & -0.0022 & -0.0020 & -0.0014 &  3.1E-4 &  0.0012 &  0.0036\\
0570 &  0.0015 &  0.0024 &  0.0036 &  0.0057 &  0.0085 &  0.0117 &  0.0163 & & -0.0017 & -0.0022 & -0.0021 & -0.0014 &  3.8E-4 &  0.0011 &  0.0034\\
0571 &  0.0015 &  0.0023 &  0.0036 &  0.0056 &  0.0084 &  0.0116 &  0.0161 & & -0.0018 & -0.0023 & -0.0021 & -0.0015 &  4.7E-4 &  0.0010 &  0.0033\\
0572 &  0.0014 &  0.0023 &  0.0036 &  0.0056 &  0.0084 &  0.0114 &  0.0162 & & -0.0018 & -0.0023 & -0.0021 & -0.0015 &  5.5E-4 &  9.4E-4 &  0.0032\\
0573 &  0.0014 &  0.0023 &  0.0036 &  0.0056 &  0.0084 &  0.0114 &  0.0163 & & -0.0019 & -0.0023 & -0.0022 & -0.0016 &  6.3E-4 &  8.3E-4 &  0.0031\\
0574 &  0.0014 &  0.0023 &  0.0035 &  0.0056 &  0.0083 &  0.0114 &  0.0161 & & -0.0019 & -0.0024 & -0.0022 & -0.0017 &  7.1E-4 &  7.3E-4 &  0.0029\\
0575 &  0.0014 &  0.0023 &  0.0035 &  0.0055 &  0.0083 &  0.0113 &  0.0161 & & -0.0019 & -0.0024 & -0.0022 & -0.0017 &  8.0E-4 &  6.2E-4 &  0.0028\\
0576 &  0.0013 &  0.0023 &  0.0035 &  0.0056 &  0.0082 &  0.0113 &  0.0163 & & -0.0020 & -0.0024 & -0.0023 & -0.0018 &  8.9E-4 &  5.1E-4 &  0.0027\\
0577 &  0.0013 &  0.0022 &  0.0035 &  0.0055 &  0.0081 &  0.0113 &  0.0160 & & -0.0020 & -0.0024 & -0.0023 & -0.0018 &  9.7E-4 &  4.0E-4 &  0.0025\\
0578 &  0.0013 &  0.0022 &  0.0035 &  0.0055 &  0.0081 &  0.0111 &  0.0161 & & -0.0021 & -0.0025 & -0.0024 & -0.0019 & -0.0011 &  2.9E-4 &  0.0024\\
0579 &  0.0013 &  0.0022 &  0.0035 &  0.0055 &  0.0080 &  0.0111 &  0.0162 & & -0.0021 & -0.0025 & -0.0024 & -0.0020 & -0.0012 &  1.8E-4 &  0.0022\\
0580 &  0.0013 &  0.0022 &  0.0034 &  0.0055 &  0.0079 &  0.0112 &  0.0160 & & -0.0021 & -0.0025 & -0.0025 & -0.0020 & -0.0012 &  6.4E-5 &  0.0021\\
0581 &  0.0013 &  0.0022 &  0.0034 &  0.0054 &  0.0079 &  0.0110 &  0.0160 & & -0.0022 & -0.0026 & -0.0025 & -0.0021 & -0.0013 &  4.9E-5 &  0.0019\\
0582 &  0.0013 &  0.0022 &  0.0034 &  0.0054 &  0.0078 &  0.0110 &  0.0161 & & -0.0022 & -0.0026 & -0.0026 & -0.0022 & -0.0014 &  1.6E-4 &  0.0018\\
0583 &  0.0013 &  0.0021 &  0.0034 &  0.0054 &  0.0077 &  0.0111 &  0.0159 & & -0.0022 & -0.0026 & -0.0026 & -0.0022 & -0.0015 &  2.8E-4 &  0.0016\\
0584 &  0.0013 &  0.0021 &  0.0034 &  0.0053 &  0.0077 &  0.0109 &  0.0159 & & -0.0023 & -0.0027 & -0.0027 & -0.0023 & -0.0016 &  3.9E-4 &  0.0015\\
0585 &  0.0012 &  0.0021 &  0.0033 &  0.0053 &  0.0076 &  0.0109 &  0.0160 & & -0.0023 & -0.0027 & -0.0027 & -0.0024 & -0.0017 &  5.0E-4 &  0.0013\\
0586 &  0.0012 &  0.0021 &  0.0033 &  0.0053 &  0.0075 &  0.0110 &  0.0157 & & -0.0023 & -0.0027 & -0.0028 & -0.0025 & -0.0018 &  6.2E-4 &  0.0012\\
0587 &  0.0012 &  0.0021 &  0.0033 &  0.0052 &  0.0075 &  0.0109 &  0.0157 & & -0.0023 & -0.0027 & -0.0028 & -0.0025 & -0.0019 &  7.3E-4 &  0.0010\\
0588 &  0.0012 &  0.0021 &  0.0033 &  0.0051 &  0.0074 &  0.0108 &  0.0158 & & -0.0024 & -0.0028 & -0.0029 & -0.0026 & -0.0020 &  8.4E-4 &  8.6E-4\\
0589 &  0.0012 &  0.0020 &  0.0032 &  0.0052 &  0.0074 &  0.0108 &  0.0155 & & -0.0024 & -0.0028 & -0.0029 & -0.0027 & -0.0021 &  9.6E-4 &  7.0E-4\\
0590 &  0.0012 &  0.0020 &  0.0032 &  0.0051 &  0.0074 &  0.0108 &  0.0154 & & -0.0024 & -0.0028 & -0.0030 & -0.0028 & -0.0022 & -0.0011 &  5.5E-4\\
0591 &  0.0012 &  0.0020 &  0.0032 &  0.0050 &  0.0073 &  0.0108 &  0.0156 & & -0.0025 & -0.0029 & -0.0030 & -0.0028 & -0.0023 & -0.0012 &  3.9E-4\\
0592 &  0.0012 &  0.0020 &  0.0032 &  0.0050 &  0.0073 &  0.0108 &  0.0152 & & -0.0025 & -0.0029 & -0.0031 & -0.0029 & -0.0024 & -0.0013 &  2.4E-4\\
0593 &  0.0012 &  0.0020 &  0.0031 &  0.0050 &  0.0072 &  0.0108 &  0.0152 & & -0.0025 & -0.0030 & -0.0031 & -0.0030 & -0.0025 & -0.0014 &  8.9E-5\\
0594 &  0.0012 &  0.0020 &  0.0031 &  0.0049 &  0.0071 &  0.0107 &  0.0153 & & -0.0025 & -0.0030 & -0.0032 & -0.0031 & -0.0026 & -0.0015 &  6.1E-5\\
0595 &  0.0012 &  0.0020 &  0.0031 &  0.0049 &  0.0071 &  0.0107 &  0.0150 & & -0.0026 & -0.0030 & -0.0032 & -0.0032 & -0.0027 & -0.0016 &  2.1E-4\\
0596 &  0.0012 &  0.0019 &  0.0030 &  0.0048 &  0.0071 &  0.0107 &  0.0149 & & -0.0026 & -0.0031 & -0.0033 & -0.0032 & -0.0028 & -0.0017 &  3.5E-4\\
0597 &  0.0012 &  0.0019 &  0.0030 &  0.0048 &  0.0070 &  0.0106 &  0.0151 & & -0.0026 & -0.0031 & -0.0034 & -0.0033 & -0.0029 & -0.0018 &  5.0E-4\\
0598 &  0.0012 &  0.0019 &  0.0030 &  0.0048 &  0.0070 &  0.0106 &  0.0147 & & -0.0026 & -0.0031 & -0.0034 & -0.0034 & -0.0030 & -0.0019 &  6.3E-4\\
0599 &  0.0012 &  0.0019 &  0.0030 &  0.0047 &  0.0070 &  0.0106 &  0.0146 & & -0.0027 & -0.0032 & -0.0035 & -0.0035 & -0.0031 & -0.0020 &  7.7E-4\\
0600 &  0.0012 &  0.0019 &  0.0030 &  0.0046 &  0.0069 &  0.0105 &  0.0148 & & -0.0027 & -0.0032 & -0.0035 & -0.0036 & -0.0032 & -0.0021 &  9.0E-4\\
0601 &  0.0012 &  0.0018 &  0.0029 &  0.0046 &  0.0069 &  0.0105 &  0.0144 & & -0.0027 & -0.0033 & -0.0036 & -0.0036 & -0.0033 & -0.0022 & -0.0010\\
0602 &  0.0012 &  0.0018 &  0.0029 &  0.0046 &  0.0069 &  0.0105 &  0.0143 & & -0.0027 & -0.0033 & -0.0037 & -0.0037 & -0.0033 & -0.0023 & -0.0012\\
0603 &  0.0012 &  0.0018 &  0.0029 &  0.0045 &  0.0068 &  0.0104 &  0.0146 & & -0.0028 & -0.0033 & -0.0037 & -0.0038 & -0.0034 & -0.0024 & -0.0013\\
0604 &  0.0012 &  0.0017 &  0.0028 &  0.0045 &  0.0068 &  0.0104 &  0.0142 & & -0.0028 & -0.0034 & -0.0038 & -0.0039 & -0.0035 & -0.0025 & -0.0014\\
0605 &  0.0012 &  0.0017 &  0.0028 &  0.0045 &  0.0068 &  0.0104 &  0.0141 & & -0.0028 & -0.0034 & -0.0039 & -0.0040 & -0.0036 & -0.0026 & -0.0015\\
0606 &  0.0012 &  0.0017 &  0.0028 &  0.0044 &  0.0067 &  0.0103 &  0.0143 & & -0.0028 & -0.0035 & -0.0039 & -0.0040 & -0.0037 & -0.0027 & -0.0016\\
0607 &  0.0012 &  0.0016 &  0.0028 &  0.0044 &  0.0067 &  0.0103 &  0.0140 & & -0.0029 & -0.0035 & -0.0040 & -0.0041 & -0.0038 & -0.0028 & -0.0017\\
0608 &  0.0011 &  0.0016 &  0.0027 &  0.0043 &  0.0067 &  0.0102 &  0.0139 & & -0.0029 & -0.0036 & -0.0040 & -0.0042 & -0.0038 & -0.0028 & -0.0018\\
0609 &  0.0011 &  0.0016 &  0.0028 &  0.0042 &  0.0066 &  0.0101 &  0.0141 & & -0.0029 & -0.0036 & -0.0041 & -0.0043 & -0.0039 & -0.0029 & -0.0019\\
0610 &  0.0011 &  0.0015 &  0.0027 &  0.0043 &  0.0066 &  0.0101 &  0.0137 & & -0.0029 & -0.0037 & -0.0042 & -0.0043 & -0.0040 & -0.0030 & -0.0020\\
0611 &  0.0011 &  0.0015 &  0.0027 &  0.0042 &  0.0066 &  0.0101 &  0.0136 & & -0.0030 & -0.0037 & -0.0042 & -0.0044 & -0.0040 & -0.0031 & -0.0021\\
0612 &  0.0011 &  0.0015 &  0.0027 &  0.0041 &  0.0066 &  0.0100 &  0.0138 & & -0.0030 & -0.0038 & -0.0043 & -0.0045 & -0.0041 & -0.0032 & -0.0021\\
0613 &  0.0011 &  0.0014 &  0.0026 &  0.0041 &  0.0066 &  0.0100 &  0.0135 & & -0.0030 & -0.0038 & -0.0044 & -0.0045 & -0.0042 & -0.0032 & -0.0022\\
0614 &  0.0010 &  0.0014 &  0.0026 &  0.0041 &  0.0066 &  0.0099 &  0.0134 & & -0.0031 & -0.0038 & -0.0044 & -0.0046 & -0.0042 & -0.0033 & -0.0023\\
0615 &  9.9E-4 &  0.0014 &  0.0026 &  0.0040 &  0.0065 &  0.0099 &  0.0136 & & -0.0031 & -0.0039 & -0.0045 & -0.0047 & -0.0043 & -0.0034 & -0.0024\\
0616 &  9.7E-4 &  0.0014 &  0.0026 &  0.0040 &  0.0065 &  0.0097 &  0.0133 & & -0.0031 & -0.0039 & -0.0045 & -0.0047 & -0.0043 & -0.0034 & -0.0024\\
0617 &  9.2E-4 &  0.0014 &  0.0026 &  0.0040 &  0.0065 &  0.0098 &  0.0132 & & -0.0031 & -0.0040 & -0.0046 & -0.0048 & -0.0044 & -0.0035 & -0.0025\\
0618 &  8.9E-4 &  0.0014 &  0.0025 &  0.0039 &  0.0065 &  0.0097 &  0.0133 & & -0.0032 & -0.0040 & -0.0046 & -0.0049 & -0.0044 & -0.0036 & -0.0026\\
0619 &  8.6E-4 &  0.0013 &  0.0025 &  0.0039 &  0.0065 &  0.0096 &  0.0130 & & -0.0032 & -0.0041 & -0.0047 & -0.0049 & -0.0045 & -0.0036 & -0.0026\\
0620 &  8.2E-4 &  0.0013 &  0.0025 &  0.0039 &  0.0065 &  0.0096 &  0.0129 & & -0.0032 & -0.0041 & -0.0048 & -0.0050 & -0.0045 & -0.0037 & -0.0027\\
0621 &  7.9E-4 &  0.0013 &  0.0024 &  0.0038 &  0.0064 &  0.0095 &  0.0131 & & -0.0033 & -0.0042 & -0.0048 & -0.0050 & -0.0046 & -0.0038 & -0.0027\\
0622 &  7.6E-4 &  0.0013 &  0.0024 &  0.0038 &  0.0065 &  0.0093 &  0.0128 & & -0.0033 & -0.0042 & -0.0049 & -0.0051 & -0.0046 & -0.0038 & -0.0027\\
0623 &  7.2E-4 &  0.0013 &  0.0024 &  0.0038 &  0.0065 &  0.0094 &  0.0127 & & -0.0033 & -0.0043 & -0.0049 & -0.0051 & -0.0047 & -0.0039 & -0.0028\\
0624 &  7.1E-4 &  0.0013 &  0.0023 &  0.0037 &  0.0064 &  0.0093 &  0.0128 & & -0.0034 & -0.0043 & -0.0050 & -0.0052 & -0.0047 & -0.0040 & -0.0028\\
0625 &  6.6E-4 &  0.0013 &  0.0023 &  0.0037 &  0.0064 &  0.0091 &  0.0126 & & -0.0034 & -0.0044 & -0.0050 & -0.0052 & -0.0048 & -0.0040 & -0.0028\\
0626 &  6.2E-4 &  0.0013 &  0.0023 &  0.0037 &  0.0064 &  0.0091 &  0.0124 & & -0.0034 & -0.0044 & -0.0051 & -0.0053 & -0.0048 & -0.0041 & -0.0029\\
0627 &  6.3E-4 &  0.0013 &  0.0022 &  0.0037 &  0.0063 &  0.0090 &  0.0125 & & -0.0035 & -0.0044 & -0.0051 & -0.0053 & -0.0048 & -0.0042 & -0.0029\\
0628 &  5.9E-4 &  0.0013 &  0.0022 &  0.0037 &  0.0063 &  0.0089 &  0.0123 & & -0.0035 & -0.0045 & -0.0052 & -0.0053 & -0.0049 & -0.0042 & -0.0029\\
0629 &  5.5E-4 &  0.0013 &  0.0022 &  0.0037 &  0.0063 &  0.0089 &  0.0122 & & -0.0035 & -0.0045 & -0.0052 & -0.0054 & -0.0049 & -0.0043 & -0.0029\\
0630 &  5.6E-4 &  0.0013 &  0.0021 &  0.0037 &  0.0062 &  0.0088 &  0.0123 & & -0.0036 & -0.0046 & -0.0052 & -0.0054 & -0.0049 & -0.0044 & -0.0029\\
0631 &  5.4E-4 &  0.0013 &  0.0021 &  0.0037 &  0.0062 &  0.0086 &  0.0121 & & -0.0036 & -0.0046 & -0.0053 & -0.0054 & -0.0050 & -0.0044 & -0.0029\\
0632 &  5.0E-4 &  0.0013 &  0.0021 &  0.0037 &  0.0062 &  0.0086 &  0.0119 & & -0.0036 & -0.0046 & -0.0053 & -0.0055 & -0.0050 & -0.0045 & -0.0029\\
0633 &  5.2E-4 &  0.0013 &  0.0020 &  0.0037 &  0.0061 &  0.0085 &  0.0121 & & -0.0037 & -0.0047 & -0.0054 & -0.0055 & -0.0051 & -0.0045 & -0.0029\\
0634 &  5.1E-4 &  0.0012 &  0.0020 &  0.0037 &  0.0061 &  0.0084 &  0.0119 & & -0.0037 & -0.0047 & -0.0054 & -0.0055 & -0.0051 & -0.0046 & -0.0029\\
0635 &  4.9E-4 &  0.0012 &  0.0020 &  0.0037 &  0.0061 &  0.0084 &  0.0117 & & -0.0037 & -0.0047 & -0.0054 & -0.0055 & -0.0051 & -0.0047 & -0.0029\\
0636 &  5.0E-4 &  0.0012 &  0.0019 &  0.0037 &  0.0060 &  0.0083 &  0.0118 & & -0.0037 & -0.0048 & -0.0055 & -0.0056 & -0.0052 & -0.0047 & -0.0029\\
0637 &  5.2E-4 &  0.0012 &  0.0019 &  0.0037 &  0.0060 &  0.0082 &  0.0116 & & -0.0038 & -0.0048 & -0.0055 & -0.0056 & -0.0052 & -0.0048 & -0.0029\\
0638 &  4.9E-4 &  0.0012 &  0.0019 &  0.0037 &  0.0059 &  0.0082 &  0.0115 & & -0.0038 & -0.0048 & -0.0055 & -0.0056 & -0.0053 & -0.0049 & -0.0030\\
0639 &  5.1E-4 &  0.0012 &  0.0018 &  0.0037 &  0.0058 &  0.0081 &  0.0116 & & -0.0038 & -0.0049 & -0.0055 & -0.0056 & -0.0053 & -0.0049 & -0.0030\\
0640 &  5.3E-4 &  0.0011 &  0.0018 &  0.0037 &  0.0058 &  0.0079 &  0.0114 & & -0.0039 & -0.0049 & -0.0056 & -0.0056 & -0.0053 & -0.0050 & -0.0030\\
0641 &  5.1E-4 &  0.0011 &  0.0018 &  0.0037 &  0.0057 &  0.0079 &  0.0112 & & -0.0039 & -0.0049 & -0.0056 & -0.0057 & -0.0054 & -0.0050 & -0.0030\\
0642 &  5.3E-4 &  0.0011 &  0.0018 &  0.0037 &  0.0056 &  0.0079 &  0.0113 & & -0.0039 & -0.0049 & -0.0056 & -0.0057 & -0.0054 & -0.0051 & -0.0030\\
0643 &  5.6E-4 &  0.0011 &  0.0018 &  0.0037 &  0.0056 &  0.0078 &  0.0112 & & -0.0039 & -0.0050 & -0.0056 & -0.0057 & -0.0055 & -0.0052 & -0.0030\\
0644 &  5.3E-4 &  0.0010 &  0.0018 &  0.0037 &  0.0055 &  0.0078 &  0.0109 & & -0.0040 & -0.0050 & -0.0057 & -0.0057 & -0.0056 & -0.0052 & -0.0030\\
0645 &  5.5E-4 &  0.0010 &  0.0018 &  0.0037 &  0.0054 &  0.0077 &  0.0110 & & -0.0040 & -0.0050 & -0.0057 & -0.0057 & -0.0056 & -0.0053 & -0.0030\\
0646 &  5.7E-4 &  9.8E-4 &  0.0018 &  0.0037 &  0.0054 &  0.0076 &  0.0109 & & -0.0040 & -0.0050 & -0.0057 & -0.0058 & -0.0057 & -0.0053 & -0.0030\\
0647 &  5.4E-4 &  9.3E-4 &  0.0018 &  0.0037 &  0.0053 &  0.0076 &  0.0107 & & -0.0040 & -0.0051 & -0.0057 & -0.0058 & -0.0057 & -0.0054 & -0.0031\\
0648 &  5.5E-4 &  9.2E-4 &  0.0018 &  0.0036 &  0.0053 &  0.0076 &  0.0108 & & -0.0041 & -0.0051 & -0.0057 & -0.0058 & -0.0058 & -0.0055 & -0.0031\\
0649 &  5.5E-4 &  8.9E-4 &  0.0018 &  0.0036 &  0.0052 &  0.0075 &  0.0107 & & -0.0041 & -0.0051 & -0.0057 & -0.0058 & -0.0058 & -0.0055 & -0.0031\\
0650 &  5.7E-4 &  8.5E-4 &  0.0018 &  0.0036 &  0.0052 &  0.0075 &  0.0105 & & -0.0041 & -0.0051 & -0.0058 & -0.0058 & -0.0059 & -0.0056 & -0.0032\\
0651 &  5.4E-4 &  8.4E-4 &  0.0018 &  0.0036 &  0.0051 &  0.0074 &  0.0105 & & -0.0041 & -0.0051 & -0.0058 & -0.0059 & -0.0060 & -0.0056 & -0.0032\\
0652 &  5.5E-4 &  8.2E-4 &  0.0018 &  0.0036 &  0.0050 &  0.0074 &  0.0105 & & -0.0041 & -0.0051 & -0.0058 & -0.0059 & -0.0060 & -0.0057 & -0.0032\\
0653 &  5.6E-4 &  7.8E-4 &  0.0018 &  0.0035 &  0.0050 &  0.0074 &  0.0103 & & -0.0041 & -0.0052 & -0.0058 & -0.0059 & -0.0061 & -0.0058 & -0.0033\\
0654 &  5.2E-4 &  7.7E-4 &  0.0018 &  0.0035 &  0.0049 &  0.0073 &  0.0103 & & -0.0042 & -0.0052 & -0.0058 & -0.0060 & -0.0062 & -0.0058 & -0.0034\\
0655 &  5.2E-4 &  7.6E-4 &  0.0018 &  0.0035 &  0.0048 &  0.0073 &  0.0103 & & -0.0042 & -0.0052 & -0.0058 & -0.0060 & -0.0062 & -0.0059 & -0.0034\\
0656 &  5.4E-4 &  7.2E-4 &  0.0019 &  0.0034 &  0.0048 &  0.0072 &  0.0101 & & -0.0042 & -0.0052 & -0.0058 & -0.0060 & -0.0063 & -0.0060 & -0.0035\\
0657 &  4.9E-4 &  7.2E-4 &  0.0019 &  0.0034 &  0.0047 &  0.0072 &  0.0101 & & -0.0042 & -0.0052 & -0.0058 & -0.0061 & -0.0064 & -0.0060 & -0.0036\\
0658 &  4.9E-4 &  7.2E-4 &  0.0019 &  0.0033 &  0.0047 &  0.0072 &  0.0101 & & -0.0042 & -0.0052 & -0.0058 & -0.0061 & -0.0065 & -0.0061 & -0.0036\\
0659 &  5.0E-4 &  6.9E-4 &  0.0019 &  0.0033 &  0.0047 &  0.0071 &  0.0099 & & -0.0042 & -0.0052 & -0.0058 & -0.0061 & -0.0065 & -0.0062 & -0.0037\\
0660 &  4.7E-4 &  7.0E-4 &  0.0019 &  0.0032 &  0.0046 &  0.0071 &  0.0100 & & -0.0042 & -0.0052 & -0.0059 & -0.0062 & -0.0066 & -0.0062 & -0.0038\\
0661 &  4.3E-4 &  7.0E-4 &  0.0019 &  0.0032 &  0.0045 &  0.0071 &  0.0100 & & -0.0042 & -0.0053 & -0.0059 & -0.0062 & -0.0067 & -0.0063 & -0.0039\\
0662 &  4.4E-4 &  6.8E-4 &  0.0019 &  0.0032 &  0.0046 &  0.0070 &  0.0098 & & -0.0042 & -0.0053 & -0.0059 & -0.0063 & -0.0068 & -0.0064 & -0.0040\\
0663 &  4.2E-4 &  6.9E-4 &  0.0019 &  0.0031 &  0.0045 &  0.0070 &  0.0099 & & -0.0042 & -0.0053 & -0.0059 & -0.0063 & -0.0068 & -0.0065 & -0.0041\\
0664 &  3.8E-4 &  7.0E-4 &  0.0020 &  0.0031 &  0.0045 &  0.0070 &  0.0099 & & -0.0042 & -0.0053 & -0.0059 & -0.0064 & -0.0069 & -0.0066 & -0.0042\\
0665 &  3.8E-4 &  6.8E-4 &  0.0020 &  0.0031 &  0.0045 &  0.0070 &  0.0097 & & -0.0042 & -0.0053 & -0.0059 & -0.0064 & -0.0070 & -0.0066 & -0.0043\\
0666 &  3.7E-4 &  6.9E-4 &  0.0020 &  0.0030 &  0.0045 &  0.0069 &  0.0098 & & -0.0042 & -0.0053 & -0.0059 & -0.0065 & -0.0071 & -0.0067 & -0.0044\\
0667 &  3.4E-4 &  7.1E-4 &  0.0020 &  0.0029 &  0.0044 &  0.0070 &  0.0099 & & -0.0043 & -0.0053 & -0.0060 & -0.0065 & -0.0072 & -0.0068 & -0.0046\\
0668 &  3.2E-4 &  6.9E-4 &  0.0020 &  0.0029 &  0.0044 &  0.0069 &  0.0096 & & -0.0043 & -0.0053 & -0.0060 & -0.0066 & -0.0072 & -0.0069 & -0.0047\\
0669 &  3.2E-4 &  7.1E-4 &  0.0020 &  0.0029 &  0.0044 &  0.0069 &  0.0097 & & -0.0043 & -0.0053 & -0.0060 & -0.0066 & -0.0073 & -0.0070 & -0.0048\\
0670 &  2.9E-4 &  7.3E-4 &  0.0019 &  0.0028 &  0.0044 &  0.0070 &  0.0098 & & -0.0043 & -0.0053 & -0.0060 & -0.0067 & -0.0074 & -0.0071 & -0.0050\\
0671 &  2.8E-4 &  7.2E-4 &  0.0019 &  0.0028 &  0.0044 &  0.0069 &  0.0096 & & -0.0043 & -0.0053 & -0.0060 & -0.0068 & -0.0075 & -0.0072 & -0.0051\\
0672 &  2.7E-4 &  7.4E-4 &  0.0019 &  0.0028 &  0.0043 &  0.0069 &  0.0096 & & -0.0043 & -0.0054 & -0.0061 & -0.0068 & -0.0076 & -0.0073 & -0.0052\\
0673 &  2.7E-4 &  7.8E-4 &  0.0019 &  0.0027 &  0.0044 &  0.0070 &  0.0098 & & -0.0043 & -0.0054 & -0.0061 & -0.0069 & -0.0076 & -0.0074 & -0.0054\\
0674 &  2.6E-4 &  7.7E-4 &  0.0019 &  0.0027 &  0.0044 &  0.0069 &  0.0095 & & -0.0043 & -0.0054 & -0.0061 & -0.0069 & -0.0077 & -0.0075 & -0.0055\\
0675 &  2.4E-4 &  8.0E-4 &  0.0019 &  0.0027 &  0.0043 &  0.0069 &  0.0096 & & -0.0043 & -0.0054 & -0.0061 & -0.0070 & -0.0078 & -0.0076 & -0.0057\\
0676 &  2.5E-4 &  8.3E-4 &  0.0019 &  0.0026 &  0.0044 &  0.0070 &  0.0097 & & -0.0043 & -0.0054 & -0.0062 & -0.0071 & -0.0079 & -0.0077 & -0.0058\\
0677 &  2.5E-4 &  8.3E-4 &  0.0019 &  0.0026 &  0.0044 &  0.0069 &  0.0095 & & -0.0043 & -0.0054 & -0.0062 & -0.0071 & -0.0080 & -0.0078 & -0.0060\\
0678 &  2.2E-4 &  8.6E-4 &  0.0018 &  0.0026 &  0.0043 &  0.0069 &  0.0095 & & -0.0043 & -0.0054 & -0.0062 & -0.0072 & -0.0081 & -0.0079 & -0.0061\\
0679 &  2.4E-4 &  9.0E-4 &  0.0018 &  0.0026 &  0.0044 &  0.0069 &  0.0097 & & -0.0043 & -0.0054 & -0.0063 & -0.0073 & -0.0082 & -0.0080 & -0.0063\\
0680 &  2.4E-4 &  9.0E-4 &  0.0018 &  0.0025 &  0.0044 &  0.0068 &  0.0094 & & -0.0043 & -0.0054 & -0.0063 & -0.0073 & -0.0082 & -0.0081 & -0.0064\\
0681 &  2.2E-4 &  9.3E-4 &  0.0018 &  0.0025 &  0.0043 &  0.0069 &  0.0095 & & -0.0043 & -0.0054 & -0.0063 & -0.0074 & -0.0083 & -0.0082 & -0.0066\\
0682 &  2.2E-4 &  9.7E-4 &  0.0018 &  0.0025 &  0.0044 &  0.0069 &  0.0097 & & -0.0043 & -0.0054 & -0.0064 & -0.0075 & -0.0084 & -0.0083 & -0.0067\\
0683 &  2.4E-4 &  9.7E-4 &  0.0017 &  0.0025 &  0.0044 &  0.0068 &  0.0094 & & -0.0043 & -0.0055 & -0.0064 & -0.0076 & -0.0085 & -0.0084 & -0.0069\\
0684 &  2.3E-4 &  9.9E-4 &  0.0017 &  0.0025 &  0.0044 &  0.0068 &  0.0095 & & -0.0043 & -0.0055 & -0.0064 & -0.0076 & -0.0086 & -0.0085 & -0.0071\\
0685 &  2.2E-4 &  0.0010 &  0.0017 &  0.0025 &  0.0044 &  0.0069 &  0.0097 & & -0.0044 & -0.0055 & -0.0065 & -0.0077 & -0.0087 & -0.0086 & -0.0072\\
0686 &  2.6E-4 &  0.0010 &  0.0016 &  0.0025 &  0.0045 &  0.0068 &  0.0094 & & -0.0044 & -0.0055 & -0.0065 & -0.0078 & -0.0088 & -0.0088 & -0.0074\\
0687 &  2.5E-4 &  0.0010 &  0.0016 &  0.0025 &  0.0044 &  0.0068 &  0.0094 & & -0.0044 & -0.0055 & -0.0065 & -0.0078 & -0.0089 & -0.0089 & -0.0075\\
0688 &  2.4E-4 &  0.0011 &  0.0016 &  0.0025 &  0.0045 &  0.0068 &  0.0096 & & -0.0044 & -0.0055 & -0.0066 & -0.0079 & -0.0090 & -0.0090 & -0.0076\\
0689 &  2.7E-4 &  0.0011 &  0.0016 &  0.0025 &  0.0045 &  0.0067 &  0.0094 & & -0.0044 & -0.0055 & -0.0066 & -0.0080 & -0.0091 & -0.0091 & -0.0078\\
0690 &  2.9E-4 &  0.0011 &  0.0015 &  0.0025 &  0.0044 &  0.0067 &  0.0094 & & -0.0044 & -0.0055 & -0.0067 & -0.0081 & -0.0091 & -0.0092 & -0.0079\\
0691 &  2.9E-4 &  0.0011 &  0.0015 &  0.0025 &  0.0045 &  0.0067 &  0.0096 & & -0.0044 & -0.0056 & -0.0067 & -0.0081 & -0.0092 & -0.0093 & -0.0081\\
0692 &  3.0E-4 &  0.0011 &  0.0015 &  0.0025 &  0.0046 &  0.0066 &  0.0093 & & -0.0044 & -0.0056 & -0.0068 & -0.0082 & -0.0093 & -0.0094 & -0.0082\\
0693 &  3.4E-4 &  0.0011 &  0.0015 &  0.0025 &  0.0045 &  0.0066 &  0.0093 & & -0.0044 & -0.0056 & -0.0068 & -0.0083 & -0.0094 & -0.0095 & -0.0083\\
0694 &  3.5E-4 &  0.0011 &  0.0015 &  0.0025 &  0.0045 &  0.0066 &  0.0095 & & -0.0044 & -0.0056 & -0.0069 & -0.0083 & -0.0095 & -0.0096 & -0.0085\\
0695 &  3.7E-4 &  0.0011 &  0.0014 &  0.0025 &  0.0046 &  0.0065 &  0.0092 & & -0.0044 & -0.0056 & -0.0069 & -0.0084 & -0.0096 & -0.0097 & -0.0086\\
0696 &  4.1E-4 &  0.0011 &  0.0014 &  0.0026 &  0.0045 &  0.0065 &  0.0092 & & -0.0044 & -0.0056 & -0.0069 & -0.0085 & -0.0097 & -0.0098 & -0.0087\\
0697 &  4.3E-4 &  0.0011 &  0.0014 &  0.0026 &  0.0045 &  0.0065 &  0.0095 & & -0.0044 & -0.0057 & -0.0070 & -0.0085 & -0.0098 & -0.0099 & -0.0088\\
0698 &  4.4E-4 &  0.0011 &  0.0014 &  0.0025 &  0.0046 &  0.0064 &  0.0091 & & -0.0044 & -0.0057 & -0.0070 & -0.0086 & -0.0098 & -0.0100 & -0.0090\\
0699 &  4.9E-4 &  0.0011 &  0.0014 &  0.0026 &  0.0045 &  0.0064 &  0.0091 & & -0.0045 & -0.0057 & -0.0071 & -0.0087 & -0.0099 & -0.0101 & -0.0091\\
0700 &  5.1E-4 &  0.0011 &  0.0014 &  0.0026 &  0.0045 &  0.0064 &  0.0093 & & -0.0045 & -0.0057 & -0.0071 & -0.0087 & -0.0100 & -0.0102 & -0.0092\\
0701 &  5.2E-4 &  0.0011 &  0.0014 &  0.0026 &  0.0045 &  0.0063 &  0.0090 & & -0.0045 & -0.0057 & -0.0072 & -0.0088 & -0.0101 & -0.0102 & -0.0093\\
0702 &  5.7E-4 &  0.0011 &  0.0014 &  0.0027 &  0.0044 &  0.0063 &  0.0090 & & -0.0045 & -0.0057 & -0.0072 & -0.0089 & -0.0102 & -0.0103 & -0.0094\\
0703 &  5.8E-4 &  0.0011 &  0.0014 &  0.0027 &  0.0045 &  0.0062 &  0.0092 & & -0.0045 & -0.0058 & -0.0073 & -0.0089 & -0.0102 & -0.0104 & -0.0095\\
0704 &  5.9E-4 &  0.0010 &  0.0014 &  0.0026 &  0.0045 &  0.0062 &  0.0089 & & -0.0045 & -0.0058 & -0.0073 & -0.0090 & -0.0103 & -0.0105 & -0.0096\\
0705 &  6.5E-4 &  0.0010 &  0.0014 &  0.0027 &  0.0044 &  0.0062 &  0.0088 & & -0.0045 & -0.0058 & -0.0074 & -0.0091 & -0.0104 & -0.0106 & -0.0097\\
0706 &  6.5E-4 &  0.0010 &  0.0014 &  0.0027 &  0.0044 &  0.0061 &  0.0091 & & -0.0045 & -0.0058 & -0.0074 & -0.0091 & -0.0105 & -0.0106 & -0.0098\\
0707 &  6.6E-4 &  1.0E-3 &  0.0014 &  0.0027 &  0.0044 &  0.0061 &  0.0087 & & -0.0045 & -0.0058 & -0.0074 & -0.0092 & -0.0105 & -0.0107 & -0.0100\\
0708 &  7.0E-4 &  9.8E-4 &  0.0014 &  0.0027 &  0.0043 &  0.0061 &  0.0087 & & -0.0045 & -0.0059 & -0.0075 & -0.0093 & -0.0106 & -0.0108 & -0.0101\\
0709 &  7.1E-4 &  1.0E-3 &  0.0014 &  0.0028 &  0.0043 &  0.0060 &  0.0089 & & -0.0045 & -0.0059 & -0.0075 & -0.0093 & -0.0107 & -0.0108 & -0.0101\\
0710 &  7.1E-4 &  9.5E-4 &  0.0014 &  0.0027 &  0.0043 &  0.0060 &  0.0086 & & -0.0045 & -0.0059 & -0.0076 & -0.0094 & -0.0107 & -0.0109 & -0.0102\\
0711 &  7.4E-4 &  9.3E-4 &  0.0014 &  0.0028 &  0.0042 &  0.0060 &  0.0085 & & -0.0045 & -0.0059 & -0.0076 & -0.0095 & -0.0108 & -0.0109 & -0.0103\\
0712 &  7.6E-4 &  9.4E-4 &  0.0014 &  0.0028 &  0.0042 &  0.0059 &  0.0087 & & -0.0045 & -0.0059 & -0.0077 & -0.0095 & -0.0108 & -0.0110 & -0.0104\\
0713 &  7.4E-4 &  9.0E-4 &  0.0014 &  0.0027 &  0.0042 &  0.0059 &  0.0084 & & -0.0045 & -0.0060 & -0.0077 & -0.0096 & -0.0109 & -0.0110 & -0.0105\\
0714 &  7.7E-4 &  8.8E-4 &  0.0015 &  0.0028 &  0.0041 &  0.0059 &  0.0083 & & -0.0045 & -0.0060 & -0.0077 & -0.0096 & -0.0109 & -0.0111 & -0.0106\\
0715 &  7.9E-4 &  8.9E-4 &  0.0014 &  0.0027 &  0.0041 &  0.0057 &  0.0085 & & -0.0045 & -0.0060 & -0.0078 & -0.0097 & -0.0110 & -0.0111 & -0.0107\\
0716 &  7.6E-4 &  8.6E-4 &  0.0015 &  0.0027 &  0.0040 &  0.0058 &  0.0083 & & -0.0045 & -0.0060 & -0.0078 & -0.0097 & -0.0110 & -0.0112 & -0.0108\\
0717 &  7.8E-4 &  8.4E-4 &  0.0015 &  0.0027 &  0.0040 &  0.0058 &  0.0082 & & -0.0045 & -0.0060 & -0.0078 & -0.0098 & -0.0111 & -0.0112 & -0.0109\\
0718 &  7.9E-4 &  8.5E-4 &  0.0015 &  0.0027 &  0.0040 &  0.0056 &  0.0084 & & -0.0046 & -0.0061 & -0.0079 & -0.0098 & -0.0111 & -0.0113 & -0.0110\\
0719 &  7.8E-4 &  8.2E-4 &  0.0015 &  0.0027 &  0.0039 &  0.0057 &  0.0081 & & -0.0046 & -0.0061 & -0.0079 & -0.0099 & -0.0112 & -0.0113 & -0.0111\\
0720 &  7.9E-4 &  8.1E-4 &  0.0015 &  0.0027 &  0.0038 &  0.0057 &  0.0080 & & -0.0046 & -0.0061 & -0.0079 & -0.0099 & -0.0112 & -0.0113 & -0.0112\\
0721 &  7.8E-4 &  8.3E-4 &  0.0015 &  0.0027 &  0.0038 &  0.0055 &  0.0082 & & -0.0046 & -0.0061 & -0.0080 & -0.0100 & -0.0112 & -0.0114 & -0.0113\\
0722 &  7.7E-4 &  8.1E-4 &  0.0015 &  0.0026 &  0.0038 &  0.0056 &  0.0080 & & -0.0046 & -0.0061 & -0.0080 & -0.0100 & -0.0113 & -0.0114 & -0.0115\\
0723 &  7.8E-4 &  8.0E-4 &  0.0015 &  0.0026 &  0.0037 &  0.0056 &  0.0079 & & -0.0046 & -0.0061 & -0.0080 & -0.0100 & -0.0113 & -0.0114 & -0.0116\\
0724 &  7.7E-4 &  8.2E-4 &  0.0015 &  0.0026 &  0.0037 &  0.0054 &  0.0080 & & -0.0046 & -0.0062 & -0.0081 & -0.0101 & -0.0113 & -0.0115 & -0.0117\\
0725 &  7.5E-4 &  8.1E-4 &  0.0015 &  0.0025 &  0.0037 &  0.0055 &  0.0078 & & -0.0046 & -0.0062 & -0.0081 & -0.0101 & -0.0113 & -0.0115 & -0.0118\\
0726 &  7.7E-4 &  8.0E-4 &  0.0015 &  0.0026 &  0.0036 &  0.0055 &  0.0077 & & -0.0046 & -0.0062 & -0.0081 & -0.0101 & -0.0114 & -0.0116 & -0.0119\\
0727 &  7.4E-4 &  8.3E-4 &  0.0015 &  0.0026 &  0.0036 &  0.0053 &  0.0079 & & -0.0046 & -0.0062 & -0.0082 & -0.0102 & -0.0114 & -0.0116 & -0.0120\\
0728 &  7.2E-4 &  8.1E-4 &  0.0014 &  0.0025 &  0.0036 &  0.0054 &  0.0077 & & -0.0046 & -0.0062 & -0.0082 & -0.0102 & -0.0114 & -0.0116 & -0.0121\\
0729 &  7.4E-4 &  8.0E-4 &  0.0015 &  0.0025 &  0.0035 &  0.0054 &  0.0076 & & -0.0046 & -0.0062 & -0.0082 & -0.0102 & -0.0114 & -0.0117 & -0.0122\\
0730 &  7.1E-4 &  8.3E-4 &  0.0015 &  0.0025 &  0.0035 &  0.0053 &  0.0078 & & -0.0046 & -0.0062 & -0.0083 & -0.0102 & -0.0114 & -0.0117 & -0.0123\\
0731 &  7.0E-4 &  8.2E-4 &  0.0014 &  0.0024 &  0.0035 &  0.0053 &  0.0077 & & -0.0046 & -0.0062 & -0.0083 & -0.0103 & -0.0114 & -0.0118 & -0.0125\\
0732 &  6.8E-4 &  8.0E-4 &  0.0015 &  0.0024 &  0.0034 &  0.0053 &  0.0076 & & -0.0046 & -0.0063 & -0.0083 & -0.0103 & -0.0114 & -0.0118 & -0.0126\\
0733 &  6.8E-4 &  8.2E-4 &  0.0014 &  0.0024 &  0.0034 &  0.0052 &  0.0077 & & -0.0046 & -0.0063 & -0.0083 & -0.0103 & -0.0114 & -0.0119 & -0.0127\\
0734 &  6.5E-4 &  8.1E-4 &  0.0014 &  0.0023 &  0.0034 &  0.0053 &  0.0076 & & -0.0046 & -0.0063 & -0.0083 & -0.0103 & -0.0115 & -0.0119 & -0.0128\\
0735 &  6.3E-4 &  7.9E-4 &  0.0014 &  0.0023 &  0.0033 &  0.0053 &  0.0075 & & -0.0046 & -0.0063 & -0.0084 & -0.0103 & -0.0115 & -0.0120 & -0.0129\\
0736 &  6.4E-4 &  8.1E-4 &  0.0014 &  0.0023 &  0.0033 &  0.0052 &  0.0077 & & -0.0046 & -0.0063 & -0.0084 & -0.0104 & -0.0115 & -0.0120 & -0.0131\\
0737 &  6.1E-4 &  7.9E-4 &  0.0014 &  0.0022 &  0.0033 &  0.0052 &  0.0076 & & -0.0046 & -0.0063 & -0.0084 & -0.0104 & -0.0115 & -0.0121 & -0.0132\\
0738 &  5.9E-4 &  7.7E-4 &  0.0014 &  0.0022 &  0.0032 &  0.0052 &  0.0075 & & -0.0046 & -0.0063 & -0.0084 & -0.0104 & -0.0115 & -0.0121 & -0.0133\\
0739 &  6.1E-4 &  7.8E-4 &  0.0014 &  0.0022 &  0.0032 &  0.0051 &  0.0076 & & -0.0046 & -0.0063 & -0.0084 & -0.0104 & -0.0115 & -0.0122 & -0.0134\\
0740 &  5.8E-4 &  7.6E-4 &  0.0013 &  0.0022 &  0.0033 &  0.0052 &  0.0075 & & -0.0046 & -0.0063 & -0.0085 & -0.0104 & -0.0115 & -0.0123 & -0.0135\\
0741 &  5.6E-4 &  7.3E-4 &  0.0014 &  0.0021 &  0.0032 &  0.0052 &  0.0074 & & -0.0046 & -0.0063 & -0.0085 & -0.0104 & -0.0115 & -0.0123 & -0.0136\\
0742 &  5.8E-4 &  7.4E-4 &  0.0014 &  0.0021 &  0.0032 &  0.0051 &  0.0076 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0115 & -0.0124 & -0.0138\\
0743 &  5.7E-4 &  7.2E-4 &  0.0013 &  0.0021 &  0.0032 &  0.0052 &  0.0075 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0115 & -0.0125 & -0.0139\\
0744 &  5.4E-4 &  6.9E-4 &  0.0013 &  0.0021 &  0.0031 &  0.0052 &  0.0073 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0115 & -0.0126 & -0.0140\\
0745 &  5.5E-4 &  6.9E-4 &  0.0013 &  0.0021 &  0.0031 &  0.0051 &  0.0075 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0115 & -0.0126 & -0.0141\\
0746 &  5.7E-4 &  6.7E-4 &  0.0013 &  0.0020 &  0.0032 &  0.0052 &  0.0074 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0116 & -0.0127 & -0.0142\\
0747 &  5.3E-4 &  6.4E-4 &  0.0013 &  0.0020 &  0.0031 &  0.0052 &  0.0073 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0116 & -0.0128 & -0.0143\\
0748 &  5.3E-4 &  6.5E-4 &  0.0013 &  0.0020 &  0.0031 &  0.0052 &  0.0074 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0116 & -0.0129 & -0.0144\\
0749 &  5.5E-4 &  6.3E-4 &  0.0013 &  0.0019 &  0.0031 &  0.0052 &  0.0073 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0116 & -0.0130 & -0.0145\\
0750 &  5.2E-4 &  6.0E-4 &  0.0013 &  0.0019 &  0.0031 &  0.0052 &  0.0072 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0116 & -0.0131 & -0.0145\\
0751 &  5.1E-4 &  6.1E-4 &  0.0013 &  0.0019 &  0.0031 &  0.0052 &  0.0073 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0117 & -0.0131 & -0.0146\\
0752 &  5.3E-4 &  6.0E-4 &  0.0012 &  0.0019 &  0.0032 &  0.0052 &  0.0072 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0117 & -0.0132 & -0.0147\\
0753 &  4.9E-4 &  5.7E-4 &  0.0012 &  0.0019 &  0.0031 &  0.0052 &  0.0071 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0117 & -0.0133 & -0.0148\\
0754 &  4.7E-4 &  5.8E-4 &  0.0012 &  0.0018 &  0.0031 &  0.0052 &  0.0072 & & -0.0045 & -0.0063 & -0.0085 & -0.0104 & -0.0117 & -0.0134 & -0.0149\\
0755 &  4.8E-4 &  5.7E-4 &  0.0012 &  0.0018 &  0.0032 &  0.0051 &  0.0072 & & -0.0044 & -0.0063 & -0.0086 & -0.0104 & -0.0118 & -0.0135 & -0.0150\\
0756 &  4.5E-4 &  5.5E-4 &  0.0012 &  0.0018 &  0.0032 &  0.0051 &  0.0070 & & -0.0044 & -0.0063 & -0.0086 & -0.0104 & -0.0118 & -0.0136 & -0.0150\\
0757 &  4.3E-4 &  5.6E-4 &  0.0012 &  0.0018 &  0.0032 &  0.0051 &  0.0071 & & -0.0044 & -0.0063 & -0.0086 & -0.0104 & -0.0119 & -0.0136 & -0.0151\\
0758 &  4.2E-4 &  5.6E-4 &  0.0012 &  0.0018 &  0.0032 &  0.0051 &  0.0071 & & -0.0044 & -0.0063 & -0.0086 & -0.0104 & -0.0119 & -0.0137 & -0.0152\\
0759 &  4.0E-4 &  5.4E-4 &  0.0012 &  0.0018 &  0.0032 &  0.0050 &  0.0069 & & -0.0044 & -0.0063 & -0.0086 & -0.0105 & -0.0119 & -0.0138 & -0.0152\\
0760 &  3.7E-4 &  5.6E-4 &  0.0012 &  0.0017 &  0.0033 &  0.0051 &  0.0070 & & -0.0044 & -0.0063 & -0.0086 & -0.0105 & -0.0120 & -0.0139 & -0.0153\\
0761 &  3.6E-4 &  5.7E-4 &  0.0011 &  0.0018 &  0.0033 &  0.0050 &  0.0070 & & -0.0044 & -0.0063 & -0.0086 & -0.0105 & -0.0120 & -0.0140 & -0.0153\\
0762 &  3.4E-4 &  5.5E-4 &  0.0011 &  0.0017 &  0.0033 &  0.0049 &  0.0068 & & -0.0044 & -0.0063 & -0.0086 & -0.0105 & -0.0121 & -0.0140 & -0.0154\\
0763 &  3.0E-4 &  5.6E-4 &  0.0011 &  0.0017 &  0.0033 &  0.0050 &  0.0069 & & -0.0044 & -0.0063 & -0.0086 & -0.0105 & -0.0121 & -0.0141 & -0.0154\\
0764 &  3.0E-4 &  5.7E-4 &  0.0011 &  0.0017 &  0.0033 &  0.0049 &  0.0070 & & -0.0043 & -0.0063 & -0.0086 & -0.0105 & -0.0122 & -0.0142 & -0.0155\\
0765 &  2.8E-4 &  5.6E-4 &  0.0011 &  0.0017 &  0.0033 &  0.0048 &  0.0068 & & -0.0043 & -0.0063 & -0.0086 & -0.0105 & -0.0122 & -0.0142 & -0.0155\\
0766 &  2.4E-4 &  5.7E-4 &  0.0011 &  0.0017 &  0.0034 &  0.0048 &  0.0069 & & -0.0043 & -0.0063 & -0.0086 & -0.0105 & -0.0123 & -0.0143 & -0.0156\\
0767 &  2.4E-4 &  5.9E-4 &  0.0011 &  0.0017 &  0.0034 &  0.0047 &  0.0070 & & -0.0043 & -0.0063 & -0.0086 & -0.0105 & -0.0123 & -0.0144 & -0.0156\\
0768 &  2.2E-4 &  5.7E-4 &  0.0010 &  0.0017 &  0.0033 &  0.0046 &  0.0068 & & -0.0043 & -0.0063 & -0.0086 & -0.0105 & -0.0124 & -0.0144 & -0.0157\\
0769 &  2.1E-4 &  5.8E-4 &  0.0010 &  0.0017 &  0.0034 &  0.0047 &  0.0069 & & -0.0043 & -0.0063 & -0.0086 & -0.0105 & -0.0124 & -0.0145 & -0.0157\\
0770 &  1.9E-4 &  6.0E-4 &  0.0010 &  0.0018 &  0.0034 &  0.0046 &  0.0070 & & -0.0043 & -0.0063 & -0.0086 & -0.0105 & -0.0125 & -0.0145 & -0.0157\\
0771 &  1.9E-4 &  5.8E-4 &  0.0010 &  0.0018 &  0.0033 &  0.0045 &  0.0068 & & -0.0043 & -0.0063 & -0.0086 & -0.0105 & -0.0125 & -0.0146 & -0.0158\\
0772 &  1.8E-4 &  5.9E-4 &  9.9E-4 &  0.0018 &  0.0034 &  0.0046 &  0.0068 & & -0.0043 & -0.0063 & -0.0086 & -0.0106 & -0.0126 & -0.0147 & -0.0158\\
0773 &  1.5E-4 &  6.1E-4 &  0.0010 &  0.0018 &  0.0034 &  0.0045 &  0.0070 & & -0.0042 & -0.0063 & -0.0086 & -0.0106 & -0.0126 & -0.0147 & -0.0158\\
0774 &  1.6E-4 &  5.9E-4 &  9.9E-4 &  0.0018 &  0.0033 &  0.0044 &  0.0067 & & -0.0042 & -0.0063 & -0.0087 & -0.0106 & -0.0127 & -0.0147 & -0.0159\\
0775 &  1.6E-4 &  6.0E-4 &  9.6E-4 &  0.0018 &  0.0034 &  0.0044 &  0.0068 & & -0.0042 & -0.0063 & -0.0087 & -0.0106 & -0.0127 & -0.0148 & -0.0159\\
0776 &  1.4E-4 &  6.2E-4 &  9.8E-4 &  0.0019 &  0.0033 &  0.0044 &  0.0069 & & -0.0042 & -0.0063 & -0.0087 & -0.0106 & -0.0128 & -0.0148 & -0.0159\\
0777 &  1.5E-4 &  6.0E-4 &  9.6E-4 &  0.0019 &  0.0032 &  0.0042 &  0.0067 & & -0.0042 & -0.0063 & -0.0087 & -0.0107 & -0.0128 & -0.0149 & -0.0160\\
0778 &  1.6E-4 &  6.1E-4 &  9.5E-4 &  0.0019 &  0.0033 &  0.0043 &  0.0067 & & -0.0042 & -0.0063 & -0.0087 & -0.0107 & -0.0129 & -0.0149 & -0.0160\\
0779 &  1.5E-4 &  6.3E-4 &  9.6E-4 &  0.0020 &  0.0032 &  0.0043 &  0.0069 & & -0.0042 & -0.0063 & -0.0087 & -0.0107 & -0.0129 & -0.0150 & -0.0160\\
0780 &  1.6E-4 &  6.0E-4 &  9.4E-4 &  0.0020 &  0.0032 &  0.0042 &  0.0066 & & -0.0042 & -0.0063 & -0.0087 & -0.0107 & -0.0130 & -0.0150 & -0.0161\\
0781 &  1.6E-4 &  6.1E-4 &  9.3E-4 &  0.0020 &  0.0032 &  0.0042 &  0.0066 & & -0.0042 & -0.0063 & -0.0087 & -0.0108 & -0.0130 & -0.0150 & -0.0161\\
0782 &  1.8E-4 &  6.3E-4 &  9.4E-4 &  0.0020 &  0.0031 &  0.0042 &  0.0067 & & -0.0042 & -0.0063 & -0.0087 & -0.0108 & -0.0131 & -0.0151 & -0.0162\\
0783 &  1.8E-4 &  6.0E-4 &  9.3E-4 &  0.0020 &  0.0030 &  0.0041 &  0.0065 & & -0.0042 & -0.0063 & -0.0087 & -0.0108 & -0.0131 & -0.0151 & -0.0162\\
0784 &  1.8E-4 &  6.1E-4 &  9.2E-4 &  0.0020 &  0.0031 &  0.0042 &  0.0065 & & -0.0041 & -0.0063 & -0.0087 & -0.0108 & -0.0132 & -0.0151 & -0.0162\\
0785 &  2.1E-4 &  6.3E-4 &  9.3E-4 &  0.0021 &  0.0030 &  0.0041 &  0.0066 & & -0.0041 & -0.0064 & -0.0087 & -0.0109 & -0.0132 & -0.0151 & -0.0163\\
0786 &  2.1E-4 &  6.0E-4 &  9.4E-4 &  0.0021 &  0.0029 &  0.0041 &  0.0063 & & -0.0041 & -0.0064 & -0.0088 & -0.0109 & -0.0132 & -0.0152 & -0.0163\\
0787 &  2.1E-4 &  6.0E-4 &  9.2E-4 &  0.0020 &  0.0029 &  0.0042 &  0.0063 & & -0.0041 & -0.0064 & -0.0088 & -0.0109 & -0.0133 & -0.0152 & -0.0163\\
0788 &  2.4E-4 &  6.2E-4 &  9.4E-4 &  0.0021 &  0.0029 &  0.0041 &  0.0065 & & -0.0041 & -0.0064 & -0.0088 & -0.0109 & -0.0133 & -0.0152 & -0.0164\\
0789 &  2.5E-4 &  5.9E-4 &  9.6E-4 &  0.0021 &  0.0028 &  0.0041 &  0.0062 & & -0.0041 & -0.0064 & -0.0088 & -0.0110 & -0.0133 & -0.0152 & -0.0164\\
0790 &  2.4E-4 &  5.9E-4 &  9.5E-4 &  0.0021 &  0.0028 &  0.0041 &  0.0061 & & -0.0041 & -0.0064 & -0.0088 & -0.0110 & -0.0134 & -0.0152 & -0.0165\\
0791 &  2.6E-4 &  6.2E-4 &  9.7E-4 &  0.0021 &  0.0028 &  0.0041 &  0.0063 & & -0.0041 & -0.0065 & -0.0088 & -0.0110 & -0.0134 & -0.0153 & -0.0165\\
0792 &  2.9E-4 &  5.9E-4 &  1.0E-3 &  0.0021 &  0.0026 &  0.0041 &  0.0060 & & -0.0041 & -0.0065 & -0.0088 & -0.0110 & -0.0134 & -0.0153 & -0.0166\\
0793 &  2.9E-4 &  5.9E-4 &  9.9E-4 &  0.0021 &  0.0027 &  0.0041 &  0.0060 & & -0.0041 & -0.0065 & -0.0088 & -0.0111 & -0.0134 & -0.0153 & -0.0166\\
0794 &  2.8E-4 &  6.1E-4 &  0.0010 &  0.0021 &  0.0026 &  0.0042 &  0.0062 & & -0.0041 & -0.0065 & -0.0088 & -0.0111 & -0.0135 & -0.0153 & -0.0166\\
0795 &  3.3E-4 &  5.8E-4 &  0.0010 &  0.0021 &  0.0025 &  0.0042 &  0.0058 & & -0.0041 & -0.0065 & -0.0088 & -0.0111 & -0.0135 & -0.0153 & -0.0167\\
0796 &  3.2E-4 &  5.8E-4 &  0.0010 &  0.0020 &  0.0026 &  0.0042 &  0.0058 & & -0.0041 & -0.0066 & -0.0088 & -0.0111 & -0.0135 & -0.0154 & -0.0167\\
0797 &  3.0E-4 &  6.0E-4 &  0.0011 &  0.0021 &  0.0025 &  0.0042 &  0.0060 & & -0.0041 & -0.0066 & -0.0089 & -0.0112 & -0.0135 & -0.0154 & -0.0167\\
0798 &  3.5E-4 &  5.7E-4 &  0.0011 &  0.0020 &  0.0024 &  0.0042 &  0.0057 & & -0.0041 & -0.0066 & -0.0089 & -0.0112 & -0.0135 & -0.0154 & -0.0168\\
0799 &  3.5E-4 &  5.6E-4 &  0.0011 &  0.0020 &  0.0025 &  0.0042 &  0.0056 & & -0.0042 & -0.0066 & -0.0089 & -0.0112 & -0.0136 & -0.0154 & -0.0168\\
0800 &  3.4E-4 &  5.9E-4 &  0.0011 &  0.0020 &  0.0025 &  0.0042 &  0.0059 & & -0.0042 & -0.0066 & -0.0089 & -0.0112 & -0.0136 & -0.0154 & -0.0169\\
0801 &  3.7E-4 &  5.5E-4 &  0.0011 &  0.0020 &  0.0024 &  0.0042 &  0.0055 & & -0.0042 & -0.0066 & -0.0089 & -0.0112 & -0.0136 & -0.0154 & -0.0169\\
0802 &  3.8E-4 &  5.5E-4 &  0.0011 &  0.0019 &  0.0024 &  0.0042 &  0.0055 & & -0.0042 & -0.0067 & -0.0089 & -0.0113 & -0.0136 & -0.0155 & -0.0169\\
0803 &  3.6E-4 &  5.8E-4 &  0.0011 &  0.0019 &  0.0024 &  0.0042 &  0.0057 & & -0.0042 & -0.0067 & -0.0089 & -0.0113 & -0.0136 & -0.0155 & -0.0170\\
0804 &  3.8E-4 &  5.4E-4 &  0.0012 &  0.0019 &  0.0023 &  0.0042 &  0.0053 & & -0.0042 & -0.0067 & -0.0089 & -0.0113 & -0.0136 & -0.0155 & -0.0170\\
0805 &  4.0E-4 &  5.4E-4 &  0.0012 &  0.0018 &  0.0024 &  0.0042 &  0.0053 & & -0.0042 & -0.0067 & -0.0089 & -0.0113 & -0.0136 & -0.0155 & -0.0170\\
0806 &  3.9E-4 &  5.6E-4 &  0.0012 &  0.0018 &  0.0024 &  0.0042 &  0.0055 & & -0.0043 & -0.0067 & -0.0089 & -0.0113 & -0.0136 & -0.0155 & -0.0171\\
0807 &  4.0E-4 &  5.3E-4 &  0.0012 &  0.0018 &  0.0023 &  0.0042 &  0.0052 & & -0.0043 & -0.0067 & -0.0089 & -0.0113 & -0.0136 & -0.0156 & -0.0171\\
0808 &  4.1E-4 &  5.3E-4 &  0.0012 &  0.0017 &  0.0024 &  0.0042 &  0.0051 & & -0.0043 & -0.0067 & -0.0089 & -0.0114 & -0.0137 & -0.0156 & -0.0171\\
0809 &  4.0E-4 &  5.6E-4 &  0.0012 &  0.0017 &  0.0024 &  0.0042 &  0.0053 & & -0.0043 & -0.0067 & -0.0090 & -0.0114 & -0.0137 & -0.0156 & -0.0171\\
0810 &  4.2E-4 &  5.3E-4 &  0.0012 &  0.0017 &  0.0023 &  0.0042 &  0.0050 & & -0.0043 & -0.0067 & -0.0090 & -0.0114 & -0.0137 & -0.0156 & -0.0172\\
0811 &  4.2E-4 &  5.3E-4 &  0.0013 &  0.0016 &  0.0024 &  0.0042 &  0.0049 & & -0.0044 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0156 & -0.0172\\
0812 &  4.3E-4 &  5.6E-4 &  0.0013 &  0.0017 &  0.0024 &  0.0042 &  0.0051 & & -0.0044 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0156 & -0.0172\\
0813 &  4.1E-4 &  5.4E-4 &  0.0012 &  0.0016 &  0.0024 &  0.0042 &  0.0048 & & -0.0044 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0173\\
0814 &  4.4E-4 &  5.4E-4 &  0.0013 &  0.0015 &  0.0025 &  0.0041 &  0.0047 & & -0.0044 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0173\\
0815 &  4.3E-4 &  5.7E-4 &  0.0013 &  0.0016 &  0.0025 &  0.0042 &  0.0049 & & -0.0045 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0173\\
0816 &  4.2E-4 &  5.5E-4 &  0.0013 &  0.0015 &  0.0025 &  0.0043 &  0.0047 & & -0.0045 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0173\\
0817 &  4.3E-4 &  5.6E-4 &  0.0013 &  0.0015 &  0.0025 &  0.0042 &  0.0046 & & -0.0045 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0174\\
0818 &  4.3E-4 &  5.9E-4 &  0.0013 &  0.0015 &  0.0026 &  0.0042 &  0.0048 & & -0.0045 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0174\\
0819 &  4.2E-4 &  5.7E-4 &  0.0012 &  0.0015 &  0.0025 &  0.0043 &  0.0046 & & -0.0045 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0174\\
0820 &  4.3E-4 &  5.7E-4 &  0.0013 &  0.0014 &  0.0026 &  0.0042 &  0.0045 & & -0.0046 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0174\\
0821 &  4.3E-4 &  6.1E-4 &  0.0013 &  0.0014 &  0.0026 &  0.0042 &  0.0047 & & -0.0046 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0174\\
0822 &  4.0E-4 &  6.0E-4 &  0.0012 &  0.0014 &  0.0026 &  0.0043 &  0.0045 & & -0.0046 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0823 &  4.1E-4 &  6.0E-4 &  0.0012 &  0.0013 &  0.0026 &  0.0042 &  0.0044 & & -0.0046 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0824 &  4.1E-4 &  6.3E-4 &  0.0012 &  0.0014 &  0.0027 &  0.0042 &  0.0046 & & -0.0046 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0825 &  3.8E-4 &  6.3E-4 &  0.0012 &  0.0014 &  0.0027 &  0.0043 &  0.0045 & & -0.0046 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0826 &  3.9E-4 &  6.3E-4 &  0.0012 &  0.0013 &  0.0027 &  0.0041 &  0.0044 & & -0.0047 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0827 &  3.9E-4 &  6.7E-4 &  0.0012 &  0.0014 &  0.0027 &  0.0042 &  0.0046 & & -0.0047 & -0.0068 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0828 &  3.6E-4 &  6.6E-4 &  0.0012 &  0.0014 &  0.0027 &  0.0042 &  0.0045 & & -0.0047 & -0.0067 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0829 &  3.7E-4 &  6.7E-4 &  0.0012 &  0.0013 &  0.0027 &  0.0041 &  0.0044 & & -0.0047 & -0.0067 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0830 &  3.6E-4 &  7.1E-4 &  0.0012 &  0.0014 &  0.0028 &  0.0041 &  0.0046 & & -0.0047 & -0.0067 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0831 &  3.4E-4 &  7.1E-4 &  0.0011 &  0.0014 &  0.0028 &  0.0042 &  0.0045 & & -0.0047 & -0.0067 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0832 &  3.5E-4 &  7.2E-4 &  0.0011 &  0.0014 &  0.0028 &  0.0041 &  0.0044 & & -0.0047 & -0.0067 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0833 &  3.4E-4 &  7.6E-4 &  0.0011 &  0.0014 &  0.0028 &  0.0041 &  0.0047 & & -0.0047 & -0.0067 & -0.0090 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0834 &  3.3E-4 &  7.6E-4 &  0.0010 &  0.0015 &  0.0028 &  0.0041 &  0.0046 & & -0.0047 & -0.0067 & -0.0089 & -0.0114 & -0.0137 & -0.0157 & -0.0175\\
0835 &  3.4E-4 &  7.7E-4 &  0.0011 &  0.0014 &  0.0029 &  0.0041 &  0.0045 & & -0.0047 & -0.0067 & -0.0089 & -0.0113 & -0.0137 & -0.0157 & -0.0174\\
0836 &  3.2E-4 &  8.0E-4 &  0.0010 &  0.0015 &  0.0029 &  0.0040 &  0.0047 & & -0.0047 & -0.0067 & -0.0089 & -0.0113 & -0.0137 & -0.0156 & -0.0174\\
0837 &  3.1E-4 &  8.1E-4 &  9.9E-4 &  0.0015 &  0.0029 &  0.0040 &  0.0047 & & -0.0047 & -0.0067 & -0.0089 & -0.0113 & -0.0137 & -0.0156 & -0.0174\\
0838 &  3.3E-4 &  8.1E-4 &  9.9E-4 &  0.0015 &  0.0030 &  0.0040 &  0.0046 & & -0.0047 & -0.0067 & -0.0089 & -0.0113 & -0.0137 & -0.0156 & -0.0174\\
0839 &  3.2E-4 &  8.4E-4 &  9.8E-4 &  0.0015 &  0.0030 &  0.0039 &  0.0048 & & -0.0047 & -0.0067 & -0.0089 & -0.0113 & -0.0137 & -0.0156 & -0.0174\\
0840 &  3.0E-4 &  8.4E-4 &  9.6E-4 &  0.0015 &  0.0030 &  0.0040 &  0.0048 & & -0.0047 & -0.0066 & -0.0089 & -0.0113 & -0.0137 & -0.0156 & -0.0174\\
0841 &  3.2E-4 &  8.4E-4 &  9.2E-4 &  0.0016 &  0.0031 &  0.0040 &  0.0047 & & -0.0047 & -0.0066 & -0.0089 & -0.0113 & -0.0137 & -0.0155 & -0.0173\\
0842 &  3.3E-4 &  8.7E-4 &  9.3E-4 &  0.0015 &  0.0030 &  0.0039 &  0.0049 & & -0.0047 & -0.0066 & -0.0089 & -0.0113 & -0.0136 & -0.0155 & -0.0173\\
0843 &  3.0E-4 &  8.7E-4 &  9.2E-4 &  0.0016 &  0.0030 &  0.0040 &  0.0049 & & -0.0047 & -0.0066 & -0.0089 & -0.0113 & -0.0136 & -0.0155 & -0.0173\\
0844 &  3.2E-4 &  8.6E-4 &  8.8E-4 &  0.0016 &  0.0031 &  0.0039 &  0.0048 & & -0.0047 & -0.0066 & -0.0088 & -0.0113 & -0.0136 & -0.0155 & -0.0173\\
0845 &  3.4E-4 &  8.9E-4 &  9.0E-4 &  0.0016 &  0.0031 &  0.0039 &  0.0049 & & -0.0047 & -0.0066 & -0.0088 & -0.0113 & -0.0136 & -0.0155 & -0.0172\\
0846 &  3.1E-4 &  8.9E-4 &  8.9E-4 &  0.0016 &  0.0031 &  0.0039 &  0.0050 & & -0.0047 & -0.0066 & -0.0088 & -0.0112 & -0.0136 & -0.0154 & -0.0172\\
0847 &  3.4E-4 &  8.8E-4 &  8.7E-4 &  0.0017 &  0.0031 &  0.0039 &  0.0048 & & -0.0046 & -0.0066 & -0.0088 & -0.0112 & -0.0135 & -0.0154 & -0.0172\\
0848 &  3.7E-4 &  9.0E-4 &  8.9E-4 &  0.0016 &  0.0031 &  0.0039 &  0.0050 & & -0.0046 & -0.0066 & -0.0088 & -0.0112 & -0.0135 & -0.0154 & -0.0171\\
0849 &  3.4E-4 &  9.0E-4 &  8.7E-4 &  0.0017 &  0.0031 &  0.0039 &  0.0051 & & -0.0046 & -0.0065 & -0.0088 & -0.0112 & -0.0135 & -0.0153 & -0.0171\\
0850 &  3.7E-4 &  8.8E-4 &  8.6E-4 &  0.0017 &  0.0032 &  0.0039 &  0.0049 & & -0.0046 & -0.0065 & -0.0088 & -0.0112 & -0.0135 & -0.0153 & -0.0170\\
0851 &  4.0E-4 &  8.9E-4 &  8.8E-4 &  0.0017 &  0.0031 &  0.0039 &  0.0051 & & -0.0046 & -0.0065 & -0.0088 & -0.0112 & -0.0135 & -0.0153 & -0.0170\\
0852 &  4.2E-4 &  8.9E-4 &  8.7E-4 &  0.0017 &  0.0031 &  0.0039 &  0.0052 & & -0.0046 & -0.0065 & -0.0087 & -0.0112 & -0.0134 & -0.0152 & -0.0169\\
0853 &  4.1E-4 &  8.7E-4 &  8.6E-4 &  0.0018 &  0.0031 &  0.0039 &  0.0050 & & -0.0046 & -0.0065 & -0.0087 & -0.0112 & -0.0134 & -0.0152 & -0.0169\\
0854 &  4.4E-4 &  8.7E-4 &  8.8E-4 &  0.0017 &  0.0031 &  0.0039 &  0.0052 & & -0.0046 & -0.0065 & -0.0087 & -0.0112 & -0.0134 & -0.0152 & -0.0169\\
0855 &  4.9E-4 &  8.7E-4 &  8.9E-4 &  0.0018 &  0.0031 &  0.0039 &  0.0053 & & -0.0046 & -0.0065 & -0.0087 & -0.0111 & -0.0133 & -0.0152 & -0.0168\\
0856 &  4.7E-4 &  8.4E-4 &  8.7E-4 &  0.0018 &  0.0031 &  0.0039 &  0.0051 & & -0.0045 & -0.0064 & -0.0087 & -0.0111 & -0.0133 & -0.0151 & -0.0168\\
0857 &  5.0E-4 &  8.4E-4 &  8.9E-4 &  0.0018 &  0.0031 &  0.0039 &  0.0053 & & -0.0045 & -0.0064 & -0.0087 & -0.0111 & -0.0133 & -0.0151 & -0.0167\\
0858 &  5.4E-4 &  8.3E-4 &  9.0E-4 &  0.0018 &  0.0031 &  0.0039 &  0.0054 & & -0.0045 & -0.0064 & -0.0086 & -0.0111 & -0.0133 & -0.0150 & -0.0167\\
0859 &  5.3E-4 &  8.0E-4 &  8.9E-4 &  0.0019 &  0.0031 &  0.0038 &  0.0052 & & -0.0045 & -0.0064 & -0.0086 & -0.0111 & -0.0132 & -0.0150 & -0.0166\\
0860 &  5.5E-4 &  8.0E-4 &  9.0E-4 &  0.0019 &  0.0031 &  0.0038 &  0.0054 & & -0.0045 & -0.0064 & -0.0086 & -0.0111 & -0.0132 & -0.0150 & -0.0166\\
0861 &  6.0E-4 &  8.0E-4 &  9.2E-4 &  0.0019 &  0.0030 &  0.0038 &  0.0055 & & -0.0045 & -0.0064 & -0.0086 & -0.0111 & -0.0132 & -0.0149 & -0.0165\\
0862 &  5.9E-4 &  7.7E-4 &  9.0E-4 &  0.0020 &  0.0031 &  0.0038 &  0.0054 & & -0.0045 & -0.0063 & -0.0086 & -0.0110 & -0.0131 & -0.0149 & -0.0165\\
0863 &  6.0E-4 &  7.7E-4 &  9.1E-4 &  0.0020 &  0.0031 &  0.0038 &  0.0055 & & -0.0044 & -0.0063 & -0.0086 & -0.0110 & -0.0131 & -0.0149 & -0.0164\\
0864 &  6.3E-4 &  7.7E-4 &  9.2E-4 &  0.0020 &  0.0030 &  0.0037 &  0.0057 & & -0.0044 & -0.0063 & -0.0085 & -0.0110 & -0.0131 & -0.0148 & -0.0164\\
0865 &  6.5E-4 &  7.4E-4 &  9.2E-4 &  0.0020 &  0.0031 &  0.0037 &  0.0055 & & -0.0044 & -0.0063 & -0.0085 & -0.0110 & -0.0130 & -0.0148 & -0.0163\\
0866 &  6.5E-4 &  7.4E-4 &  9.2E-4 &  0.0020 &  0.0031 &  0.0037 &  0.0057 & & -0.0044 & -0.0063 & -0.0085 & -0.0109 & -0.0130 & -0.0148 & -0.0163\\
0867 &  6.7E-4 &  7.4E-4 &  9.2E-4 &  0.0020 &  0.0030 &  0.0037 &  0.0058 & & -0.0044 & -0.0063 & -0.0085 & -0.0109 & -0.0130 & -0.0147 & -0.0162\\
0868 &  6.9E-4 &  7.1E-4 &  9.4E-4 &  0.0021 &  0.0031 &  0.0037 &  0.0056 & & -0.0044 & -0.0062 & -0.0085 & -0.0109 & -0.0129 & -0.0147 & -0.0162\\
0869 &  6.9E-4 &  7.1E-4 &  9.2E-4 &  0.0021 &  0.0031 &  0.0036 &  0.0058 & & -0.0044 & -0.0062 & -0.0085 & -0.0109 & -0.0129 & -0.0147 & -0.0161\\
0870 &  7.0E-4 &  7.1E-4 &  9.1E-4 &  0.0021 &  0.0030 &  0.0035 &  0.0059 & & -0.0043 & -0.0062 & -0.0084 & -0.0109 & -0.0128 & -0.0146 & -0.0160\\
0871 &  7.2E-4 &  6.8E-4 &  9.5E-4 &  0.0021 &  0.0030 &  0.0036 &  0.0058 & & -0.0043 & -0.0062 & -0.0084 & -0.0108 & -0.0128 & -0.0146 & -0.0160\\
0872 &  7.1E-4 &  6.8E-4 &  9.2E-4 &  0.0021 &  0.0030 &  0.0035 &  0.0059 & & -0.0043 & -0.0062 & -0.0084 & -0.0108 & -0.0128 & -0.0146 & -0.0159\\
0873 &  7.3E-4 &  6.8E-4 &  9.2E-4 &  0.0021 &  0.0030 &  0.0034 &  0.0061 & & -0.0043 & -0.0062 & -0.0084 & -0.0108 & -0.0127 & -0.0145 & -0.0159\\
0874 &  7.3E-4 &  6.5E-4 &  9.6E-4 &  0.0021 &  0.0030 &  0.0035 &  0.0059 & & -0.0043 & -0.0061 & -0.0084 & -0.0107 & -0.0127 & -0.0145 & -0.0158\\
0875 &  7.2E-4 &  6.5E-4 &  9.3E-4 &  0.0021 &  0.0030 &  0.0034 &  0.0060 & & -0.0043 & -0.0061 & -0.0084 & -0.0107 & -0.0127 & -0.0144 & -0.0157\\
0876 &  7.3E-4 &  6.6E-4 &  9.3E-4 &  0.0021 &  0.0029 &  0.0033 &  0.0061 & & -0.0043 & -0.0061 & -0.0083 & -0.0107 & -0.0126 & -0.0144 & -0.0157\\
0877 &  7.1E-4 &  6.2E-4 &  9.7E-4 &  0.0021 &  0.0029 &  0.0034 &  0.0059 & & -0.0042 & -0.0061 & -0.0083 & -0.0107 & -0.0126 & -0.0144 & -0.0156\\
0878 &  7.2E-4 &  6.2E-4 &  9.8E-4 &  0.0021 &  0.0029 &  0.0033 &  0.0060 & & -0.0042 & -0.0061 & -0.0083 & -0.0106 & -0.0125 & -0.0143 & -0.0156\\
0879 &  7.1E-4 &  6.3E-4 &  9.7E-4 &  0.0021 &  0.0028 &  0.0032 &  0.0062 & & -0.0042 & -0.0060 & -0.0083 & -0.0106 & -0.0125 & -0.0143 & -0.0155\\
0880 &  6.9E-4 &  6.0E-4 &  0.0010 &  0.0021 &  0.0028 &  0.0032 &  0.0060 & & -0.0042 & -0.0060 & -0.0083 & -0.0106 & -0.0125 & -0.0142 & -0.0155\\
0881 &  7.0E-4 &  5.9E-4 &  0.0010 &  0.0021 &  0.0028 &  0.0032 &  0.0060 & & -0.0042 & -0.0060 & -0.0083 & -0.0105 & -0.0124 & -0.0142 & -0.0154\\
0882 &  6.9E-4 &  6.1E-4 &  0.0010 &  0.0021 &  0.0027 &  0.0031 &  0.0062 & & -0.0042 & -0.0060 & -0.0082 & -0.0105 & -0.0124 & -0.0141 & -0.0153\\
0883 &  6.8E-4 &  5.7E-4 &  0.0011 &  0.0021 &  0.0028 &  0.0031 &  0.0059 & & -0.0041 & -0.0060 & -0.0082 & -0.0105 & -0.0124 & -0.0141 & -0.0153\\
0884 &  6.8E-4 &  5.6E-4 &  0.0011 &  0.0021 &  0.0027 &  0.0031 &  0.0060 & & -0.0041 & -0.0059 & -0.0082 & -0.0105 & -0.0123 & -0.0140 & -0.0152\\
0885 &  6.7E-4 &  5.8E-4 &  0.0011 &  0.0020 &  0.0026 &  0.0030 &  0.0062 & & -0.0041 & -0.0059 & -0.0082 & -0.0104 & -0.0123 & -0.0140 & -0.0152\\
0886 &  6.6E-4 &  5.4E-4 &  0.0011 &  0.0021 &  0.0027 &  0.0030 &  0.0059 & & -0.0041 & -0.0059 & -0.0082 & -0.0104 & -0.0123 & -0.0139 & -0.0151\\
0887 &  6.5E-4 &  5.3E-4 &  0.0011 &  0.0020 &  0.0026 &  0.0030 &  0.0059 & & -0.0041 & -0.0059 & -0.0082 & -0.0104 & -0.0122 & -0.0139 & -0.0151\\
0888 &  6.6E-4 &  5.5E-4 &  0.0011 &  0.0020 &  0.0025 &  0.0029 &  0.0061 & & -0.0040 & -0.0059 & -0.0081 & -0.0103 & -0.0122 & -0.0138 & -0.0150\\
0889 &  6.3E-4 &  5.1E-4 &  0.0011 &  0.0020 &  0.0025 &  0.0029 &  0.0058 & & -0.0040 & -0.0058 & -0.0081 & -0.0103 & -0.0122 & -0.0138 & -0.0150\\
0890 &  6.1E-4 &  5.0E-4 &  0.0011 &  0.0020 &  0.0025 &  0.0030 &  0.0059 & & -0.0040 & -0.0058 & -0.0081 & -0.0103 & -0.0121 & -0.0137 & -0.0149\\
0891 &  6.3E-4 &  5.1E-4 &  0.0011 &  0.0020 &  0.0024 &  0.0029 &  0.0061 & & -0.0040 & -0.0058 & -0.0081 & -0.0102 & -0.0121 & -0.0137 & -0.0149\\
0892 &  5.9E-4 &  4.7E-4 &  0.0012 &  0.0020 &  0.0024 &  0.0029 &  0.0058 & & -0.0040 & -0.0058 & -0.0081 & -0.0102 & -0.0121 & -0.0136 & -0.0148\\
0893 &  5.9E-4 &  4.6E-4 &  0.0011 &  0.0020 &  0.0023 &  0.0029 &  0.0058 & & -0.0040 & -0.0058 & -0.0080 & -0.0102 & -0.0120 & -0.0136 & -0.0148\\
0894 &  5.8E-4 &  4.7E-4 &  0.0011 &  0.0019 &  0.0022 &  0.0029 &  0.0060 & & -0.0039 & -0.0057 & -0.0080 & -0.0101 & -0.0120 & -0.0136 & -0.0147\\
0895 &  5.7E-4 &  4.3E-4 &  0.0012 &  0.0020 &  0.0022 &  0.0028 &  0.0057 & & -0.0039 & -0.0057 & -0.0080 & -0.0101 & -0.0120 & -0.0135 & -0.0147\\
0896 &  5.4E-4 &  4.2E-4 &  0.0011 &  0.0020 &  0.0022 &  0.0029 &  0.0057 & & -0.0039 & -0.0057 & -0.0080 & -0.0101 & -0.0119 & -0.0135 & -0.0146\\
0897 &  5.4E-4 &  4.4E-4 &  0.0011 &  0.0019 &  0.0021 &  0.0028 &  0.0060 & & -0.0039 & -0.0057 & -0.0080 & -0.0100 & -0.0119 & -0.0134 & -0.0146\\
0898 &  5.3E-4 &  3.9E-4 &  0.0011 &  0.0019 &  0.0021 &  0.0028 &  0.0057 & & -0.0039 & -0.0057 & -0.0079 & -0.0100 & -0.0119 & -0.0134 & -0.0145\\
0899 &  5.0E-4 &  3.8E-4 &  0.0011 &  0.0019 &  0.0020 &  0.0028 &  0.0057 & & -0.0038 & -0.0056 & -0.0079 & -0.0100 & -0.0118 & -0.0134 & -0.0145\\
0900 &  4.8E-4 &  4.1E-4 &  0.0011 &  0.0018 &  0.0019 &  0.0028 &  0.0060 & & -0.0038 & -0.0056 & -0.0079 & -0.0100 & -0.0118 & -0.0133 & -0.0145\\
0901 &  5.0E-4 &  3.7E-4 &  0.0011 &  0.0019 &  0.0019 &  0.0027 &  0.0057 & & -0.0038 & -0.0056 & -0.0079 & -0.0099 & -0.0117 & -0.0133 & -0.0144\\
0902 &  4.6E-4 &  3.7E-4 &  0.0011 &  0.0018 &  0.0019 &  0.0028 &  0.0057 & & -0.0038 & -0.0056 & -0.0079 & -0.0099 & -0.0117 & -0.0132 & -0.0144\\
0903 &  4.3E-4 &  4.0E-4 &  0.0011 &  0.0018 &  0.0017 &  0.0027 &  0.0059 & & -0.0038 & -0.0056 & -0.0078 & -0.0099 & -0.0117 & -0.0132 & -0.0143\\
0904 &  4.5E-4 &  3.7E-4 &  0.0011 &  0.0018 &  0.0017 &  0.0027 &  0.0056 & & -0.0037 & -0.0056 & -0.0078 & -0.0098 & -0.0116 & -0.0132 & -0.0143\\
0905 &  4.2E-4 &  3.6E-4 &  0.0011 &  0.0018 &  0.0017 &  0.0027 &  0.0056 & & -0.0037 & -0.0056 & -0.0078 & -0.0098 & -0.0116 & -0.0132 & -0.0143\\
0906 &  3.8E-4 &  4.0E-4 &  0.0011 &  0.0017 &  0.0016 &  0.0027 &  0.0059 & & -0.0037 & -0.0055 & -0.0078 & -0.0098 & -0.0115 & -0.0131 & -0.0142\\
0907 &  4.0E-4 &  3.7E-4 &  0.0011 &  0.0017 &  0.0016 &  0.0026 &  0.0056 & & -0.0037 & -0.0055 & -0.0078 & -0.0097 & -0.0115 & -0.0131 & -0.0142\\
0908 &  3.7E-4 &  3.7E-4 &  0.0011 &  0.0017 &  0.0016 &  0.0026 &  0.0055 & & -0.0037 & -0.0055 & -0.0078 & -0.0097 & -0.0114 & -0.0131 & -0.0141\\
0909 &  3.3E-4 &  4.0E-4 &  0.0011 &  0.0016 &  0.0015 &  0.0026 &  0.0058 & & -0.0036 & -0.0055 & -0.0077 & -0.0097 & -0.0114 & -0.0131 & -0.0141\\
0910 &  3.4E-4 &  3.8E-4 &  0.0010 &  0.0016 &  0.0015 &  0.0025 &  0.0055 & & -0.0036 & -0.0055 & -0.0077 & -0.0097 & -0.0114 & -0.0131 & -0.0141\\
0911 &  3.3E-4 &  3.7E-4 &  0.0010 &  0.0016 &  0.0015 &  0.0026 &  0.0054 & & -0.0036 & -0.0055 & -0.0077 & -0.0096 & -0.0113 & -0.0130 & -0.0140\\
0912 &  2.9E-4 &  4.1E-4 &  0.0010 &  0.0015 &  0.0014 &  0.0026 &  0.0056 & & -0.0036 & -0.0055 & -0.0077 & -0.0096 & -0.0113 & -0.0130 & -0.0140\\
0913 &  2.8E-4 &  3.8E-4 &  0.0010 &  0.0015 &  0.0014 &  0.0025 &  0.0054 & & -0.0036 & -0.0055 & -0.0077 & -0.0096 & -0.0113 & -0.0130 & -0.0140\\
0914 &  2.8E-4 &  3.8E-4 &  0.0010 &  0.0015 &  0.0014 &  0.0026 &  0.0053 & & -0.0035 & -0.0054 & -0.0076 & -0.0095 & -0.0112 & -0.0130 & -0.0139\\
0915 &  2.3E-4 &  4.1E-4 &  0.0010 &  0.0014 &  0.0013 &  0.0026 &  0.0054 & & -0.0035 & -0.0054 & -0.0076 & -0.0095 & -0.0112 & -0.0130 & -0.0139\\
0916 &  2.2E-4 &  3.8E-4 &  9.8E-4 &  0.0014 &  0.0013 &  0.0026 &  0.0052 & & -0.0035 & -0.0054 & -0.0076 & -0.0095 & -0.0112 & -0.0130 & -0.0139\\
0917 &  2.2E-4 &  3.8E-4 &  1.0E-3 &  0.0014 &  0.0013 &  0.0027 &  0.0050 & & -0.0035 & -0.0054 & -0.0076 & -0.0094 & -0.0111 & -0.0130 & -0.0139\\
0918 &  1.7E-4 &  4.0E-4 &  9.9E-4 &  0.0013 &  0.0013 &  0.0027 &  0.0052 & & -0.0035 & -0.0054 & -0.0076 & -0.0094 & -0.0111 & -0.0130 & -0.0138\\
0919 &  1.6E-4 &  3.7E-4 &  9.6E-4 &  0.0013 &  0.0013 &  0.0027 &  0.0049 & & -0.0034 & -0.0054 & -0.0075 & -0.0094 & -0.0111 & -0.0130 & -0.0138\\
0920 &  1.5E-4 &  3.6E-4 &  9.7E-4 &  0.0013 &  0.0013 &  0.0028 &  0.0048 & & -0.0034 & -0.0054 & -0.0075 & -0.0094 & -0.0110 & -0.0130 & -0.0138\\
0921 &  1.1E-4 &  3.8E-4 &  9.8E-4 &  0.0012 &  0.0013 &  0.0029 &  0.0049 & & -0.0034 & -0.0054 & -0.0075 & -0.0093 & -0.0110 & -0.0130 & -0.0137\\
0922 &  1.1E-4 &  3.5E-4 &  9.4E-4 &  0.0012 &  0.0013 &  0.0030 &  0.0047 & & -0.0034 & -0.0054 & -0.0075 & -0.0093 & -0.0110 & -0.0129 & -0.0137\\
0923 &  9.1E-5 &  3.4E-4 &  9.5E-4 &  0.0011 &  0.0013 &  0.0030 &  0.0045 & & -0.0034 & -0.0054 & -0.0074 & -0.0093 & -0.0110 & -0.0129 & -0.0137\\
0924 &  6.4E-5 &  3.5E-4 &  9.5E-4 &  0.0011 &  0.0013 &  0.0031 &  0.0046 & & -0.0034 & -0.0054 & -0.0074 & -0.0092 & -0.0109 & -0.0129 & -0.0136\\
0925 &  6.8E-5 &  3.2E-4 &  9.3E-4 &  0.0010 &  0.0013 &  0.0032 &  0.0043 & & -0.0033 & -0.0053 & -0.0074 & -0.0092 & -0.0109 & -0.0129 & -0.0136\\
0926 &  4.7E-5 &  3.1E-4 &  8.9E-4 &  0.0010 &  0.0012 &  0.0032 &  0.0041 & & -0.0033 & -0.0053 & -0.0074 & -0.0091 & -0.0109 & -0.0129 & -0.0136\\
0927 &  1.5E-5 &  3.2E-4 &  9.3E-4 &  9.8E-4 &  0.0012 &  0.0034 &  0.0042 & & -0.0033 & -0.0053 & -0.0074 & -0.0091 & -0.0109 & -0.0129 & -0.0135\\
0928 &  3.2E-5 &  2.9E-4 &  9.0E-4 &  9.2E-4 &  0.0012 &  0.0035 &  0.0040 & & -0.0033 & -0.0053 & -0.0073 & -0.0091 & -0.0109 & -0.0129 & -0.0135\\
0929 &  1.4E-5 &  2.7E-4 &  8.6E-4 &  9.2E-4 &  0.0012 &  0.0035 &  0.0038 & & -0.0033 & -0.0053 & -0.0073 & -0.0090 & -0.0109 & -0.0129 & -0.0135\\
0930 &  1.2E-5 &  2.9E-4 &  9.0E-4 &  8.9E-4 &  0.0012 &  0.0037 &  0.0039 & & -0.0033 & -0.0053 & -0.0073 & -0.0090 & -0.0109 & -0.0129 & -0.0135\\
0931 &  4.5E-6 &  2.7E-4 &  8.8E-4 &  8.3E-4 &  0.0012 &  0.0038 &  0.0036 & & -0.0033 & -0.0053 & -0.0073 & -0.0090 & -0.0109 & -0.0129 & -0.0134\\
0932 &  8.2E-6 &  2.5E-4 &  8.3E-4 &  8.4E-4 &  0.0012 &  0.0038 &  0.0034 & & -0.0033 & -0.0053 & -0.0072 & -0.0090 & -0.0109 & -0.0129 & -0.0134\\
0933 &  7.9E-6 &  2.6E-4 &  8.6E-4 &  8.2E-4 &  0.0012 &  0.0040 &  0.0035 & & -0.0033 & -0.0053 & -0.0072 & -0.0089 & -0.0109 & -0.0129 & -0.0134\\
0934 &  3.4E-5 &  2.5E-4 &  8.5E-4 &  7.7E-4 &  0.0012 &  0.0041 &  0.0033 & & -0.0032 & -0.0053 & -0.0072 & -0.0089 & -0.0109 & -0.0129 & -0.0133\\
0935 &  2.4E-5 &  2.3E-4 &  8.0E-4 &  7.9E-4 &  0.0012 &  0.0041 &  0.0031 & & -0.0032 & -0.0053 & -0.0072 & -0.0089 & -0.0109 & -0.0128 & -0.0133\\
0936 &  2.7E-5 &  2.4E-4 &  8.2E-4 &  7.9E-4 &  0.0012 &  0.0044 &  0.0031 & & -0.0032 & -0.0053 & -0.0071 & -0.0088 & -0.0109 & -0.0128 & -0.0133\\
0937 &  4.9E-5 &  2.3E-4 &  8.1E-4 &  7.4E-4 &  0.0013 &  0.0045 &  0.0029 & & -0.0032 & -0.0053 & -0.0071 & -0.0088 & -0.0109 & -0.0128 & -0.0132\\
0938 &  2.8E-5 &  2.2E-4 &  7.6E-4 &  7.7E-4 &  0.0013 &  0.0045 &  0.0027 & & -0.0032 & -0.0053 & -0.0071 & -0.0088 & -0.0109 & -0.0128 & -0.0132\\
0939 &  4.0E-5 &  2.4E-4 &  7.8E-4 &  7.8E-4 &  0.0013 &  0.0047 &  0.0028 & & -0.0032 & -0.0052 & -0.0071 & -0.0088 & -0.0109 & -0.0128 & -0.0132\\
0940 &  5.4E-5 &  2.3E-4 &  7.7E-4 &  7.5E-4 &  0.0014 &  0.0048 &  0.0026 & & -0.0032 & -0.0052 & -0.0070 & -0.0087 & -0.0109 & -0.0127 & -0.0131\\
0941 &  4.8E-5 &  2.1E-4 &  7.2E-4 &  7.9E-4 &  0.0014 &  0.0048 &  0.0024 & & -0.0032 & -0.0052 & -0.0070 & -0.0087 & -0.0109 & -0.0127 & -0.0131\\
0942 &  5.5E-5 &  2.3E-4 &  7.4E-4 &  8.1E-4 &  0.0014 &  0.0051 &  0.0025 & & -0.0032 & -0.0052 & -0.0070 & -0.0087 & -0.0109 & -0.0127 & -0.0131\\
0943 &  7.0E-5 &  2.3E-4 &  7.2E-4 &  7.8E-4 &  0.0015 &  0.0052 &  0.0024 & & -0.0032 & -0.0052 & -0.0070 & -0.0087 & -0.0109 & -0.0127 & -0.0130\\
0944 &  6.7E-5 &  2.2E-4 &  6.7E-4 &  8.2E-4 &  0.0015 &  0.0052 &  0.0022 & & -0.0032 & -0.0052 & -0.0069 & -0.0087 & -0.0109 & -0.0126 & -0.0130\\
0945 &  7.6E-5 &  2.4E-4 &  6.9E-4 &  8.5E-4 &  0.0016 &  0.0054 &  0.0023 & & -0.0032 & -0.0052 & -0.0069 & -0.0086 & -0.0109 & -0.0126 & -0.0130\\
0946 &  9.5E-5 &  2.4E-4 &  6.7E-4 &  8.2E-4 &  0.0017 &  0.0055 &  0.0022 & & -0.0032 & -0.0052 & -0.0069 & -0.0086 & -0.0109 & -0.0126 & -0.0130\\
0947 &  8.6E-5 &  2.2E-4 &  6.2E-4 &  8.5E-4 &  0.0017 &  0.0056 &  0.0020 & & -0.0032 & -0.0052 & -0.0068 & -0.0086 & -0.0109 & -0.0125 & -0.0129\\
0948 &  9.8E-5 &  2.4E-4 &  6.4E-4 &  9.0E-4 &  0.0018 &  0.0058 &  0.0021 & & -0.0032 & -0.0052 & -0.0068 & -0.0086 & -0.0109 & -0.0125 & -0.0129\\
0949 &  1.3E-4 &  2.4E-4 &  6.2E-4 &  8.7E-4 &  0.0019 &  0.0059 &  0.0021 & & -0.0032 & -0.0051 & -0.0068 & -0.0086 & -0.0109 & -0.0124 & -0.0129\\
0950 &  1.2E-4 &  2.2E-4 &  5.8E-4 &  9.0E-4 &  0.0019 &  0.0060 &  0.0019 & & -0.0032 & -0.0051 & -0.0068 & -0.0086 & -0.0109 & -0.0124 & -0.0128\\
0951 &  1.2E-4 &  2.4E-4 &  5.9E-4 &  9.4E-4 &  0.0020 &  0.0062 &  0.0021 & & -0.0032 & -0.0051 & -0.0067 & -0.0086 & -0.0109 & -0.0124 & -0.0128\\
0952 &  1.6E-4 &  2.4E-4 &  5.7E-4 &  9.0E-4 &  0.0021 &  0.0063 &  0.0021 & & -0.0032 & -0.0051 & -0.0067 & -0.0086 & -0.0109 & -0.0123 & -0.0128\\
0953 &  1.5E-4 &  2.2E-4 &  5.5E-4 &  9.1E-4 &  0.0021 &  0.0064 &  0.0019 & & -0.0032 & -0.0051 & -0.0067 & -0.0086 & -0.0109 & -0.0123 & -0.0127\\
0954 &  1.5E-4 &  2.3E-4 &  5.3E-4 &  9.4E-4 &  0.0022 &  0.0066 &  0.0020 & & -0.0032 & -0.0051 & -0.0067 & -0.0086 & -0.0109 & -0.0122 & -0.0127\\
0955 &  1.9E-4 &  2.4E-4 &  5.4E-4 &  8.9E-4 &  0.0023 &  0.0067 &  0.0021 & & -0.0032 & -0.0050 & -0.0066 & -0.0086 & -0.0109 & -0.0122 & -0.0127\\
0956 &  1.8E-4 &  2.2E-4 &  5.2E-4 &  8.9E-4 &  0.0024 &  0.0068 &  0.0019 & & -0.0032 & -0.0050 & -0.0066 & -0.0085 & -0.0109 & -0.0121 & -0.0127\\
0957 &  1.6E-4 &  2.3E-4 &  5.1E-4 &  9.2E-4 &  0.0024 &  0.0070 &  0.0021 & & -0.0032 & -0.0050 & -0.0066 & -0.0085 & -0.0109 & -0.0121 & -0.0126\\
0958 &  2.0E-4 &  2.3E-4 &  5.3E-4 &  8.6E-4 &  0.0026 &  0.0071 &  0.0021 & & -0.0032 & -0.0050 & -0.0066 & -0.0085 & -0.0109 & -0.0121 & -0.0126\\
0959 &  1.9E-4 &  2.1E-4 &  5.2E-4 &  8.5E-4 &  0.0026 &  0.0073 &  0.0020 & & -0.0032 & -0.0050 & -0.0066 & -0.0085 & -0.0109 & -0.0120 & -0.0126\\
0960 &  1.8E-4 &  2.3E-4 &  5.1E-4 &  8.7E-4 &  0.0027 &  0.0075 &  0.0021 & & -0.0032 & -0.0049 & -0.0065 & -0.0085 & -0.0108 & -0.0120 & -0.0125\\
0961 &  1.9E-4 &  2.3E-4 &  5.3E-4 &  8.2E-4 &  0.0028 &  0.0076 &  0.0022 & & -0.0032 & -0.0049 & -0.0065 & -0.0085 & -0.0108 & -0.0119 & -0.0125\\
0962 &  2.0E-4 &  2.1E-4 &  5.5E-4 &  8.0E-4 &  0.0029 &  0.0078 &  0.0021 & & -0.0032 & -0.0049 & -0.0065 & -0.0085 & -0.0108 & -0.0119 & -0.0125\\
0963 &  1.9E-4 &  2.2E-4 &  5.5E-4 &  8.1E-4 &  0.0029 &  0.0080 &  0.0022 & & -0.0032 & -0.0049 & -0.0065 & -0.0085 & -0.0108 & -0.0119 & -0.0124\\
0964 &  1.8E-4 &  2.3E-4 &  5.7E-4 &  7.6E-4 &  0.0031 &  0.0082 &  0.0023 & & -0.0032 & -0.0048 & -0.0065 & -0.0085 & -0.0107 & -0.0118 & -0.0124\\
0965 &  2.0E-4 &  2.1E-4 &  6.1E-4 &  7.3E-4 &  0.0031 &  0.0083 &  0.0021 & & -0.0032 & -0.0048 & -0.0064 & -0.0085 & -0.0107 & -0.0118 & -0.0124\\
0966 &  1.9E-4 &  2.1E-4 &  6.0E-4 &  7.4E-4 &  0.0032 &  0.0084 &  0.0023 & & -0.0032 & -0.0048 & -0.0064 & -0.0085 & -0.0107 & -0.0118 & -0.0124\\
0967 &  1.8E-4 &  2.2E-4 &  6.2E-4 &  6.9E-4 &  0.0033 &  0.0085 &  0.0024 & & -0.0032 & -0.0048 & -0.0064 & -0.0085 & -0.0106 & -0.0117 & -0.0123\\
0968 &  2.0E-4 &  2.0E-4 &  6.8E-4 &  6.4E-4 &  0.0034 &  0.0085 &  0.0022 & & -0.0032 & -0.0048 & -0.0064 & -0.0085 & -0.0106 & -0.0117 & -0.0123\\
0969 &  1.9E-4 &  2.0E-4 &  6.7E-4 &  6.4E-4 &  0.0034 &  0.0085 &  0.0024 & & -0.0032 & -0.0047 & -0.0064 & -0.0085 & -0.0106 & -0.0117 & -0.0123\\
0970 &  1.9E-4 &  2.1E-4 &  7.0E-4 &  5.9E-4 &  0.0035 &  0.0084 &  0.0025 & & -0.0032 & -0.0047 & -0.0064 & -0.0085 & -0.0105 & -0.0117 & -0.0122\\
0971 &  2.0E-4 &  1.8E-4 &  7.6E-4 &  5.3E-4 &  0.0036 &  0.0084 &  0.0023 & & -0.0032 & -0.0047 & -0.0064 & -0.0085 & -0.0105 & -0.0116 & -0.0122\\
0972 &  2.1E-4 &  1.8E-4 &  7.6E-4 &  5.2E-4 &  0.0036 &  0.0082 &  0.0024 & & -0.0032 & -0.0047 & -0.0063 & -0.0085 & -0.0104 & -0.0116 & -0.0122\\
0973 &  2.2E-4 &  1.8E-4 &  7.9E-4 &  4.6E-4 &  0.0038 &  0.0080 &  0.0026 & & -0.0032 & -0.0047 & -0.0063 & -0.0085 & -0.0104 & -0.0116 & -0.0122\\
0974 &  2.1E-4 &  1.5E-4 &  8.3E-4 &  3.9E-4 &  0.0038 &  0.0079 &  0.0024 & & -0.0032 & -0.0046 & -0.0063 & -0.0085 & -0.0103 & -0.0116 & -0.0121\\
0975 &  2.4E-4 &  1.5E-4 &  8.1E-4 &  3.8E-4 &  0.0039 &  0.0076 &  0.0025 & & -0.0032 & -0.0046 & -0.0063 & -0.0085 & -0.0103 & -0.0116 & -0.0121\\
0976 &  2.4E-4 &  1.5E-4 &  8.1E-4 &  3.0E-4 &  0.0040 &  0.0073 &  0.0027 & & -0.0031 & -0.0046 & -0.0063 & -0.0085 & -0.0102 & -0.0115 & -0.0121\\
0977 &  2.4E-4 &  1.1E-4 &  8.1E-4 &  2.3E-4 &  0.0041 &  0.0070 &  0.0025 & & -0.0031 & -0.0046 & -0.0063 & -0.0085 & -0.0102 & -0.0115 & -0.0120\\
0978 &  2.6E-4 &  1.1E-4 &  7.8E-4 &  2.0E-4 &  0.0041 &  0.0066 &  0.0025 & & -0.0031 & -0.0046 & -0.0063 & -0.0085 & -0.0101 & -0.0115 & -0.0120\\
0979 &  2.7E-4 &  1.1E-4 &  7.3E-4 &  1.1E-4 &  0.0042 &  0.0062 &  0.0027 & & -0.0031 & -0.0046 & -0.0063 & -0.0085 & -0.0101 & -0.0115 & -0.0120\\
0980 &  2.7E-4 &  7.1E-5 &  6.9E-4 &  2.5E-5 &  0.0043 &  0.0059 &  0.0025 & & -0.0031 & -0.0045 & -0.0062 & -0.0085 & -0.0101 & -0.0115 & -0.0120\\
0981 &  3.0E-4 &  6.4E-5 &  6.6E-4 &  1.4E-5 &  0.0043 &  0.0054 &  0.0026 & & -0.0031 & -0.0045 & -0.0062 & -0.0084 & -0.0100 & -0.0115 & -0.0119\\
0982 &  3.1E-4 &  7.3E-5 &  5.7E-4 &  1.1E-4 &  0.0045 &  0.0048 &  0.0028 & & -0.0031 & -0.0045 & -0.0062 & -0.0084 & -0.0100 & -0.0115 & -0.0119\\
0983 &  3.2E-4 &  3.5E-5 &  5.0E-4 &  2.2E-4 &  0.0045 &  0.0043 &  0.0025 & & -0.0030 & -0.0045 & -0.0062 & -0.0084 & -0.0099 & -0.0115 & -0.0119\\
0984 &  3.4E-4 &  3.0E-5 &  4.4E-4 &  2.7E-4 &  0.0046 &  0.0037 &  0.0026 & & -0.0030 & -0.0045 & -0.0062 & -0.0084 & -0.0099 & -0.0115 & -0.0118\\
0985 &  3.5E-4 &  4.5E-5 &  3.3E-4 &  3.8E-4 &  0.0047 &  0.0031 &  0.0028 & & -0.0030 & -0.0045 & -0.0062 & -0.0083 & -0.0098 & -0.0115 & -0.0118\\
0986 &  3.8E-4 &  1.1E-5 &  2.3E-4 &  5.0E-4 &  0.0048 &  0.0025 &  0.0025 & & -0.0030 & -0.0045 & -0.0062 & -0.0083 & -0.0098 & -0.0115 & -0.0118\\
0987 &  3.9E-4 &  1.1E-5 &  1.4E-4 &  5.7E-4 &  0.0049 &  0.0017 &  0.0026 & & -0.0030 & -0.0044 & -0.0062 & -0.0083 & -0.0097 & -0.0115 & -0.0118\\
0988 &  4.1E-4 &  3.3E-5 &  1.1E-5 &  6.9E-4 &  0.0048 &  9.7E-4 &  0.0028 & & -0.0030 & -0.0044 & -0.0061 & -0.0082 & -0.0097 & -0.0115 & -0.0117\\
0989 &  4.4E-4 &  2.6E-6 &  1.3E-4 &  8.4E-4 &  0.0048 &  2.4E-4 &  0.0026 & & -0.0029 & -0.0044 & -0.0061 & -0.0082 & -0.0097 & -0.0115 & -0.0117\\
0990 &  4.5E-4 &  5.7E-6 &  2.4E-4 &  9.2E-4 &  0.0047 &  6.1E-4 &  0.0026 & & -0.0029 & -0.0044 & -0.0061 & -0.0082 & -0.0096 & -0.0115 & -0.0117\\
0991 &  4.7E-4 &  3.4E-5 &  3.9E-4 & -0.0011 &  0.0045 & -0.0015 &  0.0028 & & -0.0029 & -0.0044 & -0.0061 & -0.0081 & -0.0096 & -0.0115 & -0.0116\\
0992 &  5.1E-4 &  7.3E-6 &  5.6E-4 & -0.0012 &  0.0043 & -0.0023 &  0.0026 & & -0.0029 & -0.0044 & -0.0061 & -0.0081 & -0.0096 & -0.0115 & -0.0116\\
0993 &  5.3E-4 &  1.4E-5 &  7.1E-4 & -0.0013 &  0.0040 & -0.0033 &  0.0026 & & -0.0029 & -0.0043 & -0.0061 & -0.0081 & -0.0096 & -0.0115 & -0.0116\\
0994 &  5.6E-4 &  4.9E-5 &  8.9E-4 & -0.0015 &  0.0037 & -0.0043 &  0.0029 & & -0.0029 & -0.0043 & -0.0061 & -0.0080 & -0.0095 & -0.0116 & -0.0115\\
0995 &  5.9E-4 &  2.5E-5 & -0.0011 & -0.0017 &  0.0034 & -0.0053 &  0.0026 & & -0.0029 & -0.0043 & -0.0061 & -0.0080 & -0.0095 & -0.0116 & -0.0115\\
0996 &  6.4E-4 &  3.4E-5 & -0.0013 & -0.0018 &  0.0029 & -0.0064 &  0.0026 & & -0.0029 & -0.0043 & -0.0060 & -0.0079 & -0.0095 & -0.0116 & -0.0115\\
0997 &  6.4E-4 &  7.5E-5 & -0.0015 & -0.0019 &  0.0025 & -0.0075 &  0.0029 & & -0.0028 & -0.0043 & -0.0060 & -0.0079 & -0.0095 & -0.0116 & -0.0114\\
0998 &  7.0E-4 &  5.4E-5 & -0.0017 & -0.0021 &  0.0020 & -0.0086 &  0.0026 & & -0.0028 & -0.0043 & -0.0060 & -0.0078 & -0.0094 & -0.0116 & -0.0114\\
0999 &  7.5E-4 &  6.6E-5 & -0.0019 & -0.0023 &  0.0014 & -0.0098 &  0.0026 & & -0.0028 & -0.0042 & -0.0060 & -0.0078 & -0.0094 & -0.0116 & -0.0114\\
\enddata
\tablenotetext{a}{1000 $\Delta v$ values given in units of $\delta v_\parallel\!\left(z\right) \equiv 0.25246\,z + 1.4731$ km s$^{-1}$}
\tablecomments{These are the hybrid correlation 
values for full-resolution.}
\end{deluxetable}


==> tab5_full.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                       %%
%% THIS TEX FILE WAS CREATED BY AN IDL SCRIPT AND SHOULD %%
%%  NOT BE MODIFIED - MAKE CHANGES TO SCRIPT INSTEAD...  %%
%%                                                       %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{deluxetable}{crrrrrrrrrrrrrrr}
\tablecolumns{16}
\tabletypesize{\tiny}
\tablewidth{7.25in}
\tablecaption{Cross-Correlation (\citet{2005kir360mnras1373} Mean Flux Decrement).\label{tab_cross_k05}}
\tablehead{
\colhead{$\Delta v$\tablenotemark{a}} & \multicolumn{7}{c}{$10\times\xi_\perp\!\left(\Delta v\right)$ in real-space} & 
\colhead{} & \multicolumn{7}{c}{$10\times\xi_\perp\!\left(\Delta v\right)$ in \emph{z}-space}\\
\cline{2-8}
\cline{10-16}
\colhead{($\delta v_\perp\!\left(z\right)$)} & 
\colhead{$z=1.8$} & \colhead{2.0} & \colhead{2.2} & \colhead{2.4} & 
\colhead{2.6} & \colhead{2.8} & \colhead{3.0} & 
\colhead{} & 
\colhead{$z=1.8$} & \colhead{2.0} & \colhead{2.2} & \colhead{2.4} & 
\colhead{2.6} & \colhead{2.8} & \colhead{3.0}}
\startdata
0000 &  0.3219 &  0.4503 &  0.5798 &  0.7403 &  0.9426 &  1.1868 &  1.4890 & &  0.5778 &  0.7721 &  0.9534 &  1.1649 &  1.4131 &  1.7022 &  2.0396\\
0001 &  0.3173 &  0.4449 &  0.5735 &  0.7323 &  0.9326 &  1.1738 &  1.4715 & &  0.5596 &  0.7527 &  0.9342 &  1.1448 &  1.3905 &  1.6772 &  2.0107\\
0002 &  0.3078 &  0.4319 &  0.5569 &  0.7110 &  0.9052 &  1.1389 &  1.4279 & &  0.5400 &  0.7295 &  0.9081 &  1.1144 &  1.3555 &  1.6371 &  1.9642\\
0003 &  0.2950 &  0.4143 &  0.5340 &  0.6817 &  0.8678 &  1.0918 &  1.3684 & &  0.5204 &  0.7049 &  0.8793 &  1.0807 &  1.3151 &  1.5886 &  1.9065\\
0004 &  0.2803 &  0.3933 &  0.5060 &  0.6457 &  0.8232 &  1.0356 &  1.2985 & &  0.4991 &  0.6790 &  0.8453 &  1.0414 &  1.2702 &  1.5338 &  1.8410\\
0005 &  0.2651 &  0.3722 &  0.4785 &  0.6106 &  0.7777 &  0.9778 &  1.2241 & &  0.4794 &  0.6535 &  0.8150 &  1.0045 &  1.2250 &  1.4791 &  1.7738\\
0006 &  0.2493 &  0.3499 &  0.4493 &  0.5726 &  0.7289 &  0.9159 &  1.1461 & &  0.4585 &  0.6270 &  0.7830 &  0.9650 &  1.1776 &  1.4221 &  1.7039\\
0007 &  0.2334 &  0.3268 &  0.4188 &  0.5329 &  0.6781 &  0.8520 &  1.0666 & &  0.4376 &  0.5993 &  0.7496 &  0.9252 &  1.1289 &  1.3632 &  1.6339\\
0008 &  0.2178 &  0.3049 &  0.3903 &  0.4964 &  0.6311 &  0.7919 &  0.9902 & &  0.4192 &  0.5751 &  0.7210 &  0.8890 &  1.0849 &  1.3091 &  1.5671\\
0009 &  0.2025 &  0.2830 &  0.3618 &  0.4592 &  0.5842 &  0.7332 &  0.9169 & &  0.4004 &  0.5516 &  0.6908 &  0.8524 &  1.0406 &  1.2567 &  1.5026\\
0010 &  0.1881 &  0.2626 &  0.3352 &  0.4250 &  0.5407 &  0.6786 &  0.8490 & &  0.3827 &  0.5290 &  0.6634 &  0.8183 &  0.9992 &  1.2068 &  1.4415\\
0012 &  0.1621 &  0.2259 &  0.2880 &  0.3650 &  0.4645 &  0.5837 &  0.7318 & &  0.3514 &  0.4875 &  0.6136 &  0.7572 &  0.9249 &  1.1156 &  1.3321\\
0013 &  0.1504 &  0.2098 &  0.2672 &  0.3389 &  0.4318 &  0.5435 &  0.6822 & &  0.3371 &  0.4687 &  0.5910 &  0.7306 &  0.8916 &  1.0763 &  1.2838\\
0015 &  0.1306 &  0.1821 &  0.2323 &  0.2953 &  0.3774 &  0.4764 &  0.6003 & &  0.3125 &  0.4360 &  0.5515 &  0.6824 &  0.8334 &  1.0044 &  1.1978\\
0017 &  0.1143 &  0.1594 &  0.2039 &  0.2602 &  0.3338 &  0.4232 &  0.5350 & &  0.2918 &  0.4093 &  0.5179 &  0.6405 &  0.7833 &  0.9432 &  1.1210\\
0020 &  0.0957 &  0.1340 &  0.1727 &  0.2213 &  0.2849 &  0.3624 &  0.4605 & &  0.2665 &  0.3763 &  0.4765 &  0.5898 &  0.7191 &  0.8644 &  1.0273\\
0022 &  0.0858 &  0.1207 &  0.1561 &  0.2011 &  0.2608 &  0.3334 &  0.4244 & &  0.2519 &  0.3565 &  0.4538 &  0.5616 &  0.6863 &  0.8262 &  0.9789\\
0023 &  0.0816 &  0.1151 &  0.1491 &  0.1925 &  0.2501 &  0.3202 &  0.4079 & &  0.2453 &  0.3483 &  0.4431 &  0.5485 &  0.6700 &  0.8066 &  0.9554\\
0025 &  0.0743 &  0.1052 &  0.1370 &  0.1774 &  0.2313 &  0.2967 &  0.3788 & &  0.2337 &  0.3323 &  0.4237 &  0.5247 &  0.6407 &  0.7704 &  0.9118\\
0030 &  0.0610 &  0.0870 &  0.1143 &  0.1493 &  0.1952 &  0.2508 &  0.3206 & &  0.2121 &  0.3016 &  0.3836 &  0.4756 &  0.5779 &  0.6926 &  0.8180\\
0033 &  0.0551 &  0.0790 &  0.1042 &  0.1366 &  0.1791 &  0.2306 &  0.2950 & &  0.2008 &  0.2867 &  0.3643 &  0.4506 &  0.5476 &  0.6554 &  0.7731\\
0035 &  0.0518 &  0.0745 &  0.0985 &  0.1297 &  0.1704 &  0.2193 &  0.2810 & &  0.1925 &  0.2772 &  0.3526 &  0.4355 &  0.5301 &  0.6331 &  0.7467\\
0037 &  0.0490 &  0.0706 &  0.0933 &  0.1229 &  0.1618 &  0.2087 &  0.2669 & &  0.1884 &  0.2688 &  0.3421 &  0.4224 &  0.5127 &  0.6122 &  0.7205\\
0040 &  0.0455 &  0.0656 &  0.0875 &  0.1152 &  0.1523 &  0.1959 &  0.2499 & &  0.1815 &  0.2574 &  0.3269 &  0.4043 &  0.4905 &  0.5849 &  0.6863\\
0042 &  0.0431 &  0.0625 &  0.0827 &  0.1090 &  0.1443 &  0.1870 &  0.2394 & &  0.1748 &  0.2494 &  0.3179 &  0.3917 &  0.4749 &  0.5657 &  0.6640\\
0043 &  0.0422 &  0.0611 &  0.0809 &  0.1066 &  0.1411 &  0.1831 &  0.2346 & &  0.1723 &  0.2464 &  0.3131 &  0.3862 &  0.4676 &  0.5569 &  0.6536\\
0045 &  0.0404 &  0.0585 &  0.0775 &  0.1021 &  0.1354 &  0.1758 &  0.2255 & &  0.1681 &  0.2396 &  0.3046 &  0.3751 &  0.4539 &  0.5399 &  0.6336\\
0050 &  0.0366 &  0.0529 &  0.0704 &  0.0924 &  0.1235 &  0.1615 &  0.2058 & &  0.1582 &  0.2253 &  0.2835 &  0.3489 &  0.4237 &  0.5058 &  0.5900\\
0055 &  0.0332 &  0.0480 &  0.0640 &  0.0851 &  0.1127 &  0.1458 &  0.1876 & &  0.1479 &  0.2114 &  0.2674 &  0.3281 &  0.3955 &  0.4683 &  0.5474\\
0060 &  0.0312 &  0.0447 &  0.0600 &  0.0802 &  0.1064 &  0.1369 &  0.1755 & &  0.1422 &  0.2019 &  0.2558 &  0.3121 &  0.3742 &  0.4426 &  0.5172\\
0065 &  0.0287 &  0.0412 &  0.0545 &  0.0730 &  0.0974 &  0.1265 &  0.1622 & &  0.1334 &  0.1894 &  0.2393 &  0.2921 &  0.3507 &  0.4139 &  0.4833\\
0068 &  0.0274 &  0.0395 &  0.0522 &  0.0699 &  0.0935 &  0.1215 &  0.1559 & &  0.1294 &  0.1835 &  0.2315 &  0.2822 &  0.3387 &  0.3994 &  0.4659\\
0070 &  0.0269 &  0.0384 &  0.0518 &  0.0692 &  0.0921 &  0.1191 &  0.1524 & &  0.1263 &  0.1802 &  0.2278 &  0.2778 &  0.3314 &  0.3904 &  0.4560\\
0072 &  0.0260 &  0.0374 &  0.0496 &  0.0662 &  0.0885 &  0.1155 &  0.1482 & &  0.1242 &  0.1763 &  0.2221 &  0.2701 &  0.3241 &  0.3820 &  0.4455\\
0077 &  0.0243 &  0.0350 &  0.0466 &  0.0621 &  0.0830 &  0.1087 &  0.1397 & &  0.1177 &  0.1672 &  0.2109 &  0.2557 &  0.3069 &  0.3618 &  0.4215\\
0078 &  0.0239 &  0.0345 &  0.0460 &  0.0613 &  0.0819 &  0.1073 &  0.1380 & &  0.1163 &  0.1657 &  0.2086 &  0.2531 &  0.3037 &  0.3578 &  0.4168\\
0080 &  0.0233 &  0.0336 &  0.0448 &  0.0597 &  0.0799 &  0.1047 &  0.1348 & &  0.1143 &  0.1619 &  0.2045 &  0.2479 &  0.2973 &  0.3499 &  0.4083\\
0090 &  0.0208 &  0.0299 &  0.0400 &  0.0541 &  0.0727 &  0.0966 &  0.1227 & &  0.1058 &  0.1478 &  0.1850 &  0.2253 &  0.2711 &  0.3227 &  0.3726\\
0100 &  0.0188 &  0.0269 &  0.0367 &  0.0490 &  0.0652 &  0.0856 &  0.1081 & &  0.0971 &  0.1365 &  0.1718 &  0.2082 &  0.2479 &  0.2902 &  0.3345\\
0105 &  0.0179 &  0.0254 &  0.0343 &  0.0466 &  0.0618 &  0.0803 &  0.1029 & &  0.0920 &  0.1290 &  0.1619 &  0.1980 &  0.2344 &  0.2739 &  0.3173\\
0125 &  0.0146 &  0.0208 &  0.0285 &  0.0381 &  0.0502 &  0.0655 &  0.0832 & &  0.0784 &  0.1091 &  0.1361 &  0.1652 &  0.1947 &  0.2259 &  0.2608\\
0130 &  0.0140 &  0.0198 &  0.0271 &  0.0363 &  0.0487 &  0.0634 &  0.0805 & &  0.0758 &  0.1057 &  0.1317 &  0.1575 &  0.1869 &  0.2185 &  0.2518\\
0135 &  0.0134 &  0.0188 &  0.0256 &  0.0342 &  0.0453 &  0.0588 &  0.0742 & &  0.0734 &  0.1019 &  0.1259 &  0.1518 &  0.1780 &  0.2064 &  0.2366\\
0138 &  0.0130 &  0.0183 &  0.0249 &  0.0333 &  0.0440 &  0.0566 &  0.0717 & &  0.0717 &  0.0998 &  0.1234 &  0.1482 &  0.1737 &  0.2005 &  0.2296\\
0142 &  0.0126 &  0.0176 &  0.0240 &  0.0321 &  0.0421 &  0.0541 &  0.0685 & &  0.0699 &  0.0973 &  0.1199 &  0.1434 &  0.1678 &  0.1931 &  0.2206\\
0147 &  0.0121 &  0.0169 &  0.0229 &  0.0304 &  0.0402 &  0.0516 &  0.0658 & &  0.0668 &  0.0936 &  0.1153 &  0.1367 &  0.1603 &  0.1853 &  0.2112\\
0148 &  0.0120 &  0.0168 &  0.0227 &  0.0301 &  0.0398 &  0.0512 &  0.0653 & &  0.0665 &  0.0928 &  0.1142 &  0.1355 &  0.1592 &  0.1837 &  0.2095\\
0150 &  0.0118 &  0.0165 &  0.0223 &  0.0295 &  0.0390 &  0.0502 &  0.0644 & &  0.0657 &  0.0908 &  0.1121 &  0.1327 &  0.1562 &  0.1801 &  0.2061\\
0165 &  0.0106 &  0.0147 &  0.0200 &  0.0274 &  0.0361 &  0.0468 &  0.0601 & &  0.0609 &  0.0812 &  0.1001 &  0.1190 &  0.1390 &  0.1605 &  0.1847\\
0170 &  0.0100 &  0.0141 &  0.0191 &  0.0262 &  0.0351 &  0.0458 &  0.0577 & &  0.0584 &  0.0784 &  0.0961 &  0.1151 &  0.1360 &  0.1540 &  0.1757\\
0185 &  0.0089 &  0.0127 &  0.0176 &  0.0237 &  0.0313 &  0.0421 &  0.0538 & &  0.0540 &  0.0720 &  0.0883 &  0.1044 &  0.1211 &  0.1373 &  0.1565\\
0195 &  0.0084 &  0.0120 &  0.0169 &  0.0234 &  0.0300 &  0.0400 &  0.0502 & &  0.0517 &  0.0685 &  0.0831 &  0.0979 &  0.1137 &  0.1292 &  0.1469\\
0198 &  0.0082 &  0.0119 &  0.0166 &  0.0231 &  0.0296 &  0.0389 &  0.0495 & &  0.0508 &  0.0671 &  0.0816 &  0.0959 &  0.1115 &  0.1269 &  0.1449\\
0202 &  0.0081 &  0.0115 &  0.0162 &  0.0223 &  0.0290 &  0.0377 &  0.0487 & &  0.0496 &  0.0654 &  0.0786 &  0.0926 &  0.1084 &  0.1250 &  0.1420\\
0205 &  0.0081 &  0.0113 &  0.0155 &  0.0214 &  0.0295 &  0.0369 &  0.0473 & &  0.0485 &  0.0635 &  0.0762 &  0.0898 &  0.1061 &  0.1235 &  0.1422\\
0207 &  0.0080 &  0.0110 &  0.0157 &  0.0216 &  0.0288 &  0.0364 &  0.0476 & &  0.0482 &  0.0626 &  0.0755 &  0.0886 &  0.1038 &  0.1228 &  0.1383\\
0208 &  0.0079 &  0.0110 &  0.0156 &  0.0215 &  0.0285 &  0.0363 &  0.0474 & &  0.0479 &  0.0621 &  0.0750 &  0.0878 &  0.1032 &  0.1224 &  0.1374\\
0210 &  0.0078 &  0.0108 &  0.0154 &  0.0213 &  0.0281 &  0.0360 &  0.0467 & &  0.0475 &  0.0612 &  0.0743 &  0.0866 &  0.1022 &  0.1216 &  0.1359\\
0220 &  0.0078 &  0.0109 &  0.0150 &  0.0205 &  0.0260 &  0.0345 &  0.0446 & &  0.0461 &  0.0588 &  0.0693 &  0.0824 &  0.0993 &  0.1174 &  0.1303\\
0225 &  0.0075 &  0.0102 &  0.0138 &  0.0196 &  0.0253 &  0.0337 &  0.0416 & &  0.0449 &  0.0568 &  0.0667 &  0.0801 &  0.0977 &  0.1158 &  0.1265\\
0235 &  0.0072 &  0.0097 &  0.0139 &  0.0181 &  0.0244 &  0.0313 &  0.0392 & &  0.0434 &  0.0539 &  0.0636 &  0.0773 &  0.0939 &  0.1115 &  0.1200\\
0238 &  0.0072 &  0.0096 &  0.0139 &  0.0178 &  0.0240 &  0.0304 &  0.0385 & &  0.0430 &  0.0530 &  0.0627 &  0.0762 &  0.0930 &  0.1100 &  0.1188\\
0242 &  0.0071 &  0.0096 &  0.0135 &  0.0176 &  0.0232 &  0.0293 &  0.0375 & &  0.0420 &  0.0524 &  0.0615 &  0.0746 &  0.0919 &  0.1082 &  0.1164\\
0247 &  0.0071 &  0.0096 &  0.0129 &  0.0172 &  0.0229 &  0.0282 &  0.0358 & &  0.0406 &  0.0508 &  0.0601 &  0.0725 &  0.0891 &  0.1062 &  0.1132\\
0248 &  0.0070 &  0.0096 &  0.0129 &  0.0171 &  0.0226 &  0.0280 &  0.0355 & &  0.0403 &  0.0505 &  0.0598 &  0.0721 &  0.0889 &  0.1059 &  0.1128\\
0250 &  0.0070 &  0.0096 &  0.0127 &  0.0170 &  0.0223 &  0.0276 &  0.0349 & &  0.0399 &  0.0501 &  0.0593 &  0.0714 &  0.0880 &  0.1052 &  0.1115\\
0255 &  0.0068 &  0.0094 &  0.0123 &  0.0165 &  0.0216 &  0.0262 &  0.0355 & &  0.0393 &  0.0485 &  0.0575 &  0.0695 &  0.0860 &  0.1037 &  0.1083\\
0275 &  0.0065 &  0.0085 &  0.0111 &  0.0157 &  0.0184 &  0.0209 &  0.0302 & &  0.0371 &  0.0442 &  0.0501 &  0.0616 &  0.0802 &  0.0948 &  0.0974\\
0285 &  0.0062 &  0.0077 &  0.0112 &  0.0152 &  0.0169 &  0.0177 &  0.0301 & &  0.0371 &  0.0421 &  0.0467 &  0.0594 &  0.0770 &  0.0890 &  0.0937\\
0288 &  0.0062 &  0.0076 &  0.0113 &  0.0151 &  0.0163 &  0.0166 &  0.0297 & &  0.0372 &  0.0416 &  0.0460 &  0.0588 &  0.0760 &  0.0871 &  0.0932\\
0292 &  0.0060 &  0.0074 &  0.0115 &  0.0150 &  0.0156 &  0.0149 &  0.0289 & &  0.0375 &  0.0411 &  0.0452 &  0.0582 &  0.0744 &  0.0843 &  0.0912\\
0297 &  0.0058 &  0.0074 &  0.0118 &  0.0149 &  0.0146 &  0.0131 &  0.0279 & &  0.0379 &  0.0403 &  0.0446 &  0.0575 &  0.0722 &  0.0808 &  0.0883\\
0298 &  0.0057 &  0.0074 &  0.0118 &  0.0149 &  0.0143 &  0.0127 &  0.0277 & &  0.0380 &  0.0401 &  0.0445 &  0.0573 &  0.0717 &  0.0801 &  0.0879\\
0300 &  0.0057 &  0.0074 &  0.0119 &  0.0148 &  0.0139 &  0.0119 &  0.0274 & &  0.0380 &  0.0400 &  0.0443 &  0.0570 &  0.0707 &  0.0786 &  0.0870\\
\enddata
\tablenotetext{a}{74 $\Delta v$ values given in units of $\delta v_\perp\!\left(z\right) \equiv 0.67455\,z + 0.38896$ km s$^{-1}$ (or, alternatively, arcseconds)}
\tablecomments{These are the hybrid correlation 
values for full-resolution.}
\end{deluxetable}


==> tab6_full.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                       %%
%% THIS TEX FILE WAS CREATED BY AN IDL SCRIPT AND SHOULD %%
%%  NOT BE MODIFIED - MAKE CHANGES TO SCRIPT INSTEAD...  %%
%%                                                       %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{deluxetable}{crrrrrrrrrrrrrrr}
\tablecolumns{16}
\tabletypesize{\tiny}
\tablewidth{7.25in}
\tablecaption{Autocorrelation (\citet{2005kir360mnras1373} Mean Flux Decrement).\label{tab_auto_k05}}
\tablehead{
\colhead{$\Delta v$\tablenotemark{a}} & \multicolumn{7}{c}{$10\times\xi_\parallel\!\left(\Delta v\right)$ in real-space} & 
\colhead{} & \multicolumn{7}{c}{$10\times\xi_\parallel\!\left(\Delta v\right)$ in \emph{z}-space}\\
\cline{2-8}
\cline{10-16}
\colhead{($\delta v_\parallel\!\left(z\right)$)} & 
\colhead{$z=1.8$} & \colhead{2.0} & \colhead{2.2} & \colhead{2.4} & 
\colhead{2.6} & \colhead{2.8} & \colhead{3.0} & 
\colhead{} & 
\colhead{$z=1.8$} & \colhead{2.0} & \colhead{2.2} & \colhead{2.4} & 
\colhead{2.6} & \colhead{2.8} & \colhead{3.0}}
\startdata
0000 &  0.3219 &  0.4503 &  0.5798 &  0.7403 &  0.9426 &  1.1868 &  1.4890 & &  0.5778 &  0.7721 &  0.9534 &  1.1649 &  1.4131 &  1.7022 &  2.0396\\
0001 &  0.3162 &  0.4435 &  0.5721 &  0.7312 &  0.9320 &  1.1743 &  1.4742 & &  0.5770 &  0.7709 &  0.9518 &  1.1628 &  1.4103 &  1.6987 &  2.0352\\
0002 &  0.3033 &  0.4275 &  0.5531 &  0.7087 &  0.9052 &  1.1425 &  1.4362 & &  0.5746 &  0.7674 &  0.9471 &  1.1565 &  1.4022 &  1.6883 &  2.0221\\
0003 &  0.2868 &  0.4065 &  0.5277 &  0.6782 &  0.8685 &  1.0985 &  1.3834 & &  0.5707 &  0.7616 &  0.9393 &  1.1463 &  1.3890 &  1.6715 &  2.0007\\
0004 &  0.2687 &  0.3828 &  0.4988 &  0.6430 &  0.8259 &  1.0472 &  1.3214 & &  0.5653 &  0.7537 &  0.9288 &  1.1325 &  1.3710 &  1.6487 &  1.9720\\
0005 &  0.2497 &  0.3576 &  0.4677 &  0.6050 &  0.7797 &  0.9912 &  1.2536 & &  0.5586 &  0.7439 &  0.9156 &  1.1153 &  1.3489 &  1.6206 &  1.9367\\
0006 &  0.2304 &  0.3318 &  0.4356 &  0.5656 &  0.7314 &  0.9324 &  1.1820 & &  0.5508 &  0.7324 &  0.9003 &  1.0953 &  1.3231 &  1.5879 &  1.8959\\
0007 &  0.2116 &  0.3062 &  0.4035 &  0.5258 &  0.6824 &  0.8724 &  1.1087 & &  0.5419 &  0.7194 &  0.8830 &  1.0728 &  1.2942 &  1.5516 &  1.8505\\
0008 &  0.1937 &  0.2816 &  0.3724 &  0.4869 &  0.6341 &  0.8130 &  1.0358 & &  0.5321 &  0.7051 &  0.8641 &  1.0483 &  1.2629 &  1.5122 &  1.8016\\
0009 &  0.1770 &  0.2585 &  0.3429 &  0.4497 &  0.5876 &  0.7556 &  0.9650 & &  0.5215 &  0.6898 &  0.8440 &  1.0222 &  1.2296 &  1.4705 &  1.7500\\
0010 &  0.1618 &  0.2372 &  0.3155 &  0.4150 &  0.5440 &  0.7014 &  0.8980 & &  0.5104 &  0.6737 &  0.8228 &  0.9949 &  1.1950 &  1.4273 &  1.6965\\
0011 &  0.1480 &  0.2178 &  0.2905 &  0.3832 &  0.5038 &  0.6512 &  0.8357 & &  0.4987 &  0.6570 &  0.8009 &  0.9668 &  1.1593 &  1.3829 &  1.6419\\
0012 &  0.1358 &  0.2004 &  0.2680 &  0.3544 &  0.4673 &  0.6055 &  0.7789 & &  0.4868 &  0.6398 &  0.7786 &  0.9382 &  1.1232 &  1.3381 &  1.5867\\
0013 &  0.1249 &  0.1849 &  0.2479 &  0.3287 &  0.4345 &  0.5644 &  0.7276 & &  0.4746 &  0.6224 &  0.7560 &  0.9093 &  1.0869 &  1.2931 &  1.5316\\
0014 &  0.1154 &  0.1712 &  0.2301 &  0.3058 &  0.4053 &  0.5276 &  0.6817 & &  0.4623 &  0.6049 &  0.7333 &  0.8805 &  1.0507 &  1.2484 &  1.4768\\
0015 &  0.1069 &  0.1590 &  0.2143 &  0.2855 &  0.3793 &  0.4949 &  0.6408 & &  0.4499 &  0.5875 &  0.7108 &  0.8519 &  1.0149 &  1.2042 &  1.4229\\
0016 &  0.0995 &  0.1483 &  0.2004 &  0.2675 &  0.3563 &  0.4658 &  0.6043 & &  0.4376 &  0.5701 &  0.6885 &  0.8238 &  0.9798 &  1.1609 &  1.3701\\
0017 &  0.0929 &  0.1389 &  0.1880 &  0.2516 &  0.3358 &  0.4399 &  0.5717 & &  0.4253 &  0.5530 &  0.6666 &  0.7961 &  0.9454 &  1.1187 &  1.3186\\
0018 &  0.0871 &  0.1305 &  0.1771 &  0.2374 &  0.3175 &  0.4167 &  0.5425 & &  0.4133 &  0.5362 &  0.6451 &  0.7692 &  0.9119 &  1.0777 &  1.2687\\
0019 &  0.0819 &  0.1230 &  0.1673 &  0.2248 &  0.3012 &  0.3959 &  0.5163 & &  0.4014 &  0.5197 &  0.6242 &  0.7429 &  0.8794 &  1.0380 &  1.2205\\
0020 &  0.0773 &  0.1163 &  0.1585 &  0.2134 &  0.2865 &  0.3773 &  0.4926 & &  0.3898 &  0.5037 &  0.6038 &  0.7175 &  0.8480 &  0.9997 &  1.1742\\
0021 &  0.0732 &  0.1103 &  0.1507 &  0.2033 &  0.2734 &  0.3604 &  0.4712 & &  0.3784 &  0.4881 &  0.5841 &  0.6930 &  0.8178 &  0.9629 &  1.1297\\
0022 &  0.0695 &  0.1050 &  0.1436 &  0.1941 &  0.2614 &  0.3451 &  0.4517 & &  0.3674 &  0.4729 &  0.5651 &  0.6693 &  0.7888 &  0.9277 &  1.0873\\
0023 &  0.0662 &  0.1001 &  0.1373 &  0.1858 &  0.2506 &  0.3312 &  0.4339 & &  0.3566 &  0.4583 &  0.5467 &  0.6465 &  0.7609 &  0.8940 &  1.0467\\
0024 &  0.0632 &  0.0957 &  0.1315 &  0.1782 &  0.2408 &  0.3185 &  0.4176 & &  0.3462 &  0.4441 &  0.5289 &  0.6246 &  0.7343 &  0.8618 &  1.0081\\
0025 &  0.0604 &  0.0917 &  0.1262 &  0.1713 &  0.2317 &  0.3068 &  0.4027 & &  0.3361 &  0.4304 &  0.5119 &  0.6037 &  0.7087 &  0.8311 &  0.9715\\
0026 &  0.0580 &  0.0880 &  0.1213 &  0.1650 &  0.2234 &  0.2961 &  0.3888 & &  0.3263 &  0.4172 &  0.4955 &  0.5835 &  0.6844 &  0.8019 &  0.9366\\
0027 &  0.0557 &  0.0846 &  0.1169 &  0.1591 &  0.2158 &  0.2862 &  0.3761 & &  0.3168 &  0.4045 &  0.4797 &  0.5643 &  0.6611 &  0.7741 &  0.9036\\
0028 &  0.0536 &  0.0815 &  0.1128 &  0.1537 &  0.2087 &  0.2771 &  0.3642 & &  0.3077 &  0.3923 &  0.4646 &  0.5458 &  0.6389 &  0.7477 &  0.8723\\
0029 &  0.0517 &  0.0787 &  0.1090 &  0.1488 &  0.2022 &  0.2686 &  0.3532 & &  0.2989 &  0.3805 &  0.4501 &  0.5282 &  0.6178 &  0.7226 &  0.8427\\
0030 &  0.0499 &  0.0761 &  0.1055 &  0.1441 &  0.1960 &  0.2606 &  0.3429 & &  0.2903 &  0.3692 &  0.4362 &  0.5113 &  0.5976 &  0.6987 &  0.8145\\
0031 &  0.0483 &  0.0736 &  0.1023 &  0.1398 &  0.1903 &  0.2532 &  0.3332 & &  0.2821 &  0.3583 &  0.4229 &  0.4952 &  0.5783 &  0.6760 &  0.7879\\
0032 &  0.0468 &  0.0714 &  0.0992 &  0.1358 &  0.1850 &  0.2463 &  0.3242 & &  0.2742 &  0.3478 &  0.4101 &  0.4797 &  0.5599 &  0.6543 &  0.7626\\
0033 &  0.0453 &  0.0692 &  0.0964 &  0.1320 &  0.1800 &  0.2397 &  0.3157 & &  0.2666 &  0.3378 &  0.3978 &  0.4649 &  0.5423 &  0.6337 &  0.7386\\
0034 &  0.0440 &  0.0672 &  0.0937 &  0.1285 &  0.1753 &  0.2336 &  0.3076 & &  0.2592 &  0.3281 &  0.3860 &  0.4508 &  0.5256 &  0.6141 &  0.7158\\
0035 &  0.0428 &  0.0654 &  0.0912 &  0.1252 &  0.1708 &  0.2278 &  0.3001 & &  0.2522 &  0.3188 &  0.3747 &  0.4372 &  0.5095 &  0.5954 &  0.6941\\
0036 &  0.0416 &  0.0636 &  0.0888 &  0.1220 &  0.1666 &  0.2223 &  0.2929 & &  0.2453 &  0.3099 &  0.3639 &  0.4242 &  0.4942 &  0.5776 &  0.6735\\
0037 &  0.0405 &  0.0619 &  0.0865 &  0.1190 &  0.1626 &  0.2170 &  0.2861 & &  0.2387 &  0.3012 &  0.3535 &  0.4118 &  0.4795 &  0.5605 &  0.6538\\
0038 &  0.0394 &  0.0603 &  0.0844 &  0.1162 &  0.1588 &  0.2121 &  0.2796 & &  0.2324 &  0.2930 &  0.3435 &  0.3998 &  0.4655 &  0.5442 &  0.6350\\
0039 &  0.0384 &  0.0588 &  0.0824 &  0.1135 &  0.1552 &  0.2073 &  0.2734 & &  0.2262 &  0.2850 &  0.3338 &  0.3883 &  0.4520 &  0.5286 &  0.6171\\
0040 &  0.0375 &  0.0574 &  0.0804 &  0.1109 &  0.1517 &  0.2028 &  0.2675 & &  0.2203 &  0.2773 &  0.3246 &  0.3773 &  0.4391 &  0.5137 &  0.6000\\
0041 &  0.0366 &  0.0560 &  0.0786 &  0.1085 &  0.1484 &  0.1985 &  0.2618 & &  0.2146 &  0.2699 &  0.3157 &  0.3667 &  0.4266 &  0.4994 &  0.5837\\
0042 &  0.0357 &  0.0547 &  0.0769 &  0.1061 &  0.1453 &  0.1943 &  0.2564 & &  0.2091 &  0.2627 &  0.3071 &  0.3565 &  0.4147 &  0.4856 &  0.5680\\
0043 &  0.0349 &  0.0535 &  0.0752 &  0.1039 &  0.1423 &  0.1904 &  0.2513 & &  0.2038 &  0.2558 &  0.2988 &  0.3467 &  0.4033 &  0.4724 &  0.5530\\
0044 &  0.0342 &  0.0523 &  0.0736 &  0.1018 &  0.1395 &  0.1866 &  0.2463 & &  0.1986 &  0.2492 &  0.2909 &  0.3372 &  0.3922 &  0.4598 &  0.5385\\
0045 &  0.0334 &  0.0512 &  0.0721 &  0.0998 &  0.1367 &  0.1829 &  0.2416 & &  0.1937 &  0.2428 &  0.2832 &  0.3281 &  0.3816 &  0.4476 &  0.5247\\
0046 &  0.0327 &  0.0502 &  0.0706 &  0.0978 &  0.1341 &  0.1795 &  0.2370 & &  0.1889 &  0.2366 &  0.2758 &  0.3193 &  0.3714 &  0.4358 &  0.5114\\
0047 &  0.0321 &  0.0491 &  0.0692 &  0.0960 &  0.1316 &  0.1761 &  0.2327 & &  0.1842 &  0.2306 &  0.2686 &  0.3109 &  0.3615 &  0.4245 &  0.4986\\
0048 &  0.0315 &  0.0481 &  0.0679 &  0.0942 &  0.1293 &  0.1729 &  0.2285 & &  0.1797 &  0.2249 &  0.2617 &  0.3027 &  0.3520 &  0.4136 &  0.4862\\
0049 &  0.0309 &  0.0472 &  0.0666 &  0.0925 &  0.1270 &  0.1699 &  0.2245 & &  0.1754 &  0.2193 &  0.2551 &  0.2948 &  0.3429 &  0.4031 &  0.4744\\
0050 &  0.0303 &  0.0463 &  0.0654 &  0.0909 &  0.1248 &  0.1670 &  0.2206 & &  0.1712 &  0.2139 &  0.2486 &  0.2872 &  0.3340 &  0.3929 &  0.4629\\
0051 &  0.0297 &  0.0454 &  0.0643 &  0.0893 &  0.1227 &  0.1642 &  0.2169 & &  0.1671 &  0.2087 &  0.2424 &  0.2798 &  0.3254 &  0.3831 &  0.4518\\
0052 &  0.0292 &  0.0446 &  0.0631 &  0.0878 &  0.1207 &  0.1615 &  0.2133 & &  0.1632 &  0.2036 &  0.2364 &  0.2727 &  0.3172 &  0.3737 &  0.4411\\
0053 &  0.0287 &  0.0438 &  0.0620 &  0.0863 &  0.1187 &  0.1589 &  0.2099 & &  0.1594 &  0.1988 &  0.2306 &  0.2659 &  0.3092 &  0.3645 &  0.4307\\
0054 &  0.0282 &  0.0431 &  0.0610 &  0.0849 &  0.1169 &  0.1564 &  0.2066 & &  0.1557 &  0.1941 &  0.2250 &  0.2592 &  0.3015 &  0.3556 &  0.4207\\
0055 &  0.0278 &  0.0424 &  0.0600 &  0.0836 &  0.1150 &  0.1539 &  0.2034 & &  0.1521 &  0.1895 &  0.2196 &  0.2528 &  0.2940 &  0.3470 &  0.4110\\
0056 &  0.0273 &  0.0417 &  0.0590 &  0.0823 &  0.1133 &  0.1516 &  0.2003 & &  0.1487 &  0.1851 &  0.2143 &  0.2466 &  0.2867 &  0.3387 &  0.4016\\
0057 &  0.0269 &  0.0410 &  0.0581 &  0.0810 &  0.1116 &  0.1493 &  0.1973 & &  0.1453 &  0.1808 &  0.2093 &  0.2406 &  0.2797 &  0.3306 &  0.3925\\
0058 &  0.0264 &  0.0404 &  0.0572 &  0.0798 &  0.1099 &  0.1471 &  0.1944 & &  0.1421 &  0.1767 &  0.2043 &  0.2348 &  0.2730 &  0.3228 &  0.3836\\
0059 &  0.0260 &  0.0398 &  0.0563 &  0.0786 &  0.1083 &  0.1449 &  0.1916 & &  0.1389 &  0.1727 &  0.1996 &  0.2292 &  0.2664 &  0.3152 &  0.3750\\
0060 &  0.0256 &  0.0392 &  0.0554 &  0.0774 &  0.1067 &  0.1429 &  0.1889 & &  0.1359 &  0.1688 &  0.1950 &  0.2237 &  0.2600 &  0.3079 &  0.3666\\
0061 &  0.0251 &  0.0386 &  0.0546 &  0.0763 &  0.1052 &  0.1408 &  0.1862 & &  0.1329 &  0.1650 &  0.1905 &  0.2185 &  0.2539 &  0.3008 &  0.3585\\
0062 &  0.0247 &  0.0380 &  0.0538 &  0.0752 &  0.1038 &  0.1389 &  0.1836 & &  0.1301 &  0.1614 &  0.1862 &  0.2134 &  0.2479 &  0.2939 &  0.3506\\
0063 &  0.0243 &  0.0374 &  0.0531 &  0.0742 &  0.1024 &  0.1370 &  0.1811 & &  0.1273 &  0.1578 &  0.1820 &  0.2085 &  0.2422 &  0.2872 &  0.3430\\
0064 &  0.0240 &  0.0369 &  0.0523 &  0.0731 &  0.1010 &  0.1351 &  0.1787 & &  0.1246 &  0.1544 &  0.1780 &  0.2037 &  0.2366 &  0.2807 &  0.3355\\
0065 &  0.0236 &  0.0363 &  0.0516 &  0.0721 &  0.0997 &  0.1333 &  0.1763 & &  0.1220 &  0.1511 &  0.1741 &  0.1991 &  0.2312 &  0.2744 &  0.3283\\
0066 &  0.0233 &  0.0358 &  0.0509 &  0.0712 &  0.0984 &  0.1316 &  0.1740 & &  0.1195 &  0.1479 &  0.1703 &  0.1946 &  0.2259 &  0.2683 &  0.3212\\
0067 &  0.0229 &  0.0352 &  0.0502 &  0.0702 &  0.0971 &  0.1300 &  0.1718 & &  0.1170 &  0.1447 &  0.1666 &  0.1903 &  0.2209 &  0.2624 &  0.3144\\
0068 &  0.0226 &  0.0347 &  0.0495 &  0.0693 &  0.0959 &  0.1283 &  0.1697 & &  0.1146 &  0.1417 &  0.1630 &  0.1861 &  0.2159 &  0.2566 &  0.3077\\
0069 &  0.0223 &  0.0342 &  0.0489 &  0.0684 &  0.0947 &  0.1268 &  0.1676 & &  0.1123 &  0.1387 &  0.1595 &  0.1820 &  0.2112 &  0.2510 &  0.3013\\
0070 &  0.0220 &  0.0337 &  0.0482 &  0.0675 &  0.0936 &  0.1253 &  0.1656 & &  0.1100 &  0.1358 &  0.1561 &  0.1781 &  0.2066 &  0.2457 &  0.2950\\
0071 &  0.0217 &  0.0332 &  0.0475 &  0.0666 &  0.0924 &  0.1238 &  0.1636 & &  0.1078 &  0.1330 &  0.1528 &  0.1743 &  0.2021 &  0.2404 &  0.2889\\
0072 &  0.0214 &  0.0328 &  0.0469 &  0.0657 &  0.0913 &  0.1223 &  0.1617 & &  0.1057 &  0.1303 &  0.1497 &  0.1705 &  0.1978 &  0.2354 &  0.2830\\
0073 &  0.0212 &  0.0323 &  0.0462 &  0.0649 &  0.0901 &  0.1209 &  0.1598 & &  0.1036 &  0.1277 &  0.1466 &  0.1669 &  0.1936 &  0.2304 &  0.2773\\
0074 &  0.0209 &  0.0319 &  0.0456 &  0.0641 &  0.0890 &  0.1195 &  0.1580 & &  0.1016 &  0.1251 &  0.1435 &  0.1634 &  0.1895 &  0.2257 &  0.2717\\
0075 &  0.0207 &  0.0314 &  0.0450 &  0.0632 &  0.0879 &  0.1181 &  0.1562 & &  0.0996 &  0.1226 &  0.1406 &  0.1600 &  0.1856 &  0.2211 &  0.2663\\
0076 &  0.0204 &  0.0310 &  0.0444 &  0.0624 &  0.0868 &  0.1167 &  0.1544 & &  0.0977 &  0.1201 &  0.1377 &  0.1567 &  0.1818 &  0.2166 &  0.2611\\
0077 &  0.0202 &  0.0306 &  0.0438 &  0.0616 &  0.0857 &  0.1153 &  0.1527 & &  0.0958 &  0.1177 &  0.1350 &  0.1535 &  0.1781 &  0.2122 &  0.2560\\
0078 &  0.0199 &  0.0302 &  0.0432 &  0.0608 &  0.0846 &  0.1139 &  0.1509 & &  0.0940 &  0.1154 &  0.1322 &  0.1504 &  0.1745 &  0.2080 &  0.2510\\
0079 &  0.0197 &  0.0298 &  0.0427 &  0.0601 &  0.0836 &  0.1125 &  0.1492 & &  0.0922 &  0.1132 &  0.1296 &  0.1473 &  0.1709 &  0.2039 &  0.2462\\
0080 &  0.0195 &  0.0294 &  0.0421 &  0.0593 &  0.0825 &  0.1111 &  0.1474 & &  0.0905 &  0.1110 &  0.1270 &  0.1443 &  0.1675 &  0.1999 &  0.2415\\
0081 &  0.0193 &  0.0291 &  0.0416 &  0.0585 &  0.0815 &  0.1098 &  0.1457 & &  0.0888 &  0.1088 &  0.1245 &  0.1414 &  0.1642 &  0.1961 &  0.2370\\
0082 &  0.0191 &  0.0287 &  0.0410 &  0.0578 &  0.0805 &  0.1084 &  0.1440 & &  0.0872 &  0.1067 &  0.1221 &  0.1386 &  0.1610 &  0.1923 &  0.2325\\
0083 &  0.0189 &  0.0284 &  0.0405 &  0.0571 &  0.0795 &  0.1071 &  0.1422 & &  0.0856 &  0.1047 &  0.1197 &  0.1359 &  0.1578 &  0.1886 &  0.2282\\
0084 &  0.0187 &  0.0280 &  0.0400 &  0.0564 &  0.0785 &  0.1058 &  0.1405 & &  0.0840 &  0.1027 &  0.1174 &  0.1332 &  0.1547 &  0.1850 &  0.2240\\
0085 &  0.0185 &  0.0277 &  0.0395 &  0.0557 &  0.0775 &  0.1045 &  0.1388 & &  0.0825 &  0.1007 &  0.1151 &  0.1305 &  0.1517 &  0.1816 &  0.2199\\
0086 &  0.0183 &  0.0274 &  0.0390 &  0.0550 &  0.0766 &  0.1032 &  0.1372 & &  0.0810 &  0.0989 &  0.1129 &  0.1280 &  0.1488 &  0.1782 &  0.2159\\
0087 &  0.0181 &  0.0271 &  0.0386 &  0.0543 &  0.0756 &  0.1020 &  0.1355 & &  0.0796 &  0.0970 &  0.1108 &  0.1255 &  0.1459 &  0.1749 &  0.2120\\
0088 &  0.0179 &  0.0268 &  0.0381 &  0.0537 &  0.0747 &  0.1007 &  0.1339 & &  0.0781 &  0.0952 &  0.1087 &  0.1230 &  0.1431 &  0.1716 &  0.2082\\
0089 &  0.0177 &  0.0266 &  0.0377 &  0.0530 &  0.0738 &  0.0995 &  0.1322 & &  0.0768 &  0.0935 &  0.1066 &  0.1206 &  0.1404 &  0.1685 &  0.2045\\
0090 &  0.0175 &  0.0263 &  0.0373 &  0.0524 &  0.0729 &  0.0983 &  0.1307 & &  0.0754 &  0.0918 &  0.1046 &  0.1183 &  0.1378 &  0.1654 &  0.2009\\
0091 &  0.0174 &  0.0261 &  0.0369 &  0.0518 &  0.0721 &  0.0971 &  0.1291 & &  0.0741 &  0.0901 &  0.1027 &  0.1160 &  0.1352 &  0.1623 &  0.1973\\
0092 &  0.0172 &  0.0258 &  0.0365 &  0.0513 &  0.0713 &  0.0960 &  0.1276 & &  0.0728 &  0.0885 &  0.1008 &  0.1138 &  0.1326 &  0.1594 &  0.1939\\
0093 &  0.0170 &  0.0256 &  0.0361 &  0.0507 &  0.0705 &  0.0949 &  0.1261 & &  0.0716 &  0.0869 &  0.0989 &  0.1116 &  0.1302 &  0.1565 &  0.1905\\
0094 &  0.0168 &  0.0253 &  0.0358 &  0.0502 &  0.0697 &  0.0938 &  0.1247 & &  0.0703 &  0.0853 &  0.0971 &  0.1095 &  0.1277 &  0.1537 &  0.1871\\
0095 &  0.0166 &  0.0251 &  0.0354 &  0.0496 &  0.0689 &  0.0927 &  0.1233 & &  0.0691 &  0.0838 &  0.0954 &  0.1075 &  0.1254 &  0.1510 &  0.1839\\
0096 &  0.0164 &  0.0248 &  0.0351 &  0.0491 &  0.0682 &  0.0916 &  0.1219 & &  0.0680 &  0.0824 &  0.0937 &  0.1055 &  0.1231 &  0.1483 &  0.1807\\
0097 &  0.0162 &  0.0246 &  0.0347 &  0.0486 &  0.0675 &  0.0906 &  0.1205 & &  0.0668 &  0.0809 &  0.0920 &  0.1035 &  0.1208 &  0.1456 &  0.1776\\
0098 &  0.0161 &  0.0244 &  0.0344 &  0.0481 &  0.0668 &  0.0896 &  0.1191 & &  0.0657 &  0.0795 &  0.0904 &  0.1016 &  0.1186 &  0.1431 &  0.1745\\
0099 &  0.0159 &  0.0241 &  0.0340 &  0.0476 &  0.0662 &  0.0887 &  0.1178 & &  0.0646 &  0.0782 &  0.0888 &  0.0998 &  0.1165 &  0.1406 &  0.1715\\
0100 &  0.0157 &  0.0238 &  0.0337 &  0.0472 &  0.0655 &  0.0878 &  0.1166 & &  0.0635 &  0.0768 &  0.0873 &  0.0980 &  0.1144 &  0.1381 &  0.1686\\
0101 &  0.0155 &  0.0236 &  0.0334 &  0.0467 &  0.0649 &  0.0869 &  0.1153 & &  0.0625 &  0.0755 &  0.0858 &  0.0962 &  0.1124 &  0.1357 &  0.1658\\
0102 &  0.0153 &  0.0233 &  0.0330 &  0.0462 &  0.0643 &  0.0860 &  0.1141 & &  0.0615 &  0.0742 &  0.0843 &  0.0945 &  0.1104 &  0.1334 &  0.1630\\
0103 &  0.0151 &  0.0230 &  0.0327 &  0.0458 &  0.0637 &  0.0852 &  0.1130 & &  0.0604 &  0.0730 &  0.0829 &  0.0928 &  0.1085 &  0.1311 &  0.1602\\
0104 &  0.0150 &  0.0228 &  0.0323 &  0.0453 &  0.0631 &  0.0844 &  0.1118 & &  0.0595 &  0.0718 &  0.0815 &  0.0912 &  0.1066 &  0.1289 &  0.1576\\
0105 &  0.0148 &  0.0225 &  0.0320 &  0.0448 &  0.0625 &  0.0837 &  0.1108 & &  0.0585 &  0.0706 &  0.0802 &  0.0896 &  0.1048 &  0.1268 &  0.1550\\
0106 &  0.0146 &  0.0222 &  0.0316 &  0.0444 &  0.0619 &  0.0830 &  0.1098 & &  0.0576 &  0.0694 &  0.0789 &  0.0881 &  0.1030 &  0.1247 &  0.1524\\
0107 &  0.0144 &  0.0219 &  0.0313 &  0.0439 &  0.0614 &  0.0823 &  0.1088 & &  0.0566 &  0.0683 &  0.0776 &  0.0866 &  0.1013 &  0.1226 &  0.1499\\
0108 &  0.0142 &  0.0216 &  0.0309 &  0.0435 &  0.0608 &  0.0816 &  0.1079 & &  0.0557 &  0.0672 &  0.0763 &  0.0852 &  0.0996 &  0.1206 &  0.1475\\
0109 &  0.0140 &  0.0213 &  0.0305 &  0.0430 &  0.0603 &  0.0809 &  0.1070 & &  0.0548 &  0.0661 &  0.0751 &  0.0838 &  0.0980 &  0.1187 &  0.1451\\
0110 &  0.0139 &  0.0210 &  0.0302 &  0.0426 &  0.0597 &  0.0802 &  0.1061 & &  0.0540 &  0.0650 &  0.0739 &  0.0824 &  0.0964 &  0.1168 &  0.1428\\
0111 &  0.0137 &  0.0207 &  0.0298 &  0.0422 &  0.0592 &  0.0796 &  0.1053 & &  0.0531 &  0.0640 &  0.0727 &  0.0811 &  0.0949 &  0.1150 &  0.1406\\
0112 &  0.0135 &  0.0204 &  0.0295 &  0.0417 &  0.0587 &  0.0789 &  0.1045 & &  0.0523 &  0.0630 &  0.0716 &  0.0798 &  0.0934 &  0.1132 &  0.1384\\
0113 &  0.0134 &  0.0202 &  0.0291 &  0.0413 &  0.0582 &  0.0783 &  0.1037 & &  0.0515 &  0.0620 &  0.0705 &  0.0786 &  0.0920 &  0.1115 &  0.1363\\
0114 &  0.0132 &  0.0199 &  0.0288 &  0.0409 &  0.0576 &  0.0777 &  0.1029 & &  0.0507 &  0.0610 &  0.0694 &  0.0773 &  0.0906 &  0.1098 &  0.1342\\
0115 &  0.0130 &  0.0197 &  0.0284 &  0.0405 &  0.0571 &  0.0771 &  0.1021 & &  0.0499 &  0.0600 &  0.0683 &  0.0762 &  0.0893 &  0.1082 &  0.1322\\
0116 &  0.0129 &  0.0194 &  0.0281 &  0.0401 &  0.0566 &  0.0764 &  0.1013 & &  0.0491 &  0.0591 &  0.0673 &  0.0750 &  0.0880 &  0.1067 &  0.1303\\
0117 &  0.0128 &  0.0192 &  0.0278 &  0.0397 &  0.0561 &  0.0758 &  0.1005 & &  0.0484 &  0.0582 &  0.0663 &  0.0739 &  0.0867 &  0.1052 &  0.1285\\
0118 &  0.0126 &  0.0190 &  0.0275 &  0.0393 &  0.0556 &  0.0752 &  0.0997 & &  0.0476 &  0.0573 &  0.0653 &  0.0728 &  0.0855 &  0.1037 &  0.1267\\
0119 &  0.0125 &  0.0188 &  0.0272 &  0.0389 &  0.0551 &  0.0746 &  0.0989 & &  0.0469 &  0.0564 &  0.0644 &  0.0718 &  0.0844 &  0.1023 &  0.1250\\
0120 &  0.0123 &  0.0186 &  0.0269 &  0.0386 &  0.0547 &  0.0739 &  0.0981 & &  0.0462 &  0.0556 &  0.0634 &  0.0708 &  0.0832 &  0.1010 &  0.1233\\
0121 &  0.0122 &  0.0184 &  0.0266 &  0.0382 &  0.0542 &  0.0733 &  0.0972 & &  0.0455 &  0.0547 &  0.0625 &  0.0698 &  0.0821 &  0.0997 &  0.1217\\
0122 &  0.0121 &  0.0182 &  0.0264 &  0.0379 &  0.0537 &  0.0727 &  0.0964 & &  0.0449 &  0.0539 &  0.0616 &  0.0688 &  0.0811 &  0.0984 &  0.1202\\
0123 &  0.0119 &  0.0181 &  0.0262 &  0.0376 &  0.0533 &  0.0721 &  0.0956 & &  0.0442 &  0.0531 &  0.0607 &  0.0679 &  0.0800 &  0.0972 &  0.1188\\
0124 &  0.0118 &  0.0179 &  0.0259 &  0.0373 &  0.0529 &  0.0715 &  0.0948 & &  0.0435 &  0.0523 &  0.0599 &  0.0670 &  0.0791 &  0.0961 &  0.1174\\
0125 &  0.0117 &  0.0178 &  0.0257 &  0.0370 &  0.0524 &  0.0709 &  0.0939 & &  0.0429 &  0.0515 &  0.0590 &  0.0661 &  0.0781 &  0.0950 &  0.1160\\
0126 &  0.0115 &  0.0176 &  0.0255 &  0.0367 &  0.0520 &  0.0703 &  0.0931 & &  0.0423 &  0.0508 &  0.0582 &  0.0652 &  0.0772 &  0.0939 &  0.1147\\
0127 &  0.0114 &  0.0175 &  0.0253 &  0.0364 &  0.0516 &  0.0697 &  0.0923 & &  0.0416 &  0.0500 &  0.0574 &  0.0644 &  0.0763 &  0.0929 &  0.1135\\
0128 &  0.0113 &  0.0173 &  0.0251 &  0.0362 &  0.0512 &  0.0691 &  0.0914 & &  0.0410 &  0.0493 &  0.0566 &  0.0636 &  0.0754 &  0.0919 &  0.1122\\
0129 &  0.0112 &  0.0172 &  0.0250 &  0.0359 &  0.0509 &  0.0686 &  0.0906 & &  0.0404 &  0.0486 &  0.0558 &  0.0628 &  0.0746 &  0.0909 &  0.1111\\
0130 &  0.0111 &  0.0170 &  0.0248 &  0.0356 &  0.0505 &  0.0680 &  0.0898 & &  0.0399 &  0.0479 &  0.0551 &  0.0620 &  0.0737 &  0.0900 &  0.1100\\
0131 &  0.0110 &  0.0169 &  0.0246 &  0.0354 &  0.0501 &  0.0675 &  0.0890 & &  0.0393 &  0.0472 &  0.0543 &  0.0612 &  0.0729 &  0.0891 &  0.1089\\
0132 &  0.0109 &  0.0167 &  0.0244 &  0.0351 &  0.0498 &  0.0670 &  0.0882 & &  0.0387 &  0.0465 &  0.0536 &  0.0605 &  0.0722 &  0.0882 &  0.1078\\
0133 &  0.0108 &  0.0165 &  0.0242 &  0.0348 &  0.0494 &  0.0664 &  0.0874 & &  0.0382 &  0.0458 &  0.0529 &  0.0597 &  0.0714 &  0.0874 &  0.1068\\
0134 &  0.0107 &  0.0163 &  0.0240 &  0.0346 &  0.0490 &  0.0659 &  0.0866 & &  0.0376 &  0.0452 &  0.0522 &  0.0590 &  0.0706 &  0.0866 &  0.1058\\
0135 &  0.0106 &  0.0162 &  0.0238 &  0.0343 &  0.0486 &  0.0653 &  0.0858 & &  0.0371 &  0.0445 &  0.0515 &  0.0583 &  0.0699 &  0.0858 &  0.1049\\
0136 &  0.0105 &  0.0160 &  0.0236 &  0.0340 &  0.0482 &  0.0648 &  0.0851 & &  0.0365 &  0.0439 &  0.0508 &  0.0576 &  0.0692 &  0.0850 &  0.1039\\
0137 &  0.0104 &  0.0158 &  0.0234 &  0.0337 &  0.0478 &  0.0642 &  0.0843 & &  0.0360 &  0.0433 &  0.0501 &  0.0569 &  0.0685 &  0.0842 &  0.1030\\
0138 &  0.0103 &  0.0156 &  0.0231 &  0.0334 &  0.0474 &  0.0637 &  0.0835 & &  0.0355 &  0.0427 &  0.0494 &  0.0562 &  0.0678 &  0.0834 &  0.1021\\
0139 &  0.0102 &  0.0154 &  0.0229 &  0.0331 &  0.0470 &  0.0631 &  0.0828 & &  0.0350 &  0.0421 &  0.0487 &  0.0555 &  0.0671 &  0.0827 &  0.1012\\
0140 &  0.0101 &  0.0152 &  0.0226 &  0.0327 &  0.0465 &  0.0625 &  0.0820 & &  0.0345 &  0.0415 &  0.0481 &  0.0549 &  0.0664 &  0.0819 &  0.1004\\
0141 &  0.0101 &  0.0150 &  0.0224 &  0.0324 &  0.0461 &  0.0619 &  0.0813 & &  0.0340 &  0.0409 &  0.0474 &  0.0542 &  0.0657 &  0.0812 &  0.0995\\
0142 &  0.0100 &  0.0148 &  0.0221 &  0.0320 &  0.0456 &  0.0614 &  0.0805 & &  0.0335 &  0.0403 &  0.0468 &  0.0535 &  0.0650 &  0.0805 &  0.0987\\
0143 &  0.0099 &  0.0147 &  0.0218 &  0.0317 &  0.0452 &  0.0608 &  0.0798 & &  0.0330 &  0.0397 &  0.0461 &  0.0529 &  0.0644 &  0.0797 &  0.0978\\
0144 &  0.0099 &  0.0145 &  0.0216 &  0.0313 &  0.0447 &  0.0602 &  0.0791 & &  0.0325 &  0.0392 &  0.0455 &  0.0522 &  0.0637 &  0.0790 &  0.0970\\
0145 &  0.0098 &  0.0144 &  0.0213 &  0.0310 &  0.0442 &  0.0596 &  0.0783 & &  0.0321 &  0.0386 &  0.0449 &  0.0516 &  0.0630 &  0.0783 &  0.0962\\
0146 &  0.0097 &  0.0142 &  0.0210 &  0.0306 &  0.0438 &  0.0590 &  0.0776 & &  0.0316 &  0.0380 &  0.0442 &  0.0509 &  0.0624 &  0.0776 &  0.0954\\
0147 &  0.0096 &  0.0141 &  0.0208 &  0.0303 &  0.0433 &  0.0584 &  0.0769 & &  0.0311 &  0.0375 &  0.0436 &  0.0503 &  0.0617 &  0.0768 &  0.0946\\
0148 &  0.0096 &  0.0140 &  0.0206 &  0.0300 &  0.0429 &  0.0579 &  0.0762 & &  0.0307 &  0.0370 &  0.0430 &  0.0497 &  0.0610 &  0.0761 &  0.0938\\
0149 &  0.0095 &  0.0139 &  0.0203 &  0.0297 &  0.0425 &  0.0573 &  0.0756 & &  0.0302 &  0.0364 &  0.0424 &  0.0490 &  0.0604 &  0.0754 &  0.0930\\
0150 &  0.0094 &  0.0138 &  0.0201 &  0.0294 &  0.0421 &  0.0568 &  0.0749 & &  0.0298 &  0.0359 &  0.0418 &  0.0484 &  0.0597 &  0.0747 &  0.0923\\
0151 &  0.0094 &  0.0137 &  0.0200 &  0.0291 &  0.0417 &  0.0563 &  0.0742 & &  0.0294 &  0.0354 &  0.0412 &  0.0478 &  0.0591 &  0.0740 &  0.0915\\
0152 &  0.0093 &  0.0137 &  0.0198 &  0.0288 &  0.0414 &  0.0557 &  0.0735 & &  0.0289 &  0.0348 &  0.0406 &  0.0471 &  0.0584 &  0.0733 &  0.0907\\
0153 &  0.0093 &  0.0136 &  0.0197 &  0.0286 &  0.0410 &  0.0553 &  0.0729 & &  0.0285 &  0.0343 &  0.0400 &  0.0465 &  0.0577 &  0.0726 &  0.0900\\
0154 &  0.0092 &  0.0135 &  0.0195 &  0.0284 &  0.0407 &  0.0548 &  0.0723 & &  0.0281 &  0.0338 &  0.0394 &  0.0459 &  0.0571 &  0.0719 &  0.0892\\
0155 &  0.0091 &  0.0135 &  0.0194 &  0.0282 &  0.0404 &  0.0543 &  0.0716 & &  0.0276 &  0.0333 &  0.0388 &  0.0453 &  0.0564 &  0.0712 &  0.0885\\
0156 &  0.0091 &  0.0134 &  0.0193 &  0.0280 &  0.0401 &  0.0539 &  0.0710 & &  0.0272 &  0.0328 &  0.0383 &  0.0447 &  0.0558 &  0.0705 &  0.0878\\
0157 &  0.0090 &  0.0133 &  0.0192 &  0.0278 &  0.0398 &  0.0535 &  0.0705 & &  0.0268 &  0.0323 &  0.0377 &  0.0441 &  0.0551 &  0.0698 &  0.0870\\
0158 &  0.0090 &  0.0132 &  0.0192 &  0.0277 &  0.0395 &  0.0530 &  0.0699 & &  0.0264 &  0.0318 &  0.0372 &  0.0435 &  0.0545 &  0.0692 &  0.0863\\
0159 &  0.0089 &  0.0132 &  0.0191 &  0.0275 &  0.0393 &  0.0527 &  0.0693 & &  0.0260 &  0.0314 &  0.0366 &  0.0429 &  0.0538 &  0.0685 &  0.0856\\
0160 &  0.0089 &  0.0131 &  0.0190 &  0.0274 &  0.0390 &  0.0523 &  0.0688 & &  0.0256 &  0.0309 &  0.0361 &  0.0423 &  0.0532 &  0.0678 &  0.0850\\
0161 &  0.0088 &  0.0130 &  0.0189 &  0.0272 &  0.0388 &  0.0519 &  0.0683 & &  0.0252 &  0.0304 &  0.0356 &  0.0418 &  0.0526 &  0.0672 &  0.0843\\
0162 &  0.0088 &  0.0129 &  0.0188 &  0.0271 &  0.0386 &  0.0516 &  0.0678 & &  0.0249 &  0.0300 &  0.0351 &  0.0412 &  0.0520 &  0.0666 &  0.0836\\
0163 &  0.0087 &  0.0129 &  0.0187 &  0.0270 &  0.0384 &  0.0513 &  0.0674 & &  0.0245 &  0.0295 &  0.0346 &  0.0407 &  0.0514 &  0.0659 &  0.0830\\
0164 &  0.0086 &  0.0128 &  0.0186 &  0.0268 &  0.0381 &  0.0510 &  0.0669 & &  0.0241 &  0.0291 &  0.0341 &  0.0401 &  0.0508 &  0.0653 &  0.0824\\
0165 &  0.0086 &  0.0127 &  0.0185 &  0.0267 &  0.0379 &  0.0507 &  0.0665 & &  0.0238 &  0.0287 &  0.0336 &  0.0396 &  0.0502 &  0.0647 &  0.0817\\
0166 &  0.0085 &  0.0126 &  0.0184 &  0.0266 &  0.0377 &  0.0504 &  0.0661 & &  0.0234 &  0.0282 &  0.0331 &  0.0391 &  0.0496 &  0.0641 &  0.0811\\
0167 &  0.0085 &  0.0125 &  0.0183 &  0.0264 &  0.0375 &  0.0501 &  0.0657 & &  0.0231 &  0.0278 &  0.0327 &  0.0386 &  0.0491 &  0.0635 &  0.0805\\
0168 &  0.0084 &  0.0124 &  0.0182 &  0.0263 &  0.0373 &  0.0498 &  0.0654 & &  0.0227 &  0.0274 &  0.0322 &  0.0381 &  0.0485 &  0.0630 &  0.0799\\
0169 &  0.0083 &  0.0123 &  0.0181 &  0.0262 &  0.0372 &  0.0496 &  0.0650 & &  0.0224 &  0.0270 &  0.0318 &  0.0376 &  0.0480 &  0.0624 &  0.0793\\
0170 &  0.0083 &  0.0123 &  0.0180 &  0.0261 &  0.0370 &  0.0493 &  0.0647 & &  0.0221 &  0.0267 &  0.0313 &  0.0372 &  0.0474 &  0.0618 &  0.0787\\
0171 &  0.0082 &  0.0122 &  0.0180 &  0.0259 &  0.0368 &  0.0491 &  0.0643 & &  0.0218 &  0.0263 &  0.0309 &  0.0367 &  0.0469 &  0.0613 &  0.0782\\
0172 &  0.0082 &  0.0121 &  0.0179 &  0.0258 &  0.0367 &  0.0489 &  0.0640 & &  0.0215 &  0.0259 &  0.0305 &  0.0363 &  0.0464 &  0.0607 &  0.0776\\
0173 &  0.0081 &  0.0120 &  0.0178 &  0.0257 &  0.0365 &  0.0487 &  0.0638 & &  0.0211 &  0.0255 &  0.0301 &  0.0359 &  0.0459 &  0.0602 &  0.0770\\
0174 &  0.0081 &  0.0120 &  0.0177 &  0.0256 &  0.0364 &  0.0486 &  0.0635 & &  0.0208 &  0.0252 &  0.0297 &  0.0355 &  0.0454 &  0.0596 &  0.0765\\
0175 &  0.0080 &  0.0119 &  0.0177 &  0.0255 &  0.0363 &  0.0484 &  0.0632 & &  0.0206 &  0.0249 &  0.0293 &  0.0351 &  0.0449 &  0.0591 &  0.0759\\
0176 &  0.0080 &  0.0118 &  0.0176 &  0.0255 &  0.0361 &  0.0483 &  0.0630 & &  0.0203 &  0.0245 &  0.0290 &  0.0347 &  0.0445 &  0.0586 &  0.0753\\
0177 &  0.0079 &  0.0118 &  0.0175 &  0.0254 &  0.0360 &  0.0481 &  0.0628 & &  0.0200 &  0.0242 &  0.0286 &  0.0343 &  0.0440 &  0.0580 &  0.0748\\
0178 &  0.0079 &  0.0117 &  0.0174 &  0.0253 &  0.0359 &  0.0480 &  0.0625 & &  0.0197 &  0.0239 &  0.0282 &  0.0340 &  0.0436 &  0.0575 &  0.0742\\
0179 &  0.0078 &  0.0116 &  0.0173 &  0.0252 &  0.0358 &  0.0478 &  0.0623 & &  0.0194 &  0.0236 &  0.0279 &  0.0336 &  0.0432 &  0.0570 &  0.0736\\
0180 &  0.0078 &  0.0116 &  0.0172 &  0.0251 &  0.0356 &  0.0477 &  0.0621 & &  0.0192 &  0.0232 &  0.0276 &  0.0333 &  0.0427 &  0.0565 &  0.0731\\
0181 &  0.0077 &  0.0115 &  0.0171 &  0.0249 &  0.0355 &  0.0475 &  0.0619 & &  0.0189 &  0.0229 &  0.0272 &  0.0329 &  0.0423 &  0.0560 &  0.0725\\
0182 &  0.0077 &  0.0114 &  0.0170 &  0.0248 &  0.0353 &  0.0473 &  0.0617 & &  0.0187 &  0.0227 &  0.0269 &  0.0326 &  0.0420 &  0.0555 &  0.0720\\
0183 &  0.0076 &  0.0114 &  0.0169 &  0.0246 &  0.0351 &  0.0471 &  0.0614 & &  0.0184 &  0.0224 &  0.0266 &  0.0323 &  0.0416 &  0.0551 &  0.0715\\
0184 &  0.0076 &  0.0113 &  0.0168 &  0.0244 &  0.0349 &  0.0469 &  0.0612 & &  0.0182 &  0.0221 &  0.0263 &  0.0320 &  0.0412 &  0.0546 &  0.0709\\
0185 &  0.0075 &  0.0112 &  0.0166 &  0.0242 &  0.0347 &  0.0466 &  0.0610 & &  0.0180 &  0.0218 &  0.0260 &  0.0317 &  0.0409 &  0.0542 &  0.0704\\
0186 &  0.0075 &  0.0111 &  0.0165 &  0.0240 &  0.0344 &  0.0464 &  0.0607 & &  0.0177 &  0.0215 &  0.0257 &  0.0315 &  0.0405 &  0.0537 &  0.0699\\
0187 &  0.0074 &  0.0110 &  0.0163 &  0.0238 &  0.0341 &  0.0461 &  0.0605 & &  0.0175 &  0.0213 &  0.0254 &  0.0312 &  0.0402 &  0.0533 &  0.0694\\
0188 &  0.0074 &  0.0109 &  0.0162 &  0.0235 &  0.0339 &  0.0458 &  0.0602 & &  0.0173 &  0.0210 &  0.0252 &  0.0309 &  0.0399 &  0.0529 &  0.0689\\
0189 &  0.0073 &  0.0109 &  0.0160 &  0.0233 &  0.0336 &  0.0455 &  0.0599 & &  0.0171 &  0.0208 &  0.0249 &  0.0307 &  0.0396 &  0.0525 &  0.0684\\
0190 &  0.0073 &  0.0108 &  0.0159 &  0.0230 &  0.0333 &  0.0452 &  0.0596 & &  0.0169 &  0.0205 &  0.0246 &  0.0304 &  0.0393 &  0.0521 &  0.0679\\
0191 &  0.0073 &  0.0107 &  0.0157 &  0.0228 &  0.0330 &  0.0449 &  0.0593 & &  0.0167 &  0.0203 &  0.0244 &  0.0302 &  0.0390 &  0.0517 &  0.0675\\
0192 &  0.0072 &  0.0106 &  0.0156 &  0.0226 &  0.0327 &  0.0445 &  0.0590 & &  0.0165 &  0.0201 &  0.0241 &  0.0299 &  0.0387 &  0.0513 &  0.0670\\
0193 &  0.0072 &  0.0105 &  0.0155 &  0.0224 &  0.0324 &  0.0442 &  0.0587 & &  0.0163 &  0.0198 &  0.0239 &  0.0297 &  0.0384 &  0.0510 &  0.0666\\
0194 &  0.0071 &  0.0105 &  0.0153 &  0.0222 &  0.0321 &  0.0439 &  0.0584 & &  0.0161 &  0.0196 &  0.0237 &  0.0295 &  0.0382 &  0.0506 &  0.0662\\
0195 &  0.0071 &  0.0104 &  0.0152 &  0.0220 &  0.0319 &  0.0436 &  0.0580 & &  0.0159 &  0.0194 &  0.0234 &  0.0293 &  0.0379 &  0.0503 &  0.0658\\
0196 &  0.0071 &  0.0104 &  0.0152 &  0.0219 &  0.0316 &  0.0433 &  0.0577 & &  0.0157 &  0.0192 &  0.0232 &  0.0291 &  0.0377 &  0.0500 &  0.0654\\
0197 &  0.0071 &  0.0103 &  0.0151 &  0.0218 &  0.0314 &  0.0430 &  0.0573 & &  0.0155 &  0.0190 &  0.0230 &  0.0289 &  0.0375 &  0.0497 &  0.0650\\
0198 &  0.0071 &  0.0103 &  0.0150 &  0.0217 &  0.0312 &  0.0427 &  0.0570 & &  0.0153 &  0.0188 &  0.0228 &  0.0287 &  0.0373 &  0.0494 &  0.0647\\
0199 &  0.0071 &  0.0102 &  0.0150 &  0.0216 &  0.0310 &  0.0425 &  0.0566 & &  0.0152 &  0.0186 &  0.0226 &  0.0285 &  0.0371 &  0.0492 &  0.0644\\
0200 &  0.0071 &  0.0102 &  0.0149 &  0.0215 &  0.0308 &  0.0422 &  0.0563 & &  0.0150 &  0.0184 &  0.0224 &  0.0283 &  0.0369 &  0.0489 &  0.0640\\
0201 &  0.0071 &  0.0102 &  0.0149 &  0.0214 &  0.0306 &  0.0419 &  0.0558 & &  0.0148 &  0.0182 &  0.0222 &  0.0281 &  0.0367 &  0.0487 &  0.0635\\
0202 &  0.0071 &  0.0102 &  0.0148 &  0.0213 &  0.0304 &  0.0416 &  0.0554 & &  0.0147 &  0.0180 &  0.0220 &  0.0279 &  0.0365 &  0.0485 &  0.0629\\
0203 &  0.0071 &  0.0102 &  0.0148 &  0.0213 &  0.0302 &  0.0413 &  0.0552 & &  0.0145 &  0.0178 &  0.0218 &  0.0277 &  0.0363 &  0.0483 &  0.0624\\
0204 &  0.0071 &  0.0101 &  0.0147 &  0.0212 &  0.0301 &  0.0410 &  0.0547 & &  0.0143 &  0.0176 &  0.0216 &  0.0276 &  0.0362 &  0.0481 &  0.0619\\
0205 &  0.0071 &  0.0101 &  0.0147 &  0.0211 &  0.0299 &  0.0408 &  0.0544 & &  0.0142 &  0.0174 &  0.0214 &  0.0274 &  0.0360 &  0.0477 &  0.0613\\
0206 &  0.0071 &  0.0101 &  0.0147 &  0.0210 &  0.0297 &  0.0405 &  0.0542 & &  0.0140 &  0.0172 &  0.0212 &  0.0272 &  0.0359 &  0.0473 &  0.0608\\
0207 &  0.0071 &  0.0101 &  0.0146 &  0.0210 &  0.0295 &  0.0403 &  0.0537 & &  0.0138 &  0.0171 &  0.0211 &  0.0271 &  0.0357 &  0.0469 &  0.0603\\
0208 &  0.0071 &  0.0101 &  0.0146 &  0.0209 &  0.0293 &  0.0400 &  0.0533 & &  0.0137 &  0.0169 &  0.0209 &  0.0269 &  0.0356 &  0.0465 &  0.0598\\
0209 &  0.0071 &  0.0101 &  0.0145 &  0.0208 &  0.0292 &  0.0397 &  0.0532 & &  0.0135 &  0.0167 &  0.0207 &  0.0267 &  0.0355 &  0.0461 &  0.0593\\
0210 &  0.0071 &  0.0101 &  0.0145 &  0.0207 &  0.0290 &  0.0395 &  0.0527 & &  0.0133 &  0.0165 &  0.0205 &  0.0266 &  0.0352 &  0.0458 &  0.0588\\
0211 &  0.0071 &  0.0101 &  0.0144 &  0.0206 &  0.0288 &  0.0393 &  0.0524 & &  0.0132 &  0.0163 &  0.0204 &  0.0264 &  0.0349 &  0.0454 &  0.0583\\
0212 &  0.0070 &  0.0100 &  0.0144 &  0.0205 &  0.0287 &  0.0390 &  0.0522 & &  0.0130 &  0.0162 &  0.0202 &  0.0262 &  0.0346 &  0.0450 &  0.0578\\
0213 &  0.0070 &  0.0100 &  0.0143 &  0.0205 &  0.0285 &  0.0388 &  0.0518 & &  0.0129 &  0.0160 &  0.0200 &  0.0261 &  0.0343 &  0.0446 &  0.0573\\
0214 &  0.0070 &  0.0100 &  0.0143 &  0.0204 &  0.0283 &  0.0386 &  0.0515 & &  0.0127 &  0.0158 &  0.0198 &  0.0259 &  0.0340 &  0.0442 &  0.0569\\
0215 &  0.0070 &  0.0100 &  0.0143 &  0.0203 &  0.0282 &  0.0383 &  0.0513 & &  0.0125 &  0.0156 &  0.0196 &  0.0257 &  0.0337 &  0.0439 &  0.0564\\
0216 &  0.0069 &  0.0100 &  0.0142 &  0.0202 &  0.0280 &  0.0381 &  0.0509 & &  0.0124 &  0.0154 &  0.0195 &  0.0255 &  0.0334 &  0.0435 &  0.0559\\
0217 &  0.0069 &  0.0099 &  0.0142 &  0.0201 &  0.0278 &  0.0378 &  0.0505 & &  0.0122 &  0.0152 &  0.0193 &  0.0252 &  0.0331 &  0.0431 &  0.0554\\
0218 &  0.0069 &  0.0099 &  0.0142 &  0.0200 &  0.0276 &  0.0376 &  0.0504 & &  0.0120 &  0.0150 &  0.0191 &  0.0250 &  0.0328 &  0.0428 &  0.0550\\
0219 &  0.0069 &  0.0099 &  0.0142 &  0.0198 &  0.0275 &  0.0374 &  0.0500 & &  0.0119 &  0.0149 &  0.0189 &  0.0248 &  0.0326 &  0.0424 &  0.0545\\
0220 &  0.0069 &  0.0099 &  0.0141 &  0.0197 &  0.0272 &  0.0372 &  0.0496 & &  0.0117 &  0.0147 &  0.0187 &  0.0246 &  0.0323 &  0.0421 &  0.0540\\
0221 &  0.0069 &  0.0099 &  0.0140 &  0.0196 &  0.0271 &  0.0369 &  0.0495 & &  0.0116 &  0.0145 &  0.0186 &  0.0244 &  0.0320 &  0.0417 &  0.0536\\
0222 &  0.0069 &  0.0099 &  0.0140 &  0.0195 &  0.0269 &  0.0367 &  0.0491 & &  0.0114 &  0.0143 &  0.0184 &  0.0242 &  0.0317 &  0.0414 &  0.0531\\
0223 &  0.0069 &  0.0099 &  0.0139 &  0.0194 &  0.0267 &  0.0365 &  0.0487 & &  0.0112 &  0.0141 &  0.0182 &  0.0240 &  0.0315 &  0.0410 &  0.0527\\
0224 &  0.0069 &  0.0098 &  0.0138 &  0.0193 &  0.0266 &  0.0362 &  0.0486 & &  0.0111 &  0.0139 &  0.0181 &  0.0238 &  0.0312 &  0.0407 &  0.0522\\
0225 &  0.0068 &  0.0098 &  0.0137 &  0.0191 &  0.0264 &  0.0360 &  0.0482 & &  0.0109 &  0.0137 &  0.0179 &  0.0236 &  0.0310 &  0.0403 &  0.0518\\
0226 &  0.0069 &  0.0098 &  0.0136 &  0.0190 &  0.0262 &  0.0358 &  0.0478 & &  0.0108 &  0.0136 &  0.0178 &  0.0233 &  0.0307 &  0.0400 &  0.0513\\
0227 &  0.0069 &  0.0097 &  0.0136 &  0.0189 &  0.0261 &  0.0356 &  0.0477 & &  0.0106 &  0.0135 &  0.0176 &  0.0231 &  0.0304 &  0.0397 &  0.0509\\
0228 &  0.0069 &  0.0097 &  0.0135 &  0.0187 &  0.0259 &  0.0354 &  0.0473 & &  0.0105 &  0.0134 &  0.0174 &  0.0230 &  0.0302 &  0.0393 &  0.0504\\
0229 &  0.0069 &  0.0096 &  0.0134 &  0.0186 &  0.0257 &  0.0351 &  0.0469 & &  0.0103 &  0.0132 &  0.0173 &  0.0228 &  0.0299 &  0.0390 &  0.0500\\
0230 &  0.0069 &  0.0096 &  0.0133 &  0.0185 &  0.0256 &  0.0349 &  0.0468 & &  0.0102 &  0.0131 &  0.0171 &  0.0226 &  0.0297 &  0.0387 &  0.0496\\
0231 &  0.0069 &  0.0095 &  0.0132 &  0.0184 &  0.0255 &  0.0347 &  0.0464 & &  0.0100 &  0.0130 &  0.0170 &  0.0224 &  0.0294 &  0.0383 &  0.0491\\
0232 &  0.0068 &  0.0095 &  0.0131 &  0.0183 &  0.0253 &  0.0345 &  0.0460 & &  0.0099 &  0.0129 &  0.0168 &  0.0222 &  0.0292 &  0.0380 &  0.0487\\
0233 &  0.0068 &  0.0094 &  0.0131 &  0.0182 &  0.0251 &  0.0343 &  0.0459 & &  0.0098 &  0.0128 &  0.0167 &  0.0220 &  0.0289 &  0.0377 &  0.0483\\
0234 &  0.0068 &  0.0094 &  0.0130 &  0.0180 &  0.0250 &  0.0341 &  0.0455 & &  0.0098 &  0.0127 &  0.0165 &  0.0218 &  0.0287 &  0.0374 &  0.0478\\
0235 &  0.0067 &  0.0093 &  0.0129 &  0.0179 &  0.0248 &  0.0338 &  0.0452 & &  0.0097 &  0.0125 &  0.0164 &  0.0216 &  0.0285 &  0.0370 &  0.0474\\
0236 &  0.0067 &  0.0093 &  0.0128 &  0.0178 &  0.0247 &  0.0336 &  0.0450 & &  0.0096 &  0.0124 &  0.0162 &  0.0214 &  0.0282 &  0.0367 &  0.0470\\
0237 &  0.0067 &  0.0092 &  0.0127 &  0.0177 &  0.0245 &  0.0334 &  0.0447 & &  0.0095 &  0.0123 &  0.0161 &  0.0212 &  0.0280 &  0.0364 &  0.0466\\
0238 &  0.0066 &  0.0091 &  0.0126 &  0.0176 &  0.0243 &  0.0332 &  0.0443 & &  0.0094 &  0.0122 &  0.0160 &  0.0211 &  0.0277 &  0.0361 &  0.0462\\
0239 &  0.0066 &  0.0091 &  0.0125 &  0.0175 &  0.0242 &  0.0330 &  0.0442 & &  0.0093 &  0.0121 &  0.0158 &  0.0209 &  0.0275 &  0.0358 &  0.0458\\
0240 &  0.0065 &  0.0090 &  0.0124 &  0.0173 &  0.0241 &  0.0328 &  0.0439 & &  0.0092 &  0.0120 &  0.0157 &  0.0207 &  0.0273 &  0.0355 &  0.0453\\
0241 &  0.0065 &  0.0089 &  0.0124 &  0.0172 &  0.0239 &  0.0326 &  0.0435 & &  0.0091 &  0.0119 &  0.0155 &  0.0205 &  0.0270 &  0.0352 &  0.0449\\
0242 &  0.0065 &  0.0089 &  0.0123 &  0.0171 &  0.0237 &  0.0324 &  0.0434 & &  0.0091 &  0.0118 &  0.0154 &  0.0204 &  0.0268 &  0.0348 &  0.0445\\
0243 &  0.0064 &  0.0088 &  0.0122 &  0.0170 &  0.0236 &  0.0322 &  0.0431 & &  0.0090 &  0.0117 &  0.0153 &  0.0202 &  0.0266 &  0.0345 &  0.0441\\
0244 &  0.0064 &  0.0088 &  0.0121 &  0.0169 &  0.0234 &  0.0320 &  0.0428 & &  0.0089 &  0.0116 &  0.0151 &  0.0200 &  0.0263 &  0.0342 &  0.0438\\
0245 &  0.0064 &  0.0087 &  0.0120 &  0.0168 &  0.0233 &  0.0318 &  0.0426 & &  0.0088 &  0.0114 &  0.0150 &  0.0198 &  0.0261 &  0.0339 &  0.0434\\
0246 &  0.0063 &  0.0086 &  0.0120 &  0.0167 &  0.0232 &  0.0316 &  0.0423 & &  0.0087 &  0.0113 &  0.0149 &  0.0197 &  0.0259 &  0.0336 &  0.0430\\
0247 &  0.0063 &  0.0086 &  0.0119 &  0.0166 &  0.0230 &  0.0314 &  0.0420 & &  0.0086 &  0.0112 &  0.0147 &  0.0195 &  0.0257 &  0.0333 &  0.0426\\
0248 &  0.0062 &  0.0085 &  0.0118 &  0.0165 &  0.0229 &  0.0313 &  0.0419 & &  0.0086 &  0.0111 &  0.0146 &  0.0193 &  0.0254 &  0.0330 &  0.0422\\
0249 &  0.0062 &  0.0085 &  0.0117 &  0.0164 &  0.0227 &  0.0311 &  0.0416 & &  0.0085 &  0.0110 &  0.0145 &  0.0192 &  0.0252 &  0.0327 &  0.0419\\
0250 &  0.0061 &  0.0084 &  0.0117 &  0.0163 &  0.0226 &  0.0309 &  0.0413 & &  0.0084 &  0.0109 &  0.0144 &  0.0190 &  0.0250 &  0.0324 &  0.0415\\
0251 &  0.0061 &  0.0084 &  0.0116 &  0.0162 &  0.0225 &  0.0307 &  0.0412 & &  0.0083 &  0.0108 &  0.0142 &  0.0188 &  0.0247 &  0.0321 &  0.0411\\
0252 &  0.0061 &  0.0083 &  0.0115 &  0.0161 &  0.0223 &  0.0306 &  0.0410 & &  0.0082 &  0.0107 &  0.0141 &  0.0187 &  0.0245 &  0.0318 &  0.0408\\
0253 &  0.0060 &  0.0082 &  0.0114 &  0.0160 &  0.0222 &  0.0304 &  0.0407 & &  0.0081 &  0.0106 &  0.0140 &  0.0185 &  0.0243 &  0.0316 &  0.0404\\
0254 &  0.0060 &  0.0082 &  0.0114 &  0.0159 &  0.0221 &  0.0303 &  0.0406 & &  0.0081 &  0.0105 &  0.0139 &  0.0183 &  0.0241 &  0.0313 &  0.0401\\
0255 &  0.0059 &  0.0081 &  0.0113 &  0.0158 &  0.0220 &  0.0301 &  0.0404 & &  0.0080 &  0.0104 &  0.0137 &  0.0182 &  0.0239 &  0.0310 &  0.0397\\
0256 &  0.0059 &  0.0081 &  0.0112 &  0.0157 &  0.0218 &  0.0299 &  0.0401 & &  0.0079 &  0.0103 &  0.0136 &  0.0180 &  0.0236 &  0.0307 &  0.0394\\
0257 &  0.0058 &  0.0080 &  0.0112 &  0.0156 &  0.0218 &  0.0298 &  0.0400 & &  0.0078 &  0.0102 &  0.0135 &  0.0178 &  0.0234 &  0.0304 &  0.0390\\
0258 &  0.0058 &  0.0080 &  0.0111 &  0.0156 &  0.0216 &  0.0296 &  0.0398 & &  0.0078 &  0.0102 &  0.0134 &  0.0177 &  0.0232 &  0.0302 &  0.0387\\
0259 &  0.0058 &  0.0079 &  0.0110 &  0.0155 &  0.0215 &  0.0295 &  0.0395 & &  0.0077 &  0.0101 &  0.0132 &  0.0175 &  0.0230 &  0.0299 &  0.0384\\
0260 &  0.0057 &  0.0079 &  0.0110 &  0.0154 &  0.0214 &  0.0294 &  0.0394 & &  0.0076 &  0.0100 &  0.0131 &  0.0173 &  0.0228 &  0.0296 &  0.0380\\
0261 &  0.0057 &  0.0079 &  0.0109 &  0.0153 &  0.0213 &  0.0292 &  0.0392 & &  0.0075 &  0.0099 &  0.0130 &  0.0172 &  0.0226 &  0.0293 &  0.0377\\
0262 &  0.0057 &  0.0078 &  0.0108 &  0.0152 &  0.0212 &  0.0290 &  0.0390 & &  0.0075 &  0.0098 &  0.0129 &  0.0170 &  0.0223 &  0.0291 &  0.0374\\
0263 &  0.0056 &  0.0078 &  0.0108 &  0.0151 &  0.0211 &  0.0289 &  0.0388 & &  0.0074 &  0.0097 &  0.0127 &  0.0168 &  0.0221 &  0.0288 &  0.0371\\
0264 &  0.0056 &  0.0077 &  0.0107 &  0.0151 &  0.0210 &  0.0288 &  0.0387 & &  0.0073 &  0.0096 &  0.0126 &  0.0167 &  0.0219 &  0.0286 &  0.0368\\
0265 &  0.0056 &  0.0077 &  0.0107 &  0.0150 &  0.0209 &  0.0286 &  0.0384 & &  0.0073 &  0.0095 &  0.0125 &  0.0165 &  0.0217 &  0.0283 &  0.0364\\
0266 &  0.0055 &  0.0076 &  0.0106 &  0.0149 &  0.0208 &  0.0285 &  0.0382 & &  0.0072 &  0.0094 &  0.0124 &  0.0163 &  0.0215 &  0.0280 &  0.0361\\
0267 &  0.0055 &  0.0076 &  0.0105 &  0.0148 &  0.0207 &  0.0284 &  0.0381 & &  0.0071 &  0.0093 &  0.0123 &  0.0162 &  0.0213 &  0.0278 &  0.0358\\
0268 &  0.0055 &  0.0075 &  0.0105 &  0.0147 &  0.0206 &  0.0282 &  0.0377 & &  0.0070 &  0.0092 &  0.0121 &  0.0160 &  0.0211 &  0.0275 &  0.0355\\
0269 &  0.0054 &  0.0075 &  0.0104 &  0.0147 &  0.0205 &  0.0281 &  0.0376 & &  0.0070 &  0.0091 &  0.0120 &  0.0159 &  0.0209 &  0.0273 &  0.0352\\
0270 &  0.0054 &  0.0074 &  0.0104 &  0.0146 &  0.0204 &  0.0279 &  0.0374 & &  0.0069 &  0.0090 &  0.0119 &  0.0157 &  0.0207 &  0.0270 &  0.0349\\
0271 &  0.0054 &  0.0074 &  0.0103 &  0.0145 &  0.0203 &  0.0278 &  0.0371 & &  0.0068 &  0.0090 &  0.0118 &  0.0155 &  0.0205 &  0.0268 &  0.0346\\
0272 &  0.0053 &  0.0073 &  0.0103 &  0.0144 &  0.0202 &  0.0276 &  0.0370 & &  0.0068 &  0.0089 &  0.0116 &  0.0154 &  0.0203 &  0.0265 &  0.0343\\
0273 &  0.0053 &  0.0073 &  0.0102 &  0.0144 &  0.0201 &  0.0275 &  0.0368 & &  0.0067 &  0.0088 &  0.0115 &  0.0152 &  0.0201 &  0.0263 &  0.0340\\
0274 &  0.0053 &  0.0072 &  0.0102 &  0.0143 &  0.0200 &  0.0273 &  0.0365 & &  0.0066 &  0.0087 &  0.0114 &  0.0151 &  0.0199 &  0.0260 &  0.0337\\
0275 &  0.0052 &  0.0072 &  0.0101 &  0.0142 &  0.0199 &  0.0272 &  0.0363 & &  0.0066 &  0.0086 &  0.0113 &  0.0149 &  0.0197 &  0.0258 &  0.0334\\
0276 &  0.0052 &  0.0072 &  0.0101 &  0.0142 &  0.0198 &  0.0270 &  0.0362 & &  0.0065 &  0.0085 &  0.0112 &  0.0148 &  0.0195 &  0.0256 &  0.0331\\
0277 &  0.0052 &  0.0071 &  0.0100 &  0.0141 &  0.0196 &  0.0268 &  0.0359 & &  0.0064 &  0.0084 &  0.0110 &  0.0146 &  0.0193 &  0.0253 &  0.0328\\
0278 &  0.0051 &  0.0071 &  0.0099 &  0.0140 &  0.0196 &  0.0267 &  0.0357 & &  0.0064 &  0.0083 &  0.0109 &  0.0144 &  0.0191 &  0.0251 &  0.0325\\
0279 &  0.0051 &  0.0071 &  0.0099 &  0.0140 &  0.0195 &  0.0266 &  0.0356 & &  0.0063 &  0.0082 &  0.0108 &  0.0143 &  0.0189 &  0.0249 &  0.0322\\
0280 &  0.0051 &  0.0070 &  0.0099 &  0.0139 &  0.0193 &  0.0264 &  0.0352 & &  0.0062 &  0.0081 &  0.0107 &  0.0141 &  0.0187 &  0.0246 &  0.0319\\
0281 &  0.0050 &  0.0070 &  0.0098 &  0.0138 &  0.0192 &  0.0262 &  0.0351 & &  0.0062 &  0.0080 &  0.0106 &  0.0140 &  0.0185 &  0.0244 &  0.0316\\
0282 &  0.0050 &  0.0070 &  0.0097 &  0.0138 &  0.0191 &  0.0261 &  0.0350 & &  0.0061 &  0.0079 &  0.0104 &  0.0138 &  0.0184 &  0.0242 &  0.0313\\
0283 &  0.0050 &  0.0069 &  0.0097 &  0.0137 &  0.0190 &  0.0259 &  0.0346 & &  0.0060 &  0.0079 &  0.0103 &  0.0137 &  0.0182 &  0.0240 &  0.0311\\
0284 &  0.0049 &  0.0069 &  0.0096 &  0.0136 &  0.0189 &  0.0258 &  0.0344 & &  0.0059 &  0.0078 &  0.0102 &  0.0136 &  0.0180 &  0.0237 &  0.0308\\
0285 &  0.0049 &  0.0068 &  0.0096 &  0.0135 &  0.0188 &  0.0256 &  0.0344 & &  0.0059 &  0.0077 &  0.0101 &  0.0134 &  0.0178 &  0.0235 &  0.0305\\
0286 &  0.0049 &  0.0068 &  0.0095 &  0.0135 &  0.0186 &  0.0255 &  0.0340 & &  0.0058 &  0.0076 &  0.0100 &  0.0133 &  0.0177 &  0.0233 &  0.0302\\
0287 &  0.0048 &  0.0067 &  0.0095 &  0.0134 &  0.0186 &  0.0253 &  0.0338 & &  0.0057 &  0.0075 &  0.0099 &  0.0131 &  0.0175 &  0.0231 &  0.0299\\
0288 &  0.0048 &  0.0067 &  0.0094 &  0.0133 &  0.0185 &  0.0252 &  0.0337 & &  0.0057 &  0.0074 &  0.0097 &  0.0130 &  0.0173 &  0.0229 &  0.0297\\
0289 &  0.0048 &  0.0067 &  0.0094 &  0.0132 &  0.0183 &  0.0251 &  0.0334 & &  0.0056 &  0.0073 &  0.0096 &  0.0128 &  0.0171 &  0.0227 &  0.0294\\
0290 &  0.0048 &  0.0066 &  0.0093 &  0.0131 &  0.0183 &  0.0249 &  0.0332 & &  0.0055 &  0.0072 &  0.0095 &  0.0127 &  0.0170 &  0.0225 &  0.0291\\
0291 &  0.0047 &  0.0066 &  0.0093 &  0.0131 &  0.0181 &  0.0248 &  0.0332 & &  0.0055 &  0.0071 &  0.0094 &  0.0126 &  0.0168 &  0.0222 &  0.0288\\
0292 &  0.0047 &  0.0065 &  0.0093 &  0.0130 &  0.0180 &  0.0247 &  0.0328 & &  0.0054 &  0.0071 &  0.0093 &  0.0124 &  0.0167 &  0.0220 &  0.0286\\
0293 &  0.0047 &  0.0065 &  0.0092 &  0.0129 &  0.0179 &  0.0245 &  0.0326 & &  0.0053 &  0.0070 &  0.0092 &  0.0123 &  0.0165 &  0.0218 &  0.0283\\
0294 &  0.0046 &  0.0065 &  0.0091 &  0.0129 &  0.0178 &  0.0244 &  0.0326 & &  0.0053 &  0.0069 &  0.0091 &  0.0122 &  0.0163 &  0.0216 &  0.0280\\
0295 &  0.0046 &  0.0064 &  0.0091 &  0.0128 &  0.0177 &  0.0243 &  0.0322 & &  0.0052 &  0.0068 &  0.0090 &  0.0121 &  0.0162 &  0.0215 &  0.0278\\
0296 &  0.0046 &  0.0064 &  0.0091 &  0.0127 &  0.0177 &  0.0241 &  0.0321 & &  0.0051 &  0.0067 &  0.0089 &  0.0119 &  0.0160 &  0.0213 &  0.0275\\
0297 &  0.0045 &  0.0064 &  0.0090 &  0.0126 &  0.0176 &  0.0240 &  0.0320 & &  0.0051 &  0.0066 &  0.0088 &  0.0118 &  0.0159 &  0.0211 &  0.0273\\
0298 &  0.0045 &  0.0063 &  0.0090 &  0.0126 &  0.0174 &  0.0239 &  0.0317 & &  0.0050 &  0.0066 &  0.0087 &  0.0117 &  0.0157 &  0.0209 &  0.0270\\
0299 &  0.0045 &  0.0063 &  0.0089 &  0.0125 &  0.0174 &  0.0237 &  0.0315 & &  0.0049 &  0.0065 &  0.0086 &  0.0116 &  0.0156 &  0.0207 &  0.0268\\
0300 &  0.0045 &  0.0063 &  0.0089 &  0.0124 &  0.0173 &  0.0236 &  0.0315 & &  0.0049 &  0.0064 &  0.0085 &  0.0115 &  0.0154 &  0.0205 &  0.0266\\
0301 &  0.0045 &  0.0063 &  0.0088 &  0.0124 &  0.0172 &  0.0235 &  0.0312 & &  0.0048 &  0.0063 &  0.0084 &  0.0113 &  0.0153 &  0.0203 &  0.0263\\
0302 &  0.0044 &  0.0062 &  0.0088 &  0.0123 &  0.0171 &  0.0234 &  0.0310 & &  0.0048 &  0.0062 &  0.0083 &  0.0112 &  0.0152 &  0.0202 &  0.0261\\
0303 &  0.0044 &  0.0062 &  0.0087 &  0.0122 &  0.0170 &  0.0232 &  0.0310 & &  0.0047 &  0.0062 &  0.0082 &  0.0111 &  0.0150 &  0.0200 &  0.0259\\
0304 &  0.0044 &  0.0062 &  0.0087 &  0.0122 &  0.0169 &  0.0232 &  0.0306 & &  0.0046 &  0.0061 &  0.0081 &  0.0110 &  0.0149 &  0.0198 &  0.0256\\
0305 &  0.0044 &  0.0062 &  0.0086 &  0.0120 &  0.0168 &  0.0230 &  0.0305 & &  0.0046 &  0.0060 &  0.0080 &  0.0109 &  0.0148 &  0.0197 &  0.0254\\
0306 &  0.0043 &  0.0062 &  0.0086 &  0.0120 &  0.0168 &  0.0229 &  0.0305 & &  0.0045 &  0.0059 &  0.0080 &  0.0108 &  0.0146 &  0.0195 &  0.0252\\
0307 &  0.0043 &  0.0061 &  0.0085 &  0.0120 &  0.0166 &  0.0228 &  0.0302 & &  0.0045 &  0.0059 &  0.0079 &  0.0107 &  0.0145 &  0.0193 &  0.0250\\
0308 &  0.0043 &  0.0061 &  0.0085 &  0.0119 &  0.0166 &  0.0227 &  0.0300 & &  0.0044 &  0.0058 &  0.0078 &  0.0106 &  0.0144 &  0.0192 &  0.0248\\
0309 &  0.0043 &  0.0061 &  0.0084 &  0.0118 &  0.0165 &  0.0225 &  0.0300 & &  0.0044 &  0.0057 &  0.0077 &  0.0105 &  0.0143 &  0.0190 &  0.0246\\
0310 &  0.0043 &  0.0060 &  0.0084 &  0.0118 &  0.0164 &  0.0225 &  0.0297 & &  0.0043 &  0.0057 &  0.0076 &  0.0104 &  0.0141 &  0.0188 &  0.0243\\
0311 &  0.0043 &  0.0060 &  0.0083 &  0.0117 &  0.0163 &  0.0223 &  0.0295 & &  0.0042 &  0.0056 &  0.0075 &  0.0103 &  0.0140 &  0.0187 &  0.0241\\
0312 &  0.0043 &  0.0060 &  0.0083 &  0.0116 &  0.0163 &  0.0222 &  0.0295 & &  0.0042 &  0.0055 &  0.0075 &  0.0102 &  0.0139 &  0.0185 &  0.0239\\
0313 &  0.0043 &  0.0059 &  0.0082 &  0.0116 &  0.0161 &  0.0221 &  0.0292 & &  0.0041 &  0.0055 &  0.0074 &  0.0101 &  0.0138 &  0.0184 &  0.0237\\
0314 &  0.0042 &  0.0059 &  0.0082 &  0.0115 &  0.0161 &  0.0219 &  0.0290 & &  0.0041 &  0.0054 &  0.0073 &  0.0100 &  0.0137 &  0.0182 &  0.0235\\
0315 &  0.0042 &  0.0059 &  0.0081 &  0.0114 &  0.0160 &  0.0218 &  0.0290 & &  0.0040 &  0.0054 &  0.0072 &  0.0099 &  0.0136 &  0.0181 &  0.0233\\
0316 &  0.0042 &  0.0058 &  0.0081 &  0.0114 &  0.0159 &  0.0217 &  0.0288 & &  0.0040 &  0.0053 &  0.0072 &  0.0098 &  0.0134 &  0.0179 &  0.0231\\
0317 &  0.0042 &  0.0058 &  0.0080 &  0.0113 &  0.0159 &  0.0216 &  0.0286 & &  0.0039 &  0.0052 &  0.0071 &  0.0097 &  0.0133 &  0.0178 &  0.0229\\
0318 &  0.0042 &  0.0058 &  0.0080 &  0.0113 &  0.0158 &  0.0214 &  0.0286 & &  0.0039 &  0.0052 &  0.0070 &  0.0097 &  0.0132 &  0.0176 &  0.0227\\
0319 &  0.0042 &  0.0057 &  0.0079 &  0.0112 &  0.0157 &  0.0214 &  0.0283 & &  0.0039 &  0.0051 &  0.0069 &  0.0096 &  0.0131 &  0.0174 &  0.0225\\
0320 &  0.0041 &  0.0057 &  0.0079 &  0.0111 &  0.0156 &  0.0212 &  0.0282 & &  0.0038 &  0.0051 &  0.0069 &  0.0095 &  0.0130 &  0.0173 &  0.0223\\
0321 &  0.0041 &  0.0056 &  0.0078 &  0.0111 &  0.0155 &  0.0211 &  0.0282 & &  0.0038 &  0.0050 &  0.0068 &  0.0094 &  0.0129 &  0.0171 &  0.0221\\
0322 &  0.0041 &  0.0056 &  0.0078 &  0.0110 &  0.0154 &  0.0210 &  0.0279 & &  0.0037 &  0.0049 &  0.0067 &  0.0093 &  0.0128 &  0.0170 &  0.0219\\
0323 &  0.0041 &  0.0055 &  0.0077 &  0.0110 &  0.0154 &  0.0209 &  0.0278 & &  0.0037 &  0.0049 &  0.0066 &  0.0092 &  0.0126 &  0.0168 &  0.0217\\
0324 &  0.0040 &  0.0055 &  0.0077 &  0.0109 &  0.0153 &  0.0207 &  0.0278 & &  0.0036 &  0.0048 &  0.0066 &  0.0091 &  0.0125 &  0.0167 &  0.0216\\
0325 &  0.0040 &  0.0054 &  0.0076 &  0.0109 &  0.0152 &  0.0206 &  0.0276 & &  0.0036 &  0.0048 &  0.0065 &  0.0090 &  0.0124 &  0.0165 &  0.0214\\
0326 &  0.0040 &  0.0054 &  0.0076 &  0.0108 &  0.0151 &  0.0205 &  0.0274 & &  0.0035 &  0.0047 &  0.0064 &  0.0090 &  0.0123 &  0.0164 &  0.0212\\
0327 &  0.0039 &  0.0054 &  0.0075 &  0.0107 &  0.0150 &  0.0203 &  0.0274 & &  0.0035 &  0.0047 &  0.0064 &  0.0089 &  0.0122 &  0.0162 &  0.0210\\
0328 &  0.0039 &  0.0053 &  0.0075 &  0.0107 &  0.0149 &  0.0203 &  0.0272 & &  0.0035 &  0.0046 &  0.0063 &  0.0088 &  0.0121 &  0.0161 &  0.0208\\
0329 &  0.0039 &  0.0053 &  0.0074 &  0.0106 &  0.0148 &  0.0202 &  0.0271 & &  0.0034 &  0.0045 &  0.0062 &  0.0087 &  0.0120 &  0.0159 &  0.0206\\
0330 &  0.0038 &  0.0052 &  0.0074 &  0.0106 &  0.0148 &  0.0200 &  0.0271 & &  0.0034 &  0.0045 &  0.0062 &  0.0086 &  0.0118 &  0.0158 &  0.0204\\
0331 &  0.0038 &  0.0052 &  0.0073 &  0.0105 &  0.0146 &  0.0199 &  0.0269 & &  0.0033 &  0.0044 &  0.0061 &  0.0085 &  0.0117 &  0.0156 &  0.0203\\
0332 &  0.0038 &  0.0051 &  0.0073 &  0.0104 &  0.0146 &  0.0198 &  0.0268 & &  0.0033 &  0.0044 &  0.0060 &  0.0084 &  0.0116 &  0.0155 &  0.0201\\
0333 &  0.0037 &  0.0051 &  0.0072 &  0.0104 &  0.0145 &  0.0197 &  0.0268 & &  0.0032 &  0.0043 &  0.0059 &  0.0084 &  0.0115 &  0.0153 &  0.0199\\
0334 &  0.0037 &  0.0050 &  0.0072 &  0.0104 &  0.0144 &  0.0196 &  0.0266 & &  0.0032 &  0.0042 &  0.0059 &  0.0083 &  0.0114 &  0.0152 &  0.0197\\
0335 &  0.0037 &  0.0050 &  0.0072 &  0.0103 &  0.0143 &  0.0195 &  0.0265 & &  0.0031 &  0.0042 &  0.0058 &  0.0082 &  0.0113 &  0.0150 &  0.0196\\
0336 &  0.0036 &  0.0050 &  0.0071 &  0.0102 &  0.0142 &  0.0194 &  0.0265 & &  0.0031 &  0.0041 &  0.0057 &  0.0081 &  0.0112 &  0.0149 &  0.0194\\
0337 &  0.0036 &  0.0049 &  0.0071 &  0.0102 &  0.0141 &  0.0193 &  0.0263 & &  0.0030 &  0.0041 &  0.0057 &  0.0080 &  0.0110 &  0.0147 &  0.0192\\
0338 &  0.0035 &  0.0049 &  0.0070 &  0.0101 &  0.0141 &  0.0193 &  0.0262 & &  0.0030 &  0.0040 &  0.0056 &  0.0079 &  0.0109 &  0.0146 &  0.0190\\
0339 &  0.0035 &  0.0048 &  0.0070 &  0.0101 &  0.0140 &  0.0192 &  0.0261 & &  0.0030 &  0.0040 &  0.0055 &  0.0078 &  0.0108 &  0.0145 &  0.0189\\
0340 &  0.0035 &  0.0048 &  0.0070 &  0.0100 &  0.0139 &  0.0191 &  0.0260 & &  0.0029 &  0.0039 &  0.0055 &  0.0078 &  0.0107 &  0.0143 &  0.0187\\
0341 &  0.0034 &  0.0048 &  0.0069 &  0.0100 &  0.0138 &  0.0190 &  0.0258 & &  0.0029 &  0.0038 &  0.0054 &  0.0077 &  0.0106 &  0.0142 &  0.0185\\
0342 &  0.0034 &  0.0047 &  0.0069 &  0.0099 &  0.0137 &  0.0189 &  0.0258 & &  0.0028 &  0.0038 &  0.0053 &  0.0076 &  0.0105 &  0.0140 &  0.0184\\
0343 &  0.0034 &  0.0047 &  0.0069 &  0.0099 &  0.0137 &  0.0188 &  0.0257 & &  0.0028 &  0.0037 &  0.0053 &  0.0075 &  0.0104 &  0.0139 &  0.0182\\
0344 &  0.0033 &  0.0047 &  0.0069 &  0.0098 &  0.0136 &  0.0188 &  0.0255 & &  0.0027 &  0.0037 &  0.0052 &  0.0074 &  0.0102 &  0.0138 &  0.0181\\
0345 &  0.0033 &  0.0047 &  0.0068 &  0.0097 &  0.0135 &  0.0187 &  0.0255 & &  0.0027 &  0.0036 &  0.0051 &  0.0073 &  0.0101 &  0.0137 &  0.0179\\
0346 &  0.0033 &  0.0046 &  0.0068 &  0.0097 &  0.0134 &  0.0186 &  0.0253 & &  0.0026 &  0.0036 &  0.0051 &  0.0072 &  0.0100 &  0.0135 &  0.0178\\
0347 &  0.0032 &  0.0046 &  0.0068 &  0.0096 &  0.0134 &  0.0185 &  0.0251 & &  0.0026 &  0.0035 &  0.0050 &  0.0071 &  0.0099 &  0.0134 &  0.0176\\
0348 &  0.0032 &  0.0046 &  0.0068 &  0.0096 &  0.0133 &  0.0185 &  0.0251 & &  0.0025 &  0.0034 &  0.0049 &  0.0071 &  0.0098 &  0.0133 &  0.0175\\
0349 &  0.0032 &  0.0046 &  0.0067 &  0.0095 &  0.0132 &  0.0184 &  0.0250 & &  0.0025 &  0.0034 &  0.0049 &  0.0070 &  0.0097 &  0.0132 &  0.0173\\
0350 &  0.0031 &  0.0046 &  0.0067 &  0.0095 &  0.0132 &  0.0183 &  0.0248 & &  0.0024 &  0.0033 &  0.0048 &  0.0069 &  0.0096 &  0.0130 &  0.0172\\
0351 &  0.0031 &  0.0046 &  0.0067 &  0.0094 &  0.0131 &  0.0182 &  0.0247 & &  0.0024 &  0.0033 &  0.0047 &  0.0068 &  0.0095 &  0.0129 &  0.0170\\
0352 &  0.0031 &  0.0046 &  0.0067 &  0.0094 &  0.0130 &  0.0181 &  0.0246 & &  0.0024 &  0.0032 &  0.0047 &  0.0067 &  0.0094 &  0.0128 &  0.0169\\
0353 &  0.0031 &  0.0045 &  0.0066 &  0.0093 &  0.0130 &  0.0180 &  0.0244 & &  0.0023 &  0.0032 &  0.0046 &  0.0066 &  0.0093 &  0.0127 &  0.0168\\
0354 &  0.0031 &  0.0045 &  0.0066 &  0.0093 &  0.0129 &  0.0180 &  0.0243 & &  0.0023 &  0.0031 &  0.0046 &  0.0066 &  0.0092 &  0.0126 &  0.0166\\
0355 &  0.0031 &  0.0045 &  0.0066 &  0.0092 &  0.0129 &  0.0179 &  0.0242 & &  0.0022 &  0.0031 &  0.0045 &  0.0065 &  0.0091 &  0.0125 &  0.0165\\
0356 &  0.0030 &  0.0045 &  0.0066 &  0.0092 &  0.0128 &  0.0178 &  0.0240 & &  0.0022 &  0.0030 &  0.0044 &  0.0064 &  0.0090 &  0.0124 &  0.0164\\
0357 &  0.0030 &  0.0045 &  0.0065 &  0.0091 &  0.0128 &  0.0178 &  0.0240 & &  0.0021 &  0.0030 &  0.0044 &  0.0063 &  0.0089 &  0.0123 &  0.0163\\
0358 &  0.0030 &  0.0045 &  0.0065 &  0.0091 &  0.0127 &  0.0176 &  0.0238 & &  0.0021 &  0.0029 &  0.0043 &  0.0063 &  0.0088 &  0.0121 &  0.0161\\
0359 &  0.0030 &  0.0045 &  0.0065 &  0.0090 &  0.0127 &  0.0175 &  0.0236 & &  0.0021 &  0.0029 &  0.0043 &  0.0062 &  0.0088 &  0.0120 &  0.0160\\
0360 &  0.0030 &  0.0045 &  0.0065 &  0.0090 &  0.0126 &  0.0175 &  0.0236 & &  0.0020 &  0.0029 &  0.0042 &  0.0061 &  0.0087 &  0.0119 &  0.0159\\
0361 &  0.0030 &  0.0045 &  0.0064 &  0.0089 &  0.0125 &  0.0174 &  0.0235 & &  0.0020 &  0.0028 &  0.0041 &  0.0060 &  0.0086 &  0.0118 &  0.0158\\
0362 &  0.0030 &  0.0045 &  0.0064 &  0.0089 &  0.0125 &  0.0173 &  0.0232 & &  0.0019 &  0.0028 &  0.0041 &  0.0060 &  0.0085 &  0.0118 &  0.0157\\
0363 &  0.0030 &  0.0045 &  0.0064 &  0.0088 &  0.0124 &  0.0172 &  0.0232 & &  0.0019 &  0.0027 &  0.0040 &  0.0059 &  0.0084 &  0.0117 &  0.0156\\
0364 &  0.0030 &  0.0045 &  0.0063 &  0.0088 &  0.0124 &  0.0171 &  0.0231 & &  0.0019 &  0.0027 &  0.0040 &  0.0058 &  0.0084 &  0.0116 &  0.0155\\
0365 &  0.0031 &  0.0045 &  0.0063 &  0.0088 &  0.0123 &  0.0170 &  0.0229 & &  0.0018 &  0.0026 &  0.0039 &  0.0058 &  0.0083 &  0.0115 &  0.0154\\
0366 &  0.0031 &  0.0045 &  0.0063 &  0.0087 &  0.0123 &  0.0170 &  0.0228 & &  0.0018 &  0.0026 &  0.0039 &  0.0057 &  0.0082 &  0.0114 &  0.0153\\
0367 &  0.0031 &  0.0045 &  0.0062 &  0.0087 &  0.0122 &  0.0169 &  0.0227 & &  0.0018 &  0.0026 &  0.0038 &  0.0056 &  0.0081 &  0.0113 &  0.0152\\
0368 &  0.0031 &  0.0045 &  0.0062 &  0.0086 &  0.0122 &  0.0168 &  0.0225 & &  0.0017 &  0.0025 &  0.0038 &  0.0056 &  0.0081 &  0.0112 &  0.0151\\
0369 &  0.0031 &  0.0045 &  0.0061 &  0.0086 &  0.0121 &  0.0167 &  0.0224 & &  0.0017 &  0.0025 &  0.0037 &  0.0055 &  0.0080 &  0.0111 &  0.0150\\
0370 &  0.0031 &  0.0045 &  0.0061 &  0.0085 &  0.0120 &  0.0166 &  0.0224 & &  0.0017 &  0.0024 &  0.0036 &  0.0055 &  0.0079 &  0.0110 &  0.0149\\
0371 &  0.0031 &  0.0044 &  0.0061 &  0.0085 &  0.0120 &  0.0166 &  0.0221 & &  0.0017 &  0.0024 &  0.0036 &  0.0054 &  0.0079 &  0.0109 &  0.0149\\
0372 &  0.0031 &  0.0044 &  0.0060 &  0.0085 &  0.0119 &  0.0165 &  0.0221 & &  0.0016 &  0.0024 &  0.0036 &  0.0053 &  0.0078 &  0.0109 &  0.0148\\
0373 &  0.0031 &  0.0044 &  0.0060 &  0.0084 &  0.0119 &  0.0164 &  0.0220 & &  0.0016 &  0.0023 &  0.0035 &  0.0053 &  0.0077 &  0.0108 &  0.0147\\
0374 &  0.0031 &  0.0044 &  0.0060 &  0.0084 &  0.0118 &  0.0163 &  0.0218 & &  0.0016 &  0.0023 &  0.0035 &  0.0052 &  0.0077 &  0.0107 &  0.0146\\
0375 &  0.0031 &  0.0044 &  0.0059 &  0.0084 &  0.0118 &  0.0163 &  0.0217 & &  0.0015 &  0.0022 &  0.0034 &  0.0052 &  0.0076 &  0.0106 &  0.0145\\
0376 &  0.0031 &  0.0044 &  0.0059 &  0.0083 &  0.0117 &  0.0161 &  0.0217 & &  0.0015 &  0.0022 &  0.0034 &  0.0051 &  0.0075 &  0.0105 &  0.0145\\
0377 &  0.0031 &  0.0043 &  0.0059 &  0.0083 &  0.0117 &  0.0161 &  0.0215 & &  0.0015 &  0.0022 &  0.0033 &  0.0051 &  0.0075 &  0.0104 &  0.0144\\
0378 &  0.0031 &  0.0043 &  0.0058 &  0.0082 &  0.0116 &  0.0160 &  0.0214 & &  0.0015 &  0.0021 &  0.0033 &  0.0050 &  0.0074 &  0.0104 &  0.0143\\
0379 &  0.0031 &  0.0043 &  0.0058 &  0.0082 &  0.0116 &  0.0159 &  0.0214 & &  0.0014 &  0.0021 &  0.0032 &  0.0050 &  0.0073 &  0.0103 &  0.0143\\
0380 &  0.0031 &  0.0042 &  0.0058 &  0.0082 &  0.0115 &  0.0158 &  0.0212 & &  0.0014 &  0.0021 &  0.0032 &  0.0049 &  0.0073 &  0.0102 &  0.0142\\
0381 &  0.0031 &  0.0042 &  0.0057 &  0.0081 &  0.0115 &  0.0158 &  0.0211 & &  0.0014 &  0.0020 &  0.0032 &  0.0049 &  0.0072 &  0.0101 &  0.0141\\
0382 &  0.0031 &  0.0042 &  0.0057 &  0.0081 &  0.0114 &  0.0157 &  0.0212 & &  0.0014 &  0.0020 &  0.0031 &  0.0049 &  0.0071 &  0.0101 &  0.0141\\
0383 &  0.0031 &  0.0041 &  0.0057 &  0.0081 &  0.0114 &  0.0156 &  0.0209 & &  0.0013 &  0.0020 &  0.0031 &  0.0048 &  0.0071 &  0.0100 &  0.0140\\
0384 &  0.0031 &  0.0041 &  0.0057 &  0.0080 &  0.0114 &  0.0156 &  0.0209 & &  0.0013 &  0.0019 &  0.0031 &  0.0048 &  0.0070 &  0.0099 &  0.0139\\
0385 &  0.0031 &  0.0041 &  0.0056 &  0.0080 &  0.0113 &  0.0155 &  0.0209 & &  0.0013 &  0.0019 &  0.0030 &  0.0047 &  0.0070 &  0.0099 &  0.0139\\
0386 &  0.0031 &  0.0040 &  0.0056 &  0.0080 &  0.0113 &  0.0154 &  0.0207 & &  0.0013 &  0.0019 &  0.0030 &  0.0047 &  0.0069 &  0.0098 &  0.0138\\
0387 &  0.0030 &  0.0040 &  0.0056 &  0.0080 &  0.0112 &  0.0154 &  0.0206 & &  0.0012 &  0.0018 &  0.0030 &  0.0046 &  0.0068 &  0.0097 &  0.0138\\
0388 &  0.0030 &  0.0040 &  0.0056 &  0.0079 &  0.0111 &  0.0153 &  0.0207 & &  0.0012 &  0.0018 &  0.0029 &  0.0046 &  0.0068 &  0.0096 &  0.0137\\
0389 &  0.0030 &  0.0040 &  0.0056 &  0.0079 &  0.0111 &  0.0153 &  0.0205 & &  0.0012 &  0.0018 &  0.0029 &  0.0046 &  0.0067 &  0.0096 &  0.0136\\
0390 &  0.0030 &  0.0039 &  0.0055 &  0.0079 &  0.0111 &  0.0152 &  0.0204 & &  0.0012 &  0.0018 &  0.0029 &  0.0045 &  0.0067 &  0.0095 &  0.0136\\
0391 &  0.0030 &  0.0039 &  0.0055 &  0.0078 &  0.0110 &  0.0152 &  0.0205 & &  0.0012 &  0.0017 &  0.0028 &  0.0045 &  0.0066 &  0.0094 &  0.0135\\
0392 &  0.0029 &  0.0039 &  0.0055 &  0.0078 &  0.0110 &  0.0151 &  0.0203 & &  0.0011 &  0.0017 &  0.0028 &  0.0044 &  0.0065 &  0.0094 &  0.0135\\
0393 &  0.0029 &  0.0039 &  0.0055 &  0.0078 &  0.0109 &  0.0150 &  0.0202 & &  0.0011 &  0.0017 &  0.0028 &  0.0044 &  0.0065 &  0.0093 &  0.0134\\
0394 &  0.0029 &  0.0039 &  0.0054 &  0.0077 &  0.0108 &  0.0150 &  0.0203 & &  0.0011 &  0.0017 &  0.0028 &  0.0044 &  0.0064 &  0.0092 &  0.0133\\
0395 &  0.0029 &  0.0038 &  0.0054 &  0.0078 &  0.0109 &  0.0150 &  0.0201 & &  0.0011 &  0.0016 &  0.0027 &  0.0043 &  0.0064 &  0.0092 &  0.0133\\
0396 &  0.0028 &  0.0038 &  0.0054 &  0.0077 &  0.0108 &  0.0149 &  0.0201 & &  0.0010 &  0.0016 &  0.0027 &  0.0043 &  0.0063 &  0.0091 &  0.0132\\
0397 &  0.0028 &  0.0038 &  0.0054 &  0.0077 &  0.0107 &  0.0149 &  0.0202 & &  0.0010 &  0.0016 &  0.0027 &  0.0042 &  0.0062 &  0.0091 &  0.0132\\
0398 &  0.0028 &  0.0038 &  0.0054 &  0.0077 &  0.0107 &  0.0148 &  0.0200 & &  0.0010 &  0.0016 &  0.0027 &  0.0042 &  0.0062 &  0.0090 &  0.0131\\
0399 &  0.0028 &  0.0038 &  0.0054 &  0.0076 &  0.0107 &  0.0147 &  0.0199 & &  9.9E-4 &  0.0015 &  0.0026 &  0.0042 &  0.0061 &  0.0089 &  0.0130\\
0400 &  0.0028 &  0.0038 &  0.0054 &  0.0076 &  0.0106 &  0.0148 &  0.0200 & &  9.7E-4 &  0.0015 &  0.0026 &  0.0041 &  0.0061 &  0.0089 &  0.0130\\
0401 &  0.0027 &  0.0038 &  0.0053 &  0.0076 &  0.0106 &  0.0147 &  0.0198 & &  9.5E-4 &  0.0015 &  0.0026 &  0.0041 &  0.0060 &  0.0088 &  0.0129\\
0402 &  0.0027 &  0.0038 &  0.0053 &  0.0075 &  0.0106 &  0.0146 &  0.0198 & &  9.4E-4 &  0.0015 &  0.0026 &  0.0040 &  0.0060 &  0.0088 &  0.0128\\
0403 &  0.0027 &  0.0038 &  0.0053 &  0.0075 &  0.0105 &  0.0146 &  0.0199 & &  9.2E-4 &  0.0015 &  0.0025 &  0.0040 &  0.0059 &  0.0087 &  0.0128\\
0404 &  0.0027 &  0.0037 &  0.0053 &  0.0075 &  0.0105 &  0.0146 &  0.0197 & &  9.0E-4 &  0.0015 &  0.0025 &  0.0040 &  0.0059 &  0.0087 &  0.0127\\
0405 &  0.0027 &  0.0037 &  0.0053 &  0.0075 &  0.0105 &  0.0145 &  0.0196 & &  8.9E-4 &  0.0015 &  0.0025 &  0.0039 &  0.0058 &  0.0086 &  0.0126\\
0406 &  0.0027 &  0.0037 &  0.0053 &  0.0074 &  0.0105 &  0.0145 &  0.0197 & &  8.7E-4 &  0.0014 &  0.0025 &  0.0039 &  0.0058 &  0.0086 &  0.0126\\
0407 &  0.0027 &  0.0037 &  0.0052 &  0.0074 &  0.0105 &  0.0145 &  0.0195 & &  8.6E-4 &  0.0014 &  0.0025 &  0.0038 &  0.0057 &  0.0085 &  0.0125\\
0408 &  0.0027 &  0.0037 &  0.0052 &  0.0074 &  0.0104 &  0.0144 &  0.0195 & &  8.4E-4 &  0.0014 &  0.0024 &  0.0038 &  0.0057 &  0.0085 &  0.0124\\
0409 &  0.0026 &  0.0037 &  0.0052 &  0.0073 &  0.0104 &  0.0144 &  0.0196 & &  8.3E-4 &  0.0014 &  0.0024 &  0.0038 &  0.0056 &  0.0084 &  0.0123\\
0410 &  0.0026 &  0.0037 &  0.0052 &  0.0073 &  0.0104 &  0.0144 &  0.0194 & &  8.2E-4 &  0.0014 &  0.0024 &  0.0037 &  0.0056 &  0.0084 &  0.0123\\
0411 &  0.0026 &  0.0037 &  0.0052 &  0.0073 &  0.0103 &  0.0143 &  0.0193 & &  8.1E-4 &  0.0014 &  0.0024 &  0.0037 &  0.0055 &  0.0083 &  0.0122\\
0412 &  0.0026 &  0.0037 &  0.0051 &  0.0073 &  0.0103 &  0.0143 &  0.0194 & &  8.0E-4 &  0.0014 &  0.0024 &  0.0037 &  0.0055 &  0.0083 &  0.0121\\
0413 &  0.0026 &  0.0037 &  0.0051 &  0.0073 &  0.0103 &  0.0143 &  0.0192 & &  7.9E-4 &  0.0014 &  0.0023 &  0.0036 &  0.0055 &  0.0082 &  0.0120\\
0414 &  0.0026 &  0.0036 &  0.0051 &  0.0072 &  0.0103 &  0.0142 &  0.0192 & &  7.8E-4 &  0.0014 &  0.0023 &  0.0036 &  0.0054 &  0.0082 &  0.0119\\
0415 &  0.0026 &  0.0036 &  0.0051 &  0.0072 &  0.0102 &  0.0142 &  0.0192 & &  7.7E-4 &  0.0014 &  0.0023 &  0.0036 &  0.0054 &  0.0081 &  0.0118\\
0416 &  0.0026 &  0.0036 &  0.0050 &  0.0072 &  0.0102 &  0.0141 &  0.0191 & &  7.7E-4 &  0.0014 &  0.0023 &  0.0035 &  0.0054 &  0.0081 &  0.0118\\
0417 &  0.0026 &  0.0036 &  0.0050 &  0.0072 &  0.0102 &  0.0140 &  0.0190 & &  7.6E-4 &  0.0014 &  0.0023 &  0.0035 &  0.0053 &  0.0080 &  0.0117\\
0418 &  0.0026 &  0.0036 &  0.0050 &  0.0072 &  0.0101 &  0.0140 &  0.0191 & &  7.5E-4 &  0.0013 &  0.0023 &  0.0035 &  0.0053 &  0.0079 &  0.0116\\
0419 &  0.0026 &  0.0036 &  0.0050 &  0.0071 &  0.0101 &  0.0140 &  0.0189 & &  7.5E-4 &  0.0013 &  0.0022 &  0.0034 &  0.0052 &  0.0079 &  0.0115\\
0420 &  0.0026 &  0.0036 &  0.0049 &  0.0071 &  0.0101 &  0.0139 &  0.0188 & &  7.5E-4 &  0.0013 &  0.0022 &  0.0034 &  0.0052 &  0.0078 &  0.0114\\
0421 &  0.0025 &  0.0035 &  0.0049 &  0.0071 &  0.0100 &  0.0139 &  0.0188 & &  7.4E-4 &  0.0013 &  0.0022 &  0.0034 &  0.0052 &  0.0078 &  0.0113\\
0422 &  0.0026 &  0.0035 &  0.0049 &  0.0071 &  0.0100 &  0.0138 &  0.0187 & &  7.4E-4 &  0.0013 &  0.0022 &  0.0034 &  0.0051 &  0.0077 &  0.0112\\
0423 &  0.0025 &  0.0035 &  0.0049 &  0.0071 &  0.0100 &  0.0137 &  0.0186 & &  7.4E-4 &  0.0013 &  0.0022 &  0.0033 &  0.0051 &  0.0077 &  0.0111\\
0424 &  0.0025 &  0.0035 &  0.0049 &  0.0071 &  0.0099 &  0.0137 &  0.0186 & &  7.4E-4 &  0.0013 &  0.0022 &  0.0033 &  0.0051 &  0.0076 &  0.0110\\
0425 &  0.0025 &  0.0034 &  0.0049 &  0.0070 &  0.0099 &  0.0136 &  0.0184 & &  7.4E-4 &  0.0013 &  0.0022 &  0.0033 &  0.0050 &  0.0075 &  0.0109\\
0426 &  0.0025 &  0.0034 &  0.0049 &  0.0070 &  0.0099 &  0.0135 &  0.0183 & &  7.4E-4 &  0.0013 &  0.0021 &  0.0033 &  0.0050 &  0.0075 &  0.0108\\
0427 &  0.0025 &  0.0034 &  0.0049 &  0.0070 &  0.0098 &  0.0135 &  0.0183 & &  7.5E-4 &  0.0013 &  0.0021 &  0.0032 &  0.0049 &  0.0074 &  0.0107\\
0428 &  0.0025 &  0.0034 &  0.0049 &  0.0069 &  0.0098 &  0.0134 &  0.0182 & &  7.5E-4 &  0.0013 &  0.0021 &  0.0032 &  0.0049 &  0.0074 &  0.0106\\
0429 &  0.0025 &  0.0034 &  0.0048 &  0.0069 &  0.0097 &  0.0133 &  0.0180 & &  7.5E-4 &  0.0013 &  0.0021 &  0.0032 &  0.0049 &  0.0073 &  0.0105\\
0430 &  0.0025 &  0.0034 &  0.0048 &  0.0069 &  0.0097 &  0.0132 &  0.0180 & &  7.6E-4 &  0.0013 &  0.0021 &  0.0032 &  0.0048 &  0.0072 &  0.0104\\
0431 &  0.0025 &  0.0033 &  0.0048 &  0.0069 &  0.0097 &  0.0132 &  0.0179 & &  7.6E-4 &  0.0013 &  0.0021 &  0.0031 &  0.0048 &  0.0072 &  0.0103\\
0432 &  0.0024 &  0.0033 &  0.0048 &  0.0069 &  0.0096 &  0.0131 &  0.0177 & &  7.7E-4 &  0.0013 &  0.0021 &  0.0031 &  0.0047 &  0.0071 &  0.0101\\
0433 &  0.0024 &  0.0033 &  0.0048 &  0.0068 &  0.0095 &  0.0130 &  0.0177 & &  7.7E-4 &  0.0013 &  0.0020 &  0.0031 &  0.0047 &  0.0070 &  0.0100\\
0434 &  0.0024 &  0.0033 &  0.0048 &  0.0068 &  0.0095 &  0.0129 &  0.0176 & &  7.8E-4 &  0.0013 &  0.0020 &  0.0031 &  0.0047 &  0.0070 &  0.0099\\
0435 &  0.0024 &  0.0033 &  0.0047 &  0.0068 &  0.0094 &  0.0128 &  0.0174 & &  7.8E-4 &  0.0013 &  0.0020 &  0.0030 &  0.0046 &  0.0069 &  0.0098\\
0436 &  0.0023 &  0.0033 &  0.0047 &  0.0068 &  0.0094 &  0.0128 &  0.0174 & &  7.9E-4 &  0.0013 &  0.0020 &  0.0030 &  0.0046 &  0.0068 &  0.0097\\
0437 &  0.0023 &  0.0033 &  0.0047 &  0.0067 &  0.0093 &  0.0127 &  0.0172 & &  8.0E-4 &  0.0013 &  0.0020 &  0.0030 &  0.0045 &  0.0068 &  0.0096\\
0438 &  0.0023 &  0.0033 &  0.0047 &  0.0067 &  0.0092 &  0.0126 &  0.0170 & &  8.0E-4 &  0.0013 &  0.0020 &  0.0030 &  0.0045 &  0.0067 &  0.0095\\
0439 &  0.0023 &  0.0033 &  0.0047 &  0.0067 &  0.0092 &  0.0126 &  0.0170 & &  8.1E-4 &  0.0013 &  0.0020 &  0.0029 &  0.0045 &  0.0066 &  0.0094\\
0440 &  0.0023 &  0.0032 &  0.0046 &  0.0066 &  0.0091 &  0.0125 &  0.0169 & &  8.1E-4 &  0.0013 &  0.0020 &  0.0029 &  0.0044 &  0.0066 &  0.0093\\
0441 &  0.0023 &  0.0032 &  0.0046 &  0.0066 &  0.0091 &  0.0124 &  0.0167 & &  8.2E-4 &  0.0013 &  0.0019 &  0.0029 &  0.0044 &  0.0065 &  0.0091\\
0442 &  0.0023 &  0.0032 &  0.0046 &  0.0066 &  0.0090 &  0.0124 &  0.0167 & &  8.2E-4 &  0.0013 &  0.0019 &  0.0029 &  0.0043 &  0.0064 &  0.0090\\
0443 &  0.0022 &  0.0032 &  0.0046 &  0.0065 &  0.0089 &  0.0123 &  0.0165 & &  8.3E-4 &  0.0013 &  0.0019 &  0.0028 &  0.0043 &  0.0064 &  0.0089\\
0444 &  0.0022 &  0.0032 &  0.0046 &  0.0065 &  0.0089 &  0.0122 &  0.0163 & &  8.3E-4 &  0.0013 &  0.0019 &  0.0028 &  0.0042 &  0.0063 &  0.0088\\
0445 &  0.0022 &  0.0032 &  0.0045 &  0.0065 &  0.0088 &  0.0122 &  0.0163 & &  8.4E-4 &  0.0013 &  0.0019 &  0.0028 &  0.0042 &  0.0062 &  0.0087\\
0446 &  0.0022 &  0.0032 &  0.0045 &  0.0064 &  0.0088 &  0.0121 &  0.0162 & &  8.4E-4 &  0.0013 &  0.0019 &  0.0028 &  0.0041 &  0.0062 &  0.0086\\
0447 &  0.0022 &  0.0031 &  0.0045 &  0.0064 &  0.0087 &  0.0121 &  0.0160 & &  8.5E-4 &  0.0013 &  0.0019 &  0.0027 &  0.0041 &  0.0061 &  0.0085\\
0448 &  0.0022 &  0.0031 &  0.0045 &  0.0063 &  0.0086 &  0.0120 &  0.0160 & &  8.5E-4 &  0.0013 &  0.0019 &  0.0027 &  0.0041 &  0.0060 &  0.0084\\
0449 &  0.0022 &  0.0031 &  0.0045 &  0.0063 &  0.0086 &  0.0119 &  0.0159 & &  8.5E-4 &  0.0013 &  0.0018 &  0.0027 &  0.0040 &  0.0060 &  0.0083\\
0450 &  0.0022 &  0.0031 &  0.0045 &  0.0062 &  0.0085 &  0.0119 &  0.0157 & &  8.5E-4 &  0.0013 &  0.0018 &  0.0026 &  0.0040 &  0.0059 &  0.0082\\
0451 &  0.0022 &  0.0031 &  0.0045 &  0.0062 &  0.0085 &  0.0118 &  0.0156 & &  8.6E-4 &  0.0013 &  0.0018 &  0.0026 &  0.0039 &  0.0058 &  0.0081\\
0452 &  0.0022 &  0.0031 &  0.0044 &  0.0062 &  0.0085 &  0.0117 &  0.0156 & &  8.6E-4 &  0.0013 &  0.0018 &  0.0026 &  0.0039 &  0.0058 &  0.0080\\
0453 &  0.0021 &  0.0030 &  0.0044 &  0.0061 &  0.0084 &  0.0117 &  0.0154 & &  8.6E-4 &  0.0013 &  0.0018 &  0.0025 &  0.0038 &  0.0057 &  0.0080\\
0454 &  0.0021 &  0.0030 &  0.0044 &  0.0061 &  0.0084 &  0.0116 &  0.0154 & &  8.6E-4 &  0.0013 &  0.0018 &  0.0025 &  0.0038 &  0.0057 &  0.0079\\
0455 &  0.0021 &  0.0030 &  0.0044 &  0.0060 &  0.0084 &  0.0115 &  0.0153 & &  8.6E-4 &  0.0013 &  0.0017 &  0.0025 &  0.0038 &  0.0056 &  0.0078\\
0456 &  0.0021 &  0.0030 &  0.0044 &  0.0060 &  0.0083 &  0.0115 &  0.0151 & &  8.6E-4 &  0.0013 &  0.0017 &  0.0025 &  0.0037 &  0.0055 &  0.0077\\
0457 &  0.0021 &  0.0030 &  0.0043 &  0.0060 &  0.0083 &  0.0114 &  0.0151 & &  8.6E-4 &  0.0012 &  0.0017 &  0.0024 &  0.0037 &  0.0055 &  0.0076\\
0458 &  0.0021 &  0.0030 &  0.0043 &  0.0059 &  0.0083 &  0.0113 &  0.0150 & &  8.6E-4 &  0.0012 &  0.0017 &  0.0024 &  0.0036 &  0.0054 &  0.0076\\
0459 &  0.0021 &  0.0030 &  0.0043 &  0.0059 &  0.0082 &  0.0113 &  0.0149 & &  8.6E-4 &  0.0012 &  0.0017 &  0.0024 &  0.0036 &  0.0054 &  0.0075\\
0460 &  0.0021 &  0.0030 &  0.0043 &  0.0058 &  0.0082 &  0.0112 &  0.0149 & &  8.6E-4 &  0.0012 &  0.0016 &  0.0023 &  0.0036 &  0.0053 &  0.0074\\
0461 &  0.0020 &  0.0030 &  0.0043 &  0.0058 &  0.0082 &  0.0111 &  0.0148 & &  8.5E-4 &  0.0012 &  0.0016 &  0.0023 &  0.0035 &  0.0053 &  0.0074\\
0462 &  0.0020 &  0.0030 &  0.0043 &  0.0058 &  0.0081 &  0.0111 &  0.0146 & &  8.5E-4 &  0.0012 &  0.0016 &  0.0023 &  0.0035 &  0.0052 &  0.0073\\
0463 &  0.0020 &  0.0030 &  0.0042 &  0.0058 &  0.0081 &  0.0110 &  0.0146 & &  8.5E-4 &  0.0012 &  0.0016 &  0.0022 &  0.0035 &  0.0052 &  0.0072\\
0464 &  0.0020 &  0.0030 &  0.0042 &  0.0057 &  0.0081 &  0.0110 &  0.0146 & &  8.5E-4 &  0.0012 &  0.0015 &  0.0022 &  0.0034 &  0.0051 &  0.0072\\
0465 &  0.0020 &  0.0030 &  0.0042 &  0.0057 &  0.0080 &  0.0109 &  0.0144 & &  8.5E-4 &  0.0012 &  0.0015 &  0.0022 &  0.0034 &  0.0051 &  0.0071\\
0466 &  0.0020 &  0.0030 &  0.0042 &  0.0057 &  0.0080 &  0.0109 &  0.0144 & &  8.4E-4 &  0.0012 &  0.0015 &  0.0022 &  0.0034 &  0.0050 &  0.0071\\
0467 &  0.0020 &  0.0030 &  0.0041 &  0.0057 &  0.0080 &  0.0108 &  0.0144 & &  8.4E-4 &  0.0011 &  0.0015 &  0.0021 &  0.0033 &  0.0050 &  0.0070\\
0468 &  0.0020 &  0.0030 &  0.0041 &  0.0056 &  0.0079 &  0.0108 &  0.0143 & &  8.4E-4 &  0.0011 &  0.0014 &  0.0021 &  0.0033 &  0.0049 &  0.0070\\
0469 &  0.0020 &  0.0030 &  0.0041 &  0.0056 &  0.0079 &  0.0107 &  0.0142 & &  8.3E-4 &  0.0011 &  0.0014 &  0.0021 &  0.0033 &  0.0049 &  0.0069\\
0470 &  0.0020 &  0.0030 &  0.0041 &  0.0056 &  0.0079 &  0.0106 &  0.0143 & &  8.3E-4 &  0.0011 &  0.0014 &  0.0021 &  0.0032 &  0.0048 &  0.0069\\
0471 &  0.0020 &  0.0030 &  0.0040 &  0.0056 &  0.0078 &  0.0106 &  0.0141 & &  8.2E-4 &  0.0011 &  0.0014 &  0.0020 &  0.0032 &  0.0048 &  0.0068\\
0472 &  0.0020 &  0.0030 &  0.0040 &  0.0056 &  0.0078 &  0.0105 &  0.0141 & &  8.2E-4 &  0.0011 &  0.0013 &  0.0020 &  0.0032 &  0.0047 &  0.0068\\
0473 &  0.0020 &  0.0030 &  0.0040 &  0.0056 &  0.0078 &  0.0105 &  0.0141 & &  8.1E-4 &  0.0011 &  0.0013 &  0.0020 &  0.0031 &  0.0047 &  0.0067\\
0474 &  0.0020 &  0.0030 &  0.0040 &  0.0055 &  0.0077 &  0.0105 &  0.0139 & &  8.1E-4 &  0.0010 &  0.0013 &  0.0020 &  0.0031 &  0.0046 &  0.0067\\
0475 &  0.0020 &  0.0030 &  0.0040 &  0.0055 &  0.0076 &  0.0104 &  0.0139 & &  8.0E-4 &  0.0010 &  0.0013 &  0.0019 &  0.0031 &  0.0046 &  0.0066\\
0476 &  0.0020 &  0.0030 &  0.0039 &  0.0055 &  0.0076 &  0.0103 &  0.0140 & &  7.9E-4 &  1.0E-3 &  0.0013 &  0.0019 &  0.0030 &  0.0045 &  0.0066\\
0477 &  0.0020 &  0.0029 &  0.0039 &  0.0055 &  0.0076 &  0.0103 &  0.0138 & &  7.8E-4 &  9.8E-4 &  0.0012 &  0.0019 &  0.0030 &  0.0045 &  0.0066\\
0478 &  0.0020 &  0.0029 &  0.0039 &  0.0055 &  0.0075 &  0.0102 &  0.0138 & &  7.7E-4 &  9.5E-4 &  0.0012 &  0.0019 &  0.0030 &  0.0044 &  0.0065\\
0479 &  0.0020 &  0.0029 &  0.0039 &  0.0055 &  0.0075 &  0.0102 &  0.0138 & &  7.6E-4 &  9.3E-4 &  0.0012 &  0.0018 &  0.0029 &  0.0044 &  0.0065\\
0480 &  0.0020 &  0.0029 &  0.0039 &  0.0054 &  0.0075 &  0.0102 &  0.0136 & &  7.5E-4 &  9.1E-4 &  0.0012 &  0.0018 &  0.0029 &  0.0044 &  0.0064\\
0481 &  0.0021 &  0.0029 &  0.0039 &  0.0054 &  0.0074 &  0.0101 &  0.0136 & &  7.4E-4 &  8.9E-4 &  0.0011 &  0.0018 &  0.0029 &  0.0043 &  0.0064\\
0482 &  0.0021 &  0.0029 &  0.0039 &  0.0054 &  0.0074 &  0.0101 &  0.0137 & &  7.2E-4 &  8.7E-4 &  0.0011 &  0.0018 &  0.0028 &  0.0043 &  0.0063\\
0483 &  0.0021 &  0.0029 &  0.0038 &  0.0053 &  0.0074 &  0.0100 &  0.0135 & &  7.1E-4 &  8.5E-4 &  0.0011 &  0.0018 &  0.0028 &  0.0042 &  0.0063\\
0484 &  0.0021 &  0.0029 &  0.0038 &  0.0053 &  0.0073 &  0.0100 &  0.0134 & &  7.0E-4 &  8.3E-4 &  0.0011 &  0.0017 &  0.0028 &  0.0042 &  0.0062\\
0485 &  0.0021 &  0.0029 &  0.0038 &  0.0053 &  0.0073 &  0.0100 &  0.0135 & &  6.8E-4 &  8.1E-4 &  0.0011 &  0.0017 &  0.0027 &  0.0041 &  0.0062\\
0486 &  0.0021 &  0.0028 &  0.0038 &  0.0052 &  0.0072 &  0.0099 &  0.0133 & &  6.7E-4 &  7.9E-4 &  0.0010 &  0.0017 &  0.0027 &  0.0041 &  0.0061\\
0487 &  0.0021 &  0.0028 &  0.0038 &  0.0052 &  0.0072 &  0.0099 &  0.0133 & &  6.5E-4 &  7.7E-4 &  0.0010 &  0.0017 &  0.0026 &  0.0040 &  0.0060\\
0488 &  0.0021 &  0.0028 &  0.0038 &  0.0052 &  0.0072 &  0.0099 &  0.0133 & &  6.3E-4 &  7.5E-4 &  1.0E-3 &  0.0016 &  0.0026 &  0.0040 &  0.0060\\
0489 &  0.0021 &  0.0028 &  0.0038 &  0.0051 &  0.0071 &  0.0099 &  0.0131 & &  6.2E-4 &  7.3E-4 &  9.8E-4 &  0.0016 &  0.0026 &  0.0039 &  0.0059\\
0490 &  0.0021 &  0.0028 &  0.0038 &  0.0051 &  0.0071 &  0.0099 &  0.0131 & &  6.0E-4 &  7.1E-4 &  9.6E-4 &  0.0016 &  0.0025 &  0.0039 &  0.0059\\
0491 &  0.0021 &  0.0028 &  0.0037 &  0.0051 &  0.0071 &  0.0099 &  0.0131 & &  5.8E-4 &  6.8E-4 &  9.4E-4 &  0.0015 &  0.0025 &  0.0038 &  0.0058\\
0492 &  0.0021 &  0.0027 &  0.0037 &  0.0051 &  0.0070 &  0.0098 &  0.0129 & &  5.7E-4 &  6.6E-4 &  9.2E-4 &  0.0015 &  0.0024 &  0.0038 &  0.0057\\
0493 &  0.0021 &  0.0027 &  0.0037 &  0.0051 &  0.0070 &  0.0098 &  0.0129 & &  5.5E-4 &  6.4E-4 &  8.9E-4 &  0.0015 &  0.0024 &  0.0037 &  0.0057\\
0494 &  0.0021 &  0.0027 &  0.0037 &  0.0050 &  0.0070 &  0.0098 &  0.0130 & &  5.3E-4 &  6.2E-4 &  8.7E-4 &  0.0015 &  0.0023 &  0.0037 &  0.0056\\
0495 &  0.0021 &  0.0027 &  0.0036 &  0.0050 &  0.0070 &  0.0098 &  0.0128 & &  5.1E-4 &  6.0E-4 &  8.5E-4 &  0.0014 &  0.0023 &  0.0037 &  0.0055\\
0496 &  0.0021 &  0.0027 &  0.0036 &  0.0050 &  0.0069 &  0.0098 &  0.0127 & &  5.0E-4 &  5.8E-4 &  8.3E-4 &  0.0014 &  0.0023 &  0.0036 &  0.0055\\
0497 &  0.0021 &  0.0027 &  0.0036 &  0.0049 &  0.0069 &  0.0098 &  0.0128 & &  4.8E-4 &  5.6E-4 &  8.0E-4 &  0.0014 &  0.0022 &  0.0036 &  0.0054\\
0498 &  0.0021 &  0.0027 &  0.0036 &  0.0049 &  0.0069 &  0.0097 &  0.0126 & &  4.6E-4 &  5.4E-4 &  7.8E-4 &  0.0013 &  0.0022 &  0.0035 &  0.0053\\
0499 &  0.0020 &  0.0027 &  0.0036 &  0.0049 &  0.0069 &  0.0097 &  0.0126 & &  4.4E-4 &  5.2E-4 &  7.5E-4 &  0.0013 &  0.0021 &  0.0035 &  0.0052\\
0500 &  0.0020 &  0.0027 &  0.0035 &  0.0049 &  0.0069 &  0.0097 &  0.0127 & &  4.2E-4 &  4.9E-4 &  7.3E-4 &  0.0013 &  0.0021 &  0.0034 &  0.0052\\
0501 &  0.0020 &  0.0026 &  0.0035 &  0.0048 &  0.0069 &  0.0096 &  0.0125 & &  4.0E-4 &  4.7E-4 &  7.0E-4 &  0.0012 &  0.0020 &  0.0034 &  0.0051\\
0502 &  0.0020 &  0.0026 &  0.0035 &  0.0048 &  0.0069 &  0.0096 &  0.0125 & &  3.9E-4 &  4.5E-4 &  6.8E-4 &  0.0012 &  0.0020 &  0.0033 &  0.0050\\
0503 &  0.0020 &  0.0026 &  0.0034 &  0.0048 &  0.0069 &  0.0096 &  0.0126 & &  3.7E-4 &  4.3E-4 &  6.5E-4 &  0.0011 &  0.0019 &  0.0033 &  0.0050\\
0504 &  0.0020 &  0.0026 &  0.0034 &  0.0048 &  0.0069 &  0.0096 &  0.0124 & &  3.5E-4 &  4.0E-4 &  6.2E-4 &  0.0011 &  0.0019 &  0.0032 &  0.0049\\
0505 &  0.0020 &  0.0026 &  0.0034 &  0.0047 &  0.0069 &  0.0096 &  0.0123 & &  3.3E-4 &  3.8E-4 &  5.9E-4 &  0.0011 &  0.0018 &  0.0032 &  0.0048\\
0506 &  0.0019 &  0.0026 &  0.0034 &  0.0047 &  0.0069 &  0.0096 &  0.0124 & &  3.1E-4 &  3.6E-4 &  5.6E-4 &  0.0010 &  0.0018 &  0.0031 &  0.0047\\
0507 &  0.0019 &  0.0025 &  0.0033 &  0.0047 &  0.0069 &  0.0095 &  0.0123 & &  2.9E-4 &  3.3E-4 &  5.4E-4 &  9.8E-4 &  0.0018 &  0.0031 &  0.0047\\
0508 &  0.0019 &  0.0025 &  0.0033 &  0.0047 &  0.0069 &  0.0095 &  0.0122 & &  2.7E-4 &  3.1E-4 &  5.1E-4 &  9.3E-4 &  0.0017 &  0.0030 &  0.0046\\
0509 &  0.0019 &  0.0025 &  0.0033 &  0.0047 &  0.0069 &  0.0095 &  0.0123 & &  2.5E-4 &  2.9E-4 &  4.7E-4 &  8.9E-4 &  0.0017 &  0.0030 &  0.0045\\
0510 &  0.0019 &  0.0025 &  0.0033 &  0.0047 &  0.0069 &  0.0094 &  0.0122 & &  2.3E-4 &  2.6E-4 &  4.4E-4 &  8.5E-4 &  0.0016 &  0.0030 &  0.0045\\
0511 &  0.0019 &  0.0024 &  0.0032 &  0.0047 &  0.0069 &  0.0094 &  0.0121 & &  2.1E-4 &  2.3E-4 &  4.1E-4 &  8.0E-4 &  0.0016 &  0.0029 &  0.0044\\
0512 &  0.0019 &  0.0024 &  0.0032 &  0.0047 &  0.0069 &  0.0094 &  0.0122 & &  1.8E-4 &  2.1E-4 &  3.8E-4 &  7.6E-4 &  0.0015 &  0.0029 &  0.0043\\
0513 &  0.0019 &  0.0024 &  0.0032 &  0.0047 &  0.0069 &  0.0093 &  0.0121 & &  1.6E-4 &  1.8E-4 &  3.5E-4 &  7.2E-4 &  0.0015 &  0.0028 &  0.0043\\
0514 &  0.0018 &  0.0023 &  0.0032 &  0.0047 &  0.0069 &  0.0093 &  0.0120 & &  1.4E-4 &  1.6E-4 &  3.1E-4 &  6.7E-4 &  0.0015 &  0.0028 &  0.0042\\
0515 &  0.0018 &  0.0023 &  0.0032 &  0.0047 &  0.0069 &  0.0092 &  0.0121 & &  1.2E-4 &  1.3E-4 &  2.8E-4 &  6.3E-4 &  0.0014 &  0.0027 &  0.0041\\
0516 &  0.0018 &  0.0023 &  0.0032 &  0.0047 &  0.0068 &  0.0091 &  0.0120 & &  9.8E-5 &  1.0E-4 &  2.4E-4 &  5.8E-4 &  0.0014 &  0.0027 &  0.0041\\
0517 &  0.0018 &  0.0023 &  0.0032 &  0.0047 &  0.0069 &  0.0091 &  0.0119 & &  7.5E-5 &  7.6E-5 &  2.1E-4 &  5.4E-4 &  0.0014 &  0.0026 &  0.0040\\
0518 &  0.0018 &  0.0023 &  0.0032 &  0.0047 &  0.0069 &  0.0091 &  0.0120 & &  5.3E-5 &  4.8E-5 &  1.7E-4 &  5.0E-4 &  0.0013 &  0.0026 &  0.0039\\
0519 &  0.0018 &  0.0022 &  0.0031 &  0.0047 &  0.0068 &  0.0090 &  0.0119 & &  2.9E-5 &  2.0E-5 &  1.3E-4 &  4.6E-4 &  0.0013 &  0.0025 &  0.0039\\
0520 &  0.0017 &  0.0022 &  0.0031 &  0.0047 &  0.0068 &  0.0090 &  0.0118 & &  6.1E-6 &  7.5E-6 &  9.6E-5 &  4.2E-4 &  0.0012 &  0.0025 &  0.0038\\
0521 &  0.0017 &  0.0022 &  0.0031 &  0.0047 &  0.0068 &  0.0089 &  0.0119 & &  1.8E-5 &  3.6E-5 &  5.8E-5 &  3.7E-4 &  0.0012 &  0.0025 &  0.0038\\
0522 &  0.0017 &  0.0022 &  0.0031 &  0.0047 &  0.0067 &  0.0088 &  0.0118 & &  4.2E-5 &  6.4E-5 &  1.9E-5 &  3.3E-4 &  0.0012 &  0.0024 &  0.0037\\
0523 &  0.0017 &  0.0022 &  0.0031 &  0.0047 &  0.0067 &  0.0088 &  0.0117 & &  6.6E-5 &  9.2E-5 &  2.0E-5 &  3.0E-4 &  0.0011 &  0.0024 &  0.0037\\
0524 &  0.0017 &  0.0022 &  0.0031 &  0.0047 &  0.0067 &  0.0088 &  0.0118 & &  9.1E-5 &  1.2E-4 &  6.0E-5 &  2.6E-4 &  0.0011 &  0.0023 &  0.0036\\
0525 &  0.0016 &  0.0021 &  0.0031 &  0.0048 &  0.0066 &  0.0087 &  0.0116 & &  1.2E-4 &  1.5E-4 &  9.9E-5 &  2.2E-4 &  0.0011 &  0.0023 &  0.0036\\
0526 &  0.0016 &  0.0021 &  0.0031 &  0.0047 &  0.0066 &  0.0087 &  0.0115 & &  1.4E-4 &  1.8E-4 &  1.4E-4 &  1.8E-4 &  0.0010 &  0.0022 &  0.0036\\
0527 &  0.0016 &  0.0021 &  0.0031 &  0.0047 &  0.0066 &  0.0086 &  0.0116 & &  1.7E-4 &  2.1E-4 &  1.8E-4 &  1.5E-4 &  0.0010 &  0.0022 &  0.0035\\
0528 &  0.0016 &  0.0021 &  0.0031 &  0.0047 &  0.0065 &  0.0086 &  0.0115 & &  1.9E-4 &  2.4E-4 &  2.2E-4 &  1.1E-4 &  9.8E-4 &  0.0021 &  0.0035\\
0529 &  0.0016 &  0.0021 &  0.0031 &  0.0047 &  0.0065 &  0.0085 &  0.0114 & &  2.2E-4 &  2.7E-4 &  2.6E-4 &  7.6E-5 &  9.5E-4 &  0.0021 &  0.0034\\
0530 &  0.0015 &  0.0021 &  0.0031 &  0.0047 &  0.0065 &  0.0085 &  0.0114 & &  2.4E-4 &  3.0E-4 &  3.0E-4 &  4.2E-5 &  9.2E-4 &  0.0021 &  0.0034\\
0531 &  0.0015 &  0.0021 &  0.0031 &  0.0047 &  0.0064 &  0.0084 &  0.0113 & &  2.7E-4 &  3.3E-4 &  3.4E-4 &  8.6E-6 &  8.9E-4 &  0.0020 &  0.0033\\
0532 &  0.0015 &  0.0021 &  0.0031 &  0.0047 &  0.0063 &  0.0084 &  0.0112 & &  2.9E-4 &  3.6E-4 &  3.8E-4 &  2.4E-5 &  8.6E-4 &  0.0020 &  0.0033\\
0533 &  0.0015 &  0.0021 &  0.0031 &  0.0047 &  0.0063 &  0.0083 &  0.0113 & &  3.2E-4 &  3.9E-4 &  4.2E-4 &  5.5E-5 &  8.3E-4 &  0.0019 &  0.0033\\
0534 &  0.0015 &  0.0021 &  0.0031 &  0.0047 &  0.0062 &  0.0083 &  0.0111 & &  3.4E-4 &  4.2E-4 &  4.6E-4 &  8.6E-5 &  7.9E-4 &  0.0019 &  0.0032\\
0535 &  0.0015 &  0.0020 &  0.0031 &  0.0046 &  0.0062 &  0.0083 &  0.0110 & &  3.7E-4 &  4.6E-4 &  5.0E-4 &  1.2E-4 &  7.6E-4 &  0.0018 &  0.0032\\
0536 &  0.0014 &  0.0020 &  0.0031 &  0.0046 &  0.0061 &  0.0082 &  0.0111 & &  3.9E-4 &  4.9E-4 &  5.4E-4 &  1.5E-4 &  7.3E-4 &  0.0018 &  0.0031\\
0537 &  0.0014 &  0.0020 &  0.0031 &  0.0046 &  0.0061 &  0.0082 &  0.0110 & &  4.2E-4 &  5.2E-4 &  5.7E-4 &  1.7E-4 &  7.0E-4 &  0.0018 &  0.0031\\
0538 &  0.0014 &  0.0020 &  0.0031 &  0.0045 &  0.0060 &  0.0082 &  0.0108 & &  4.4E-4 &  5.6E-4 &  6.1E-4 &  2.0E-4 &  6.6E-4 &  0.0017 &  0.0031\\
0539 &  0.0014 &  0.0020 &  0.0031 &  0.0045 &  0.0060 &  0.0081 &  0.0109 & &  4.7E-4 &  5.9E-4 &  6.5E-4 &  2.3E-4 &  6.3E-4 &  0.0017 &  0.0030\\
0540 &  0.0014 &  0.0020 &  0.0031 &  0.0045 &  0.0059 &  0.0081 &  0.0108 & &  4.9E-4 &  6.3E-4 &  6.9E-4 &  2.6E-4 &  6.0E-4 &  0.0016 &  0.0030\\
0541 &  0.0014 &  0.0020 &  0.0031 &  0.0044 &  0.0059 &  0.0081 &  0.0106 & &  5.1E-4 &  6.6E-4 &  7.2E-4 &  2.8E-4 &  5.6E-4 &  0.0016 &  0.0029\\
0542 &  0.0014 &  0.0020 &  0.0031 &  0.0044 &  0.0058 &  0.0081 &  0.0107 & &  5.4E-4 &  7.0E-4 &  7.6E-4 &  3.1E-4 &  5.3E-4 &  0.0016 &  0.0029\\
0543 &  0.0014 &  0.0020 &  0.0031 &  0.0044 &  0.0058 &  0.0081 &  0.0106 & &  5.6E-4 &  7.3E-4 &  7.9E-4 &  3.3E-4 &  4.9E-4 &  0.0015 &  0.0028\\
0544 &  0.0014 &  0.0020 &  0.0031 &  0.0043 &  0.0057 &  0.0080 &  0.0104 & &  5.9E-4 &  7.7E-4 &  8.2E-4 &  3.6E-4 &  4.6E-4 &  0.0015 &  0.0028\\
0545 &  0.0014 &  0.0020 &  0.0030 &  0.0043 &  0.0057 &  0.0080 &  0.0105 & &  6.1E-4 &  8.1E-4 &  8.6E-4 &  3.8E-4 &  4.2E-4 &  0.0014 &  0.0027\\
0546 &  0.0014 &  0.0020 &  0.0030 &  0.0042 &  0.0057 &  0.0080 &  0.0104 & &  6.4E-4 &  8.4E-4 &  8.9E-4 &  4.1E-4 &  3.9E-4 &  0.0014 &  0.0027\\
0547 &  0.0014 &  0.0020 &  0.0030 &  0.0042 &  0.0056 &  0.0079 &  0.0102 & &  6.7E-4 &  8.8E-4 &  9.2E-4 &  4.3E-4 &  3.5E-4 &  0.0013 &  0.0026\\
0548 &  0.0013 &  0.0020 &  0.0030 &  0.0041 &  0.0056 &  0.0079 &  0.0103 & &  6.9E-4 &  9.2E-4 &  9.5E-4 &  4.6E-4 &  3.1E-4 &  0.0013 &  0.0026\\
0549 &  0.0013 &  0.0020 &  0.0030 &  0.0041 &  0.0056 &  0.0079 &  0.0102 & &  7.2E-4 &  9.5E-4 &  9.8E-4 &  4.9E-4 &  2.8E-4 &  0.0013 &  0.0025\\
0550 &  0.0013 &  0.0020 &  0.0030 &  0.0040 &  0.0056 &  0.0079 &  0.0101 & &  7.5E-4 &  9.9E-4 & -0.0010 &  5.1E-4 &  2.4E-4 &  0.0012 &  0.0024\\
0551 &  0.0013 &  0.0020 &  0.0029 &  0.0040 &  0.0056 &  0.0078 &  0.0101 & &  7.7E-4 & -0.0010 & -0.0010 &  5.4E-4 &  2.0E-4 &  0.0012 &  0.0024\\
0552 &  0.0013 &  0.0020 &  0.0029 &  0.0040 &  0.0055 &  0.0078 &  0.0100 & &  8.0E-4 & -0.0011 & -0.0011 &  5.7E-4 &  1.6E-4 &  0.0011 &  0.0023\\
0553 &  0.0013 &  0.0019 &  0.0029 &  0.0039 &  0.0055 &  0.0078 &  0.0099 & &  8.3E-4 & -0.0011 & -0.0011 &  5.9E-4 &  1.2E-4 &  0.0011 &  0.0022\\
0554 &  0.0013 &  0.0019 &  0.0028 &  0.0039 &  0.0055 &  0.0077 &  0.0099 & &  8.6E-4 & -0.0011 & -0.0011 &  6.2E-4 &  8.4E-5 &  0.0010 &  0.0022\\
0555 &  0.0013 &  0.0019 &  0.0028 &  0.0039 &  0.0055 &  0.0077 &  0.0099 & &  8.9E-4 & -0.0012 & -0.0011 &  6.5E-4 &  4.3E-5 &  9.8E-4 &  0.0021\\
0556 &  0.0013 &  0.0019 &  0.0028 &  0.0038 &  0.0055 &  0.0077 &  0.0098 & &  9.2E-4 & -0.0012 & -0.0012 &  6.8E-4 &  2.7E-6 &  9.3E-4 &  0.0021\\
0557 &  0.0013 &  0.0019 &  0.0027 &  0.0038 &  0.0055 &  0.0076 &  0.0098 & &  9.5E-4 & -0.0012 & -0.0012 &  7.1E-4 &  3.9E-5 &  8.8E-4 &  0.0020\\
0558 &  0.0012 &  0.0019 &  0.0027 &  0.0038 &  0.0055 &  0.0076 &  0.0098 & &  9.8E-4 & -0.0013 & -0.0012 &  7.4E-4 &  8.0E-5 &  8.2E-4 &  0.0019\\
0559 &  0.0012 &  0.0018 &  0.0027 &  0.0037 &  0.0055 &  0.0075 &  0.0097 & & -0.0010 & -0.0013 & -0.0012 &  7.7E-4 &  1.2E-4 &  7.7E-4 &  0.0018\\
0560 &  0.0012 &  0.0018 &  0.0027 &  0.0037 &  0.0055 &  0.0075 &  0.0097 & & -0.0010 & -0.0013 & -0.0013 &  8.0E-4 &  1.7E-4 &  7.1E-4 &  0.0018\\
0561 &  0.0012 &  0.0018 &  0.0026 &  0.0037 &  0.0055 &  0.0075 &  0.0097 & & -0.0011 & -0.0014 & -0.0013 &  8.4E-4 &  2.1E-4 &  6.6E-4 &  0.0017\\
0562 &  0.0012 &  0.0018 &  0.0026 &  0.0037 &  0.0054 &  0.0074 &  0.0096 & & -0.0011 & -0.0014 & -0.0013 &  8.7E-4 &  2.5E-4 &  6.0E-4 &  0.0016\\
0563 &  0.0012 &  0.0018 &  0.0026 &  0.0036 &  0.0054 &  0.0073 &  0.0097 & & -0.0011 & -0.0014 & -0.0013 &  9.0E-4 &  3.0E-4 &  5.4E-4 &  0.0016\\
0564 &  0.0012 &  0.0018 &  0.0025 &  0.0037 &  0.0054 &  0.0073 &  0.0097 & & -0.0012 & -0.0015 & -0.0013 &  9.4E-4 &  3.4E-4 &  4.8E-4 &  0.0015\\
0565 &  0.0012 &  0.0017 &  0.0025 &  0.0036 &  0.0054 &  0.0073 &  0.0096 & & -0.0012 & -0.0015 & -0.0014 &  9.8E-4 &  3.9E-4 &  4.2E-4 &  0.0014\\
0566 &  0.0011 &  0.0017 &  0.0025 &  0.0036 &  0.0054 &  0.0072 &  0.0097 & & -0.0012 & -0.0015 & -0.0014 & -0.0010 &  4.4E-4 &  3.6E-4 &  0.0013\\
0567 &  0.0011 &  0.0017 &  0.0025 &  0.0036 &  0.0054 &  0.0072 &  0.0097 & & -0.0013 & -0.0015 & -0.0014 & -0.0010 &  4.9E-4 &  2.9E-4 &  0.0013\\
0568 &  0.0011 &  0.0017 &  0.0024 &  0.0036 &  0.0053 &  0.0071 &  0.0096 & & -0.0013 & -0.0016 & -0.0014 & -0.0011 &  5.3E-4 &  2.3E-4 &  0.0012\\
0569 &  0.0011 &  0.0017 &  0.0024 &  0.0036 &  0.0053 &  0.0071 &  0.0097 & & -0.0013 & -0.0016 & -0.0015 & -0.0011 &  5.8E-4 &  1.6E-4 &  0.0011\\
0570 &  0.0011 &  0.0017 &  0.0024 &  0.0036 &  0.0053 &  0.0071 &  0.0097 & & -0.0013 & -0.0016 & -0.0015 & -0.0012 &  6.3E-4 &  9.7E-5 &  0.0010\\
0571 &  0.0011 &  0.0016 &  0.0024 &  0.0036 &  0.0052 &  0.0070 &  0.0096 & & -0.0014 & -0.0016 & -0.0015 & -0.0012 &  6.8E-4 &  2.9E-5 &  9.5E-4\\
0572 &  0.0010 &  0.0016 &  0.0024 &  0.0036 &  0.0052 &  0.0069 &  0.0097 & & -0.0014 & -0.0017 & -0.0015 & -0.0012 &  7.4E-4 &  4.0E-5 &  8.7E-4\\
0573 &  0.0010 &  0.0016 &  0.0024 &  0.0036 &  0.0052 &  0.0069 &  0.0097 & & -0.0014 & -0.0017 & -0.0016 & -0.0013 &  7.9E-4 &  1.1E-4 &  7.9E-4\\
0574 &  0.0010 &  0.0016 &  0.0023 &  0.0036 &  0.0051 &  0.0069 &  0.0096 & & -0.0015 & -0.0017 & -0.0016 & -0.0013 &  8.4E-4 &  1.8E-4 &  7.0E-4\\
0575 &  0.0010 &  0.0016 &  0.0023 &  0.0035 &  0.0051 &  0.0068 &  0.0096 & & -0.0015 & -0.0017 & -0.0016 & -0.0014 &  9.0E-4 &  2.5E-4 &  6.1E-4\\
0576 &  9.8E-4 &  0.0016 &  0.0023 &  0.0035 &  0.0051 &  0.0069 &  0.0097 & & -0.0015 & -0.0017 & -0.0017 & -0.0014 &  9.5E-4 &  3.3E-4 &  5.2E-4\\
0577 &  9.8E-4 &  0.0016 &  0.0023 &  0.0035 &  0.0050 &  0.0068 &  0.0096 & & -0.0015 & -0.0018 & -0.0017 & -0.0015 & -0.0010 &  4.0E-4 &  4.3E-4\\
0578 &  9.8E-4 &  0.0015 &  0.0023 &  0.0035 &  0.0050 &  0.0068 &  0.0096 & & -0.0016 & -0.0018 & -0.0017 & -0.0015 & -0.0011 &  4.7E-4 &  3.3E-4\\
0579 &  9.6E-4 &  0.0015 &  0.0023 &  0.0035 &  0.0050 &  0.0068 &  0.0097 & & -0.0016 & -0.0018 & -0.0018 & -0.0015 & -0.0011 &  5.5E-4 &  2.4E-4\\
0580 &  9.5E-4 &  0.0015 &  0.0023 &  0.0035 &  0.0049 &  0.0068 &  0.0096 & & -0.0016 & -0.0018 & -0.0018 & -0.0016 & -0.0012 &  6.3E-4 &  1.4E-4\\
0581 &  9.5E-4 &  0.0015 &  0.0023 &  0.0034 &  0.0049 &  0.0067 &  0.0096 & & -0.0016 & -0.0018 & -0.0018 & -0.0016 & -0.0012 &  7.0E-4 &  3.7E-5\\
0582 &  9.3E-4 &  0.0015 &  0.0023 &  0.0034 &  0.0049 &  0.0067 &  0.0097 & & -0.0017 & -0.0019 & -0.0019 & -0.0017 & -0.0013 &  7.8E-4 &  6.5E-5\\
0583 &  9.3E-4 &  0.0015 &  0.0022 &  0.0034 &  0.0048 &  0.0067 &  0.0095 & & -0.0017 & -0.0019 & -0.0019 & -0.0017 & -0.0014 &  8.6E-4 &  1.7E-4\\
0584 &  9.3E-4 &  0.0015 &  0.0022 &  0.0034 &  0.0048 &  0.0066 &  0.0095 & & -0.0017 & -0.0019 & -0.0019 & -0.0018 & -0.0014 &  9.3E-4 &  2.7E-4\\
0585 &  9.2E-4 &  0.0015 &  0.0022 &  0.0034 &  0.0048 &  0.0066 &  0.0096 & & -0.0017 & -0.0019 & -0.0020 & -0.0018 & -0.0015 & -0.0010 &  3.8E-4\\
0586 &  9.1E-4 &  0.0015 &  0.0022 &  0.0033 &  0.0047 &  0.0067 &  0.0094 & & -0.0018 & -0.0020 & -0.0020 & -0.0019 & -0.0015 & -0.0011 &  4.9E-4\\
0587 &  9.1E-4 &  0.0015 &  0.0022 &  0.0033 &  0.0047 &  0.0066 &  0.0094 & & -0.0018 & -0.0020 & -0.0020 & -0.0019 & -0.0016 & -0.0012 &  5.9E-4\\
0588 &  9.1E-4 &  0.0015 &  0.0022 &  0.0033 &  0.0046 &  0.0066 &  0.0095 & & -0.0018 & -0.0020 & -0.0021 & -0.0020 & -0.0017 & -0.0012 &  7.0E-4\\
0589 &  9.0E-4 &  0.0014 &  0.0021 &  0.0033 &  0.0046 &  0.0066 &  0.0093 & & -0.0018 & -0.0020 & -0.0021 & -0.0020 & -0.0017 & -0.0013 &  8.1E-4\\
0590 &  9.1E-4 &  0.0014 &  0.0021 &  0.0033 &  0.0046 &  0.0066 &  0.0092 & & -0.0018 & -0.0021 & -0.0022 & -0.0021 & -0.0018 & -0.0014 &  9.1E-4\\
0591 &  9.0E-4 &  0.0014 &  0.0021 &  0.0032 &  0.0045 &  0.0065 &  0.0093 & & -0.0018 & -0.0021 & -0.0022 & -0.0021 & -0.0019 & -0.0015 & -0.0010\\
0592 &  8.9E-4 &  0.0014 &  0.0021 &  0.0032 &  0.0045 &  0.0065 &  0.0091 & & -0.0019 & -0.0021 & -0.0022 & -0.0022 & -0.0019 & -0.0016 & -0.0011\\
0593 &  9.1E-4 &  0.0014 &  0.0021 &  0.0032 &  0.0045 &  0.0065 &  0.0091 & & -0.0019 & -0.0021 & -0.0023 & -0.0022 & -0.0020 & -0.0016 & -0.0012\\
0594 &  9.0E-4 &  0.0014 &  0.0021 &  0.0031 &  0.0044 &  0.0065 &  0.0091 & & -0.0019 & -0.0022 & -0.0023 & -0.0023 & -0.0021 & -0.0017 & -0.0013\\
0595 &  8.9E-4 &  0.0014 &  0.0020 &  0.0031 &  0.0044 &  0.0065 &  0.0089 & & -0.0019 & -0.0022 & -0.0024 & -0.0023 & -0.0021 & -0.0018 & -0.0014\\
0596 &  9.1E-4 &  0.0014 &  0.0020 &  0.0031 &  0.0044 &  0.0065 &  0.0089 & & -0.0019 & -0.0022 & -0.0024 & -0.0024 & -0.0022 & -0.0018 & -0.0015\\
0597 &  9.1E-4 &  0.0014 &  0.0020 &  0.0031 &  0.0044 &  0.0064 &  0.0090 & & -0.0019 & -0.0022 & -0.0024 & -0.0024 & -0.0023 & -0.0019 & -0.0016\\
0598 &  8.9E-4 &  0.0013 &  0.0020 &  0.0031 &  0.0044 &  0.0064 &  0.0087 & & -0.0020 & -0.0023 & -0.0025 & -0.0025 & -0.0023 & -0.0020 & -0.0017\\
0599 &  9.1E-4 &  0.0013 &  0.0019 &  0.0030 &  0.0043 &  0.0064 &  0.0087 & & -0.0020 & -0.0023 & -0.0025 & -0.0025 & -0.0024 & -0.0021 & -0.0018\\
0600 &  9.1E-4 &  0.0013 &  0.0019 &  0.0030 &  0.0043 &  0.0064 &  0.0088 & & -0.0020 & -0.0023 & -0.0026 & -0.0026 & -0.0025 & -0.0021 & -0.0019\\
0601 &  8.9E-4 &  0.0013 &  0.0019 &  0.0030 &  0.0043 &  0.0064 &  0.0086 & & -0.0020 & -0.0024 & -0.0026 & -0.0026 & -0.0025 & -0.0022 & -0.0020\\
0602 &  9.0E-4 &  0.0012 &  0.0019 &  0.0030 &  0.0043 &  0.0064 &  0.0085 & & -0.0020 & -0.0024 & -0.0026 & -0.0027 & -0.0026 & -0.0023 & -0.0021\\
0603 &  9.0E-4 &  0.0012 &  0.0019 &  0.0029 &  0.0042 &  0.0063 &  0.0086 & & -0.0021 & -0.0024 & -0.0027 & -0.0027 & -0.0026 & -0.0023 & -0.0022\\
0604 &  8.8E-4 &  0.0012 &  0.0019 &  0.0029 &  0.0042 &  0.0063 &  0.0084 & & -0.0021 & -0.0025 & -0.0027 & -0.0028 & -0.0027 & -0.0024 & -0.0022\\
0605 &  8.8E-4 &  0.0012 &  0.0018 &  0.0029 &  0.0042 &  0.0063 &  0.0084 & & -0.0021 & -0.0025 & -0.0028 & -0.0028 & -0.0028 & -0.0025 & -0.0023\\
0606 &  8.9E-4 &  0.0012 &  0.0018 &  0.0028 &  0.0041 &  0.0063 &  0.0085 & & -0.0021 & -0.0025 & -0.0028 & -0.0029 & -0.0028 & -0.0025 & -0.0024\\
0607 &  8.7E-4 &  0.0011 &  0.0018 &  0.0028 &  0.0041 &  0.0062 &  0.0083 & & -0.0021 & -0.0026 & -0.0029 & -0.0029 & -0.0029 & -0.0026 & -0.0024\\
0608 &  8.6E-4 &  0.0011 &  0.0018 &  0.0028 &  0.0041 &  0.0062 &  0.0083 & & -0.0022 & -0.0026 & -0.0029 & -0.0030 & -0.0029 & -0.0026 & -0.0025\\
0609 &  8.6E-4 &  0.0011 &  0.0018 &  0.0027 &  0.0041 &  0.0062 &  0.0083 & & -0.0022 & -0.0026 & -0.0029 & -0.0030 & -0.0030 & -0.0027 & -0.0026\\
0610 &  8.4E-4 &  0.0010 &  0.0018 &  0.0027 &  0.0041 &  0.0062 &  0.0082 & & -0.0022 & -0.0027 & -0.0030 & -0.0031 & -0.0030 & -0.0027 & -0.0026\\
0611 &  8.1E-4 &  0.0010 &  0.0018 &  0.0027 &  0.0041 &  0.0061 &  0.0081 & & -0.0022 & -0.0027 & -0.0030 & -0.0031 & -0.0031 & -0.0028 & -0.0027\\
0612 &  8.0E-4 &  0.0010 &  0.0018 &  0.0026 &  0.0041 &  0.0061 &  0.0082 & & -0.0022 & -0.0027 & -0.0031 & -0.0032 & -0.0031 & -0.0028 & -0.0027\\
0613 &  7.9E-4 &  9.8E-4 &  0.0018 &  0.0026 &  0.0041 &  0.0061 &  0.0080 & & -0.0023 & -0.0028 & -0.0031 & -0.0032 & -0.0032 & -0.0029 & -0.0028\\
0614 &  7.6E-4 &  9.5E-4 &  0.0017 &  0.0026 &  0.0041 &  0.0060 &  0.0080 & & -0.0023 & -0.0028 & -0.0031 & -0.0033 & -0.0032 & -0.0029 & -0.0028\\
0615 &  7.4E-4 &  9.6E-4 &  0.0017 &  0.0025 &  0.0040 &  0.0060 &  0.0080 & & -0.0023 & -0.0028 & -0.0032 & -0.0033 & -0.0032 & -0.0030 & -0.0029\\
0616 &  7.2E-4 &  9.3E-4 &  0.0017 &  0.0025 &  0.0040 &  0.0059 &  0.0079 & & -0.0023 & -0.0029 & -0.0032 & -0.0034 & -0.0033 & -0.0030 & -0.0029\\
0617 &  6.8E-4 &  9.1E-4 &  0.0017 &  0.0025 &  0.0040 &  0.0059 &  0.0078 & & -0.0024 & -0.0029 & -0.0033 & -0.0034 & -0.0033 & -0.0031 & -0.0030\\
0618 &  6.6E-4 &  9.2E-4 &  0.0017 &  0.0025 &  0.0040 &  0.0059 &  0.0079 & & -0.0024 & -0.0029 & -0.0033 & -0.0034 & -0.0034 & -0.0031 & -0.0030\\
0619 &  6.3E-4 &  9.0E-4 &  0.0017 &  0.0025 &  0.0040 &  0.0058 &  0.0077 & & -0.0024 & -0.0030 & -0.0033 & -0.0035 & -0.0034 & -0.0032 & -0.0030\\
0620 &  6.0E-4 &  8.9E-4 &  0.0016 &  0.0024 &  0.0040 &  0.0058 &  0.0076 & & -0.0024 & -0.0030 & -0.0034 & -0.0035 & -0.0034 & -0.0032 & -0.0031\\
0621 &  5.8E-4 &  9.0E-4 &  0.0016 &  0.0024 &  0.0040 &  0.0057 &  0.0077 & & -0.0024 & -0.0030 & -0.0034 & -0.0036 & -0.0035 & -0.0033 & -0.0031\\
0622 &  5.5E-4 &  8.8E-4 &  0.0016 &  0.0024 &  0.0040 &  0.0057 &  0.0076 & & -0.0025 & -0.0031 & -0.0034 & -0.0036 & -0.0035 & -0.0033 & -0.0031\\
0623 &  5.2E-4 &  8.8E-4 &  0.0016 &  0.0024 &  0.0040 &  0.0057 &  0.0075 & & -0.0025 & -0.0031 & -0.0035 & -0.0036 & -0.0035 & -0.0034 & -0.0031\\
0624 &  5.1E-4 &  8.9E-4 &  0.0015 &  0.0023 &  0.0040 &  0.0056 &  0.0076 & & -0.0025 & -0.0031 & -0.0035 & -0.0037 & -0.0035 & -0.0034 & -0.0031\\
0625 &  4.7E-4 &  8.8E-4 &  0.0015 &  0.0024 &  0.0040 &  0.0055 &  0.0074 & & -0.0025 & -0.0032 & -0.0035 & -0.0037 & -0.0036 & -0.0034 & -0.0032\\
0626 &  4.4E-4 &  8.7E-4 &  0.0015 &  0.0024 &  0.0040 &  0.0055 &  0.0073 & & -0.0026 & -0.0032 & -0.0036 & -0.0037 & -0.0036 & -0.0035 & -0.0032\\
0627 &  4.4E-4 &  8.8E-4 &  0.0014 &  0.0023 &  0.0039 &  0.0054 &  0.0074 & & -0.0026 & -0.0032 & -0.0036 & -0.0037 & -0.0036 & -0.0035 & -0.0032\\
0628 &  4.1E-4 &  8.7E-4 &  0.0014 &  0.0023 &  0.0040 &  0.0054 &  0.0073 & & -0.0026 & -0.0033 & -0.0036 & -0.0038 & -0.0036 & -0.0036 & -0.0032\\
0629 &  3.8E-4 &  8.6E-4 &  0.0014 &  0.0023 &  0.0040 &  0.0053 &  0.0072 & & -0.0027 & -0.0033 & -0.0037 & -0.0038 & -0.0037 & -0.0036 & -0.0032\\
0630 &  3.8E-4 &  8.8E-4 &  0.0014 &  0.0023 &  0.0039 &  0.0053 &  0.0073 & & -0.0027 & -0.0033 & -0.0037 & -0.0038 & -0.0037 & -0.0037 & -0.0032\\
0631 &  3.7E-4 &  8.6E-4 &  0.0014 &  0.0023 &  0.0039 &  0.0052 &  0.0072 & & -0.0027 & -0.0033 & -0.0037 & -0.0038 & -0.0037 & -0.0037 & -0.0032\\
0632 &  3.4E-4 &  8.5E-4 &  0.0013 &  0.0023 &  0.0039 &  0.0052 &  0.0071 & & -0.0027 & -0.0034 & -0.0037 & -0.0039 & -0.0037 & -0.0037 & -0.0032\\
0633 &  3.5E-4 &  8.6E-4 &  0.0013 &  0.0023 &  0.0038 &  0.0051 &  0.0072 & & -0.0028 & -0.0034 & -0.0038 & -0.0039 & -0.0038 & -0.0038 & -0.0031\\
0634 &  3.4E-4 &  8.4E-4 &  0.0013 &  0.0023 &  0.0038 &  0.0050 &  0.0071 & & -0.0028 & -0.0034 & -0.0038 & -0.0039 & -0.0038 & -0.0038 & -0.0031\\
0635 &  3.2E-4 &  8.2E-4 &  0.0013 &  0.0024 &  0.0038 &  0.0050 &  0.0070 & & -0.0028 & -0.0034 & -0.0038 & -0.0039 & -0.0038 & -0.0039 & -0.0031\\
0636 &  3.3E-4 &  8.3E-4 &  0.0012 &  0.0023 &  0.0037 &  0.0050 &  0.0070 & & -0.0028 & -0.0034 & -0.0038 & -0.0039 & -0.0038 & -0.0039 & -0.0031\\
0637 &  3.4E-4 &  8.1E-4 &  0.0012 &  0.0024 &  0.0037 &  0.0049 &  0.0069 & & -0.0028 & -0.0035 & -0.0038 & -0.0039 & -0.0039 & -0.0039 & -0.0031\\
0638 &  3.3E-4 &  7.9E-4 &  0.0012 &  0.0024 &  0.0037 &  0.0049 &  0.0068 & & -0.0029 & -0.0035 & -0.0039 & -0.0040 & -0.0039 & -0.0040 & -0.0031\\
0639 &  3.4E-4 &  7.9E-4 &  0.0012 &  0.0023 &  0.0036 &  0.0048 &  0.0069 & & -0.0029 & -0.0035 & -0.0039 & -0.0040 & -0.0039 & -0.0040 & -0.0031\\
0640 &  3.5E-4 &  7.7E-4 &  0.0012 &  0.0024 &  0.0036 &  0.0047 &  0.0068 & & -0.0029 & -0.0035 & -0.0039 & -0.0040 & -0.0040 & -0.0041 & -0.0031\\
0641 &  3.4E-4 &  7.4E-4 &  0.0012 &  0.0024 &  0.0035 &  0.0047 &  0.0067 & & -0.0029 & -0.0035 & -0.0039 & -0.0040 & -0.0040 & -0.0041 & -0.0031\\
0642 &  3.5E-4 &  7.4E-4 &  0.0011 &  0.0024 &  0.0035 &  0.0047 &  0.0067 & & -0.0030 & -0.0036 & -0.0039 & -0.0040 & -0.0040 & -0.0041 & -0.0031\\
0643 &  3.7E-4 &  7.2E-4 &  0.0012 &  0.0024 &  0.0034 &  0.0046 &  0.0066 & & -0.0030 & -0.0036 & -0.0039 & -0.0040 & -0.0041 & -0.0042 & -0.0031\\
0644 &  3.5E-4 &  6.9E-4 &  0.0012 &  0.0024 &  0.0034 &  0.0046 &  0.0065 & & -0.0030 & -0.0036 & -0.0040 & -0.0040 & -0.0041 & -0.0042 & -0.0030\\
0645 &  3.6E-4 &  6.8E-4 &  0.0012 &  0.0024 &  0.0033 &  0.0046 &  0.0066 & & -0.0030 & -0.0036 & -0.0040 & -0.0040 & -0.0041 & -0.0042 & -0.0030\\
0646 &  3.8E-4 &  6.6E-4 &  0.0011 &  0.0024 &  0.0033 &  0.0045 &  0.0065 & & -0.0030 & -0.0036 & -0.0040 & -0.0041 & -0.0042 & -0.0043 & -0.0031\\
0647 &  3.6E-4 &  6.3E-4 &  0.0012 &  0.0024 &  0.0033 &  0.0045 &  0.0064 & & -0.0030 & -0.0036 & -0.0040 & -0.0041 & -0.0042 & -0.0043 & -0.0031\\
0648 &  3.7E-4 &  6.2E-4 &  0.0012 &  0.0023 &  0.0032 &  0.0045 &  0.0064 & & -0.0031 & -0.0036 & -0.0040 & -0.0041 & -0.0043 & -0.0043 & -0.0031\\
0649 &  3.7E-4 &  6.0E-4 &  0.0012 &  0.0023 &  0.0032 &  0.0045 &  0.0064 & & -0.0031 & -0.0036 & -0.0040 & -0.0041 & -0.0043 & -0.0044 & -0.0031\\
0650 &  3.8E-4 &  5.7E-4 &  0.0012 &  0.0023 &  0.0031 &  0.0044 &  0.0062 & & -0.0031 & -0.0037 & -0.0040 & -0.0041 & -0.0043 & -0.0044 & -0.0031\\
0651 &  3.6E-4 &  5.6E-4 &  0.0012 &  0.0023 &  0.0031 &  0.0044 &  0.0063 & & -0.0031 & -0.0037 & -0.0040 & -0.0041 & -0.0044 & -0.0045 & -0.0031\\
0652 &  3.7E-4 &  5.4E-4 &  0.0012 &  0.0023 &  0.0030 &  0.0044 &  0.0062 & & -0.0031 & -0.0037 & -0.0040 & -0.0042 & -0.0044 & -0.0045 & -0.0031\\
0653 &  3.8E-4 &  5.1E-4 &  0.0012 &  0.0023 &  0.0030 &  0.0044 &  0.0061 & & -0.0031 & -0.0037 & -0.0040 & -0.0042 & -0.0045 & -0.0045 & -0.0032\\
0654 &  3.5E-4 &  5.1E-4 &  0.0012 &  0.0022 &  0.0030 &  0.0043 &  0.0061 & & -0.0031 & -0.0037 & -0.0040 & -0.0042 & -0.0045 & -0.0046 & -0.0032\\
0655 &  3.5E-4 &  5.0E-4 &  0.0012 &  0.0022 &  0.0029 &  0.0043 &  0.0061 & & -0.0031 & -0.0037 & -0.0040 & -0.0042 & -0.0046 & -0.0046 & -0.0032\\
0656 &  3.6E-4 &  4.7E-4 &  0.0012 &  0.0022 &  0.0029 &  0.0043 &  0.0060 & & -0.0031 & -0.0037 & -0.0041 & -0.0042 & -0.0046 & -0.0046 & -0.0033\\
0657 &  3.3E-4 &  4.7E-4 &  0.0012 &  0.0021 &  0.0029 &  0.0043 &  0.0060 & & -0.0031 & -0.0037 & -0.0041 & -0.0043 & -0.0047 & -0.0047 & -0.0033\\
0658 &  3.3E-4 &  4.7E-4 &  0.0012 &  0.0021 &  0.0028 &  0.0043 &  0.0060 & & -0.0031 & -0.0037 & -0.0041 & -0.0043 & -0.0047 & -0.0047 & -0.0034\\
0659 &  3.4E-4 &  4.5E-4 &  0.0013 &  0.0021 &  0.0028 &  0.0042 &  0.0059 & & -0.0032 & -0.0037 & -0.0041 & -0.0043 & -0.0048 & -0.0048 & -0.0034\\
0660 &  3.2E-4 &  4.6E-4 &  0.0013 &  0.0021 &  0.0028 &  0.0042 &  0.0059 & & -0.0032 & -0.0037 & -0.0041 & -0.0043 & -0.0048 & -0.0048 & -0.0035\\
0661 &  3.0E-4 &  4.6E-4 &  0.0013 &  0.0020 &  0.0027 &  0.0042 &  0.0060 & & -0.0032 & -0.0037 & -0.0041 & -0.0044 & -0.0049 & -0.0049 & -0.0035\\
0662 &  3.0E-4 &  4.5E-4 &  0.0013 &  0.0020 &  0.0027 &  0.0042 &  0.0058 & & -0.0032 & -0.0037 & -0.0041 & -0.0044 & -0.0049 & -0.0049 & -0.0036\\
0663 &  2.9E-4 &  4.5E-4 &  0.0013 &  0.0020 &  0.0027 &  0.0041 &  0.0059 & & -0.0032 & -0.0037 & -0.0041 & -0.0044 & -0.0050 & -0.0050 & -0.0037\\
0664 &  2.6E-4 &  4.6E-4 &  0.0013 &  0.0019 &  0.0027 &  0.0042 &  0.0059 & & -0.0032 & -0.0037 & -0.0041 & -0.0045 & -0.0050 & -0.0050 & -0.0037\\
0665 &  2.6E-4 &  4.5E-4 &  0.0013 &  0.0019 &  0.0027 &  0.0041 &  0.0058 & & -0.0032 & -0.0038 & -0.0041 & -0.0045 & -0.0051 & -0.0051 & -0.0038\\
0666 &  2.5E-4 &  4.6E-4 &  0.0013 &  0.0019 &  0.0027 &  0.0041 &  0.0058 & & -0.0032 & -0.0038 & -0.0041 & -0.0046 & -0.0051 & -0.0051 & -0.0039\\
0667 &  2.3E-4 &  4.7E-4 &  0.0013 &  0.0018 &  0.0026 &  0.0042 &  0.0058 & & -0.0032 & -0.0038 & -0.0041 & -0.0046 & -0.0052 & -0.0052 & -0.0040\\
0668 &  2.2E-4 &  4.6E-4 &  0.0013 &  0.0018 &  0.0026 &  0.0041 &  0.0057 & & -0.0032 & -0.0038 & -0.0042 & -0.0046 & -0.0052 & -0.0052 & -0.0041\\
0669 &  2.2E-4 &  4.7E-4 &  0.0013 &  0.0018 &  0.0026 &  0.0041 &  0.0058 & & -0.0032 & -0.0038 & -0.0042 & -0.0047 & -0.0053 & -0.0053 & -0.0042\\
0670 &  2.0E-4 &  4.9E-4 &  0.0013 &  0.0018 &  0.0026 &  0.0042 &  0.0058 & & -0.0032 & -0.0038 & -0.0042 & -0.0047 & -0.0053 & -0.0053 & -0.0043\\
0671 &  1.9E-4 &  4.8E-4 &  0.0013 &  0.0017 &  0.0026 &  0.0041 &  0.0057 & & -0.0032 & -0.0038 & -0.0042 & -0.0048 & -0.0054 & -0.0054 & -0.0044\\
0672 &  1.8E-4 &  5.0E-4 &  0.0013 &  0.0017 &  0.0026 &  0.0041 &  0.0057 & & -0.0032 & -0.0038 & -0.0042 & -0.0048 & -0.0055 & -0.0055 & -0.0045\\
0673 &  1.8E-4 &  5.2E-4 &  0.0013 &  0.0017 &  0.0026 &  0.0042 &  0.0057 & & -0.0032 & -0.0038 & -0.0042 & -0.0048 & -0.0055 & -0.0055 & -0.0046\\
0674 &  1.7E-4 &  5.2E-4 &  0.0013 &  0.0016 &  0.0026 &  0.0041 &  0.0056 & & -0.0032 & -0.0038 & -0.0043 & -0.0049 & -0.0056 & -0.0056 & -0.0047\\
0675 &  1.6E-4 &  5.4E-4 &  0.0012 &  0.0016 &  0.0026 &  0.0041 &  0.0056 & & -0.0032 & -0.0038 & -0.0043 & -0.0049 & -0.0056 & -0.0057 & -0.0048\\
0676 &  1.7E-4 &  5.6E-4 &  0.0012 &  0.0016 &  0.0026 &  0.0042 &  0.0057 & & -0.0032 & -0.0038 & -0.0043 & -0.0050 & -0.0057 & -0.0057 & -0.0049\\
0677 &  1.6E-4 &  5.6E-4 &  0.0012 &  0.0016 &  0.0026 &  0.0041 &  0.0056 & & -0.0032 & -0.0038 & -0.0043 & -0.0050 & -0.0057 & -0.0058 & -0.0050\\
0678 &  1.5E-4 &  5.9E-4 &  0.0012 &  0.0016 &  0.0026 &  0.0041 &  0.0056 & & -0.0032 & -0.0038 & -0.0043 & -0.0051 & -0.0058 & -0.0059 & -0.0051\\
0679 &  1.6E-4 &  6.2E-4 &  0.0012 &  0.0016 &  0.0026 &  0.0042 &  0.0057 & & -0.0032 & -0.0038 & -0.0044 & -0.0051 & -0.0059 & -0.0060 & -0.0052\\
0680 &  1.6E-4 &  6.2E-4 &  0.0012 &  0.0015 &  0.0026 &  0.0041 &  0.0056 & & -0.0032 & -0.0038 & -0.0044 & -0.0052 & -0.0059 & -0.0060 & -0.0053\\
0681 &  1.5E-4 &  6.4E-4 &  0.0012 &  0.0015 &  0.0026 &  0.0041 &  0.0056 & & -0.0032 & -0.0038 & -0.0044 & -0.0052 & -0.0060 & -0.0061 & -0.0054\\
0682 &  1.5E-4 &  6.7E-4 &  0.0012 &  0.0015 &  0.0026 &  0.0042 &  0.0057 & & -0.0032 & -0.0038 & -0.0044 & -0.0053 & -0.0060 & -0.0062 & -0.0055\\
0683 &  1.6E-4 &  6.7E-4 &  0.0011 &  0.0015 &  0.0026 &  0.0041 &  0.0056 & & -0.0032 & -0.0039 & -0.0045 & -0.0053 & -0.0061 & -0.0063 & -0.0056\\
0684 &  1.5E-4 &  6.9E-4 &  0.0011 &  0.0015 &  0.0026 &  0.0041 &  0.0056 & & -0.0032 & -0.0039 & -0.0045 & -0.0054 & -0.0062 & -0.0063 & -0.0057\\
0685 &  1.4E-4 &  7.2E-4 &  0.0011 &  0.0015 &  0.0027 &  0.0041 &  0.0057 & & -0.0032 & -0.0039 & -0.0045 & -0.0054 & -0.0062 & -0.0064 & -0.0058\\
0686 &  1.6E-4 &  7.1E-4 &  0.0011 &  0.0015 &  0.0027 &  0.0041 &  0.0055 & & -0.0032 & -0.0039 & -0.0045 & -0.0055 & -0.0063 & -0.0065 & -0.0059\\
0687 &  1.6E-4 &  7.3E-4 &  0.0010 &  0.0015 &  0.0026 &  0.0041 &  0.0056 & & -0.0032 & -0.0039 & -0.0046 & -0.0055 & -0.0063 & -0.0066 & -0.0060\\
0688 &  1.5E-4 &  7.5E-4 &  0.0010 &  0.0015 &  0.0027 &  0.0041 &  0.0057 & & -0.0032 & -0.0039 & -0.0046 & -0.0056 & -0.0064 & -0.0066 & -0.0061\\
0689 &  1.8E-4 &  7.4E-4 &  0.0010 &  0.0015 &  0.0027 &  0.0040 &  0.0055 & & -0.0032 & -0.0039 & -0.0046 & -0.0056 & -0.0065 & -0.0067 & -0.0062\\
0690 &  1.9E-4 &  7.5E-4 &  9.9E-4 &  0.0015 &  0.0027 &  0.0040 &  0.0055 & & -0.0032 & -0.0039 & -0.0047 & -0.0057 & -0.0065 & -0.0068 & -0.0063\\
0691 &  1.9E-4 &  7.7E-4 &  9.9E-4 &  0.0015 &  0.0027 &  0.0040 &  0.0057 & & -0.0032 & -0.0039 & -0.0047 & -0.0057 & -0.0066 & -0.0069 & -0.0064\\
0692 &  2.0E-4 &  7.6E-4 &  9.6E-4 &  0.0015 &  0.0028 &  0.0040 &  0.0055 & & -0.0032 & -0.0039 & -0.0047 & -0.0058 & -0.0066 & -0.0069 & -0.0065\\
0693 &  2.3E-4 &  7.6E-4 &  9.4E-4 &  0.0015 &  0.0027 &  0.0039 &  0.0055 & & -0.0032 & -0.0040 & -0.0048 & -0.0058 & -0.0067 & -0.0070 & -0.0066\\
0694 &  2.4E-4 &  7.8E-4 &  9.4E-4 &  0.0015 &  0.0028 &  0.0039 &  0.0056 & & -0.0032 & -0.0040 & -0.0048 & -0.0059 & -0.0068 & -0.0071 & -0.0067\\
0695 &  2.5E-4 &  7.6E-4 &  9.1E-4 &  0.0015 &  0.0028 &  0.0039 &  0.0054 & & -0.0032 & -0.0040 & -0.0048 & -0.0059 & -0.0068 & -0.0071 & -0.0068\\
0696 &  2.8E-4 &  7.6E-4 &  8.9E-4 &  0.0015 &  0.0027 &  0.0038 &  0.0054 & & -0.0032 & -0.0040 & -0.0049 & -0.0060 & -0.0069 & -0.0072 & -0.0068\\
0697 &  3.0E-4 &  7.7E-4 &  9.0E-4 &  0.0015 &  0.0028 &  0.0039 &  0.0056 & & -0.0032 & -0.0040 & -0.0049 & -0.0060 & -0.0069 & -0.0073 & -0.0069\\
0698 &  3.1E-4 &  7.5E-4 &  8.7E-4 &  0.0015 &  0.0028 &  0.0038 &  0.0054 & & -0.0033 & -0.0040 & -0.0049 & -0.0061 & -0.0070 & -0.0073 & -0.0070\\
0699 &  3.4E-4 &  7.4E-4 &  8.6E-4 &  0.0016 &  0.0027 &  0.0038 &  0.0053 & & -0.0033 & -0.0040 & -0.0050 & -0.0061 & -0.0071 & -0.0074 & -0.0071\\
0700 &  3.6E-4 &  7.6E-4 &  8.5E-4 &  0.0016 &  0.0028 &  0.0038 &  0.0055 & & -0.0033 & -0.0040 & -0.0050 & -0.0061 & -0.0071 & -0.0074 & -0.0071\\
0701 &  3.7E-4 &  7.3E-4 &  8.5E-4 &  0.0016 &  0.0028 &  0.0037 &  0.0053 & & -0.0033 & -0.0041 & -0.0050 & -0.0062 & -0.0072 & -0.0075 & -0.0072\\
0702 &  4.0E-4 &  7.2E-4 &  8.5E-4 &  0.0016 &  0.0027 &  0.0037 &  0.0052 & & -0.0033 & -0.0041 & -0.0051 & -0.0062 & -0.0072 & -0.0076 & -0.0073\\
0703 &  4.2E-4 &  7.3E-4 &  8.4E-4 &  0.0016 &  0.0027 &  0.0037 &  0.0054 & & -0.0033 & -0.0041 & -0.0051 & -0.0063 & -0.0073 & -0.0076 & -0.0074\\
0704 &  4.2E-4 &  7.0E-4 &  8.5E-4 &  0.0016 &  0.0027 &  0.0037 &  0.0052 & & -0.0033 & -0.0041 & -0.0051 & -0.0063 & -0.0073 & -0.0077 & -0.0074\\
0705 &  4.6E-4 &  6.9E-4 &  8.5E-4 &  0.0017 &  0.0027 &  0.0037 &  0.0051 & & -0.0033 & -0.0041 & -0.0052 & -0.0064 & -0.0074 & -0.0077 & -0.0075\\
0706 &  4.7E-4 &  7.0E-4 &  8.4E-4 &  0.0017 &  0.0027 &  0.0036 &  0.0052 & & -0.0033 & -0.0041 & -0.0052 & -0.0064 & -0.0074 & -0.0078 & -0.0076\\
0707 &  4.7E-4 &  6.7E-4 &  8.5E-4 &  0.0016 &  0.0027 &  0.0036 &  0.0051 & & -0.0033 & -0.0041 & -0.0052 & -0.0065 & -0.0075 & -0.0078 & -0.0076\\
0708 &  5.0E-4 &  6.6E-4 &  8.6E-4 &  0.0017 &  0.0026 &  0.0036 &  0.0050 & & -0.0033 & -0.0042 & -0.0053 & -0.0065 & -0.0075 & -0.0079 & -0.0077\\
0709 &  5.1E-4 &  6.7E-4 &  8.5E-4 &  0.0017 &  0.0026 &  0.0035 &  0.0051 & & -0.0033 & -0.0042 & -0.0053 & -0.0065 & -0.0076 & -0.0079 & -0.0078\\
0710 &  5.1E-4 &  6.4E-4 &  8.7E-4 &  0.0017 &  0.0026 &  0.0036 &  0.0050 & & -0.0033 & -0.0042 & -0.0053 & -0.0066 & -0.0076 & -0.0079 & -0.0078\\
0711 &  5.2E-4 &  6.2E-4 &  8.7E-4 &  0.0017 &  0.0025 &  0.0036 &  0.0049 & & -0.0033 & -0.0042 & -0.0053 & -0.0066 & -0.0076 & -0.0080 & -0.0079\\
0712 &  5.4E-4 &  6.3E-4 &  8.7E-4 &  0.0017 &  0.0025 &  0.0035 &  0.0050 & & -0.0033 & -0.0042 & -0.0054 & -0.0067 & -0.0077 & -0.0080 & -0.0079\\
0713 &  5.2E-4 &  6.0E-4 &  8.8E-4 &  0.0017 &  0.0025 &  0.0035 &  0.0048 & & -0.0033 & -0.0042 & -0.0054 & -0.0067 & -0.0077 & -0.0080 & -0.0080\\
0714 &  5.4E-4 &  5.9E-4 &  8.9E-4 &  0.0017 &  0.0024 &  0.0035 &  0.0048 & & -0.0033 & -0.0042 & -0.0054 & -0.0067 & -0.0078 & -0.0081 & -0.0081\\
0715 &  5.5E-4 &  5.9E-4 &  8.9E-4 &  0.0017 &  0.0024 &  0.0034 &  0.0049 & & -0.0033 & -0.0043 & -0.0055 & -0.0068 & -0.0078 & -0.0081 & -0.0081\\
0716 &  5.3E-4 &  5.6E-4 &  9.0E-4 &  0.0017 &  0.0024 &  0.0034 &  0.0047 & & -0.0033 & -0.0043 & -0.0055 & -0.0068 & -0.0078 & -0.0081 & -0.0082\\
0717 &  5.5E-4 &  5.5E-4 &  9.1E-4 &  0.0017 &  0.0024 &  0.0034 &  0.0047 & & -0.0033 & -0.0043 & -0.0055 & -0.0069 & -0.0078 & -0.0082 & -0.0083\\
0718 &  5.5E-4 &  5.6E-4 &  9.0E-4 &  0.0017 &  0.0024 &  0.0033 &  0.0048 & & -0.0033 & -0.0043 & -0.0055 & -0.0069 & -0.0079 & -0.0082 & -0.0083\\
0719 &  5.4E-4 &  5.4E-4 &  9.1E-4 &  0.0016 &  0.0023 &  0.0033 &  0.0046 & & -0.0033 & -0.0043 & -0.0056 & -0.0069 & -0.0079 & -0.0082 & -0.0084\\
0720 &  5.5E-4 &  5.2E-4 &  9.2E-4 &  0.0017 &  0.0023 &  0.0033 &  0.0046 & & -0.0033 & -0.0043 & -0.0056 & -0.0070 & -0.0079 & -0.0082 & -0.0085\\
0721 &  5.4E-4 &  5.4E-4 &  9.1E-4 &  0.0017 &  0.0023 &  0.0032 &  0.0047 & & -0.0033 & -0.0043 & -0.0056 & -0.0070 & -0.0079 & -0.0082 & -0.0085\\
0722 &  5.3E-4 &  5.2E-4 &  9.2E-4 &  0.0016 &  0.0023 &  0.0033 &  0.0046 & & -0.0033 & -0.0044 & -0.0056 & -0.0070 & -0.0080 & -0.0083 & -0.0086\\
0723 &  5.4E-4 &  5.1E-4 &  9.2E-4 &  0.0016 &  0.0022 &  0.0033 &  0.0045 & & -0.0033 & -0.0044 & -0.0057 & -0.0070 & -0.0080 & -0.0083 & -0.0087\\
0724 &  5.3E-4 &  5.3E-4 &  9.1E-4 &  0.0016 &  0.0022 &  0.0032 &  0.0046 & & -0.0034 & -0.0044 & -0.0057 & -0.0071 & -0.0080 & -0.0083 & -0.0088\\
0725 &  5.2E-4 &  5.2E-4 &  9.2E-4 &  0.0016 &  0.0022 &  0.0032 &  0.0045 & & -0.0034 & -0.0044 & -0.0057 & -0.0071 & -0.0080 & -0.0083 & -0.0088\\
0726 &  5.3E-4 &  5.1E-4 &  9.2E-4 &  0.0016 &  0.0022 &  0.0032 &  0.0044 & & -0.0034 & -0.0044 & -0.0057 & -0.0071 & -0.0080 & -0.0084 & -0.0089\\
0727 &  5.1E-4 &  5.3E-4 &  9.1E-4 &  0.0016 &  0.0022 &  0.0031 &  0.0045 & & -0.0034 & -0.0044 & -0.0057 & -0.0071 & -0.0080 & -0.0084 & -0.0090\\
0728 &  5.0E-4 &  5.2E-4 &  9.0E-4 &  0.0015 &  0.0022 &  0.0032 &  0.0044 & & -0.0034 & -0.0044 & -0.0058 & -0.0071 & -0.0081 & -0.0084 & -0.0091\\
0729 &  5.1E-4 &  5.2E-4 &  9.1E-4 &  0.0015 &  0.0021 &  0.0031 &  0.0044 & & -0.0034 & -0.0044 & -0.0058 & -0.0072 & -0.0081 & -0.0084 & -0.0092\\
0730 &  4.9E-4 &  5.4E-4 &  9.1E-4 &  0.0015 &  0.0021 &  0.0031 &  0.0045 & & -0.0034 & -0.0044 & -0.0058 & -0.0072 & -0.0081 & -0.0085 & -0.0092\\
0731 &  4.8E-4 &  5.3E-4 &  8.9E-4 &  0.0015 &  0.0021 &  0.0031 &  0.0044 & & -0.0034 & -0.0045 & -0.0058 & -0.0072 & -0.0081 & -0.0085 & -0.0093\\
0732 &  4.7E-4 &  5.2E-4 &  9.0E-4 &  0.0015 &  0.0020 &  0.0031 &  0.0043 & & -0.0034 & -0.0045 & -0.0058 & -0.0072 & -0.0081 & -0.0085 & -0.0094\\
0733 &  4.7E-4 &  5.3E-4 &  8.9E-4 &  0.0015 &  0.0020 &  0.0031 &  0.0044 & & -0.0034 & -0.0045 & -0.0058 & -0.0072 & -0.0081 & -0.0085 & -0.0095\\
0734 &  4.5E-4 &  5.2E-4 &  8.7E-4 &  0.0014 &  0.0020 &  0.0031 &  0.0044 & & -0.0034 & -0.0045 & -0.0059 & -0.0072 & -0.0081 & -0.0086 & -0.0096\\
0735 &  4.3E-4 &  5.1E-4 &  8.9E-4 &  0.0014 &  0.0020 &  0.0031 &  0.0043 & & -0.0034 & -0.0045 & -0.0059 & -0.0072 & -0.0081 & -0.0086 & -0.0097\\
0736 &  4.4E-4 &  5.2E-4 &  8.8E-4 &  0.0014 &  0.0020 &  0.0031 &  0.0044 & & -0.0034 & -0.0045 & -0.0059 & -0.0072 & -0.0081 & -0.0086 & -0.0098\\
0737 &  4.2E-4 &  5.1E-4 &  8.6E-4 &  0.0014 &  0.0020 &  0.0031 &  0.0044 & & -0.0034 & -0.0045 & -0.0059 & -0.0073 & -0.0081 & -0.0087 & -0.0098\\
0738 &  4.0E-4 &  4.9E-4 &  8.8E-4 &  0.0013 &  0.0020 &  0.0031 &  0.0043 & & -0.0034 & -0.0045 & -0.0059 & -0.0073 & -0.0081 & -0.0087 & -0.0099\\
0739 &  4.1E-4 &  5.0E-4 &  8.7E-4 &  0.0013 &  0.0020 &  0.0031 &  0.0044 & & -0.0034 & -0.0045 & -0.0059 & -0.0073 & -0.0081 & -0.0088 & -0.0100\\
0740 &  4.0E-4 &  4.8E-4 &  8.5E-4 &  0.0013 &  0.0020 &  0.0031 &  0.0044 & & -0.0034 & -0.0045 & -0.0059 & -0.0073 & -0.0081 & -0.0088 & -0.0101\\
0741 &  3.8E-4 &  4.7E-4 &  8.7E-4 &  0.0013 &  0.0019 &  0.0031 &  0.0043 & & -0.0034 & -0.0045 & -0.0059 & -0.0073 & -0.0081 & -0.0089 & -0.0102\\
0742 &  3.9E-4 &  4.7E-4 &  8.6E-4 &  0.0013 &  0.0019 &  0.0031 &  0.0044 & & -0.0034 & -0.0045 & -0.0060 & -0.0073 & -0.0081 & -0.0089 & -0.0102\\
0743 &  3.8E-4 &  4.6E-4 &  8.3E-4 &  0.0013 &  0.0019 &  0.0031 &  0.0043 & & -0.0034 & -0.0045 & -0.0060 & -0.0073 & -0.0081 & -0.0090 & -0.0103\\
0744 &  3.7E-4 &  4.4E-4 &  8.5E-4 &  0.0013 &  0.0019 &  0.0031 &  0.0043 & & -0.0034 & -0.0045 & -0.0060 & -0.0073 & -0.0081 & -0.0090 & -0.0104\\
0745 &  3.7E-4 &  4.4E-4 &  8.4E-4 &  0.0013 &  0.0019 &  0.0031 &  0.0043 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0081 & -0.0091 & -0.0105\\
0746 &  3.8E-4 &  4.2E-4 &  8.1E-4 &  0.0012 &  0.0019 &  0.0031 &  0.0043 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0082 & -0.0091 & -0.0105\\
0747 &  3.6E-4 &  4.0E-4 &  8.2E-4 &  0.0012 &  0.0019 &  0.0031 &  0.0042 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0082 & -0.0092 & -0.0106\\
0748 &  3.6E-4 &  4.0E-4 &  8.2E-4 &  0.0012 &  0.0019 &  0.0031 &  0.0043 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0082 & -0.0092 & -0.0107\\
0749 &  3.7E-4 &  3.9E-4 &  7.9E-4 &  0.0012 &  0.0019 &  0.0031 &  0.0043 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0082 & -0.0093 & -0.0107\\
0750 &  3.5E-4 &  3.7E-4 &  8.0E-4 &  0.0012 &  0.0019 &  0.0031 &  0.0042 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0082 & -0.0093 & -0.0108\\
0751 &  3.5E-4 &  3.8E-4 &  8.0E-4 &  0.0012 &  0.0019 &  0.0031 &  0.0042 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0082 & -0.0094 & -0.0109\\
0752 &  3.6E-4 &  3.7E-4 &  7.7E-4 &  0.0012 &  0.0019 &  0.0031 &  0.0042 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0082 & -0.0094 & -0.0109\\
0753 &  3.3E-4 &  3.5E-4 &  7.8E-4 &  0.0011 &  0.0019 &  0.0031 &  0.0041 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0082 & -0.0095 & -0.0110\\
0754 &  3.2E-4 &  3.6E-4 &  7.7E-4 &  0.0011 &  0.0019 &  0.0031 &  0.0041 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0083 & -0.0096 & -0.0110\\
0755 &  3.3E-4 &  3.6E-4 &  7.6E-4 &  0.0011 &  0.0020 &  0.0031 &  0.0041 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0083 & -0.0096 & -0.0111\\
0756 &  3.0E-4 &  3.4E-4 &  7.5E-4 &  0.0011 &  0.0020 &  0.0031 &  0.0040 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0083 & -0.0097 & -0.0111\\
0757 &  2.9E-4 &  3.5E-4 &  7.5E-4 &  0.0011 &  0.0020 &  0.0031 &  0.0041 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0083 & -0.0097 & -0.0112\\
0758 &  2.8E-4 &  3.5E-4 &  7.5E-4 &  0.0011 &  0.0020 &  0.0030 &  0.0041 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0083 & -0.0098 & -0.0112\\
0759 &  2.7E-4 &  3.4E-4 &  7.3E-4 &  0.0011 &  0.0020 &  0.0030 &  0.0040 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0084 & -0.0098 & -0.0113\\
0760 &  2.4E-4 &  3.5E-4 &  7.3E-4 &  0.0011 &  0.0021 &  0.0030 &  0.0040 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0084 & -0.0099 & -0.0113\\
0761 &  2.3E-4 &  3.6E-4 &  7.3E-4 &  0.0011 &  0.0021 &  0.0030 &  0.0040 & & -0.0033 & -0.0045 & -0.0060 & -0.0073 & -0.0084 & -0.0099 & -0.0114\\
0762 &  2.2E-4 &  3.5E-4 &  7.1E-4 &  0.0011 &  0.0021 &  0.0029 &  0.0039 & & -0.0032 & -0.0045 & -0.0060 & -0.0073 & -0.0085 & -0.0100 & -0.0114\\
0763 &  2.0E-4 &  3.6E-4 &  7.1E-4 &  0.0011 &  0.0021 &  0.0030 &  0.0040 & & -0.0032 & -0.0045 & -0.0060 & -0.0073 & -0.0085 & -0.0100 & -0.0114\\
0764 &  1.9E-4 &  3.7E-4 &  7.1E-4 &  0.0011 &  0.0021 &  0.0029 &  0.0040 & & -0.0032 & -0.0045 & -0.0060 & -0.0073 & -0.0085 & -0.0101 & -0.0115\\
0765 &  1.8E-4 &  3.6E-4 &  7.0E-4 &  0.0011 &  0.0021 &  0.0028 &  0.0039 & & -0.0032 & -0.0045 & -0.0060 & -0.0073 & -0.0086 & -0.0101 & -0.0115\\
0766 &  1.5E-4 &  3.7E-4 &  6.9E-4 &  0.0011 &  0.0021 &  0.0029 &  0.0039 & & -0.0032 & -0.0045 & -0.0060 & -0.0073 & -0.0086 & -0.0102 & -0.0115\\
0767 &  1.5E-4 &  3.8E-4 &  6.8E-4 &  0.0011 &  0.0021 &  0.0028 &  0.0040 & & -0.0032 & -0.0045 & -0.0060 & -0.0073 & -0.0086 & -0.0102 & -0.0115\\
0768 &  1.3E-4 &  3.7E-4 &  6.8E-4 &  0.0011 &  0.0021 &  0.0028 &  0.0039 & & -0.0032 & -0.0045 & -0.0060 & -0.0073 & -0.0087 & -0.0102 & -0.0116\\
0769 &  1.2E-4 &  3.8E-4 &  6.6E-4 &  0.0011 &  0.0021 &  0.0028 &  0.0039 & & -0.0032 & -0.0045 & -0.0060 & -0.0073 & -0.0087 & -0.0103 & -0.0116\\
0770 &  1.1E-4 &  4.0E-4 &  6.7E-4 &  0.0012 &  0.0021 &  0.0027 &  0.0040 & & -0.0032 & -0.0045 & -0.0061 & -0.0074 & -0.0087 & -0.0103 & -0.0116\\
0771 &  1.1E-4 &  3.8E-4 &  6.6E-4 &  0.0012 &  0.0021 &  0.0026 &  0.0038 & & -0.0032 & -0.0045 & -0.0061 & -0.0074 & -0.0088 & -0.0104 & -0.0116\\
0772 &  1.0E-4 &  3.9E-4 &  6.5E-4 &  0.0012 &  0.0021 &  0.0027 &  0.0039 & & -0.0032 & -0.0045 & -0.0061 & -0.0074 & -0.0088 & -0.0104 & -0.0116\\
0773 &  8.3E-5 &  4.1E-4 &  6.6E-4 &  0.0012 &  0.0021 &  0.0026 &  0.0039 & & -0.0032 & -0.0045 & -0.0061 & -0.0074 & -0.0088 & -0.0104 & -0.0117\\
0774 &  8.7E-5 &  3.9E-4 &  6.5E-4 &  0.0012 &  0.0021 &  0.0026 &  0.0038 & & -0.0032 & -0.0045 & -0.0061 & -0.0074 & -0.0089 & -0.0105 & -0.0117\\
0775 &  8.8E-5 &  4.0E-4 &  6.3E-4 &  0.0012 &  0.0021 &  0.0026 &  0.0038 & & -0.0032 & -0.0045 & -0.0061 & -0.0074 & -0.0089 & -0.0105 & -0.0117\\
0776 &  7.5E-5 &  4.2E-4 &  6.5E-4 &  0.0012 &  0.0021 &  0.0025 &  0.0039 & & -0.0032 & -0.0045 & -0.0061 & -0.0074 & -0.0089 & -0.0105 & -0.0117\\
0777 &  8.0E-5 &  4.0E-4 &  6.3E-4 &  0.0013 &  0.0020 &  0.0025 &  0.0038 & & -0.0031 & -0.0045 & -0.0061 & -0.0074 & -0.0090 & -0.0105 & -0.0117\\
0778 &  8.9E-5 &  4.1E-4 &  6.3E-4 &  0.0013 &  0.0020 &  0.0025 &  0.0038 & & -0.0031 & -0.0045 & -0.0061 & -0.0074 & -0.0090 & -0.0106 & -0.0118\\
0779 &  8.3E-5 &  4.2E-4 &  6.4E-4 &  0.0013 &  0.0020 &  0.0025 &  0.0038 & & -0.0031 & -0.0045 & -0.0061 & -0.0075 & -0.0090 & -0.0106 & -0.0118\\
0780 &  9.0E-5 &  4.1E-4 &  6.3E-4 &  0.0013 &  0.0020 &  0.0024 &  0.0037 & & -0.0031 & -0.0045 & -0.0061 & -0.0075 & -0.0090 & -0.0106 & -0.0118\\
0781 &  9.4E-5 &  4.1E-4 &  6.2E-4 &  0.0013 &  0.0020 &  0.0025 &  0.0037 & & -0.0031 & -0.0045 & -0.0061 & -0.0075 & -0.0091 & -0.0106 & -0.0118\\
0782 &  1.0E-4 &  4.3E-4 &  6.3E-4 &  0.0013 &  0.0019 &  0.0024 &  0.0038 & & -0.0031 & -0.0045 & -0.0061 & -0.0075 & -0.0091 & -0.0106 & -0.0119\\
0783 &  1.1E-4 &  4.1E-4 &  6.2E-4 &  0.0013 &  0.0019 &  0.0024 &  0.0036 & & -0.0031 & -0.0045 & -0.0061 & -0.0075 & -0.0091 & -0.0106 & -0.0119\\
0784 &  1.1E-4 &  4.1E-4 &  6.2E-4 &  0.0013 &  0.0019 &  0.0024 &  0.0036 & & -0.0031 & -0.0045 & -0.0061 & -0.0075 & -0.0092 & -0.0107 & -0.0119\\
0785 &  1.3E-4 &  4.3E-4 &  6.3E-4 &  0.0014 &  0.0019 &  0.0024 &  0.0037 & & -0.0031 & -0.0046 & -0.0061 & -0.0076 & -0.0092 & -0.0107 & -0.0119\\
0786 &  1.4E-4 &  4.1E-4 &  6.4E-4 &  0.0014 &  0.0018 &  0.0024 &  0.0035 & & -0.0031 & -0.0046 & -0.0062 & -0.0076 & -0.0092 & -0.0107 & -0.0120\\
0787 &  1.4E-4 &  4.1E-4 &  6.3E-4 &  0.0014 &  0.0018 &  0.0024 &  0.0035 & & -0.0031 & -0.0046 & -0.0062 & -0.0076 & -0.0092 & -0.0107 & -0.0120\\
0788 &  1.5E-4 &  4.2E-4 &  6.4E-4 &  0.0014 &  0.0018 &  0.0024 &  0.0036 & & -0.0031 & -0.0046 & -0.0062 & -0.0076 & -0.0092 & -0.0107 & -0.0120\\
0789 &  1.7E-4 &  4.0E-4 &  6.6E-4 &  0.0014 &  0.0017 &  0.0024 &  0.0035 & & -0.0031 & -0.0046 & -0.0062 & -0.0076 & -0.0093 & -0.0107 & -0.0120\\
0790 &  1.7E-4 &  4.0E-4 &  6.5E-4 &  0.0014 &  0.0017 &  0.0024 &  0.0034 & & -0.0031 & -0.0046 & -0.0062 & -0.0076 & -0.0093 & -0.0107 & -0.0121\\
0791 &  1.8E-4 &  4.2E-4 &  6.7E-4 &  0.0014 &  0.0017 &  0.0024 &  0.0035 & & -0.0031 & -0.0046 & -0.0062 & -0.0077 & -0.0093 & -0.0107 & -0.0121\\
0792 &  2.0E-4 &  4.0E-4 &  6.9E-4 &  0.0014 &  0.0016 &  0.0024 &  0.0034 & & -0.0031 & -0.0046 & -0.0062 & -0.0077 & -0.0093 & -0.0107 & -0.0121\\
0793 &  2.0E-4 &  4.0E-4 &  6.8E-4 &  0.0013 &  0.0016 &  0.0024 &  0.0034 & & -0.0031 & -0.0046 & -0.0062 & -0.0077 & -0.0093 & -0.0108 & -0.0122\\
0794 &  1.9E-4 &  4.2E-4 &  7.0E-4 &  0.0014 &  0.0016 &  0.0024 &  0.0035 & & -0.0031 & -0.0047 & -0.0062 & -0.0077 & -0.0093 & -0.0108 & -0.0122\\
0795 &  2.3E-4 &  3.9E-4 &  7.2E-4 &  0.0014 &  0.0015 &  0.0024 &  0.0033 & & -0.0031 & -0.0047 & -0.0062 & -0.0077 & -0.0093 & -0.0108 & -0.0122\\
0796 &  2.2E-4 &  3.9E-4 &  7.1E-4 &  0.0013 &  0.0015 &  0.0024 &  0.0033 & & -0.0031 & -0.0047 & -0.0062 & -0.0077 & -0.0094 & -0.0108 & -0.0122\\
0797 &  2.1E-4 &  4.1E-4 &  7.3E-4 &  0.0013 &  0.0015 &  0.0024 &  0.0034 & & -0.0031 & -0.0047 & -0.0062 & -0.0078 & -0.0094 & -0.0108 & -0.0123\\
0798 &  2.5E-4 &  3.9E-4 &  7.5E-4 &  0.0013 &  0.0015 &  0.0024 &  0.0032 & & -0.0031 & -0.0047 & -0.0062 & -0.0078 & -0.0094 & -0.0108 & -0.0123\\
0799 &  2.5E-4 &  3.9E-4 &  7.5E-4 &  0.0013 &  0.0015 &  0.0024 &  0.0032 & & -0.0031 & -0.0047 & -0.0062 & -0.0078 & -0.0094 & -0.0108 & -0.0123\\
0800 &  2.4E-4 &  4.1E-4 &  7.6E-4 &  0.0013 &  0.0015 &  0.0024 &  0.0033 & & -0.0031 & -0.0047 & -0.0062 & -0.0078 & -0.0094 & -0.0108 & -0.0123\\
0801 &  2.6E-4 &  3.8E-4 &  7.8E-4 &  0.0013 &  0.0014 &  0.0024 &  0.0031 & & -0.0031 & -0.0048 & -0.0062 & -0.0078 & -0.0094 & -0.0108 & -0.0124\\
0802 &  2.6E-4 &  3.8E-4 &  7.8E-4 &  0.0012 &  0.0014 &  0.0024 &  0.0031 & & -0.0032 & -0.0048 & -0.0063 & -0.0078 & -0.0094 & -0.0108 & -0.0124\\
0803 &  2.5E-4 &  3.9E-4 &  7.8E-4 &  0.0012 &  0.0014 &  0.0024 &  0.0032 & & -0.0032 & -0.0048 & -0.0063 & -0.0078 & -0.0094 & -0.0108 & -0.0124\\
0804 &  2.6E-4 &  3.7E-4 &  8.1E-4 &  0.0012 &  0.0014 &  0.0024 &  0.0030 & & -0.0032 & -0.0048 & -0.0063 & -0.0078 & -0.0094 & -0.0109 & -0.0124\\
0805 &  2.8E-4 &  3.7E-4 &  8.1E-4 &  0.0012 &  0.0014 &  0.0024 &  0.0030 & & -0.0032 & -0.0048 & -0.0063 & -0.0078 & -0.0094 & -0.0109 & -0.0124\\
0806 &  2.6E-4 &  3.8E-4 &  8.1E-4 &  0.0012 &  0.0014 &  0.0024 &  0.0031 & & -0.0032 & -0.0048 & -0.0063 & -0.0078 & -0.0094 & -0.0109 & -0.0125\\
0807 &  2.7E-4 &  3.6E-4 &  8.3E-4 &  0.0012 &  0.0014 &  0.0024 &  0.0029 & & -0.0032 & -0.0048 & -0.0063 & -0.0079 & -0.0094 & -0.0109 & -0.0125\\
0808 &  2.8E-4 &  3.6E-4 &  8.4E-4 &  0.0011 &  0.0014 &  0.0024 &  0.0028 & & -0.0032 & -0.0048 & -0.0063 & -0.0079 & -0.0094 & -0.0109 & -0.0125\\
0809 &  2.7E-4 &  3.8E-4 &  8.3E-4 &  0.0011 &  0.0014 &  0.0024 &  0.0029 & & -0.0032 & -0.0048 & -0.0063 & -0.0079 & -0.0094 & -0.0109 & -0.0125\\
0810 &  2.8E-4 &  3.6E-4 &  8.4E-4 &  0.0011 &  0.0014 &  0.0024 &  0.0028 & & -0.0033 & -0.0048 & -0.0063 & -0.0079 & -0.0094 & -0.0109 & -0.0125\\
0811 &  2.8E-4 &  3.6E-4 &  8.6E-4 &  0.0010 &  0.0014 &  0.0024 &  0.0027 & & -0.0033 & -0.0048 & -0.0063 & -0.0079 & -0.0094 & -0.0110 & -0.0125\\
0812 &  2.8E-4 &  3.8E-4 &  8.6E-4 &  0.0010 &  0.0015 &  0.0024 &  0.0028 & & -0.0033 & -0.0049 & -0.0063 & -0.0079 & -0.0094 & -0.0110 & -0.0125\\
0813 &  2.7E-4 &  3.7E-4 &  8.5E-4 &  0.0010 &  0.0014 &  0.0024 &  0.0027 & & -0.0033 & -0.0049 & -0.0063 & -0.0079 & -0.0094 & -0.0110 & -0.0125\\
0814 &  2.9E-4 &  3.7E-4 &  8.7E-4 &  9.7E-4 &  0.0015 &  0.0024 &  0.0026 & & -0.0033 & -0.0049 & -0.0063 & -0.0079 & -0.0094 & -0.0110 & -0.0126\\
0815 &  2.8E-4 &  3.9E-4 &  8.7E-4 &  9.8E-4 &  0.0015 &  0.0024 &  0.0027 & & -0.0033 & -0.0049 & -0.0063 & -0.0079 & -0.0094 & -0.0110 & -0.0126\\
0816 &  2.8E-4 &  3.8E-4 &  8.5E-4 &  9.6E-4 &  0.0015 &  0.0024 &  0.0026 & & -0.0034 & -0.0049 & -0.0063 & -0.0079 & -0.0094 & -0.0110 & -0.0126\\
0817 &  2.9E-4 &  3.8E-4 &  8.7E-4 &  9.1E-4 &  0.0015 &  0.0024 &  0.0025 & & -0.0034 & -0.0049 & -0.0063 & -0.0079 & -0.0094 & -0.0110 & -0.0126\\
0818 &  2.8E-4 &  4.0E-4 &  8.7E-4 &  9.2E-4 &  0.0015 &  0.0024 &  0.0026 & & -0.0034 & -0.0049 & -0.0063 & -0.0079 & -0.0094 & -0.0110 & -0.0126\\
0819 &  2.7E-4 &  3.9E-4 &  8.5E-4 &  9.1E-4 &  0.0015 &  0.0025 &  0.0025 & & -0.0034 & -0.0049 & -0.0063 & -0.0079 & -0.0094 & -0.0110 & -0.0126\\
0820 &  2.8E-4 &  3.9E-4 &  8.6E-4 &  8.6E-4 &  0.0016 &  0.0024 &  0.0024 & & -0.0034 & -0.0049 & -0.0063 & -0.0079 & -0.0094 & -0.0110 & -0.0126\\
0821 &  2.8E-4 &  4.1E-4 &  8.6E-4 &  8.8E-4 &  0.0016 &  0.0024 &  0.0025 & & -0.0034 & -0.0049 & -0.0063 & -0.0079 & -0.0094 & -0.0110 & -0.0126\\
0822 &  2.6E-4 &  4.0E-4 &  8.3E-4 &  8.7E-4 &  0.0016 &  0.0025 &  0.0024 & & -0.0034 & -0.0049 & -0.0063 & -0.0079 & -0.0094 & -0.0110 & -0.0126\\
0823 &  2.7E-4 &  4.0E-4 &  8.4E-4 &  8.3E-4 &  0.0016 &  0.0024 &  0.0024 & & -0.0035 & -0.0049 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0126\\
0824 &  2.7E-4 &  4.2E-4 &  8.4E-4 &  8.6E-4 &  0.0016 &  0.0024 &  0.0025 & & -0.0035 & -0.0049 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0126\\
0825 &  2.4E-4 &  4.2E-4 &  8.0E-4 &  8.5E-4 &  0.0016 &  0.0025 &  0.0024 & & -0.0035 & -0.0049 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0126\\
0826 &  2.5E-4 &  4.2E-4 &  8.1E-4 &  8.2E-4 &  0.0016 &  0.0024 &  0.0024 & & -0.0035 & -0.0049 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0126\\
0827 &  2.4E-4 &  4.4E-4 &  8.1E-4 &  8.5E-4 &  0.0016 &  0.0024 &  0.0025 & & -0.0035 & -0.0049 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0126\\
0828 &  2.2E-4 &  4.4E-4 &  7.7E-4 &  8.6E-4 &  0.0016 &  0.0024 &  0.0024 & & -0.0035 & -0.0049 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0126\\
0829 &  2.3E-4 &  4.5E-4 &  7.7E-4 &  8.3E-4 &  0.0016 &  0.0024 &  0.0024 & & -0.0035 & -0.0049 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0126\\
0830 &  2.2E-4 &  4.8E-4 &  7.7E-4 &  8.6E-4 &  0.0016 &  0.0024 &  0.0025 & & -0.0035 & -0.0049 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0125\\
0831 &  2.1E-4 &  4.8E-4 &  7.3E-4 &  8.8E-4 &  0.0016 &  0.0024 &  0.0025 & & -0.0035 & -0.0049 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0125\\
0832 &  2.1E-4 &  4.9E-4 &  7.3E-4 &  8.6E-4 &  0.0016 &  0.0024 &  0.0024 & & -0.0035 & -0.0049 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0125\\
0833 &  2.0E-4 &  5.1E-4 &  7.2E-4 &  8.9E-4 &  0.0017 &  0.0024 &  0.0025 & & -0.0035 & -0.0049 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0125\\
0834 &  1.9E-4 &  5.2E-4 &  6.9E-4 &  9.2E-4 &  0.0017 &  0.0024 &  0.0025 & & -0.0035 & -0.0048 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0125\\
0835 &  2.0E-4 &  5.3E-4 &  6.9E-4 &  9.0E-4 &  0.0017 &  0.0023 &  0.0025 & & -0.0035 & -0.0048 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0125\\
0836 &  1.9E-4 &  5.5E-4 &  6.8E-4 &  9.3E-4 &  0.0017 &  0.0023 &  0.0026 & & -0.0035 & -0.0048 & -0.0063 & -0.0078 & -0.0094 & -0.0110 & -0.0125\\
0837 &  1.8E-4 &  5.6E-4 &  6.5E-4 &  9.5E-4 &  0.0017 &  0.0023 &  0.0026 & & -0.0035 & -0.0048 & -0.0062 & -0.0077 & -0.0094 & -0.0110 & -0.0125\\
0838 &  1.9E-4 &  5.6E-4 &  6.5E-4 &  9.4E-4 &  0.0017 &  0.0023 &  0.0025 & & -0.0035 & -0.0048 & -0.0062 & -0.0077 & -0.0094 & -0.0110 & -0.0124\\
0839 &  1.8E-4 &  5.8E-4 &  6.4E-4 &  9.6E-4 &  0.0018 &  0.0023 &  0.0026 & & -0.0035 & -0.0048 & -0.0062 & -0.0077 & -0.0094 & -0.0109 & -0.0124\\
0840 &  1.7E-4 &  5.8E-4 &  6.3E-4 &  9.7E-4 &  0.0018 &  0.0023 &  0.0026 & & -0.0035 & -0.0048 & -0.0062 & -0.0077 & -0.0094 & -0.0109 & -0.0124\\
0841 &  1.8E-4 &  5.8E-4 &  6.0E-4 &  9.9E-4 &  0.0018 &  0.0023 &  0.0025 & & -0.0035 & -0.0048 & -0.0062 & -0.0077 & -0.0094 & -0.0109 & -0.0124\\
0842 &  1.8E-4 &  6.0E-4 &  6.1E-4 &  9.8E-4 &  0.0018 &  0.0023 &  0.0027 & & -0.0035 & -0.0048 & -0.0062 & -0.0077 & -0.0094 & -0.0109 & -0.0124\\
0843 &  1.7E-4 &  6.0E-4 &  6.0E-4 &  1.0E-3 &  0.0018 &  0.0023 &  0.0026 & & -0.0035 & -0.0048 & -0.0062 & -0.0077 & -0.0094 & -0.0109 & -0.0124\\
0844 &  1.8E-4 &  6.0E-4 &  5.8E-4 &  0.0010 &  0.0018 &  0.0023 &  0.0026 & & -0.0035 & -0.0048 & -0.0062 & -0.0077 & -0.0094 & -0.0109 & -0.0123\\
0845 &  1.9E-4 &  6.1E-4 &  5.9E-4 &  1.0E-3 &  0.0018 &  0.0023 &  0.0027 & & -0.0035 & -0.0048 & -0.0062 & -0.0077 & -0.0093 & -0.0108 & -0.0123\\
0846 &  1.7E-4 &  6.1E-4 &  5.8E-4 &  0.0010 &  0.0018 &  0.0023 &  0.0027 & & -0.0035 & -0.0048 & -0.0062 & -0.0077 & -0.0093 & -0.0108 & -0.0123\\
0847 &  1.9E-4 &  6.0E-4 &  5.7E-4 &  0.0010 &  0.0019 &  0.0023 &  0.0026 & & -0.0035 & -0.0048 & -0.0062 & -0.0077 & -0.0093 & -0.0108 & -0.0123\\
0848 &  2.1E-4 &  6.1E-4 &  5.8E-4 &  0.0010 &  0.0019 &  0.0023 &  0.0027 & & -0.0035 & -0.0048 & -0.0061 & -0.0077 & -0.0093 & -0.0108 & -0.0122\\
0849 &  2.0E-4 &  6.1E-4 &  5.7E-4 &  0.0010 &  0.0019 &  0.0023 &  0.0027 & & -0.0035 & -0.0048 & -0.0061 & -0.0077 & -0.0093 & -0.0108 & -0.0122\\
0850 &  2.2E-4 &  6.0E-4 &  5.7E-4 &  0.0010 &  0.0019 &  0.0023 &  0.0027 & & -0.0035 & -0.0047 & -0.0061 & -0.0077 & -0.0093 & -0.0107 & -0.0122\\
0851 &  2.4E-4 &  6.1E-4 &  5.8E-4 &  0.0010 &  0.0019 &  0.0023 &  0.0028 & & -0.0035 & -0.0047 & -0.0061 & -0.0077 & -0.0093 & -0.0107 & -0.0122\\
0852 &  2.6E-4 &  6.0E-4 &  5.8E-4 &  0.0010 &  0.0019 &  0.0023 &  0.0028 & & -0.0035 & -0.0047 & -0.0061 & -0.0076 & -0.0093 & -0.0107 & -0.0121\\
0853 &  2.6E-4 &  5.9E-4 &  5.8E-4 &  0.0011 &  0.0019 &  0.0023 &  0.0027 & & -0.0035 & -0.0047 & -0.0061 & -0.0076 & -0.0092 & -0.0107 & -0.0121\\
0854 &  2.8E-4 &  5.9E-4 &  5.9E-4 &  0.0011 &  0.0019 &  0.0023 &  0.0028 & & -0.0035 & -0.0047 & -0.0061 & -0.0076 & -0.0092 & -0.0106 & -0.0121\\
0855 &  3.1E-4 &  5.8E-4 &  5.9E-4 &  0.0011 &  0.0019 &  0.0023 &  0.0029 & & -0.0035 & -0.0047 & -0.0061 & -0.0076 & -0.0092 & -0.0106 & -0.0120\\
0856 &  3.1E-4 &  5.6E-4 &  5.9E-4 &  0.0011 &  0.0019 &  0.0022 &  0.0028 & & -0.0035 & -0.0047 & -0.0060 & -0.0076 & -0.0092 & -0.0106 & -0.0120\\
0857 &  3.3E-4 &  5.6E-4 &  6.0E-4 &  0.0011 &  0.0019 &  0.0022 &  0.0029 & & -0.0035 & -0.0047 & -0.0060 & -0.0076 & -0.0092 & -0.0106 & -0.0120\\
0858 &  3.6E-4 &  5.5E-4 &  6.1E-4 &  0.0011 &  0.0019 &  0.0022 &  0.0029 & & -0.0034 & -0.0047 & -0.0060 & -0.0076 & -0.0092 & -0.0105 & -0.0119\\
0859 &  3.6E-4 &  5.3E-4 &  6.0E-4 &  0.0012 &  0.0019 &  0.0022 &  0.0029 & & -0.0034 & -0.0047 & -0.0060 & -0.0076 & -0.0091 & -0.0105 & -0.0119\\
0860 &  3.8E-4 &  5.3E-4 &  6.1E-4 &  0.0012 &  0.0019 &  0.0022 &  0.0029 & & -0.0034 & -0.0046 & -0.0060 & -0.0076 & -0.0091 & -0.0105 & -0.0119\\
0861 &  4.1E-4 &  5.3E-4 &  6.2E-4 &  0.0012 &  0.0019 &  0.0022 &  0.0030 & & -0.0034 & -0.0046 & -0.0060 & -0.0076 & -0.0091 & -0.0105 & -0.0118\\
0862 &  4.0E-4 &  5.1E-4 &  6.1E-4 &  0.0012 &  0.0019 &  0.0022 &  0.0029 & & -0.0034 & -0.0046 & -0.0060 & -0.0075 & -0.0091 & -0.0105 & -0.0118\\
0863 &  4.2E-4 &  5.1E-4 &  6.2E-4 &  0.0012 &  0.0019 &  0.0022 &  0.0030 & & -0.0034 & -0.0046 & -0.0060 & -0.0075 & -0.0091 & -0.0104 & -0.0118\\
0864 &  4.3E-4 &  5.1E-4 &  6.2E-4 &  0.0012 &  0.0019 &  0.0021 &  0.0031 & & -0.0034 & -0.0046 & -0.0059 & -0.0075 & -0.0090 & -0.0104 & -0.0117\\
0865 &  4.4E-4 &  4.9E-4 &  6.2E-4 &  0.0013 &  0.0019 &  0.0021 &  0.0030 & & -0.0034 & -0.0046 & -0.0059 & -0.0075 & -0.0090 & -0.0104 & -0.0117\\
0866 &  4.5E-4 &  4.9E-4 &  6.2E-4 &  0.0013 &  0.0019 &  0.0021 &  0.0031 & & -0.0034 & -0.0046 & -0.0059 & -0.0075 & -0.0090 & -0.0104 & -0.0117\\
0867 &  4.6E-4 &  4.9E-4 &  6.2E-4 &  0.0013 &  0.0018 &  0.0021 &  0.0032 & & -0.0034 & -0.0046 & -0.0059 & -0.0075 & -0.0090 & -0.0103 & -0.0116\\
0868 &  4.7E-4 &  4.7E-4 &  6.3E-4 &  0.0013 &  0.0019 &  0.0021 &  0.0031 & & -0.0034 & -0.0045 & -0.0059 & -0.0075 & -0.0089 & -0.0103 & -0.0116\\
0869 &  4.7E-4 &  4.7E-4 &  6.1E-4 &  0.0013 &  0.0019 &  0.0021 &  0.0032 & & -0.0034 & -0.0045 & -0.0059 & -0.0075 & -0.0089 & -0.0103 & -0.0116\\
0870 &  4.8E-4 &  4.8E-4 &  6.1E-4 &  0.0013 &  0.0018 &  0.0020 &  0.0033 & & -0.0034 & -0.0045 & -0.0059 & -0.0074 & -0.0089 & -0.0103 & -0.0115\\
0871 &  4.9E-4 &  4.5E-4 &  6.2E-4 &  0.0013 &  0.0019 &  0.0020 &  0.0032 & & -0.0033 & -0.0045 & -0.0059 & -0.0074 & -0.0089 & -0.0103 & -0.0115\\
0872 &  4.8E-4 &  4.5E-4 &  6.0E-4 &  0.0013 &  0.0018 &  0.0020 &  0.0033 & & -0.0033 & -0.0045 & -0.0059 & -0.0074 & -0.0088 & -0.0102 & -0.0115\\
0873 &  4.9E-4 &  4.6E-4 &  6.0E-4 &  0.0013 &  0.0018 &  0.0019 &  0.0034 & & -0.0033 & -0.0045 & -0.0058 & -0.0074 & -0.0088 & -0.0102 & -0.0114\\
0874 &  4.9E-4 &  4.4E-4 &  6.2E-4 &  0.0013 &  0.0018 &  0.0019 &  0.0033 & & -0.0033 & -0.0045 & -0.0058 & -0.0074 & -0.0088 & -0.0102 & -0.0114\\
0875 &  4.8E-4 &  4.4E-4 &  6.1E-4 &  0.0013 &  0.0018 &  0.0019 &  0.0034 & & -0.0033 & -0.0045 & -0.0058 & -0.0074 & -0.0088 & -0.0102 & -0.0114\\
0876 &  4.8E-4 &  4.5E-4 &  6.0E-4 &  0.0013 &  0.0018 &  0.0018 &  0.0035 & & -0.0033 & -0.0044 & -0.0058 & -0.0073 & -0.0087 & -0.0101 & -0.0113\\
0877 &  4.7E-4 &  4.3E-4 &  6.3E-4 &  0.0013 &  0.0018 &  0.0019 &  0.0034 & & -0.0033 & -0.0044 & -0.0058 & -0.0073 & -0.0087 & -0.0101 & -0.0113\\
0878 &  4.7E-4 &  4.3E-4 &  6.3E-4 &  0.0013 &  0.0017 &  0.0018 &  0.0034 & & -0.0033 & -0.0044 & -0.0058 & -0.0073 & -0.0087 & -0.0101 & -0.0113\\
0879 &  4.7E-4 &  4.3E-4 &  6.2E-4 &  0.0013 &  0.0017 &  0.0018 &  0.0035 & & -0.0033 & -0.0044 & -0.0058 & -0.0073 & -0.0087 & -0.0101 & -0.0112\\
0880 &  4.5E-4 &  4.1E-4 &  6.5E-4 &  0.0013 &  0.0017 &  0.0017 &  0.0034 & & -0.0033 & -0.0044 & -0.0058 & -0.0073 & -0.0086 & -0.0100 & -0.0112\\
0881 &  4.5E-4 &  4.1E-4 &  6.5E-4 &  0.0013 &  0.0017 &  0.0018 &  0.0034 & & -0.0032 & -0.0044 & -0.0057 & -0.0073 & -0.0086 & -0.0100 & -0.0112\\
0882 &  4.5E-4 &  4.2E-4 &  6.5E-4 &  0.0013 &  0.0016 &  0.0017 &  0.0035 & & -0.0032 & -0.0044 & -0.0057 & -0.0072 & -0.0086 & -0.0100 & -0.0111\\
0883 &  4.4E-4 &  4.0E-4 &  6.8E-4 &  0.0013 &  0.0017 &  0.0017 &  0.0034 & & -0.0032 & -0.0043 & -0.0057 & -0.0072 & -0.0086 & -0.0099 & -0.0111\\
0884 &  4.4E-4 &  4.0E-4 &  6.8E-4 &  0.0013 &  0.0016 &  0.0017 &  0.0034 & & -0.0032 & -0.0043 & -0.0057 & -0.0072 & -0.0086 & -0.0099 & -0.0111\\
0885 &  4.3E-4 &  4.1E-4 &  6.9E-4 &  0.0013 &  0.0016 &  0.0016 &  0.0035 & & -0.0032 & -0.0043 & -0.0057 & -0.0072 & -0.0085 & -0.0099 & -0.0110\\
0886 &  4.2E-4 &  3.8E-4 &  7.1E-4 &  0.0013 &  0.0016 &  0.0016 &  0.0033 & & -0.0032 & -0.0043 & -0.0057 & -0.0072 & -0.0085 & -0.0098 & -0.0110\\
0887 &  4.2E-4 &  3.8E-4 &  7.0E-4 &  0.0013 &  0.0016 &  0.0016 &  0.0033 & & -0.0032 & -0.0043 & -0.0057 & -0.0071 & -0.0085 & -0.0098 & -0.0110\\
0888 &  4.2E-4 &  3.9E-4 &  7.2E-4 &  0.0013 &  0.0015 &  0.0016 &  0.0034 & & -0.0032 & -0.0043 & -0.0057 & -0.0071 & -0.0085 & -0.0098 & -0.0109\\
0889 &  4.1E-4 &  3.6E-4 &  7.4E-4 &  0.0013 &  0.0015 &  0.0016 &  0.0033 & & -0.0032 & -0.0042 & -0.0056 & -0.0071 & -0.0085 & -0.0097 & -0.0109\\
0890 &  4.0E-4 &  3.6E-4 &  7.3E-4 &  0.0013 &  0.0015 &  0.0016 &  0.0033 & & -0.0031 & -0.0042 & -0.0056 & -0.0071 & -0.0084 & -0.0097 & -0.0109\\
0891 &  4.1E-4 &  3.7E-4 &  7.4E-4 &  0.0012 &  0.0014 &  0.0015 &  0.0034 & & -0.0031 & -0.0042 & -0.0056 & -0.0071 & -0.0084 & -0.0097 & -0.0109\\
0892 &  3.9E-4 &  3.4E-4 &  7.5E-4 &  0.0013 &  0.0014 &  0.0015 &  0.0032 & & -0.0031 & -0.0042 & -0.0056 & -0.0070 & -0.0084 & -0.0097 & -0.0108\\
0893 &  3.8E-4 &  3.3E-4 &  7.4E-4 &  0.0012 &  0.0014 &  0.0015 &  0.0032 & & -0.0031 & -0.0042 & -0.0056 & -0.0070 & -0.0084 & -0.0096 & -0.0108\\
0894 &  3.8E-4 &  3.4E-4 &  7.5E-4 &  0.0012 &  0.0013 &  0.0015 &  0.0034 & & -0.0031 & -0.0042 & -0.0056 & -0.0070 & -0.0084 & -0.0096 & -0.0108\\
0895 &  3.7E-4 &  3.1E-4 &  7.5E-4 &  0.0012 &  0.0013 &  0.0015 &  0.0032 & & -0.0031 & -0.0042 & -0.0056 & -0.0070 & -0.0083 & -0.0096 & -0.0108\\
0896 &  3.5E-4 &  3.0E-4 &  7.4E-4 &  0.0012 &  0.0013 &  0.0015 &  0.0032 & & -0.0031 & -0.0041 & -0.0056 & -0.0070 & -0.0083 & -0.0095 & -0.0107\\
0897 &  3.5E-4 &  3.2E-4 &  7.5E-4 &  0.0012 &  0.0012 &  0.0015 &  0.0033 & & -0.0030 & -0.0041 & -0.0055 & -0.0069 & -0.0083 & -0.0095 & -0.0107\\
0898 &  3.5E-4 &  2.9E-4 &  7.4E-4 &  0.0012 &  0.0012 &  0.0015 &  0.0032 & & -0.0030 & -0.0041 & -0.0055 & -0.0069 & -0.0083 & -0.0095 & -0.0107\\
0899 &  3.3E-4 &  2.8E-4 &  7.4E-4 &  0.0012 &  0.0012 &  0.0015 &  0.0031 & & -0.0030 & -0.0041 & -0.0055 & -0.0069 & -0.0082 & -0.0095 & -0.0107\\
0900 &  3.2E-4 &  3.0E-4 &  7.3E-4 &  0.0011 &  0.0011 &  0.0015 &  0.0033 & & -0.0030 & -0.0041 & -0.0055 & -0.0069 & -0.0082 & -0.0094 & -0.0107\\
0901 &  3.3E-4 &  2.7E-4 &  7.3E-4 &  0.0012 &  0.0011 &  0.0014 &  0.0031 & & -0.0030 & -0.0041 & -0.0055 & -0.0069 & -0.0082 & -0.0094 & -0.0106\\
0902 &  3.1E-4 &  2.7E-4 &  7.2E-4 &  0.0011 &  0.0010 &  0.0014 &  0.0031 & & -0.0030 & -0.0041 & -0.0055 & -0.0068 & -0.0082 & -0.0094 & -0.0106\\
0903 &  2.9E-4 &  2.9E-4 &  7.2E-4 &  0.0011 &  9.7E-4 &  0.0014 &  0.0032 & & -0.0030 & -0.0041 & -0.0055 & -0.0068 & -0.0081 & -0.0094 & -0.0106\\
0904 &  3.1E-4 &  2.7E-4 &  7.1E-4 &  0.0011 &  9.7E-4 &  0.0014 &  0.0031 & & -0.0029 & -0.0040 & -0.0055 & -0.0068 & -0.0081 & -0.0094 & -0.0106\\
0905 &  2.9E-4 &  2.7E-4 &  7.1E-4 &  0.0011 &  9.4E-4 &  0.0014 &  0.0031 & & -0.0029 & -0.0040 & -0.0054 & -0.0068 & -0.0081 & -0.0094 & -0.0106\\
0906 &  2.6E-4 &  2.9E-4 &  7.0E-4 &  0.0011 &  8.7E-4 &  0.0013 &  0.0032 & & -0.0029 & -0.0040 & -0.0054 & -0.0068 & -0.0081 & -0.0093 & -0.0105\\
0907 &  2.8E-4 &  2.7E-4 &  6.9E-4 &  0.0011 &  8.7E-4 &  0.0013 &  0.0030 & & -0.0029 & -0.0040 & -0.0054 & -0.0068 & -0.0080 & -0.0093 & -0.0105\\
0908 &  2.6E-4 &  2.7E-4 &  6.9E-4 &  0.0011 &  8.5E-4 &  0.0013 &  0.0030 & & -0.0029 & -0.0040 & -0.0054 & -0.0067 & -0.0080 & -0.0093 & -0.0105\\
0909 &  2.4E-4 &  2.9E-4 &  6.8E-4 &  0.0010 &  7.9E-4 &  0.0013 &  0.0031 & & -0.0029 & -0.0040 & -0.0054 & -0.0067 & -0.0080 & -0.0093 & -0.0105\\
0910 &  2.5E-4 &  2.7E-4 &  6.7E-4 &  0.0010 &  7.9E-4 &  0.0013 &  0.0030 & & -0.0029 & -0.0040 & -0.0054 & -0.0067 & -0.0080 & -0.0093 & -0.0105\\
0911 &  2.4E-4 &  2.7E-4 &  6.7E-4 &  0.0010 &  7.8E-4 &  0.0013 &  0.0029 & & -0.0028 & -0.0040 & -0.0054 & -0.0067 & -0.0079 & -0.0093 & -0.0105\\
0912 &  2.1E-4 &  2.9E-4 &  6.6E-4 &  9.5E-4 &  7.3E-4 &  0.0013 &  0.0030 & & -0.0028 & -0.0039 & -0.0054 & -0.0067 & -0.0079 & -0.0093 & -0.0104\\
0913 &  2.1E-4 &  2.8E-4 &  6.4E-4 &  9.5E-4 &  7.3E-4 &  0.0012 &  0.0029 & & -0.0028 & -0.0039 & -0.0053 & -0.0066 & -0.0079 & -0.0093 & -0.0104\\
0914 &  2.1E-4 &  2.8E-4 &  6.5E-4 &  9.4E-4 &  7.3E-4 &  0.0013 &  0.0028 & & -0.0028 & -0.0039 & -0.0053 & -0.0066 & -0.0079 & -0.0093 & -0.0104\\
0915 &  1.8E-4 &  3.0E-4 &  6.4E-4 &  8.8E-4 &  6.9E-4 &  0.0013 &  0.0029 & & -0.0028 & -0.0039 & -0.0053 & -0.0066 & -0.0078 & -0.0093 & -0.0104\\
0916 &  1.8E-4 &  2.8E-4 &  6.2E-4 &  8.9E-4 &  6.9E-4 &  0.0013 &  0.0027 & & -0.0028 & -0.0039 & -0.0053 & -0.0066 & -0.0078 & -0.0093 & -0.0104\\
0917 &  1.7E-4 &  2.7E-4 &  6.3E-4 &  8.6E-4 &  7.0E-4 &  0.0013 &  0.0027 & & -0.0027 & -0.0039 & -0.0053 & -0.0066 & -0.0078 & -0.0093 & -0.0104\\
0918 &  1.5E-4 &  2.9E-4 &  6.3E-4 &  8.1E-4 &  6.6E-4 &  0.0013 &  0.0027 & & -0.0027 & -0.0039 & -0.0053 & -0.0066 & -0.0078 & -0.0093 & -0.0104\\
0919 &  1.4E-4 &  2.7E-4 &  6.1E-4 &  8.1E-4 &  6.7E-4 &  0.0013 &  0.0026 & & -0.0027 & -0.0039 & -0.0053 & -0.0065 & -0.0077 & -0.0093 & -0.0103\\
0920 &  1.3E-4 &  2.6E-4 &  6.1E-4 &  7.9E-4 &  6.8E-4 &  0.0014 &  0.0025 & & -0.0027 & -0.0039 & -0.0052 & -0.0065 & -0.0077 & -0.0093 & -0.0103\\
0921 &  1.1E-4 &  2.7E-4 &  6.2E-4 &  7.4E-4 &  6.4E-4 &  0.0014 &  0.0025 & & -0.0027 & -0.0039 & -0.0052 & -0.0065 & -0.0077 & -0.0093 & -0.0103\\
0922 &  1.1E-4 &  2.5E-4 &  6.0E-4 &  7.3E-4 &  6.5E-4 &  0.0015 &  0.0024 & & -0.0027 & -0.0039 & -0.0052 & -0.0065 & -0.0077 & -0.0093 & -0.0103\\
0923 &  9.5E-5 &  2.4E-4 &  6.0E-4 &  7.1E-4 &  6.6E-4 &  0.0015 &  0.0023 & & -0.0027 & -0.0038 & -0.0052 & -0.0064 & -0.0077 & -0.0093 & -0.0103\\
0924 &  7.6E-5 &  2.5E-4 &  6.1E-4 &  6.8E-4 &  6.4E-4 &  0.0016 &  0.0023 & & -0.0026 & -0.0038 & -0.0052 & -0.0064 & -0.0077 & -0.0093 & -0.0102\\
0925 &  8.0E-5 &  2.3E-4 &  5.9E-4 &  6.4E-4 &  6.4E-4 &  0.0016 &  0.0022 & & -0.0026 & -0.0038 & -0.0052 & -0.0064 & -0.0077 & -0.0093 & -0.0102\\
0926 &  6.7E-5 &  2.2E-4 &  5.8E-4 &  6.3E-4 &  6.2E-4 &  0.0016 &  0.0021 & & -0.0026 & -0.0038 & -0.0052 & -0.0064 & -0.0077 & -0.0093 & -0.0102\\
0927 &  4.6E-5 &  2.3E-4 &  5.9E-4 &  6.1E-4 &  6.1E-4 &  0.0017 &  0.0021 & & -0.0026 & -0.0038 & -0.0051 & -0.0064 & -0.0077 & -0.0093 & -0.0102\\
0928 &  5.6E-5 &  2.1E-4 &  5.8E-4 &  5.7E-4 &  6.2E-4 &  0.0018 &  0.0019 & & -0.0026 & -0.0038 & -0.0051 & -0.0063 & -0.0076 & -0.0093 & -0.0101\\
0929 &  4.5E-5 &  1.9E-4 &  5.6E-4 &  5.7E-4 &  5.9E-4 &  0.0018 &  0.0018 & & -0.0026 & -0.0038 & -0.0051 & -0.0063 & -0.0076 & -0.0093 & -0.0101\\
0930 &  2.8E-5 &  2.0E-4 &  5.8E-4 &  5.5E-4 &  6.0E-4 &  0.0019 &  0.0018 & & -0.0026 & -0.0038 & -0.0051 & -0.0063 & -0.0076 & -0.0093 & -0.0101\\
0931 &  3.8E-5 &  1.8E-4 &  5.7E-4 &  5.1E-4 &  6.2E-4 &  0.0019 &  0.0017 & & -0.0026 & -0.0038 & -0.0051 & -0.0063 & -0.0076 & -0.0093 & -0.0101\\
0932 &  3.0E-5 &  1.7E-4 &  5.5E-4 &  5.1E-4 &  5.9E-4 &  0.0020 &  0.0016 & & -0.0025 & -0.0038 & -0.0051 & -0.0062 & -0.0076 & -0.0093 & -0.0100\\
0933 &  2.9E-5 &  1.7E-4 &  5.6E-4 &  5.0E-4 &  6.0E-4 &  0.0021 &  0.0016 & & -0.0025 & -0.0038 & -0.0051 & -0.0062 & -0.0076 & -0.0093 & -0.0100\\
0934 &  1.2E-5 &  1.6E-4 &  5.6E-4 &  4.7E-4 &  6.2E-4 &  0.0021 &  0.0015 & & -0.0025 & -0.0038 & -0.0050 & -0.0062 & -0.0076 & -0.0093 & -0.0100\\
0935 &  1.7E-5 &  1.4E-4 &  5.3E-4 &  4.8E-4 &  6.0E-4 &  0.0022 &  0.0013 & & -0.0025 & -0.0038 & -0.0050 & -0.0062 & -0.0076 & -0.0093 & -0.0100\\
0936 &  1.5E-5 &  1.5E-4 &  5.4E-4 &  4.8E-4 &  6.1E-4 &  0.0023 &  0.0014 & & -0.0025 & -0.0038 & -0.0050 & -0.0062 & -0.0076 & -0.0092 & -0.0099\\
0937 &  1.1E-7 &  1.4E-4 &  5.4E-4 &  4.5E-4 &  6.4E-4 &  0.0024 &  0.0012 & & -0.0025 & -0.0038 & -0.0050 & -0.0061 & -0.0076 & -0.0092 & -0.0099\\
0938 &  1.2E-5 &  1.3E-4 &  5.1E-4 &  4.7E-4 &  6.3E-4 &  0.0024 &  0.0011 & & -0.0025 & -0.0038 & -0.0050 & -0.0061 & -0.0076 & -0.0092 & -0.0099\\
0939 &  5.0E-6 &  1.4E-4 &  5.2E-4 &  4.8E-4 &  6.5E-4 &  0.0025 &  0.0011 & & -0.0025 & -0.0038 & -0.0049 & -0.0061 & -0.0076 & -0.0092 & -0.0099\\
0940 &  5.3E-6 &  1.4E-4 &  5.1E-4 &  4.6E-4 &  7.0E-4 &  0.0026 &  0.0010 & & -0.0025 & -0.0038 & -0.0049 & -0.0061 & -0.0076 & -0.0092 & -0.0098\\
0941 &  1.4E-6 &  1.3E-4 &  4.8E-4 &  4.9E-4 &  6.9E-4 &  0.0026 &  9.2E-4 & & -0.0025 & -0.0038 & -0.0049 & -0.0061 & -0.0077 & -0.0092 & -0.0098\\
0942 &  6.4E-6 &  1.4E-4 &  5.0E-4 &  5.0E-4 &  7.2E-4 &  0.0027 &  9.6E-4 & & -0.0025 & -0.0037 & -0.0049 & -0.0061 & -0.0077 & -0.0092 & -0.0098\\
0943 &  1.8E-5 &  1.4E-4 &  4.9E-4 &  4.9E-4 &  7.8E-4 &  0.0028 &  8.8E-4 & & -0.0025 & -0.0037 & -0.0049 & -0.0060 & -0.0077 & -0.0092 & -0.0097\\
0944 &  1.7E-5 &  1.3E-4 &  4.6E-4 &  5.2E-4 &  7.8E-4 &  0.0028 &  7.7E-4 & & -0.0025 & -0.0037 & -0.0049 & -0.0060 & -0.0077 & -0.0091 & -0.0097\\
0945 &  2.4E-5 &  1.5E-4 &  4.7E-4 &  5.4E-4 &  8.2E-4 &  0.0029 &  8.1E-4 & & -0.0025 & -0.0037 & -0.0048 & -0.0060 & -0.0077 & -0.0091 & -0.0097\\
0946 &  3.9E-5 &  1.4E-4 &  4.6E-4 &  5.3E-4 &  8.8E-4 &  0.0030 &  7.6E-4 & & -0.0025 & -0.0037 & -0.0048 & -0.0060 & -0.0077 & -0.0091 & -0.0097\\
0947 &  3.5E-5 &  1.4E-4 &  4.3E-4 &  5.5E-4 &  8.9E-4 &  0.0030 &  6.6E-4 & & -0.0025 & -0.0037 & -0.0048 & -0.0060 & -0.0077 & -0.0091 & -0.0096\\
0948 &  4.3E-5 &  1.5E-4 &  4.4E-4 &  5.8E-4 &  9.3E-4 &  0.0032 &  7.1E-4 & & -0.0025 & -0.0037 & -0.0048 & -0.0060 & -0.0077 & -0.0090 & -0.0096\\
0949 &  6.7E-5 &  1.5E-4 &  4.3E-4 &  5.7E-4 &  1.0E-3 &  0.0032 &  6.9E-4 & & -0.0024 & -0.0037 & -0.0048 & -0.0060 & -0.0077 & -0.0090 & -0.0096\\
0950 &  6.4E-5 &  1.4E-4 &  4.1E-4 &  5.9E-4 &  0.0010 &  0.0033 &  6.0E-4 & & -0.0024 & -0.0037 & -0.0047 & -0.0060 & -0.0077 & -0.0090 & -0.0096\\
0951 &  6.8E-5 &  1.5E-4 &  4.1E-4 &  6.2E-4 &  0.0010 &  0.0034 &  6.7E-4 & & -0.0024 & -0.0037 & -0.0047 & -0.0060 & -0.0077 & -0.0090 & -0.0095\\
0952 &  9.3E-5 &  1.5E-4 &  4.0E-4 &  6.0E-4 &  0.0011 &  0.0035 &  6.7E-4 & & -0.0024 & -0.0036 & -0.0047 & -0.0060 & -0.0077 & -0.0089 & -0.0095\\
0953 &  9.1E-5 &  1.4E-4 &  3.9E-4 &  6.1E-4 &  0.0012 &  0.0036 &  5.9E-4 & & -0.0024 & -0.0036 & -0.0047 & -0.0060 & -0.0077 & -0.0089 & -0.0095\\
0954 &  9.2E-5 &  1.5E-4 &  3.8E-4 &  6.3E-4 &  0.0012 &  0.0037 &  6.6E-4 & & -0.0024 & -0.0036 & -0.0047 & -0.0060 & -0.0077 & -0.0089 & -0.0095\\
0955 &  1.2E-4 &  1.5E-4 &  3.8E-4 &  6.1E-4 &  0.0013 &  0.0037 &  6.9E-4 & & -0.0024 & -0.0036 & -0.0047 & -0.0060 & -0.0077 & -0.0088 & -0.0094\\
0956 &  1.2E-4 &  1.4E-4 &  3.7E-4 &  6.1E-4 &  0.0013 &  0.0038 &  6.1E-4 & & -0.0024 & -0.0036 & -0.0046 & -0.0060 & -0.0077 & -0.0088 & -0.0094\\
0957 &  1.1E-4 &  1.4E-4 &  3.6E-4 &  6.3E-4 &  0.0013 &  0.0040 &  6.9E-4 & & -0.0024 & -0.0036 & -0.0046 & -0.0059 & -0.0077 & -0.0088 & -0.0094\\
0958 &  1.4E-4 &  1.5E-4 &  3.7E-4 &  6.0E-4 &  0.0014 &  0.0040 &  7.2E-4 & & -0.0024 & -0.0036 & -0.0046 & -0.0059 & -0.0077 & -0.0088 & -0.0094\\
0959 &  1.4E-4 &  1.3E-4 &  3.7E-4 &  5.9E-4 &  0.0015 &  0.0042 &  6.4E-4 & & -0.0024 & -0.0035 & -0.0046 & -0.0059 & -0.0077 & -0.0087 & -0.0093\\
0960 &  1.3E-4 &  1.4E-4 &  3.7E-4 &  6.0E-4 &  0.0015 &  0.0043 &  7.2E-4 & & -0.0024 & -0.0035 & -0.0046 & -0.0059 & -0.0076 & -0.0087 & -0.0093\\
0961 &  1.4E-4 &  1.5E-4 &  3.8E-4 &  5.8E-4 &  0.0016 &  0.0044 &  7.7E-4 & & -0.0024 & -0.0035 & -0.0046 & -0.0059 & -0.0076 & -0.0087 & -0.0093\\
0962 &  1.5E-4 &  1.3E-4 &  4.0E-4 &  5.6E-4 &  0.0016 &  0.0045 &  6.9E-4 & & -0.0024 & -0.0035 & -0.0045 & -0.0059 & -0.0076 & -0.0086 & -0.0093\\
0963 &  1.4E-4 &  1.4E-4 &  4.0E-4 &  5.7E-4 &  0.0016 &  0.0046 &  7.7E-4 & & -0.0024 & -0.0035 & -0.0045 & -0.0059 & -0.0076 & -0.0086 & -0.0093\\
0964 &  1.4E-4 &  1.5E-4 &  4.2E-4 &  5.4E-4 &  0.0017 &  0.0048 &  8.3E-4 & & -0.0024 & -0.0035 & -0.0045 & -0.0059 & -0.0076 & -0.0086 & -0.0092\\
0965 &  1.5E-4 &  1.3E-4 &  4.5E-4 &  5.2E-4 &  0.0018 &  0.0048 &  7.5E-4 & & -0.0024 & -0.0035 & -0.0045 & -0.0059 & -0.0076 & -0.0086 & -0.0092\\
0966 &  1.4E-4 &  1.4E-4 &  4.5E-4 &  5.2E-4 &  0.0018 &  0.0049 &  8.3E-4 & & -0.0024 & -0.0034 & -0.0045 & -0.0059 & -0.0075 & -0.0085 & -0.0092\\
0967 &  1.4E-4 &  1.4E-4 &  4.7E-4 &  4.9E-4 &  0.0019 &  0.0050 &  9.0E-4 & & -0.0024 & -0.0034 & -0.0045 & -0.0059 & -0.0075 & -0.0085 & -0.0092\\
0968 &  1.5E-4 &  1.2E-4 &  5.0E-4 &  4.6E-4 &  0.0019 &  0.0050 &  8.2E-4 & & -0.0024 & -0.0034 & -0.0045 & -0.0059 & -0.0075 & -0.0085 & -0.0091\\
0969 &  1.5E-4 &  1.3E-4 &  5.1E-4 &  4.6E-4 &  0.0019 &  0.0050 &  8.9E-4 & & -0.0024 & -0.0034 & -0.0045 & -0.0059 & -0.0075 & -0.0085 & -0.0091\\
0970 &  1.5E-4 &  1.3E-4 &  5.3E-4 &  4.3E-4 &  0.0020 &  0.0050 &  9.8E-4 & & -0.0024 & -0.0034 & -0.0044 & -0.0059 & -0.0074 & -0.0084 & -0.0091\\
0971 &  1.6E-4 &  1.1E-4 &  5.7E-4 &  3.9E-4 &  0.0021 &  0.0050 &  8.9E-4 & & -0.0024 & -0.0034 & -0.0044 & -0.0059 & -0.0074 & -0.0084 & -0.0091\\
0972 &  1.6E-4 &  1.1E-4 &  5.8E-4 &  3.9E-4 &  0.0021 &  0.0049 &  9.5E-4 & & -0.0024 & -0.0033 & -0.0044 & -0.0059 & -0.0074 & -0.0084 & -0.0091\\
0973 &  1.7E-4 &  1.2E-4 &  6.1E-4 &  3.5E-4 &  0.0022 &  0.0048 &  0.0010 & & -0.0024 & -0.0033 & -0.0044 & -0.0059 & -0.0074 & -0.0084 & -0.0090\\
0974 &  1.7E-4 &  9.1E-5 &  6.3E-4 &  3.0E-4 &  0.0022 &  0.0047 &  9.4E-4 & & -0.0024 & -0.0033 & -0.0044 & -0.0059 & -0.0073 & -0.0084 & -0.0090\\
0975 &  1.9E-4 &  8.7E-5 &  6.3E-4 &  2.9E-4 &  0.0022 &  0.0046 &  1.0E-3 & & -0.0024 & -0.0033 & -0.0044 & -0.0059 & -0.0073 & -0.0084 & -0.0090\\
0976 &  1.9E-4 &  8.8E-5 &  6.3E-4 &  2.4E-4 &  0.0023 &  0.0045 &  0.0011 & & -0.0024 & -0.0033 & -0.0044 & -0.0059 & -0.0073 & -0.0083 & -0.0090\\
0977 &  2.0E-4 &  6.1E-5 &  6.3E-4 &  1.9E-4 &  0.0024 &  0.0043 &  9.9E-4 & & -0.0024 & -0.0033 & -0.0044 & -0.0059 & -0.0072 & -0.0083 & -0.0089\\
0978 &  2.2E-4 &  5.5E-5 &  6.2E-4 &  1.7E-4 &  0.0024 &  0.0041 &  0.0010 & & -0.0023 & -0.0033 & -0.0044 & -0.0059 & -0.0072 & -0.0083 & -0.0089\\
0979 &  2.2E-4 &  5.7E-5 &  6.0E-4 &  1.1E-4 &  0.0025 &  0.0039 &  0.0011 & & -0.0023 & -0.0033 & -0.0044 & -0.0059 & -0.0072 & -0.0083 & -0.0089\\
0980 &  2.3E-4 &  2.8E-5 &  5.7E-4 &  5.9E-5 &  0.0025 &  0.0038 &  0.0010 & & -0.0023 & -0.0032 & -0.0043 & -0.0059 & -0.0071 & -0.0083 & -0.0089\\
0981 &  2.5E-4 &  2.2E-5 &  5.5E-4 &  3.0E-5 &  0.0025 &  0.0035 &  0.0011 & & -0.0023 & -0.0032 & -0.0043 & -0.0059 & -0.0071 & -0.0083 & -0.0089\\
0982 &  2.6E-4 &  2.6E-5 &  5.0E-4 &  3.3E-5 &  0.0026 &  0.0032 &  0.0012 & & -0.0023 & -0.0032 & -0.0043 & -0.0058 & -0.0071 & -0.0083 & -0.0088\\
0983 &  2.7E-4 &  8.7E-7 &  4.6E-4 &  1.0E-4 &  0.0027 &  0.0030 &  0.0011 & & -0.0023 & -0.0032 & -0.0043 & -0.0058 & -0.0070 & -0.0083 & -0.0088\\
0984 &  2.9E-4 &  4.9E-6 &  4.2E-4 &  1.4E-4 &  0.0027 &  0.0026 &  0.0011 & & -0.0023 & -0.0032 & -0.0043 & -0.0058 & -0.0070 & -0.0083 & -0.0088\\
0985 &  3.0E-4 &  4.8E-6 &  3.5E-4 &  2.1E-4 &  0.0028 &  0.0023 &  0.0012 & & -0.0023 & -0.0032 & -0.0043 & -0.0058 & -0.0070 & -0.0083 & -0.0088\\
0986 &  3.3E-4 &  1.8E-5 &  2.9E-4 &  2.9E-4 &  0.0029 &  0.0020 &  0.0011 & & -0.0022 & -0.0032 & -0.0043 & -0.0058 & -0.0069 & -0.0083 & -0.0087\\
0987 &  3.4E-4 &  1.8E-5 &  2.3E-4 &  3.4E-4 &  0.0029 &  0.0016 &  0.0011 & & -0.0022 & -0.0032 & -0.0043 & -0.0057 & -0.0069 & -0.0083 & -0.0087\\
0988 &  3.5E-4 &  2.8E-6 &  1.5E-4 &  4.2E-4 &  0.0029 &  0.0012 &  0.0013 & & -0.0022 & -0.0031 & -0.0043 & -0.0057 & -0.0069 & -0.0082 & -0.0087\\
0989 &  3.8E-4 &  2.2E-5 &  6.3E-5 &  5.2E-4 &  0.0029 &  7.8E-4 &  0.0012 & & -0.0022 & -0.0031 & -0.0043 & -0.0057 & -0.0069 & -0.0082 & -0.0087\\
0990 &  3.9E-4 &  1.9E-5 &  1.3E-5 &  5.7E-4 &  0.0028 &  3.2E-4 &  0.0012 & & -0.0022 & -0.0031 & -0.0042 & -0.0057 & -0.0068 & -0.0082 & -0.0087\\
0991 &  4.1E-4 &  8.0E-7 &  1.1E-4 &  6.6E-4 &  0.0028 &  1.6E-4 &  0.0013 & & -0.0022 & -0.0031 & -0.0042 & -0.0057 & -0.0068 & -0.0082 & -0.0086\\
0992 &  4.4E-4 &  1.6E-5 &  2.2E-4 &  7.7E-4 &  0.0026 &  6.1E-4 &  0.0012 & & -0.0022 & -0.0031 & -0.0042 & -0.0056 & -0.0068 & -0.0082 & -0.0086\\
0993 &  4.6E-4 &  1.1E-5 &  3.1E-4 &  8.3E-4 &  0.0025 & -0.0011 &  0.0012 & & -0.0022 & -0.0031 & -0.0042 & -0.0056 & -0.0068 & -0.0082 & -0.0086\\
0994 &  4.8E-4 &  1.4E-5 &  4.3E-4 &  9.3E-4 &  0.0023 & -0.0017 &  0.0013 & & -0.0021 & -0.0031 & -0.0042 & -0.0056 & -0.0067 & -0.0083 & -0.0085\\
0995 &  5.1E-4 &  1.0E-6 &  5.5E-4 & -0.0011 &  0.0021 & -0.0022 &  0.0012 & & -0.0021 & -0.0031 & -0.0042 & -0.0055 & -0.0067 & -0.0083 & -0.0085\\
0996 &  5.5E-4 &  6.6E-6 &  6.7E-4 & -0.0011 &  0.0019 & -0.0028 &  0.0012 & & -0.0021 & -0.0030 & -0.0042 & -0.0055 & -0.0067 & -0.0083 & -0.0085\\
0997 &  5.6E-4 &  3.5E-5 &  8.0E-4 & -0.0012 &  0.0017 & -0.0034 &  0.0014 & & -0.0021 & -0.0030 & -0.0042 & -0.0055 & -0.0067 & -0.0083 & -0.0085\\
0998 &  6.0E-4 &  2.2E-5 &  9.5E-4 & -0.0014 &  0.0014 & -0.0040 &  0.0012 & & -0.0021 & -0.0030 & -0.0041 & -0.0054 & -0.0067 & -0.0083 & -0.0084\\
0999 &  6.4E-4 &  3.2E-5 & -0.0011 & -0.0015 &  0.0011 & -0.0047 &  0.0012 & & -0.0021 & -0.0030 & -0.0041 & -0.0054 & -0.0067 & -0.0083 & -0.0084\\
\enddata
\tablenotetext{a}{1000 $\Delta v$ values given in units of $\delta v_\parallel\!\left(z\right) \equiv 0.25246\,z + 1.4731$ km s$^{-1}$}
\tablecomments{These are the hybrid correlation 
values for full-resolution.}
\end{deluxetable}

